Introduction into Calculus over Banach algebra

Let $A$, $B$ be Banach $D$-algebras. The map $f:A\rightarrow B$ is called differentiable on the set $U\subset A$, if at every point $x\in U$ the increment of map $f$ can be represented as $$f(x+dx)-f(x) =\frac{d f(x)}{d x}\circ dx +o(dx)$$ where $$\frac{d f(x)}{d x}:A\rightarrow B$$ is linear map and $o:A\rightarrow B$ is such continuous map that $$\lim_{a\rightarrow 0}\frac{\|o(a)\|_B}{\|a\|_A}=0$$ Linear map $\displaystyle\frac{d f(x)}{d x}$ is called derivative of map $f$. I considered differential forms in Banach Algebra. Differential form $\omega\in\mathcal{LA}(D;A\rightarrow B)$ is defined by map $g:A\rightarrow B\otimes B$, $\omega=g\circ dx$. If the map $g$, is derivative of the map $f:A\rightarrow B$, then the map $f$ is called indefinite integral of the map $g$ $$f(x)=\int g(x)\circ dx=\int\omega$$ Then, for any $A$-numbers $a$, $b$, we define definite integral by the equality $$\int_a^b\omega=\int_{\gamma}\omega$$ for any path $\gamma$ from $a$ to $b$.

==> Biblio.Russian.tex <==
%auto-ignore
\OpenBiblio

\BiblioItem{Doctor Ouch}
{
Корней Чуковский. Айболит.
\\
Детский мир, ISBN 978-5-91315-875-8, 2012
}%

\BiblioItem{Einstein: Electrodynamics of Moving Bodies}
{
Альберт Эйнштейн,
К электродинамике движущихся тел, 1905,
Собрание научных трудов, I, 7 - 35,
М., Наука, 1965
\\
Zur Elektrodynamik der bewegter K\"orper. Ann. Phys., 1905, 17, 891-921. 
}%

\BiblioItem{Einstein: On the Relativity Principle}
{
Альберт Эйнштейн,
О принципе относительности и его следствиях, 1907,
Собрание научных трудов, I, 65 - 114,
М., Наука, 1965
\\
\"Uber das Relativit\"atsprinzip und die aus demselben gezogenen Folgerungen. 
Jahrb. d. Radioaktivit\"at u. Elektronik, 1907, 4, 411-462. 
}%

\BiblioItem{Einstein: Foundations of general relativity}
{
Альберт Эйнштейн,
Основы общей теории относительности, 1916,
Собрание научных трудов, I, 452 - 504,
М., Наука, 1965
}%

\BiblioItem{Einstein: Geometry and Experience}
{
Альберт Эйнштейн,
Геометрия и опыт, (1921)
Собрание научных трудов, II, 83 - 84,
М., Наука, 1966
}%

\BiblioItem{Einstein: Main problems of general relativity}
{
Альберт Эйнштейн,
Основные идеи и проблемы теории относительности, (1923)
Собрание научных трудов, II, 120 - 129,
М., Наука, 1966
}%

\BiblioItem{Einstein: Noneuclidean Geometry and Physics}
{
Альберт Эйнштейн,
Неэвклидова геометрия и физика, (1926)
Собрание научных трудов, II, 178 - 182,
М., Наука, 1966
}%

\BiblioItem{Einstein: Isaak Newton}
{
Альберт Эйнштейн,
Исаак Ньютон, 1927,
Собрание научных трудов, IV, 78 - 81,
М., Наука, 1967
}%

\BiblioItem{Einstein: On Science}
{
Альберт Эйнштейн,
О науке, 1931,
Собрание научных трудов, IV, 142 - 146,
М., Наука, 1967
}%

\BiblioItem{Einstein: Autobiographical Notes}
{
Альберт Эйнштейн,
Автобиографические заметки, 1949,
Собрание научных трудов, IV, 259 - 293,
М., Наука, 1967
}%

\BiblioItem{Feynman 3}
{
Фейнман Р., Лейтон Р., Сэндс М..
Фейнмановские лекции по физике (том 3). Излучение. Волны. Кванты.
М., Мир, 1976
}%

\BiblioItem{0538731877}
{
James Shipman, Jerry D. Wilson and Aaron Todd.
Introduction to Physical Science.
Cengage Learning, 2009; ISBN 0538731877.
}%

\BiblioItem{Cite: 104}
{
Ссылка 104, Источник неизвестен
}%

\BiblioItem{Ghez}
{
Ghez et al.,
The First Measurement of Spectral Lines in a Short-Period Star Bound to the Galaxy's Central Black Hole: A Paradox of Youth,
\href{http://www.journals.uchicago.edu/ApJ/journal/issues/ApJL/v586n2/16990/brief/16990.abstract.html}{ApJL, 586, L127} (2003),
eprint \href{http://arxiv.org/abs/astro-ph/0302299}{arXiv:astro-ph/0302299} (2003)
}%

\BiblioItem{Schodel}
{
R. Sch\"odel et al.,
A star in a 15.2-year orbit around the supermassive black hole at the centre of the Milky Way,
\href{http://www.nature.com/cgi-taf/DynaPage.taf?file=/nature/journal/v419/n6908/abs/nature01121_fs.html}{Nature 419, 694} (2002)
}%

\BiblioItem{Mielke}
{
Eckehard W. Mielke, Affine generalization of the Komar complex of general relativity,
\href{http://prola.aps.org/searchabstract/PRD/v63/i4/e044018}{Phys. Rev. D 63, 044018} (2001)
}%

\BiblioItem{Obukhov}
{
Yu. N. Obukhov and J. G. Pereira, Metric\hyph affine approach to teleparallel gravity,
\href{http://scitation.aip.org/getabs/servlet/GetabsServlet?prog=normal&id=PRVDAQ000067000004044016000001&idtype=cvips&gifs=Yes}
{Phys. Rev. D 67, 044016} (2003),
eprint \href{http://arxiv.org/abs/gr-qc/0212080}{arXiv:gr-qc/0212080} (2002)
}%

\BiblioItem{Sardanashvily}
{
Giovanni Giachetta, Gennadi Sardanashvily, Dirac Equation in Gauge and Affine-Metric Gravitation Theories,
eprint \href{http://arxiv.org/abs/gr-qc/9511035}{arXiv:gr-qc/9511035} (1995)
}%

\BiblioItem{Gauge}
{
Frank Gronwald and Friedrich W. Hehl, On the Gauge Aspects of Gravity, eprint
\href{http://arxiv.org/abs/gr-qc/9602013}{arXiv:gr-qc/9602013} (1996)
}%

\begin{otherlanguage}{english}
\BiblioItem{Neeman}
{
Yuval Neeman, Friedrich W. Hehl, Test Matter in a Spacetime with Nonmetricity, eprint
\href{http://arxiv.org/abs/gr-qc/9604047}{arXiv:gr-qc/9604047} (1996)
}%
\end{otherlanguage}

\BiblioItem{torsion}
{
F. W. Hehl, P. von der Heyde, G. D. Kerlick, and J. M. Nester,
General relativity with spin and torsion: Foundations and prospects,\\
\href{http://prola.aps.org/abstract/RMP/v48/i3/p393_1}{Rev. Mod. Phys. 48, 393} (1976)
}%

\BiblioItem{Megged}
{
O. Megged, Post-Riemannian Merger of Yang-Mills Interactions with Gravity,
eprint \href{http://arxiv.org/abs/hep-th/0008135}{arXiv:hep-th/0008135} (2001)
}%

%\BiblioItem{Hehl}
%{
%Friedrich W. Hehl, Uwe Muench,
%eprint \href{http://arxiv.org/abs/gr-qc/9708007}{arXiv:gr-qc/9708007} (1997)
%}%

\BiblioItem{gr-qc-9604027}
{
Yu.N. Obukhov, E.J. Vlachynsky, W. Esser, R. Tresguerres and F.W. Hehl,
An exact solution of the metric\hyph affine gauge theory with dilation, shear, and spin charges,
eprint \href{http://arxiv.org/abs/gr-qc/9604027}{arXiv:gr-qc/9604027} (1996)
}%

\BiblioItem{4419-7514}
{
Mari\'an Fabian, Petr Habala, Petr H\'ajek, Vicente Montesinos, V\'aclav Zizler.
Banach Space Theory: The Basis for Linear and Nonlinear Analysis.
\\
Springer; New York, 2010; ISBN-13: 978-1441975140
}%

\BiblioItem{Weinberg I}
{
Стивен Вайнберг.
Квантовая теория полей. Том 1. Основы.
\\
Перевод на русский язык А. В. Беркова под редакцией Б. Л. Воронова,
М., Физико-математическая литература, 2001
}%

\BiblioItem{Weinberg II}
{
Стивен Вайнберг.
Квантовая теория полей. Том 2. Современные приложения.
\\
Перевод на русский язык А. В. Беркова,
М., Физико-математическая литература, 2001
}%

\BiblioItem{Reinhardt}
{
Walter Greiner, Joachim Reinhardt. Field Quantization. Springer.
}%

\BiblioItem{978-3540875604}
{
Walter Greiner, Joachim Reinhardt. Quantum Electrodynamics. Springer, 2009.
}%

\BiblioItem{978-1898563020}
{
H. Robert Mills. Practical Astronomy. Woodhead Publishing, 1994. ISBN-13: 978-1898563020.v
}%

\BiblioItem{Landau I}
{
Л. Д. Ландау, Е. М. Лифшич,
Теоретическая физика, механика,
М., Наука, 1988
}%

\BiblioItem{Landau}
{
Л. Д. Ландау, Е. М. Лифшич,
Теоретическая физика, теория поля,
М., Наука, 1988
}%

\BiblioItem{Landau III}
{
Л. Д. Ландау, Е. М. Лифшич,
Теоретическая физика, том III, квантовая механика,
нерелятивистская теория,
М., Наука, 1989
}%

\BiblioItem{Wheeler}
{
Ignazio Ciufolini, John Wheeler. Gravitation and Inertia.
Princeton university press.
}%

\BiblioItem{Gravitation MTW 1}
{
Ч. Мизнер, К. Торн, Дж. Уилер.
Гравитация, том $1$.
\\
Перевод с английского М. М. Баско
под редакцией В. Б. Брагинского и И. Д. Новикова.
\\
М. Мир, 1977.
}%

\BiblioItem{Gravitation MTW 2}
{
Ч. Мизнер, К. Торн, Дж. Уилер.
Гравитация, том $2$.
\\
Перевод с английского A. А. Рузмайкина 
под редакцией В. Б. Брагинского и И. Д. Новикова.
\\
М. Мир, 1977.
}%

\BiblioItem{Gravitation MTW 3}
{
Ч. Мизнер, К. Торн, Дж. Уилер.
Гравитация, том $3$.
\\
Перевод с английского A. А. Рузмайкина 
под редакцией В. Б. Брагинского и И. Д. Новикова.
\\
М. Мир, 1977.
}%

\BiblioItem{Anderson98}
{
J. D. Anderson, P. A. Laing, E. L. Lau, A. S. Liu, M. M. Nieto, and S. G. Turyshev,
Indication, from Pioneer 10/11, Galileo, and Ulysses Data, of an Apparent Anomalous, Weak, Long-Range Acceleration,
\href{http://prola.aps.org/abstract/PRL/v81/i14/p2858_1}{Phys. Rev. Lett. 81, 2858}, (1998),
eprint \href{http://arxiv.org/abs/gr-qc/9808081}{arXiv:gr-qc/9808081} (1998)
}%

\BiblioItem{Anderson02}
{
J. D. Anderson, P. A. Laing, E. L. Lau, A. S. Liu, M. M. Nieto, and S. G. Turyshev,
Study of the anomalous acceleration of Pioneer 10 and 11,
\href{http://prola.aps.org/searchabstract/PRD/v65/i8/e082004}{Phys. Rev. D 65, 082004, 50 pp.}, (2002),
eprint \href{http://arxiv.org/abs/gr-qc/0104064}{arXiv:gr-qc/0104064} (2001)
}%

%\BiblioItem{Havas} Peter Havas, The Classical Equations of Motion of Point Particles, I,
%{
%\href{http://prola.aps.org/abstract/PR/v87/i2/p309_1}{Phys. Rev. 87, 309} (1952)
%}%

\BiblioItem{H. Aslaksen}
{
H. Aslaksen.  Quaternionic determinants \textit{Math.
Intelligencer} {\bf 18}(3), pp.57-65, (1996).
}%

\BiblioItem{L. Chen: Definition of determinant}
{
L. Chen, Definition of determinant and Cramer solutions over
quaternion field, \textit{Acta Math. Sinica (N.S.)} {\bf 7},
pp.171-180, (1991).
}%

\BiblioItem{L. Chen: Inverse matrix}
{
L. Chen,
Inverse matrix and properties of double determinant over quaternion
field, \textit{Sci. China, Ser. A} {\bf 34}, pp.528-540, (1991).
}%

\BiblioItem{N. Cohen S. De Leo}
{
N. Cohen, S. De Leo, The quaternionic determinant, \textit{The Electronic Journal Linear
Algebra} {\bf 7}, pp.100-111, (2000).
}%

\BiblioItem{Dyson: Quaternion determinants}
{
F. J. Dyson, Quaternion determinants, \textit{Helvetica Phys.
Acta} {\bf 45}, pp. 289-302, (1972).
}%

\BiblioItem{Melvin Hausner}
{
Melvin Hausner,
A Vector Space Approach to Geometry,
Dover Publications, 1998
}%

\BiblioItem{Serge Lang}
{
Серж Ленг,
Алгебра, М. Мир, 1968
}%

\BiblioItem{9780534423230}
{
Charles Lanski.
Concepts In Abstract Algebra.
American Mathematical Soc., 2005, ISBN 978-0534423230
}%

\BiblioItem{Burris Sankappanavar}
{
S. Burris, H.P. Sankappanavar,
A Course in Universal Algebra, Springer-Verlag (March, 1982),
\\eprint
\href{http://www.math.uwaterloo.ca/~snburris/htdocs/ualg.html}
{http://www.math.uwaterloo.ca/~snburris/htdocs/ualg.html}
\\(The Millennium Edition)
}%

\BiblioItem{Shilov single 12}
{
Г. Е. Шилов. Математический анализ,
Функции одного переменного, части 1 - 2,
М., Наука, 1969
}%

\BiblioItem{Shilov single 3}
{
Г. Е. Шилов. Математический анализ,
Функции одного переменного, часть 3,
М., Наука, 1970
}%

\BiblioItem{Shilov}
{
Г. Е. Шилов. Математический анализ,
Функции нескольких вещественных переменных, части 1 - 2,
М., Наука, 1972
}%

\BiblioItem{Kolmogorov Fomin}
{
А. Н. Колмогоров, С. В. Фомин.
Элементы теории функций и функционального анализа.
М., Наука, 1976
}%

\BiblioItem{Lebedev Vorovich}
{
И. И. Ворович, Л. П. Лебедев,
Функциональный анализ и его приложения в механике сплошной среды,
М., Вузовская книга, 2000
}%

\BiblioItem{8176-4374}
{
Mariano Giaquinta, Giuseppe Modica,
Mathematical Analysis: Linear and Metric Structures and Continuity.
\\
Springer, 2007, ISBN-13: 978-0-8176-4374-4
}%

\BiblioItem
{Rashevsky}
{
П. К. Рашевский,
Риманова геометрия и тензорный анализ,\\
М., Наука, 1967
}%

\BiblioItem
{Kurosh: High Algebra}
{
А. Г. Курош,
Курс высшей алгебры,
М., Наука, 1968
}%

\BiblioItem
{Kurosh: General Algebra}
{
А. Г. Курош,
Общая алгебра, (лекции 1969 - 70 учебного года),
М., МГУ, 1970
}%

\BiblioItem{Sabinin: Smooth Quasigroups}
{
Lev V. Sabinin, Smooth Quasigroups and Loops,
Kluwer Academic Publisher, 1999 
}%

\BiblioItem{978-0-8176-8384-9}
{
Garret Sobczyk, New Foundations in Mathematics: The Geometric Concept of Number,
\\
Springer, 2013, ISBN: 978-0-8176-8384-9
}%

\BiblioItem{Dubrovin Fomenko Novikov part 1}
{
Б. А. Дубровин, С. П. Новиков, А. Т. Фоменко,
Современная геометрия, Методы и приложения,\\
Том I, Геометрия поверхностей, групп преобразований и полей,\\
Эдиториал УРСС, М. 1998
}%

\BiblioItem{Dubrovin Fomenko Novikov part 2}
{
Б. А. Дубровин, С. П. Новиков, А. Т. Фоменко,
Современная геометрия, Методы и приложения,\\
Том II, Геометрия и топология многообразий,\\
Эдиториал УРСС, М. 1998
}%

\BiblioItem{Kobayashi Nomizu vol 1}
{
Ш. Кобаяси, К. Номидзу,
Основы дифференциальной геометрии, Том I,
перевод с английского Л. В. Сабинина,
М., Наука, 1981
}%

\BiblioItem{Lichnerowicz}
{
Андрэ Лихнерович,
Теория связностей в целом и группы голономий,
перевод с французкого С. П. Финикова под редакцией В. В. Рыжкова,
М., Иностранная литература, 1960
}%

\BiblioItem{Korn}
{
Г. Корн, Т. Корн,
Справочник по математике для научных работников и инженеров,
М., Наука, 1974
}%

\BiblioItem{Hocking Young Topology}
{
John G. Hocking, Gail S. Young,
Topology,\\
Courier Dover Publications, 1988
}%

\BiblioItem{Olver: Lie groups to differential equations}
{
П. Олвер,
Приложения групп Ли к дифференциальным уравнениям,\\
М. Мир, 1989
}%

\BiblioItem{1708.01190}
{
Nathan BeDell,
Doing Algebra over an Associative Algebra,
\\
eprint \href{https://arxiv.org/abs/1708.01190}{arXiv:1708.01190} (2017)
}%

\BiblioItem{Tartaglia}
{
Angelo Tartaglia and Matteo Luca Ruggiero,
Angular Momentum Effects in Michelson\Hyph Morley Type Experiments,
Gen.Rel.Grav. 34, 1371-1382 (2002),\\
eprint \href{http://arxiv.org/abs/gr-qc/0110015}{arXiv:gr-qc/0110015} (2001)
}%

\BiblioItem{Tomozawa}
{
Yukio Tomozawa, Speed of Light in Gravitational Fields, eprint
\href{http://arxiv.org/abs/astro-ph/0303047}{arXiv:astro-ph/0303047} (2004)
}%

\BiblioItem{Magueijo}
{
Joao Magueijo,
Covariant and locally Lorentz-invariant varying speed of light theories,
\href{http://prola.aps.org/abstract/PRD/v62/i10/e103521}{Phys. Rev. D 62, 103521} (2000),
eprint \href{http://arxiv.org/abs/gr-qc/0007036}{arXiv:gr-qc/0007036} (2000)
}%

\BiblioItem{Bassett}
{
Bruce A. Bassett, Stefano Liberati, Carmen Molina-Paris, and Matt Visser,
Geometrodynamics of variable-speed-of-light cosmologies,
\href{http://prola.aps.org/abstract/PRD/v62/i10/e103518}{Phys. Rev. D 62}, 103518 (2000),
eprint \href{http://arxiv.org/abs/astro-ph/0001441}{arXiv:astro-ph/0001441} (2000)
}%

\BiblioItem{C.A. Deavours The Quaternion Calculus}
{
C.A. Deavours, The Quaternion Calculus, 
American Mathematical Monthly, {\bf 80} (1973), pp. 995 - 1008
}%

\BiblioItem{Straumann}
{
Lochlainn O'Raifeartaigh and Norbert Straumann,
Gauge theory: Historical origins and some modern developments,
\href{http://prola.aps.org/abstract/RMP/v72/i1/p1_1}{Rev. Mod. Phys. 72, 1} (2000)
}%

\begin{otherlanguage}{english}
\BiblioItem{Lammerzahl}
{
Claus L\"ammerzahl, Mark P. Haugan,
On the interpretation of Michelson\Hyph Morley experiments,
%\href{http://www.sciencedirect.comyph /science?_ob=ArticleURL&_udi=B6TVM-42WP7CR-1&_user=10&_handle=W-WA-A-A-AZ-MsSAYZW-UUW-AUDDYZYZAU-WZCBYCEDW-AZ-U&_fmt=summary&_coverDate=04%2F23%2F2001&_rdoc=1&_orig=browse&_srch=%23toc%235538%232001%23997179995%23246657!&_cdi=5538&view=c&_acct=C000050221&_version=1&_urlVersion=0&_userid=10&md5=385478cda8c5568dea1aeaf0c43669da}
{Phys. Lett. A282 223-229} (2001),\\
eprint \href{http://arxiv.org/abs/gr-qc/0103052}{arXiv:gr-qc/0103052} (2001)
}%
\end{otherlanguage}

\begin{otherlanguage}{english}
\BiblioItem{0305117}
{
Holger Mueller, Sven Herrmann, Claus Braxmaier, Stephan Schiller, Achim Peters.
Modern Michelson-Morley Experiment using Cryogenic Optical Resonators.
eprint \href{http://arxiv.org/abs/physics/0305117}{arXiv:physics/0305117} (2003)
\\
Phys. Rev. Lett. 91:020401, 2003
}%
\end{otherlanguage}

\BiblioItem{0706.2031}
{
Holger Mueller, Paul Louis Stanwix, Michael Edmund Tobar,
Eugene Ivanov, Peter Wolf, Sven Herrmann, Alexander Senger,
Evgeny Kovalchuk, Achim Peters.
Relativity tests by complementary rotating Michelson-Morley experiments.
eprint \href{http://arxiv.org/abs/0706.2031}{arXiv:0706.2031 [physics.class-ph]} (2006)
\\
Phys. Rev. Lett. 99:050401, 2007
}%

\BiblioItem{1008.1205}
{
M. Nagel, K. M\"ohle, K. D\"oringshoff, S. Herrmann, A. Senger, E.V. Kovalchuk, A. Peters.
Testing Lorentz Invariance by Comparing Light Propagation in Vacuum and Matter.
eprint \href{http://arxiv.org/abs/1008.1205}{arXiv:1008.1205 [physics.ins-det]} (2010)
}%

\BiblioItem{1109.4897}
{
The OPERA Collaboration.
Measurement of the neutrino velocity with the OPERA detector in the CNGS beam.
eprint \href{http://arxiv.org/abs/1109.4897}{arXiv:1109.4897 [hep-ex]} (2011)
}%

\begin{otherlanguage}{english}
\BiblioItem{Ranada}
{
Antonio F. Ranada,
Pioneer acceleration and variation of light speed: experimental situation,
eprint \href{http://arxiv.org/abs/gr-qc/0402120}{arXiv:gr-qc/0402120} (2004)
}%
\end{otherlanguage}

\BiblioItem{Gelfand Minlos: rotation and Lorentz groups}
{
И. М. Гельфанд, Р. А. Минлос, З. Я. Шапиро,
Представления группы вращений и группы Лоренца, их применения,\\
М., Наука, 1958
}%

\BiblioItem{math.QA-0208146}
{
I. Gelfand, S. Gelfand, V. Retakh, R. Wilson,
Quasideterminants,\\
eprint \href{http://arxiv.org/abs/math.QA/0208146}{arXiv:math.QA/0208146} (2002)
}%

\BiblioItem{q-alg-9705026}
{
I. Gelfand, V. Retakh,
Quasideterminants, I,\\
eprint \href{http://arxiv.org/abs/q-alg/9705026}{arXiv:q-alg/9705026} (1997)
}%

\BiblioItem{Gelfand Retakh 1991}
{
И. М. Гельфанд, В. С. Ретах,  Детерминанты матриц над некоммутативными кольцами,
\textit{Функциональный анализ и его приложения} {\bf 25}(2), c. 13-35, (1991).
}%

\BiblioItem{Gelfand Retakh 1992}
{
И. М. Гельфанд, В. С. Ретах,  Теория некоммутативных
детерминантов и характеристические функции графов,\\
\textit{Функциональный анализ и его приложения} {\bf 26} (4), c.
33-45, (1992).
}%

\BiblioItem{hep-th-9407124}
{
I. M. Gelfand, D. Krob, A. Lascoux, B. Leclerc, V.S. Retakh and J.-Y. Thibon,
Noncommutative symmetric functions,\\
eprint \href{http://arxiv.org/abs/hep-th/9407124}{arXiv:hep-th/9407124} (1994)
}%

\BiblioItem{0911.4454}
{
Vladimir Retakh,
From factorizations of noncommutative polynomials to combinatorial topology,\\
eprint \href{http://arxiv.org/abs/0911.4454}{arXiv:0911.4454} (2009)
}%

\BiblioItem{Naimark Shtern: Theory of group representations}
{
М. А. Наймарк,
Теория представления групп,\\
М., Наука, 1976
}%

\BiblioItem{Barut Raczka: Theory of group representations}
{
А. Барут, Р. Рончка,
Теория представления групп и её приложения,\\
Перевод с английского А. У. Климыка и А. М. Гаврилика
под редакцией Я. А. Смородинского,\\
М., Мир, 1980
}%

\BiblioItem{Mihalev Pilz: concise handbook of algebra}
{
Aleksandr Vasilevich Mikhalev; G\"{u}nter Pilz;
The concise handbook of algebra;\\
Kluwer Academic Publishers, 2002
}%

\BiblioItem{McCrimmon: Jordan Algebras}
{
Kevin McCrimmon;
A Taste of Jordan Algebras;\\
Springer, 2004
}%

\BiblioItem{Shafarevich: Basic notions of algebra}
{
И. Р. Шафаревич,
Основные понятия алгебры,\\
В сборнике "Современные проблемы математики. Фундаментальные направления
(Итоги науки и техники. ВИНИТИ АН СССР",
М., 1986, {\bf 11} 3 - 289
М., Мир, 1980
}%

\BiblioItem{Coppel: Number Theory}
{
W.A. Coppel,
Number Theory: An Introduction to Mathematics,\\
Springer, 2009
}%

\BiblioItem{978-0486497952}
{
Michael J. Field,
Differential Calculus and Its Applications,\\
Dover Publications, 2012; ISBN-13: 978-0486497952
}%

\BiblioItem{Elsgolts: Differential Equations}
{
Л. Э. Эльсгольц,
Дифференциальные уравнения и вариационное исчисление,
М., Наука, 1971 
}%

\BiblioItem{Baez Huerta: algebra of grand unified theories}
{
John Baez; John Huerta;
The algebra of grand unified theories;\\
Bull. Amer. Math. Soc. {\bf 47} (2010), 483-552
}%

\BiblioItem{J. Fan: Determinants}
{
J. Fan, Determinants and multiplicative functionals
on quaternion matrices, \textit{Linear Algebra and Its
Applications} {\bf 369}, pp. 193-201, (2003).
}%

\BiblioItem{Carl Faith 1}
{
К. Фейс, Алгебра: кольца, модули и категории, том I,
М., Мир, 1973
}%

\BiblioItem{Gilson Nimmo Ohta}
{
 C.R.Gilson, J.J.C.Nimmo, Y.Ohta, Quasideterminant solutions of a non-Abelian Hirota-Miwa
 equation, \textit{Journal of Physics A: Mathematical and Theoretical} {\bf 40}(42), pp.
 12607-12617,(2007).
}%

\BiblioItem{Haider Hassan}
{
B. Haider, M. Hassan, Quasideterminant solutions of an integrable chiral model in two
 dimensions, \textit{Journal of Physics A: Mathematical and Theoretical} {\bf 42} (35), art. no.
 355211, (2009).
}%

%\BiblioItem{Pareigis}
%{
%Bodo Pareigis, Categories and Functors,
%Academic Press - New York - London, 1970
%}%

%\BiblioItem{Beachy}
%{
%John A. Beachy, Introductory Lectures on Rings i Modules,
%Cambridge University Press, 1999
%}%

\BiblioItem{0702447}
{
I.I. Kyrchei, Cramer's rule for quaternion systems of linear equations,
\textit{Journal of Mathematical Sciences} {\bf 155}(6), 839-858, (2008).
 Translated from  \textit{Fundamental and Appl. Math.}
 {\bf 13}(4), pp.67-94, (2007). (in Russian)\\
eprint
\href{http://arxiv.org/abs/math/0702447}{arXiv:math.RA/0702447}
(2007)
}%

\BiblioItem{1004.4380}
{
I.I. Kyrchei, Cramer's rule for some quaternion matrix
    equations,  \textit{Applied Mathematics and Computation} {\bf 217}(5), pp.2024-2030, (2010).\\eprint
\href{http://arxiv.org/abs/1004.4380
}{arXiv:math.RA/arXiv:1004.4380 } (2010)
}%

\BiblioItem{1005.0736}
{
I.I. Kyrchei,Determinantal representations of the Moore-Penrose inverse
 over the quaternion skew field and corresponding Cramer's rules,
 \\
eprint
\href{http://arxiv.org/abs/1005.0736}{arXiv:math.RA/1005.0736}
(2010)
}%

\BiblioItem{0412.391}
{
Александр Клейн,
Многообразие базисов,\\
eprint \href{http://arxiv.org/abs/math.DG/0412391}{arXiv:math.DG/0412391} (2007)
}%

\BiblioItem{0405.027}
{
Александр Клейн,
Система отсчета в общей теории относительности,
eprint \href{http://arxiv.org/abs/gr-qc/0405027}{arXiv:gr-qc/0405027} (2008)
}%

\BiblioItem{0405.028}
{
Александр Клейн,
Метрико\hyph аффинное многообразие,\\
eprint \href{http://arxiv.org/abs/gr-qc/0405028}{arXiv:gr-qc/0405028} (2008)
}%

\BiblioItem{0612.111}
{
Александр Клейн,
Бикольцо матриц,\\
eprint \href{http://arxiv.org/abs/math.OA/0612111}{arXiv:math.OA/0612111} (2007)
}%

\BiblioItem{0701.238}
{
Александр Клейн,
Лекции по линейной алгебре над телом,\\
eprint \href{http://arxiv.org/abs/math.GM/0701238}{arXiv:math.GM/0701238} (2010)
}%

\BiblioItem{0702.561}
{
Александр Клейн,
Расслоенная универсальная алгебра,\\
eprint \href{http://arxiv.org/abs/math.DG/0702561}{arXiv:math.DG/0702561} (2007)
}%

\BiblioItem{math.RA-0501237}
{
Александр Клейн,
Векторное пространство над телом,\\
eprint \href{http://arxiv.org/abs/math.RA/0412391}{arXiv:math.RA/0501237} (2007)
}%

\BiblioItem{math.RA-0501237v1}
{
Aleks Kleyn,
Module Over Division Ring, version 1,\\
eprint \href{http://arxiv.org/abs/math/0501237v1}{arXiv:math.RA/0501237v1} (2005)
}%

\BiblioItem{0707.2246}
{
Александр Клейн,
Расслоенное соответствие,\\
eprint \href{http://arxiv.org/abs/0707.2246}{arXiv:0707.2246} (2007)
}%

\BiblioItem{0803.2620}
{
Александр Клейн,
Морфизм \Ts{T}представлений,\\
eprint \href{http://arxiv.org/abs/0803.2620}{arXiv:0803.2620} (2008)
}%

\BiblioItem{0803.3276}
{
Александр Клейн,
Преобразование Лоренца и принцип общековариантности,\\
eprint \href{http://arxiv.org/abs/0803.3276}{arXiv:0803.3276} (2009)
}%

\BiblioItem{0812.4763}
{
Александр Клейн,
Введение в математический анализ над телом,\\
eprint \href{http://arxiv.org/abs/0812.4763}{arXiv:0812.4763} (2010)
}%

\BiblioItem{0906.0135}
{
Александр Клейн,
Введение в геометрию над телом,\\
eprint \href{http://arxiv.org/abs/0906.0135}{arXiv:0906.0135} (2010)
}%

\BiblioItem{0909.0855}
{
Александр Клейн,
Этюд о кватернионах,\\
eprint \href{http://arxiv.org/abs/0909.0855}{arXiv:0909.0855} (2010)
}%

\BiblioItem{0912.3315}
{
Александр Клейн,
Представление универсальной алгебры,\\
eprint \href{http://arxiv.org/abs/0912.3315}{arXiv:0912.3315} (2010)
}%

\BiblioItem{0912.4061}
{
Александр Клейн,
Линейное уравнение в конечномерной алгебре,\\
eprint \href{http://arxiv.org/abs/0912.4061}{arXiv:0912.4061} (2010)
}%

\BiblioItem{1001.4852}
{
Александр Клейн,
Матрица линейных отображений,\\
eprint \href{http://arxiv.org/abs/1001.4852}{arXiv:1001.4852} (2010)
}%

\BiblioItem{1003.1544}
{
Александр Клейн,
Линейные отображения свободной алгебры,\\
eprint \href{http://arxiv.org/abs/1003.1544}{arXiv:1003.1544} (2010)
}%

\BiblioItem{1006.2597}
{
Александр Клейн,
Производная Гато и интеграл над банаховой алгеброй,\\
eprint \href{http://arxiv.org/abs/1006.2597}{arXiv:1006.2597} (2010)
}%

\BiblioItem{1011.3102}
{
Александр Клейн,
Полилинейное отображение свободной алгебры,\\
eprint \href{http://arxiv.org/abs/1011.3102}{arXiv:1011.3102} (2010)
}%

\BiblioItem{1104.5197}
{
Александр Клейн,
$C^*$-рапсодия,\\
eprint \href{http://arxiv.org/abs/1104.5197}{arXiv:1104.5197} (2011)
}%

\BiblioItem{1105.4307}
{
Александр Клейн,
Алгебра с сопряжением,\\
eprint \href{http://arxiv.org/abs/1105.4307}{arXiv:1105.4307} (2011)
}%

\BiblioItem{1107.1139}
{
Александр Клейн,
Линейные отображения алгебры кватернионов,\\
eprint \href{http://arxiv.org/abs/1107.1139}{arXiv:1107.1139} (2011)
}%

\BiblioItem{1107.5037}
{
Александр Клейн,
Ортогональный базис и движение в финслеровой геометрии,\\
eprint \href{http://arxiv.org/abs/1107.5037}{arXiv:1107.5037} (2011)
}%

\BiblioItem{1111.6035}
{
Александр Клейн,
Базис представления универсальной алгебры,\\
eprint \href{http://arxiv.org/abs/1111.6035}{arXiv:1111.6035} (2011)
}%

\BiblioItem{1201.4158}
{
Александр Клейн, Александер Ложье,
Ортонормированный базис в пространстве Минковского,\\
eprint \href{http://arxiv.org/abs/1201.4158}{arXiv:1201.4158} (2012)
}%

\BiblioItem{1202.6021}
{
Александр Клейн,
Отображения сопряжения алгебры кватернионов,\\
eprint \href{http://arxiv.org/abs/1202.6021}{arXiv:1202.6021} (2012)
}%

\BiblioItem{1206.0200}
{
Александр Клейн,
Алгебра частных алгебры с сопряжением,\\
eprint \href{http://arxiv.org/abs/1206.0200}{arXiv:1206.0200} (2012)
}

\BiblioItem{1211.6965}
{
Александр Клейн,
Свободная алгебра со счётным базисом,\\
eprint \href{http://arxiv.org/abs/1211.6965}{arXiv:1211.6965} (2012)
}%

\BiblioItem{1302.7204}
{
Александр Клейн,
Многочлен над ассоциативной $D$-алгеброй,\\
eprint \href{http://arxiv.org/abs/1302.7204}{arXiv:1302.7204} (2013)
}%

\BiblioItem{1305.4547}
{
Александр Клейн,
Нормированная $\Omega$-группа,\\
eprint \href{http://arxiv.org/abs/1305.4547}{arXiv:1305.4547} (2013)
}%

\BiblioItem{1310.5591}
{
Александр Клейн,
Интеграл отображения в абелевую $\Omega$\Hyph группу,\\
eprint \href{http://arxiv.org/abs/1310.5591}{arXiv:1310.5591} (2013)
}%

\BiblioItem{1502.04063}
{
Александр Клейн,
Линейное отображение $D$\Hyph алгебры,\\
eprint \href{http://arxiv.org/abs/1502.04063}{arXiv:1502.04063} (2015)
}%

\BiblioItem{1505.03625}
{
Александр Клейн,
Производная отображения банаховой алгебры,\\
eprint \href{http://arxiv.org/abs/1505.03625}{arXiv:1505.03625} (2015)
}%

\BiblioItem{1601.03259}
{
Александр Клейн,
Введение в математический анализ над банаховой алгеброй,\\
eprint \href{http://arxiv.org/abs/1601.03259}{arXiv:1601.03259} (2016)
}%

\BiblioItem{MRepro}
{
Александр Клейн,
Теория представлений универсальной алгебры,\\
eprint \href{http://arxiv.org/abs/MRepro}{arXiv:MRepro} (2015)
}%

\BiblioItem{MVector}
{
Александр Клейн,
Линейное отображение D-алгебры,\\
eprint \href{http://arxiv.org/abs/MVector}{arXiv:MVector} (2017)
}%

\BiblioItem{8433-5163}
{
Aleks Kleyn,
Linear Maps of Free Algebra: First Steps in Noncommutative Linear Algebra,\\
Lambert Academic Publishing, 2010
}%

\BiblioItem{8443-0072}
{
Aleks Kleyn,
Representation Theory: Representation of Universal Algebra,\\
Lambert Academic Publishing, 2011
}%

\BiblioItem{4776-3181}
{
Александр Клейн.\\
Линейная алгебра над телом: Система линейных уравнений.\\
CreateSpace Independent Publishing Platform, 2014;\\
ISBN-13: 978-1502982476
}%

\BiblioItem{4993-2400}
{
Александр Клейн.\\
Линейная алгебра над телом: Векторное пространство.\\
CreateSpace Independent Publishing Platform, 2014;\\
ISBN-13: 978-1499323948
}%

\BiblioItem{5059-9176}
{
Александр Клейн.\\
Нормированная \(\Omega\)-группа.\\
CreateSpace Independent Publishing Platform, 2015;\\
ISBN-13: 978-1505992359
}%

\BiblioItem{5114-6019}
{
Александр Клейн.\\
Представление универсальной алгебры: Полиморфизм.\\
CreateSpace Independent Publishing Platform, 2015;\\
ISBN-13: 978-1511464949
}%

\BiblioItem{5148-4632}
{
Александр Клейн.\\
Представление универсальной алгебры: Полиморфизм.\\
CreateSpace Independent Publishing Platform, 2015;\\
ISBN-13: 978-1511464949
}%

\BiblioItem{5410-9916}
{
Александр Клейн.\\
Интеграл Лебега в абелевой $\Omega$-группе.\\
CreateSpace Independent Publishing Platform, 2016;\\
ISBN-13: 978-1541099845
}%

\BiblioItem{BRepro}
{
Александр Клейн,
Теория представлений универсальной алгебры,\\
CreateSpace Independent Publishing Platform, 2015;\\
ISBN-13: %978-1511464949
}%

\BiblioItem{CACAA.01.291}
{
Aleks Kleyn,
Introduction into Calculus over Division Ring.\\
Clifford Analysis, Clifford Algebras and their applications,
volume 1, Issue 4, pages 291 - 355, 2012
}%

\BiblioItem{CACAA.02.097}
{
Aleks Kleyn,
Polynomial over Associative $D$-Algebra.\\
Clifford Analysis, Clifford Algebras and their applications,
volume 2, Issue 2, pages 97 - 115, 2013
}%

\BiblioItem{CACAA.04.001}
{
Aleks Kleyn,
Integral of Map into Abelian $\Omega$-group.\\
Clifford Analysis, Clifford Algebras and their applications,
volume 4, Issue 1, pages 1 - 68, 2013
}%

\BiblioItem{CACAA.05.001}
{
Aleks Kleyn,
Introduction into Calculus over Division Ring.\\
Clifford Analysis, Clifford Algebras and their applications,
volume 5, issue 1, pages 1 - 68, 2016 
}%

\BiblioItem{GJSFRA.13.1.39}
{
Aleks Kleyn,
Reference frame and Lorentz transformation,\\
Global Journals of Science Frontier Research A,
volume 13, issue 1, pages 39 - 55, 2013 
}%

\BiblioItem{1506.05848}
{
Rida T. Farouki, Graziano Gentili, Carlotta Giannelli, Alessandra Sestini,
Caterina Stoppato,\\
Solution of a quadratic quaternion equation with mixed coefficients,\\
eprint \href{http://arxiv.org/abs/1506.05848}{arXiv:1506.05848} (2015)
}%

\BiblioItem{Lauve: Quantum coordinates}
{
A. Lauve, Quantum- and quasi-Plucker coordinates,
\textit{Journal of Algebra} {\bf 296}(2), pp.440-461,
(2006).
}%

\BiblioItem{Lewis D. W. Quaternion algebras}
{
Lewis D. W. Quaternion algebras and the algebraic legacy
of Hamilton's quaternions, \textit{Irish Math. Soc. Bulletin} {\bf
57}, pp. 41-64, (2006).
}%

\BiblioItem{0812.2865}
{
Jos\'e Miguel Figueroa-O'Farrill,
Three lectures on 3-algebras,
eprint \href{http://arxiv.org/abs/0812.2865}{arXiv:0812.2865} (2008)
}%

\BiblioItem{1202.0951}
{
Daniel Edward Clark,
Deconvolution of point processes,
eprint \href{http://arxiv.org/abs/1202.0951}{arXiv:1202.0951} (2012)
}%

\BiblioItem{1202.4546}
{
Ming-Liang Hu,
Disentanglement, Bell-nonlocality violation
and teleportation capacity of the decaying tripartite states,
eprint \href{http://arxiv.org/abs/1202.4546}{arXiv:1202.4546} (2012)
}%

\BiblioItem{1203.1629}
{
Borivoje Dakic, Yannick Ole Lipp, Xiaosong Ma, Martin Ringbauer,
Sebastian Kropatschek, Stefanie Barz, Tomasz Paterek, Vlatko Vedral,
Anton Zeilinger, Caslav Brukner, Philip Walther,
Quantum Discord as Optimal Resource for Quantum Communication,
eprint \href{http://arxiv.org/abs/1203.1629}{arXiv:1203.1629} (2012)
}%

\BiblioItem{Li Nimmo: Darboux transformations}
{
C.X.Li, J.J.C. Nimmo, Darboux transformations for a twisted
derivation and quasideterminant solutions to the super KdV
equation, \textit{Proceedings of the Royal Society A:
Mathematical, Physical and Engineering Sciences} {\bf 466} (2120),
pp. 2471-2493, (2010).
}%

\BiblioItem{Schiebold: Cauchy-type determinants}
{
C. Schiebold, Cauchy-type determinants and integrable
systems, \textit{Linear Algebra and Its Applications} {\bf 433}
(2), pp. 447-475, (2010)
}%

\BiblioItem{Suzuki: Noncommutative spectral decomposition}
{
T. Suzuki, Noncommutative
spectral decomposition with qua\-si\-de\-ter\-mi\-nant, \textit{Advances in
Mathematics} {\bf 217}(5), pp. 2141-2158, (2008).
}%

\BiblioItem{1105.3456}
{
C. W. F. Everitt, D. B. DeBra, B. W. Parkinson, J. P. Turneaure, J. W. Conklin,
M. I. Heifetz, G. M. Keiser, A. S. Silbergleit, T. Holmes, J. Kolodziejczak,
M. Al-Meshari, J. C. Mester, B. Muhlfelder, V. Solomonik, K. Stahl, P. Worden,
W. Bencze, S. Buchman, B. Clarke, A. Al-Jadaan, H. Al-Jibreen, J. Li, J. A. Lipa,
J. M. Lockhart, B. Al-Suwaidan, M. Taber, S. Wang,\\
Gravity Probe B: Final Results of a Space Experiment to Test General Relativity,\\
eprint \href{http://arxiv.org/abs/1105.3456}{arXiv:1105.3456[math-ph]} (2011)
}%

\BiblioItem{0009305}
{
G. S. Asanov.
Can Neutrinos and High-Energy Particles Test Finsler Metric of Space-Time?\\
eprint \href{http://arxiv.org/abs/hep-ph/0009305}{arXiv:hep-ph/0009305} (2000)
}%

\BiblioItem{Asanov 2004}
{
Г. С. Асанов.
Финслероид - пространство с углом и скалярным произведением.\\
Гиперкомплексные числа в геометрии и физике, {\bf 1}, 2004, с. 43 - 67
}%

\BiblioItem{1004.3007}
{
Sergiu I. Vacaru,
Principles of Einstein-Finsler Gravity and Perspectives in Modern Cosmology,\\
eprint \href{http://arxiv.org/abs/1004.3007}{arXiv:1004.3007[gr-qc]} (2010)
}%

\BiblioItem{1012.4148}
{
Sergiu I. Vacaru.
Principles of Einstein-Finsler Gravity and Cosmology.\\
eprint \href{http://arxiv.org/abs/1012.4148}{arXiv:1012.4148[physics.gen-ph]} (2010)
}%

\BiblioItem{1112.5641}
{
Christian Pfeifer, Mattias N.R. Wohlfarth.
Finsler geometric extension of Einstein gravity.\\
eprint \href{http://arxiv.org/abs/1112.5641}{arXiv:1112.5641[gr-qc]} (2011)
}%

\BiblioItem{0711.0056}
{
Zhe Chang, Xin Li.
Lorentz Invariance Violation and Symmetry in Randers\Hyph Finsler Spaces.\\
eprint \href{http://arxiv.org/abs/0711.0056}{arXiv:0711.0056[hep-th]} (2011)
}%

\BiblioItem{Zharinov Kursy NOC, 9}
{
V. V. Zharinov,
Algebraic and geometric foundation of mathematical physics.
\\
Lekts. Kursy NOC, 9, Steklov Math. Institute of RAS, Moscow, 2008, 3–209 
}%

\BiblioItem{Rund Finsler geometry}
{
Х. Рунд,
Дифференциальная геометрия финслеровых пространств.
\\
Перевод с английского Г. С. Асанова под редакцией Э. Г. Позняка,
М., Наука, 1981
}%

\BiblioItem{Smirnov vol 1}
{
В. И. Смирнов,
Курс высшей математики, том первый.
\\
М., Наука, 1974
}%

\BiblioItem{Beem Dostoglou Ehrlich}
{
John K. Beem, Stamatis A. Dostoglou, Paul E. Ehrlich,
Advances in differential geometry and general relativity.
\\
American Mathematical Society, 2004
}%

\BiblioItem{978-0719033414}
{
Malcolm Pemberton, Nicholas Rau,
Mathematics for economists: an introductory textbook.
\\
Manchester University Press, November 2001; ISBN-13: 978-0719033414
}%

\BiblioItem{0 521 59180 5}
{
Cyrus D. Cantrell,
Modern mathematical methods for physicists and engineers.
\\
Cambridge University Press, 2000
}%

\BiblioItem{Arveson spectral theory}
{
William Arveson,
A short course on spectral theory.
\\
Springer - Verlag, New York, 2002
}%

\BiblioItem{Robert Hermann}
{
Robert Hermann,
Topics in the mathematics of quantum mechanics.
\\
Math Sci Press, 1973
}%

\BiblioItem{9705.009}%q-alg-9705009
{
John C. Baez,
An Introduction to n-Categories,\\
eprint \href{http://arxiv.org/abs/q-alg/9705009}{arXiv:q-alg/9705009} (1997)
}%

\BiblioItem{0105.155}
{
John C. Baez,
The Octonions,\\
eprint \href{http://arxiv.org/abs/math.RA/0105155}{arXiv:math.RA/0105155} (2002)
}%

\BiblioItem{John Baez: Math Blogs}
{
John C. Baez,
What do mathematicians need to know about blogging?,\\
Notices of the American Mathematical Society,
(2010), 3, {\bf 57}, 333,\\
\url{http://www.ams.org/notices/201003/rtx100300333p.pdf}
}%

\BiblioItem{Tolstoi about Anna Karenina}
{
Константин Паустовский. Золотая роза, в сборнике Книга скитаний.
Картя молдовеняскэ, Кишинёв, 1978
}%
%Л. Н. Толстой в воспоминаниях современиков, т. 1, М. 1955, с. 231 - 232

\BiblioItem
{Cohn: Universal Algebra}
{
П. Кон,
Универсальная алгебра,
М., Мир, 1968
}%

\BiblioItem
{Cohn: Algebra 1}
{
Paul M. Cohn,
Algebra, Volume 1,
John Wiley \& Sons, 1982
}%

\BiblioItem
{Cohn: Algebra 3}
{
Paul M. Cohn,
Algebra, Volume 3,
John Wiley \& Sons, 1991
}%

\BiblioItem
{Cohn: Skew Fields}
{
Paul M. Cohn,
Skew Fields,
Cambridge University Press, 1995
}%

\BiblioItem
{Lam: Noncommutative Rings}
{
T. Y. Lam,
A First Course in
Noncommutative Rings,
Springer-Verlag, 1991
}%

\BiblioItem
{Maunder: Algebraic Topology}
{
C. R. F. Maunder,
Algebraic Topology,
Dover Publications, Inc, Mineola, New York, 1996
}%

\BiblioItem{Pommaret: Partial Differential Equations}
{
Ж. Поммаре,
Системы уравнений с частными производными и псевдогруппы Ли,
М., Мир, 1983
}%

\BiblioItem{Bourbaki: Set Theory}
{
Н. Бурбаки,
Теория множеств, перевод с французского Г. Н. Поварова и Ю. А.
Шихановича под редакцией В. А. Успенского,
М. Мир, 1965
}%

\BiblioItem{Bourbaki: Algebra 1}
{
Н. Бурбаки,
Алгебра: алгебраические структуры, линейная и полилинейная алгебра,
перевод с французского Д. А. Райкова,
М.,
государственное издательство физико\Hyph математической литературы, 1962
}%

\BiblioItem{Bourbaki: Algebra 2}
{
Н. Бурбаки,
Алгебра: алгебраические структуры, линейная и полилинейная алгебра,
перевод с французского Д. А. Райкова,
М.,
государственное издательство физико\Hyph математической литературы, 1962
}%

\BiblioItem
{Bourbaki: General Topology 1}
{
Н. Бурбаки,
Общая топология, основные структуры,
перевод с французского Д. А. Райкова,
М. Наука, 1968
}

\BiblioItem{Bourbaki: General Topology: Chapter 3 - 8}
{
Н. Бурбаки,
Общая топология. Топологические группы.
Числа и связанные с ними группы и пространства.
\\
перевод с французского С. Н. Крачковского под редакцией Д. А. Райкова,
\\
М. Наука, 1975
}

\BiblioItem{Bourbaki: General Topology: Chapter 5 - 10}
{
Н. Бурбаки,
Общая топология. Использование вещественных чисел в общей топологии.
\\
перевод с французского С. Н. Крачковского под редакцией Д. А. Райкова,
\\
М. Наука, 1975
}

\BiblioItem{Bourbaki: Topological Vector Space}
{
Н. Бурбаки,
Топологические векторные пространства,
перевод с французского Д. А. Райкова,
М. Иностранная литература, 1959
}

\BiblioItem{Bourbaki: Coxeter Group Lie}
{
Н. Бурбаки,
Группы и алгебры Ли, главы 4 - 6,
Перевод с французского А. И. Кострикина и А. Н. Тюрина
под редакцией А. И. Кострикина,
М. Мир, 1986
}

\BiblioItem{Bourbaki: Real Group Lie}
{
Н. Бурбаки,
Группы и алгебры Ли, Компактные вещественные группы,
Перевод с французского И. А. Кострикина под редакцией А. А. Кирилова,
М. Мир, 1986
}

\BiblioItem{Shabat: Complex Analysis}
{
Шабат Б. В.,
Введение в комплексный анализ,
М. Наука, 1969
}

\BiblioItem{Pontryagin: Topological Group}
{
Понтрягин Л. С.,
Непрерывные группы,
М. Едиториал УРСС, 2004
}

\BiblioItem
{Eisenhart: Riemannian Geometry}
{
Eisenhart,
Riemannian Geometry,
Princeton University Press, Princeton, 1949
}

\BiblioItem
{Eisenhart: Continuous Groups of Transformations}
{
Л. П. Эйзенхарт,
Непрерывные группы преобразований,
перевод с английского М. М. Постникова,
М., Иностранная литература, 1947
}

\BiblioItem
{Condon Odabasi}
{
Edward Uhler Condon, Halis Odabasi,
Atomic Structure,
CUP Archive, 1980
}

\BiblioItem{Postnikov: Differential Geometry}
{
Постников М. М.,
Лекции по геометрии, семестр IV, Дифференциальная геометрия,
М. Наука, 1983
}

\BiblioItem{Fikhtengolts: Calculus volume 1}
{
Фихтенгольц Г. М.,
Курс дифференциального и интегрального исчисления, том 1,
М. Наука, 1969
}

\BiblioItem{Fikhtengolts: Calculus volume 2}
{
Фихтенгольц Г. М.,
Курс дифференциального и интегрального исчисления, том 2,
М. Наука, 1969
}

\BiblioItem{Fikhtengolts: Calculus volume 3}
{
Фихтенгольц Г. М.,
Курс дифференциального и интегрального исчисления, том 3,
М. Наука, 1969
}

\BiblioItem{Hatcher: Algebraic Topology}
{
Allen Hatcher,
Algebraic Topology,
Cambridge University Press, 2002
}

\BiblioItem{geometry of differential equations}
{
А. М. Виноградов, И. С. Красильщик, В. В. Лычагин,
Введение в геометрию нелинейных дифференциальных уравнений,
М. Наука, 1986
}

\BiblioItem{Basic Concepts of Differential Geometry}
{
Алексеевский Д. В., Виноградов А. М., Лычагин В. В.,
Основные понятия дифференциальной геометрии
\\
Итоги ВИНИТИ 28
\\
М. ВИНИТИ, 1988
}

\BiblioItem{cohomological analysis}
{
A. M. Vinogradov,
Cohomological Analysis of Partial Differential Equations
and Secondary Calculus,
American Mathematical Society, 2001
}

\BiblioItem{0801.1734}
{
Brandon S. DiNunno, Richard A. Matzner,
The Volume Inside a Black Hole,\\
eprint \href{http://arxiv.org/abs/0801.1734v1}{arXiv:0801.1734v1} (2008)
}

\BiblioItem{0702.447}
{
Ivan Kyrchei,
Cramer's rule for some quaternion matrix equations,\\
eprint \href{http://arxiv.org/abs/math/0702447}{arXiv:math.RA/0702447} (2007)
}

\BiblioItem{Izrail M. Gelfand: Quaternion Groups}
{
I. M. Gelfand, M. I. Graev,
Representation of Quaternion Groups over Localy Compact and
Functional Fields,\\
Functs. Anal. Prilozh. {\bf 2} (1968) 20 - 35;\\
Izrail Moiseevich Gelfand, Semen Grigorevich Gindikin,\\
Izrail M. Gelfand: Collected Papers, volume II, 435 - 449,\\
Springer, 1989
}

\BiblioItem{Richard D. Schafer}
{
Richard D. Schafer,
An Introduction to Nonassociative Algebras,
Dover Publications, Inc., New York, 1995
}

\BiblioItem{Bamberg Sternberg}
{
Paul Bamberg, Shlomo Sternberg,
A course in mathematics for students of physics,
Cambridge University Press, 1991
}

\BiblioItem{Conway Smith}
{
John Horton Conway, Derek Alan Smith,
On quaternions and octonions: their geometry, arithmetic, and symmetry,
A K Peters, Natick, Massachussets, 2003
}

\BiblioItem{Fueter}
{
Fueter, R.
Die Funktionentheorie der Differentialgleichungen $\Delta u = 0$ und
$\Delta \Delta u = 0$ mit vier reellen Variablen.
Comment. Math. Helv. {\bf 7} (1935), 307-330
}

\BiblioItem{Sudbery Quaternionic Analysis}
{
A. Sudbery,
Quaternionic Analysis,
Math. Proc. Camb. Phil. Soc. (1979), {\bf 85}, 199 - 225
}

\BiblioItem{0902.4771}
{
Fabrizio Colombo, Graziano Gentili, Irene Sabadini,
A Cauchy kernel for slice regular functions,\\
eprint \href{http://arxiv.org/abs/0902.4771v1}{arXiv:0902.4771v1} (2009)
}

\BiblioItem{Vadim Komkov}
{
Vadim Komkov,
Variational Principles of Continuum Mechanics with Engineering Applications: Critical Points Theory,\\
Springer, 1986
}

\BiblioItem{Alain Connes 1994}
{
Alain Connes,
Noncommutative Geometry,\\
Academic Press, 1994
}

\BiblioItem{Hamilton papers 3}
{
Sir William Rowan Hamilton,
The Mathematical Papers, Vol. III, Algebra,\\
Cambridge at the University Press, 1967
}

\BiblioItem{Hamilton Elements of Quaternions 1}
{
Sir William Rowan Hamilton,
Elements of Quaternions, Volume I,\\
Longmans, Green, and Co., London, New York, and Bombay, 1899
}

\BiblioItem{Cartan geometry in reper}
{
Эли Картан,
Риманова геометрия в ортогональном репере,
По лекциям Эли Картана, читанным в Сорбонне в 1926 - 1927 гг.,\\
перевод и редакция проф. С. П. Финикова,\\
издательство МГУ, 1960
}

\BiblioItem{Cartan differential form}
{
Анри Картан.
Дифференцииальное исчисление. Дифференциальные формы.\\
М. Мир, 1971
}

\BiblioItem{Arnautov Glavatsky Mikhalev}
{
V. I. Arnautov, S. T. Glavatsky, A. V. Mikhalev,\\
Introduction to the theory of topological rings and modules,
Volume 1995,\\
Marcel Dekker, Inc, 1996
}

\BiblioItem{Moore Yaqub}
{
Hal G. Moore, Adil Yaqub,
A first course in linear algebra with applications,
Edition 3, Academic Press, 1998 
}

\BiblioItem{math.CV-0405471}
{
S. V. Ludkovsky,
Differentiable functions of Cayley-Dickson numbers,\\
eprint \href{http://arxiv.org/abs/math.CV/0405471}{arXiv:math.CV/0405471} (2004)
}%

\BiblioItem{W.Bertram H.Glockner K.Neeb}
{
W.Bertram, H.Glockner, K.Neeb,
Differential Calculus over General Base Fields and Rings,
Expositiones Mathematicae (2004), Volume 22, Issue 3, Pages 213-282
}

\CloseBiblio



==> Calculus.16.Absract.Russian.tex <==
%auto-ignore

\input{Calculus.16.Absract.Eq}
%\def\KeyWords{ассоциативная алгебра; частное; остаток}

\begin{abstract}
Пусть $A$, $B$ - банаховые $D$\Hyph алгебры.% с нормой $\|a\|$.
Отображение
\ShowEq{f:A->B abs}
дифференцируемо
на множестве $U\subset A$,
если в каждой точке $x\in U$
изменение отображения
$f$ может быть представлено в виде
\ShowEq{derivative of map def}
где
\ShowEq{df:A->B abstract}
линейное отображение и
\ShowEq{map o:A->B}
такое непрерывное отображение, что
\ShowEq{derivative of map, algebra, 2}
Линейное отображение
$\displaystyle\frac{d f(x)}{d x}$
называется
производной отображения
$f$.

Рассмотренна теория дифференциальных форм в банаховой алгебре.
Дифференциальная форма
\ShowEq{omega in A->B}
определена отображением
\ShowEq{g:A->BxB}
Если отображение $g$
является производной отображения
\ShowEq{f:A->B abs},
то отображение $f$ называется неопределённым интегралом отображения $g$
\ShowEq{f=int g abs}
В этом случае, для любых $A$\Hyph чисел $a$, $b$,
мы определим определённый интеграл с помощью равенства
\ShowEq{definite integral omega ab}
для любого пути $\gamma$ из $a$ в $b$.
\end{abstract}



==> Derivative.16.Russian.tex <==
%auto-ignore

\input{Derivative.16.Eq}

\Chapter{Дифференцируемые отображения}
\labelChapter{Differentiable maps}

\Section{Топологическое кольцо}
\labelSection{Topological Ring}

\begin{definition}
Кольцо $D$ называется 
\AddIndex{топологическим кольцом}{topological ring}\,\footnote{
Определение дано согласно
определению из \citeBib{Pontryagin: Topological Group},
глава 4},
если $D$ является топологическим пространством, и алгебраические операции,
определённые в $D$, непрерывны в топологическом пространстве $D$.
\qed
\end{definition}

Согласно определению, для произвольных элементов $a$, $b\in D$
и для произвольных окрестностей $W_{a-b}$ элемента $a-b$,
$W_{ab}$ элемента $ab$ существуют такие окрестности $W_a$
элемента $a$ и $W_b$ элемента $b$, что $W_a-W_b\subset W_{a-b}$,
$W_aW_b\subset W_{ab}$.

\begin{definition}
\labelDefinition{norm on ring}
\AddIndex{Норма на кольце}{norm on ring}
$D$ - это отображение\,\footnote{
Определение дано согласно определению из
\citeBib{Bourbaki: General Topology: Chapter 5 - 10},
гл. IX, \S 3, п${}^\circ$2,
а также согласно определению
\citeBib{Arnautov Glavatsky Mikhalev}-1.1.12,
с. 23.}
\[d\in D\rightarrow |d|\in R\]
такое, что
\begin{itemize}
\item $|a|\ge 0$
\item $|a|=0$ равносильно $a=0$
\item $|ab|=|a|\ |b|$
\item $|a+b|\le|a|+|b|$
\end{itemize}

Кольцо $D$, наделённое структурой, определяемой заданием на
$D$ нормы, называется
\AddIndex{нормированным кольцом}{normed ring}.
\qed
\end{definition}

Инвариантное расстояние на аддитивной группе кольца $D$
\[d(a,b)=|a-b|\]
определяет топологию метрического пространства,
согласующуюся со структурой кольца в $D$.

\begin{definition}
\labelDefinition{limit of sequence, normed ring}
Пусть $D$ - нормированное кольцо.
Элемент $a\in D$ называется 
\AddIndex{пределом последовательности}{limit of sequence}
\ShowEq{limit of sequence, normed ring}
если для любого $\epsilon\in R$, $\epsilon>0$,
существует, зависящее от $\epsilon$, натуральное число $n_0$ такое,
что
\ShowEq{an-a}
для любого $n>n_0$.
\qed
\end{definition}

\begin{theorem}
\labelTheorem{limit of sequence, normed ring, product on scalar}
Пусть $D$ - нормированное кольцо характеристики $0$ и пусть $d\in D$.
Пусть $a\in D$ - предел последовательности $\{a_n\}$.
Тогда
\[
\lim_{n\rightarrow\infty}(a_nd)=ad
\]
\[
\lim_{n\rightarrow\infty}(da_n)=da
\]
\end{theorem}
\begin{proof}
Утверждение теоремы тривиально, однако я привожу доказательство
для полноты текста. 
Поскольку $a\in D$ - предел последовательности $\{a_n\}$,
то согласно определению
\RefDefinition{limit of sequence, normed ring}
для заданного $\epsilon\in R$, $\epsilon>0$,
существует натуральное число $n_0$ такое, что
\ShowEq{an-a d}
для любого $n>n_0$.
Согласно определению \RefDefinition{norm on ring}
утверждение теоремы следует из неравенств
\ShowEq{an-a d1}
для любого $n>n_0$.
\end{proof}

\begin{definition}
Пусть $D$ - нормированное кольцо.
Последовательность $\{a_n\}$, $a_n\in D$ называется 
\AddIndex{фундаментальной}{fundamental sequence}
или \AddIndex{последовательностью Коши}{Cauchy sequence},
если для любого $\epsilon\in R$, $\epsilon>0$
существует, зависящее от $ \epsilon$, натуральное число $n_0$ такое,
что $|a_p-a_q|<\epsilon$ для любых $p$, $q>n_0$.
\qed
\end{definition}

\begin{definition}
Нормированное кольцо $D$ называется 
\AddIndex{полным}{complete ring}
если любая фундаментальная последовательность элементов
данного кольца сходится, т. е.
имеет предел в этом кольце.
\qed
\end{definition}

В дальнейшем, говоря о нормированном кольце характеристики $0$,
мы будем предполагать, что определён гомеоморфизм поля рациональных
чисел $Q$ в кольцо $D$.

\begin{theorem}
\labelTheorem{complete ring contains real number}
Полное кольцо $D$ характеристики $0$
содержит в качестве подполя изоморфный образ поля $R$
действительных чисел.
Это поле обычно отождествляют с $R$.
\end{theorem}
\begin{proof}
Рассмотрим фундаментальную последовательность рациональных чисел $\{p_n\}$.
Пусть $p'$ - предел этой последовательности в кольце $D$.
Пусть $p$ - предел этой последовательности в поле $R$.
Так как вложение поля $Q$ в тело $D$ гомеоморфно,
то мы можем отождествить $p'\in D$ и $p\in R$.
\end{proof}

\begin{theorem}
\labelTheorem{complete ring and real number}
Пусть $D$ - полное кольцо характеристики $0$ и пусть $d\in D$.
Тогда любое действительное число $p\in R$ коммутирует с $d$.
\end{theorem}
\begin{proof}
Мы можем представить действительное число $p\in R$ в
виде фундаментальной последовательности рациональных чисел $\{p_n\}$.
Утверждение теоремы следует из цепочки равенств
\ShowEq{complete ring and real number}
основанной на утверждении теоремы
\RefTheorem{limit of sequence, normed ring, product on scalar}.
\end{proof}

\Section{Топологическая \texorpdfstring{$D$}{D}-алгебра}

\begin{definition}
\labelDefinition{norm on D module}
Пусть $D$ - нормированное коммутативное кольцо.\,\footnote{Определение
дано согласно
определению из \citeBib{Bourbaki: General Topology: Chapter 5 - 10},
гл. IX, \S 3, п${}^\circ$3.
Для нормы мы пользуемся обозначением $|a|$ или $\|a\|$.
}
\AddIndex{Норма в $D$\Hyph модуле}
{norm on D module} $A$
 - это отображение
\ShowEq{norm on D module}
такое, что
\StartLabelItem
\begin{enumerate}
\ShowEq{norm on D module 1}
\ShowEq{norm on D module 2, 1}
равносильно
\ShowEq{norm on D module 2, 2}
\ShowEq{norm on D module 3}
\end{enumerate}
$D$\Hyph модуль $A$,
наделённый структурой, определяемой заданием на
$A$ нормы, называется
\AddIndex{нормированным $D$\Hyph модулем}{normed D module}.
\qed
\end{definition}

\ShowEq{=module}

\ShowDefinition{open ball}

\ShowDefinition{closed ball}

\begin{theorem}
\labelTheorem{b in Bar}
\ShowEq{b in Bar}
тогда и только тогда, когда
\ShowEq{b-a in Br}
\end{theorem}
\begin{proof}
Теорема является следствием определения
\RefDefinition{closed ball}.
\end{proof}

%\begin{definition}
%Пусть $A$
%- нормированный $D$\Hyph модуль.
%Множество
%\ShowEq{B subset A}{}
%называется
%\AddIndex{открытым}{open set},
%если для любого $A$\Hyph числа $a\in B$
%существует открытый шар
%\ShowEq{B(a)in B}
%\qed
%\end{definition}

%\begin{theorem}
%Норма $\|x\|$,
%определённая на $D$\Hyph модуле $A$,
%порождает топологию, определённую
%множеством открытых множеств.
%\end{theorem}
%\begin{proof}
%\end{proof}

\ShowDefinition{limit of sequence}

\ShowTheorem{limit of sequence}
\ShowProof{limit of sequence}

\ShowDefinition{fundamental sequence}

\ShowTheorem{fundamental sequence}
\ShowProof{fundamental sequence}

\begin{definition}
Нормы\,\footnote{
Смотри также определение
\citeBib{Shilov single 3}\Hyph 12.35.а
на странице 53.
}
\ShowEq{|1,|2},
определённые на $D$\Hyph модуле $A$,
называются
\AddIndex{эквивалентными}{equivalent norms},
%если они порождают одну и туже топологию.
если утверждение
\DrawEq{a=lim an}{}
не зависит от выбранной нормы.
\qed
\end{definition}

%\begin{theorem}
%Пусть нормы\,\footnote{
%Смотри также замечание к определению
%\citeBib{Shilov single 3}\Hyph 12.35.а
%на странице 53.
%}
%\ShowEq{|1,|2},
%определённые на $D$\Hyph модуле $A$,
%эквивалентны.
%\end{theorem}
%\begin{proof}
%\end{proof}

В теоремах
\RefTheorem{B1o in B2o},
мы рассмотрим нормы
\ShowEq{|1,|2},
определённые на $D$\Hyph модуле $A$.
Мы также будем рассматривать открытые и замкнутые шары
\ShowEq{B1o,B2o}

\begin{theorem}
\labelTheorem{B1o in B2o}
Нормы\,\footnote{
Смотри также лемму
\citeBib{Shilov single 3}\Hyph 12.35.б
на странице 54.
}
\ShowEq{|1,|2},
определённые на $D$\Hyph модуле $A$,
эквивалентны тогда и только тогда, когда
существуют постоянные
\ShowEq{c12>0}
такие, что для любого $\rho>0$
\ShowEq{cB1c in B2c}
\ShowEq{cB2c in B1c}
\end{theorem}
\begin{proof}
Пусть постоянные $c_1$, $c_2$ существуют.
Пусть
\DrawEq{a=lim an}{}
по норме $\|x\|_1$.
Согласно теоремам
\RefTheorem{b in Bar},
\RefTheorem{limit of sequence, normed module}
и определениям
\RefDefinition{open ball},
\RefDefinition{closed ball},
для любого
\ShowEq{epsilon in R}
существует натуральное число $n_0$ такое, что
\ShowEq{a-an in B1e}
Утверждение
\ShowEq{a-an in B2}
является следствием утверждений
\EqRef{cB1c in B2c},
\EqRef{a-an in B1e}
и определения
\RefDefinition{closed ball}.
Согласно теореме
\RefTheorem{limit of sequence, normed module}
\DrawEq{a=lim an}{}
по норме $\|x\|_2$.

Аналогичным образом мы доказываем, что утверждение
\DrawEq{a=lim an}{}
по норме $\|x\|_1$
является следствием утверждения
\DrawEq{a=lim an}{}
по норме $\|x\|_2$.

Пусть нормы
\ShowEq{|1,|2}{}
эквивалентны.
Пусть не существует константы $c_2$ такой, что утверждение
\EqRef{cB2c in B1c}
верно.
Тогда для любого
\ShowEq{n,1.}
мы найдём замкнутые шары
\ShowEq{B1rn B2rn}
такие, что
\ShowEq{cB2c not in B1c}
Из утверждения
\EqRef{cB2c not in B1c}
и определения
\RefDefinition{closed ball},
следует, что существует $x_n$ такой, что
\ShowEq{xn rn <>}
Пусть
\ShowEq{yn=xn/n}
Из равенства
\EqRef{yn=xn/n}
и утверждений
\RefItem{norm on D module 3, 2},
\EqRef{xn rn <>}
следует, что
\ShowEq{yn rn <>}
Из утверждения
\EqRef{yn rn <>}
следует, что утверждение
\ShowEq{lim y =0}
верно относительно нормы $\|x\|_2$ и
не верно относительно нормы $\|x\|_1$.
Это противоречит утверждению о эквивалентности норм,
следовательно, константа $c_2$ существует.
Аналогичным образом мы доказываем, что константа $c_1$ существует.
\end{proof}

\begin{theorem}
\labelTheorem{Norms are equivalent iff |1<|2<|1}
Нормы\,\footnote{
Смотри также следствие
\citeBib{Shilov single 3}\Hyph 12.35.в
на странице 54.
Смотри также определение
\citeBib{8176-4374}\Hyph 9.9
и утверждение
\citeBib{8176-4374}\Hyph 9.10
на странице 288.
}
\ShowEq{|1,|2},
определённые на $D$\Hyph модуле $A$,
эквивалентны тогда и только тогда, когда
существуют постоянные
\ShowEq{c12>0}
такие, что для любого $x\in A$
\ShowEq{|1<|2<|1}
\end{theorem}
\begin{proof}
Согласно теореме
\RefTheorem{B1o in B2o},
существуют постоянная
$c_1$
такая, что
для
\ShowEq{r=x|1}
\ShowEq{B1x in B2x}
Утверждение
\ShowEq{|2<|1}
является следствием утверждения
\EqRef{B1x in B2x}.
Согласно теореме
\RefTheorem{B1o in B2o},
существуют постоянная
$c_2$
такая, что
для
\ShowEq{r=x|2}
\ShowEq{B2x in B1x}
Утверждение
\ShowEq{|1<|2}
является следствием утверждения
\EqRef{B2x in B1x}.
Утверждение
является следствием утверждений
\EqRef{|2<|1},
\EqRef{|1<|2}.
\end{proof}

\begin{definition}
Нормированный $D$\Hyph модуль $A$ называется 
\AddIndex{банаховым $D$\Hyph модулем}{Banach module}
если любая фундаментальная последовательность элементов
модуля $A$ сходится, т. е.
имеет предел в модуле $A$.
\qed
\end{definition}

\ifx\texFuture\Defined
\begin{definition}
Пусть $D$ - топологическое коммутативное кольцо.
$D$\Hyph алгебра $A$ называется 
\AddIndex{топологической $D$\Hyph алгеброй}
{topological D algebra}\,\footnote{
Определение дано согласно
определению из \citeBib{Bourbaki: Topological Vector Space},
с. 21},
если $A$ наделено топологией, согласующейся со
структурой аддитивной группы в $A$,
и отображения
\ShowEq{topological D algebra}
непрерывны.
\qed
\end{definition}
\fi

\begin{definition}
\labelDefinition{continuous map, algebra}
Отображение
\ShowEq{f:A->B}f{A_1}{A_2}
банахового $D_1$\Hyph модуля $A_1$ с нормой $|x|_1$
в банаховый $D_2$\Hyph модуль $A_2$ с нормой $|y|_2$
называется \AddIndex{непрерывным}{continuous map}, если
для любого сколь угодно малого $\epsilon>0$
существует такое $\delta>0$, что
\[
|x'-x|_1<\delta
\]
влечёт
\[
|f(x')-f(x)|_2<\epsilon
\]
\qed
\end{definition}

\ShowTheorem{set of A->B is D module}
\begin{proof}
Мы определим сумму отображений
\ShowEq{fg in BA}
согласно равенству
\ShowEq{(f+g)(a)=}
Согласно определению
\RefDefinition{module over commutative ring},
множество $B^A$ является абелевой группой.
Мы определим представление кольца $D$
в абелевой группе $B^A$
согласно равенству
\ShowEq{(df)(a)=}
Мы можем записывать равенство
\EqRef{(df)(a)=},
не пользуясь скобками.
Следовательно, утверждение
\RefItem{norm of map}
верно.

Утверждения
\RefItem{norm on D module 1},
\RefItem{norm on D module 2}
очевидны для величины $\|f\|$.
Утверждение
\RefItem{norm on D module 3, 1}
является следствием неравенства
\ShowEq{|(f+g)(a)|<}
и определения
\EqRef{norm of map, algebra}.
Утверждение
\RefItem{norm on D module 3, 2}
для величины $\|f\|$
является следствием равенства
\EqRef{(df)(a)=},
утверждения
\RefItem{norm on D module 3, 2}
для величины $\|a\|_B$
и определения
\EqRef{norm of map, algebra}.
Следовательно, утверждение
\RefItem{set of A->B is D module}
верно.
\end{proof}

\begin{theorem}
Пусть
\ShowEq{f:A->B}f{A_1}{A_2}
линейное отображение банахового $D$\Hyph модуля $A_1$ с нормой $|x|_1$
в банаховый $D$\Hyph модуль $A_2$ с нормой $|y|_2$.
Тогда
\ShowEq{norm of linear map, algebra}
\end{theorem}
\begin{proof}
Из определений
\EqParm{ref definition linear map from A1 to A2}{=z}
и теорем
\RefTheorem{complete ring contains real number},
\RefTheorem{complete ring and real number}
следует
\ShowEq{linear map and real number}
Из равенства \EqRef{linear map and real number}
и определения \RefDefinition{norm on d algebra}
следует
\ShowEq{linear map and real number, 1}
Полагая $\displaystyle r=\frac 1{|x|_1}$, мы получим
\ShowEq{norm of linear map, algebra, 1}
Равенство \EqRef{norm of linear map, algebra}
следует из равенств \EqRef{norm of linear map, algebra, 1}
и \EqRef{norm of map, algebra}.
\end{proof}

\begin{theorem}
Пусть
\ShowEq{f:A->B}f{A_1}{A_2}
линейное отображение банахового $D_1$\Hyph модуля $A_1$ с нормой $|x|_1$
в банаховый $D_2$\Hyph модуль $A_2$ с нормой $|y|_2$.
Отображение $f$ непрерывно, если $\|f\|<\infty$.
\end{theorem}
\begin{proof}
Поскольку отображение $f$ линейно, то
согласно теореме \RefTheorem{set of A->B is D module}
\[
|f(x)-f(y)|_2=|f(x-y)|_2\le \|f\|\ |x-y|_1
\]
Возьмём произвольное $\epsilon>0$. Положим
\ShowEq{delta=epsilon/|f|}
Тогда из неравенства
\[
|x-y|_1<\delta
\]
следует
\[
|f(x)-f(y)|_2\le \|f\|\ \delta=\epsilon
\]
Согласно определению \RefDefinition{continuous map, algebra}
отображение $f$ непрерывно.
\end{proof}

\begin{theorem}
\labelTheorem{L(A;B) is Banach module}
Пусть $A$ - банаховый $D$\Hyph модуль с нормой $|x|_A$.
Пусть $B$ - банаховый $D$\Hyph модуль с нормой $|y|_B$.
$D$\Hyph модуль
\ShowEq{L(A;B)}DAB,
оснащённый нормой
\ShowEq{norm of map to algebra}
является банаховым $D$\Hyph модулем.
\end{theorem}
\begin{proof}
Для доказательства теоремы мы должны доказать,
что предел последовательности линейных отображений
является линейным отображением.
Утверждение является следствием равенств
\ShowEq{lim f(a+b)=}
\ShowEq{lim f(ca)=}
\end{proof}

\ShowDefinition{norm of polylinear map}

\ShowTheorem{|f(a)|<|f||a| 1n}
\ShowProof{|f(a)|<|f||a| 1n}

\ShowTheorem{|on|->0 ona1p->0}
\ShowProof{|on|->0 ona1p->0}

Согласно определению
\RefDefinition{algebra over ring},
$D$\Hyph алгебра $A$ - это
$D$\Hyph модуль $A$,
на котором задано билинейное отображение
\ShowEq{*:AA->A}
называемое произведением.
Вообще говоря, норма $\|*\|$ произведения отлична от $1$.

\ShowEq{def H2}
\begin{example}
\labelExample{algebra of hyperbolic numbers}
{\it
Пусть\,\footnote{
Я признателен замечанию, сделанному Натаном БиДел,
где он обратил моё внимание,
что существуют алгебры,
в которых норма $\|*\|$ произведения отлична от $1$.
Пример
\RefExample{algebra of hyperbolic numbers}
опирается на определение
\citeBib{1708.01190}\Hyph 3.1
на странице 3
в статье
\citeBib{1708.01190}
Натана БиДел.
Смотри также определение на странице
\citeBib{978-0-8176-8384-9}\Hyph 24.
}
\HH\ - алгебра гиперболических чисел.
\HH\Hyph число имеет вид
\ShowEq{H2 number}{},
где $a$, $b$ - действительные числа.
Произведение \HH\Hyph чисел
\ShowEq{H2 number}1,
\ShowEq{H2 number}2{}
имеет вид
\ShowEq{product hyperbolic numbers}
Из равенства
\EqRef{product hyperbolic numbers}
следует, что $j^2=1$.
Рассмотрим норму\,\footnote{
Эта норма предложена в
\citeBib{978-0-8176-8384-9}
на странице 25.
}
\HH\Hyph числа
\ShowEq{H2 number}{},
определенную равенством
\ShowEq{H2 number norm}

Из равенств
\EqRef{product hyperbolic numbers},
\EqRef{H2 number norm}
следует, что норма произведения имеет значение
\ShowEq{norm hyperbolic numbers product}
%Естественно предположить, что отображение $f$ имеет максимум, когда
%\ShowEq{map f has maximum when}
Следовательно, $\|*\|=1$ в алгебре \HH.
}
\qed
\end{example}

\begin{example}
{\it
Норма $\|x\|$ \HH\Hyph числа,
рассмотренная в примере
\RefExample{algebra of hyperbolic numbers},
не удовлетворяет утверждению
\RefItem{norm on D module 2}.\,\footnote{
Garret Sobczyk обратил наше внимание, что эта норма
соответствует геометрии пространства событий в специальной теории относительности.
}
Поэтому мы рассмотрим другую норму.
Если норма \HH\Hyph числа
\ShowEq{H2 number}{}{}
определена равенством
\ShowEq{H2 number norm 1}
то норма произведения равна максимуму отображения
\ShowEq{norm of product is maximum of map}
Отображение $f$ симметрично по переменным, поэтому достигает своего экстремума,
когда значения переменных равны.
Пусть
\ShowEq{x1...=}
Тогда
\ShowEq{faaaa=}
Это значение максимально, так как
\ShowEq{f1010=}
Следовательно,
\ShowEq{|*|=v2}
}
\qed
\end{example}

Согласно теореме
\RefTheorem{Norms are equivalent iff |1<|2<|1},
если в алгебре \HH\ определена норма $\|x\|_1$,
то любая норма $\|x\|_2$, определённая равенством
\ShowEq{|2=r|1}
эквивалентна норме $\|x\|_1$.

\begin{theorem}
\labelTheorem{there exists equivalent norm |*|=1}
Пусть $A$ - $D$\Hyph алгебра.
Если в $D$\Hyph модуле $A$ определена норма $\|x\|_1$ такая, что
норма $\|*\|_1$ произведения в $D$\Hyph алгебре $A$ отлична от $1$,
то в $D$\Hyph модуле $A$ существует эквивалентная норма
\ShowEq{|2=*|1 |1}
такая, что
\ShowEq{|*|2=1}
\end{theorem}
\begin{proof}
Равенство
\ShowEq{|*|2=1 1}
является следствием равенств
\EqRef{norm of map, module},
\EqRef{|2=*|1 |1}.
Равенство
\EqRef{|*|2=1}
является следствием равенства
\EqRef{|*|2=1 1}.
\end{proof}

Согласно теореме
\RefTheorem{there exists equivalent norm |*|=1},
если в алгебре \HH\ определить норму
\ShowEq{|2=v2|1}
то норма произведения $\|*\|_2=1$.

\begin{definition}
\labelDefinition{norm on d algebra}
Пусть $D$ - нормированное коммутативное кольцо.
Пусть $A$ - $D$\Hyph алгебра.
Норма\,\footnote{
Определение дано согласно
определению из \citeBib{Bourbaki: General Topology: Chapter 5 - 10},
гл. IX, \S 3, п${}^\circ$3.
Если $D$\Hyph алгебра $A$ является алгеброй с делением,
то норма называется
\AddIndex{абсолютной величиной}{absolute value}
и мы пользуемся записью $|a|$ для нормы $A$\Hyph числа $a$.
Смотри определение из
\citeBib{Bourbaki: General Topology: Chapter 5 - 10},
гл. IX, \S 3, п${}^\circ$2.
}
\ShowEq{norm on d algebra}
в $D$\Hyph модуле $A$ такая, что\,\footnote{
Неравенство
\EqRef{norm on d algebra 3}
является следствием теоремы
\RefTheorem{there exists equivalent norm |*|=1}.
В противном случае мы должны были бы писать
\ShowEq{norm on d algebra 3 1}
}
\ShowEq{norm on d algebra 3}
называется
\AddIndex{нормой в $D$\Hyph алгебре}
{norm on D algebra} $A$.
$D$\Hyph алгебра $A$,
наделённая структурой, определяемой заданием на
$A$ нормы, называется
\AddIndex{нормированной $D$\Hyph алгеброй}{normed D algebra}.
\qed
\end{definition}

\begin{definition}
Нормированная $D$\Hyph алгебра $A$ называется 
\AddIndex{банаховой $D$\Hyph алгеброй}{Banach algebra}
если любая фундаментальная последовательность элементов
алгебры $A$ сходится, т. е.
имеет предел в алгебре $A$.
\qed
\end{definition}

\Section{Производная отображений \texorpdfstring{$D$}{D}-алгебры}
\labelSection{The Derivative of Map in Algebra}

\ShowDefinition{differentiable map}DAB{algebra}

\begin{definition}
\labelDefinition{differential of map}
{\it
Если, для данного $x\in A$, приращение
\eqRef{derivative of map, def}{algebra}
отображения
\ShowEq{f:A->B}fAB
рассматривать как функцию дифференциала $dx$ переменной $x$,
то линейная часть этой функции
\ShowEq{differential of independent variable}
\ShowEq{differential of map}
\DrawEq{differential of map =}{}
называется
\AddIndex{дифференциалом отображения}{differential of map}
$f$.
}
\qed
\end{definition}

\ShowEq{remark: differential L(A,A)}

\ShowTheorem{derivative, representation in algebra}
\begin{proof}
Из определений
\EqParm{ref definition linear map from A1 to A2}{=z}
и теоремы
\RefTheorem{complete ring contains real number}
следует
\ShowEq{differential is multiplicative over field R, algebra}
\ShowEq{t ne 0 in R, a ne 0 in A}
Комбинируя равенство
\EqRef{differential is multiplicative over field R, algebra}
и определение
\RefDefinition{differentiable map, algebra},
мы получим определение
\EqRef{derivative, linear path}
производной.
\end{proof}

\begin{corollary}
{\it
Отображение $f$
дифференцируемо на множестве $U\subset D$,
если в каждой точке $x\in U$
приращение отображения $f$ может быть представлен в виде
\ShowEq{differential of map, t, algebra}
где
$o:R\rightarrow A$ - такое непрерывное отображение, что
\[
\lim_{t\rightarrow 0}\frac{|o(t)|}{|t|}=0
\]
}
\qed
\end{corollary}

\ShowTheorem{representation of derivative, algebra A->B}
\begin{proof}
Теорема
является следствием определения
\RefDefinition{differentiable map, algebra}
и утверждения
\ShowEq{ref map f generated by basis I}
\end{proof}

\ShowDefinition{coordinates of derivative, algebra A->B}

\ShowTheorem{representation of differential, algebra A->B}
\begin{proof}
Теорема
является следствием теоремы
\RefTheorem{representation of derivative, algebra A->B}
и определения
\RefDefinition{coordinates of derivative, algebra A->B}.
\end{proof}

\begin{remark}
\labelRemark{linear maps generated by map I0}
Если $D$\Hyph модуль
\ShowEq{L(A;A)}
порождён отображением $F_0\circ x=x$,
то равенство
\EqRef{df=sum dsf/dx dx A->B}
принимает вид
\ShowEq{df=sum dsf/dx dx}
где выражение
\ShowEq{component of derivative}
\ShowEq{component of derivative =}
называется
\AddIndex{компонентой производной}
{component of derivative} отображения $f(x)$.
\qed
\end{remark}

\begin{theorem}
\labelTheorem{derivative, standard form, algebra}
Пусть $A$ - свободный банаховый $D$\Hyph модуль.
Пусть $B$ - свободная банаховая $D$\Hyph алгебра.
Пусть $\Basis F$ - базис левого \BoxB{B}модуля\newline
\ShowEq{L(A;B)}DAB.
Пусть $\Basis e$ - базис $D$\Hyph модуля $B$.
\AddIndex{Стандартное представление производной}
{derivative, standard representation} отображения
\ShowEq{f:A->B}fAB
имеет вид
\ShowEq{standard component of derivative}
\ShowEq{derivative, algebra, standard representation}
Выражение
\ShowEq{standard component of derivative, algebra}
в равенстве
\EqRef{derivative, algebra, standard representation}
называется
\AddIndex{стандартной компонентой производной}
{standard component of derivative} отображения $f$.
\end{theorem}
\begin{proof}
Утверждение теоремы является следствием определения
\RefDefinition{differentiable map, algebra}
и утверждения
\ShowEq{ref standard representation of map A1 A2, associative algebra}
\end{proof}

\begin{theorem}
\labelTheorem{derivative and jacobian, algebra}
Пусть $A$ - свободный банаховый $D$\Hyph модуль.
Пусть $B$ - свободная банаховая $D$\Hyph алгебра.
Пусть $\Basis F$ - базис левого \BoxB{B}модуля\newline
\ShowEq{L(A;B)}DAB.
Пусть $\Basis e_A$ - базис свободного конечно мерного
$D$\Hyph модуля $A$.
Пусть $\Basis e_B$ - базис свободной конечно мерной ассоциативной
$D$\Hyph алгебры $B$.
Пусть
\ShowEq{structural constants, algebra}
- структурные константы алгебры $B$.
Тогда производную отображения
\ShowEq{f:A->B}fAB
можно записать в виде
\ShowEq{derivative and jacobian, algebra}
где $dx\in A$ имеет разложение
\ShowEq{derivative and jacobian, 1, algebra}
относительно базиса $\Basis e_A$ и матрица Якоби отображения $f$ имеет вид
\ShowEq{standard components and Jacobian, algebra A->B}
\end{theorem}
\begin{proof}
Утверждение теоремы является следствием теоремы
\ShowEq{ref theorem coordinates of map A1 A2, algebra}
\end{proof}

\begin{remark}
Если $D$\Hyph модуль
\ShowEq{L(A;A)}
порождён отображением $F_0\circ x=x$,
то равенства
\EqRef{derivative, algebra, standard representation},
\EqRef{standard components and Jacobian, algebra A->B}
принимают вид
\ShowEq{standard component of derivative I0}
\ShowEq{derivative, algebra, standard representation I0}
\ShowEq{standard components and Jacobian, algebra}
где выражение
\ShowEq{standard component of derivative, algebra I0}
называется
\AddIndex{стандартной компонентой производной}
{standard component of derivative} отображения $f$.
\qed
\end{remark}

\ShowTheorem{derivative of the sum}
\begin{proof}
Согласно определению
\EqRef{derivative, linear path},
\ShowEq{derivative of the sum, 4}
Равенство \EqRef{derivative of the sum, 3}
следует из равенства \EqRef{derivative of the sum, 4}.
\end{proof}

\ShowTheorem{dfa1p/dx=df/dx a1p}
\ShowProof{dfa1p/dx=df/dx a1p}

\begin{convention}
\labelConvention{bilinear map, parameter linear map}
Для заданного билинейного отображения
\ShowEq{h:BxB->B}
мы рассмотрим отображения
\ShowEq{h1:A3->A}
\ShowEq{h2:A3->A}
определённые равенствами
\ShowEq{h1()=}
\ShowEq{h2()=}
Мы будем пользоваться буквой $h$ для обозначения отображений $h_1$, $h_2$.
\qed
\end{convention}

\ShowTheorem{bilinear map and differential}
\begin{proof}
Равенство \EqRef{bilinear map and derivative, 3}
следует из цепочки равенств
\ShowEq{bilinear map and derivative, 4}
основанной на определении
\EqRef{derivative, linear path}.
Равенство \EqRef{bilinear map and derivative, 5}
следует из равенства
\EqRef{bilinear map and derivative, 3}
и соглашения
\RefConvention{bilinear map, parameter linear map}.
\end{proof}

\ShowTheorem{derivative of product, algebra}
\begin{proof}
Теорема является следствием теорем
\RefTheorem{bilinear map and differential}
и определения
\ShowEq{ref algebra over ring}
\end{proof}

\begin{theorem}
Пусть $A$ - банаховый $D$\Hyph модуль.
Пусть $B$ - банаховая $D$\Hyph алгебра.
Допустим производная отображения
\ShowEq{f:A->B}fAB
имеет разложение
\DrawEq{derivative of f, algebra}{product}
Допустим производная отображения
\ShowEq{g:A->B}
имеет разложение
\DrawEq{derivative of g, algebra}{product}
Производная отображения $f(x)g(x)$
имеет вид
\ShowEq{derivative, fg, algebra}
\ShowEq{component of derivative, fg, algebra}
\end{theorem}
\begin{proof}
Подставим \eqRef{derivative of f, algebra}{product}
и \eqRef{derivative of g, algebra}{product}
в равенство \EqRef{derivative of product, algebra}
\ShowEq{derivative of fg, division ring}
Опираясь на \EqRef{derivative of fg, division ring},
мы определяем равенства
\EqRef{component of derivative, fg, algebra}.
\end{proof}

\begin{theorem}
\labelTheorem{derivative of representation}
Пусть $A$ - банаховый $D$\Hyph модуль.
Пусть $B$, $C$ - банаховые $D$\Hyph алгебры.
Пусть
\ShowEq{h:B->*C}
представление $D$\Hyph модуля $B$
в $D$\Hyph модуле $C$.
Пусть $f$, $g$ - дифференцируемые отображения
\ShowEq{f,g:A->BC}
Производная отображения
\ShowEq{h(f)(g)}
имеет вид
\ShowEq{derivative of representation}
\end{theorem}
\begin{proof}
Так как отображение
\ShowEq{h:B->End C}
является гомоморфизмом абелевой группы
и представление
\ShowEq{h(a):C->C}
является эндоморфизмом аддитивной группы,
то отображение $h(b)(c)$ является билинейным отображением.
Теорема является следствием теоремы
\RefTheorem{bilinear map and differential}.
\end{proof}

\ShowTheorem{derivative of tensor product}
\begin{proof}
Теорема является следствием теорем
\RefTheorem{bilinear map and differential},
\ShowEq{ref theorem V times->V otimes}
и определения
\ShowEq{ref algebra over ring}
\end{proof}

\ifx\texFuture\Defined
\begin{remark}
Пусть
\DrawEq{derivative of f, algebra}{tensor}
\DrawEq{derivative of g, algebra}{tensor}
Тогда
\ShowEq{derivative of tensor product 1, algebra}
Мы не пишем скобки, так как тензорное произведение
ассоциативно и дистрибутивно относительно сложения
(теоремы
\ShowEq{ref tensor product is associative and distributive}
).
\qed
\end{remark}
\fi

\ShowTheorem{map is continuous, derivative}
\begin{proof}
Из теоремы \RefTheorem{set of A->B is D module}
следует
\ShowEq{derivative and continuos map, algebra, 1}
Из \eqRef{derivative of map, def}{algebra},
\EqRef{derivative and continuos map, algebra, 1}
следует
\ShowEq{derivative and continuos map, algebra, 2}
Возьмём произвольное $\epsilon>0$. Положим
\ShowEq{delta=epsilon/|df|}
Тогда из неравенства
\ShowEq{|a|<delta}
следует
\ShowEq{derivative and continuos map, algebra, 3}
Согласно определению \RefDefinition{continuous map, algebra}
отображение $f$ непрерывно в точке $x$.
\end{proof}

\begin{theorem}
\labelTheorem{derivative, 0, D algebra}
Пусть $A$ - банаховый $D$\Hyph модуль.
Пусть $B$ - банаховая $D$\Hyph алгебра.
Пусть отображение
\ShowEq{f:A->B}fAB
дифференцируемо в точке
$x$.
Тогда
\ShowEq{derivative, 0, D algebra}
\end{theorem}
\begin{proof}
Следствие определения
\RefDefinition{differentiable map, algebra}
и теоремы
\ShowEq{ref linear map, 0}
\end{proof}

\ShowTheorem{composite map, derivative, D algebra}
\begin{proof}
Согласно определению
\RefDefinition{differentiable map, algebra}
\ShowEq{derivative of map g, D algebra}
где
\ShowEq{o1:B->C}
- такое непрерывное отображение, что
\ShowEq{o1:B->C, 1}
Согласно определению
\RefDefinition{differentiable map, algebra}
\ShowEq{derivative of map f, D algebra}
где
\ShowEq{o2:A->B}
- такое непрерывное отображение, что
\ShowEq{o2:A->B, 1}
Согласно
\EqRef{derivative of map f, D algebra}
смещение $a$ значения $x\in A$
приводит к смещению
\ShowEq{composite map, b fxa, D algebra}
значения $y$.
Используя \EqRef{composite map, y fx, D algebra},
\EqRef{composite map, b fxa, D algebra}
в равенстве \EqRef{derivative of map g, D algebra},
мы получим
\ShowEq{derivative of map gf, 1, D algebra}
Согласно определениям
\RefDefinition{differentiable map, algebra},
\EqParm{ref definition linear map from A1 to A2}{=c}
из равенства \EqRef{derivative of map gf, 1, D algebra}
следует
\ShowEq{derivative of map gf, 2, D algebra}
Согласно определению \RefDefinition{norm on d algebra}
\ShowEq{derivative of map gf, 3, D algebra}
Из \EqRef{composite map, norm g, D algebra}
следует
\ShowEq{derivative of map gf, 4, D algebra}
Из \EqRef{composite map, norm f, D algebra}
следует
\ShowEq{derivative of map gf, 6, D algebra}
Согласно теореме \RefTheorem{derivative, 0, D algebra}
\ShowEq{derivative of map gf, 7, D algebra}
Следовательно,
\ShowEq{derivative of map gf, 5, D algebra}
Из равенств
\EqRef{derivative of map gf, 3, D algebra},
\EqRef{derivative of map gf, 4, D algebra},
\EqRef{derivative of map gf, 5, D algebra}
следует
\ShowEq{derivative of map gf, 8, D algebra}
Согласно определению
\RefDefinition{differentiable map, algebra}
\ShowEq{derivative of map gf, 9, D algebra}
где
\ShowEq{o:A->B}oAC
такое непрерывное отображение, что
\ShowEq{lim |o|/|a|}AC
Равенство \EqRef{composite map, derivative, D algebra}
следует из
\EqRef{derivative of map gf, 2, D algebra},
\EqRef{derivative of map gf, 8, D algebra},
\EqRef{derivative of map gf, 9, D algebra}.

Из равенства \EqRef{composite map, derivative, D algebra}
и теоремы
\RefTheorem{representation of derivative, algebra A->B}
следует
\ShowEq{composite map, derivative 2, D algebra}
\EqRef{composite map, derivative 01, D algebra}
следуют из равенства
\EqRef{composite map, derivative 2, D algebra}.
\end{proof}

\begin{theorem}
Пусть $A$ - свободный банаховый $D$\Hyph модуль.
Пусть $B$, $C$ - свободные ассоциативные банаховые $D$\Hyph алгебры.
Пусть $\Basis F$ - базис левого \BoxB{B}модуля
\ShowEq{L(A;B)}DAB.
Пусть $\Basis G$ - базис левого \BoxB{C}модуля
\ShowEq{L(A;B)}DBC.
Пусть производная отображения
\ShowEq{f:A->B}fAB
имеет разложение
\ShowEq{expansion of derivative of f with respect to basis I}
относительно базиса $\Basis F$.
Пусть производная отображения
\ShowEq{f:A->B}gBC
имеет разложение
\ShowEq{expansion of derivative of g with respect to basis J}
относительно базиса $\Basis G$.
Тогда производная отображения
\DrawEq{h=g o f}{}
имеет разложение
\ShowEq{expansion of derivative of h with respect to basis K}
относительно базиса
\DrawEq{JlIk}{}
где
\ShowEq{expansion of derivative of h with respect to basis K =}
\end{theorem}
\begin{proof}
Теорема является следствием теорем
\RefTheorem{representation of composition of linear maps},
\RefTheorem{representation of derivative, algebra A->B}
и определения
\RefDefinition{differentiable map, algebra}.
\end{proof}

\begin{theorem}
Пусть $A$ - свободная ассоциативная $D$\Hyph алгеба.
Пусть левый \BoxB{A}модуль
\ShowEq{L(A;B)}DAA.
порождён тождественным отображением $F_0=\delta$.
Пусть производная отображения
\ShowEq{f:A->B}fAA
имеет разложение
\ShowEq{expansion of derivative of f A->A}
Пусть производная отображения
\ShowEq{f:A->B}gAA
имеет разложение
\ShowEq{expansion of derivative of g A->A}
Тогда производная отображения
\DrawEq{h=g o f}{}
имеет разложение
\ShowEq{expansion of derivative of h A->A}
где
\ShowEq{composite map, derivative 01, D algebra}
\end{theorem}
\begin{proof}
Теорема является следствием теоремы
\RefTheorem{representation of composition of linear maps A->A},
замечания
\ref{remark: linear maps generated by map I0}
и определения
\RefDefinition{differentiable map, algebra}.
\end{proof}


==> Diff.Form.1.Ref.tex <==
%auto-ignore

\DefEq
{
\ePrints{1601.03259,1610.309618526}
%\ifx\Semafor\ValueOn
%\RefDefinition[1601.03259]{differential of map},
%\else
\RefDefinition{differential of map},
%\fi
}
{ref definition: differential of map}

%\DefEq
%{
%%\ePrints{1601.03259,1610.309618526}
%%\ifx\Semafor\ValueOn
%%\RefTheorem[1502.04063]{linear map from A1 to A2, commutative module},
%%\else
%\RefTheorem{linear map from A1 to A2, commutative module},
%%\fi
%}
%{ref theorem: linear map from A1 to A2, commutative module}



==> Diff.Form.1.Russian.tex <==
%auto-ignore

\input{Diff.Form.1.Eq}

\Chapter{Дифференциальная форма}

\Section{Структура полилинейного отображения}

\begin{definition}
\labelDefinition{symmetric polylinear map}
{\it
Пусть $A$, $B$ - алгебры над коммутативным кольцом $D$.
Полилинейное отображение
\ShowEq{f in L(A->B)}{A^n}B{}
называется
\AddIndex{симметричным}{symmetric polylinear map},
если
\ShowEq{fa=fsa}
для любой перестановки $\sigma$ множества
\ShowEq{set a1n}
}
\qed
\end{definition}

\begin{theorem}
Пусть
\ShowEq{f in L(A->B)}{A^n}B{}
- полилинейное отображение.
Тогда отображение
\ShowEq{symmetrization of polylinear map}
\EqParm{<f>}{=c}
определённое равенством
\ShowEq{symmetrization of polylinear map =}
является симметричным полилинейным отображением
и называется
\AddIndex{симметрированием полилинейного отображения}{symmetrization of polylinear map}
$f$.
\end{theorem}
\begin{proof}
Теорема является следствием равенства
\ShowEq{gs=sum fss}
и определения
\RefDefinition{symmetric polylinear map}.
\end{proof}

\begin{definition}
\labelDefinition{skew symmetric polylinear map}
{\it
Пусть $A$, $B$ - алгебры над коммутативным кольцом $D$.
Полилинейное отображение
\ShowEq{f in L(A->B)}{A^n}B{}
называется
\AddIndex{косо симметричным}{skew symmetric polylinear map},
если
\ShowEq{fa=sfsa}
для любой перестановки $\sigma$ множества
\EqParm{set a1n}{=.}
}
\qed
\end{definition}

\begin{theorem}
Пусть
\ShowEq{f in L(A->B)}{A^n}B{}
- полилинейное отображение.
Тогда отображение
\ShowEq{alternation of polylinear map}
\EqParm{[f]}{=c}
определённое равенством
\ShowEq{alternation of polylinear map =}
является косо симметричным полилинейным отображением
и называется
\AddIndex{альтернацией полилинейного отображения}{alternation of polylinear map}
$f$.
\end{theorem}
\begin{proof}
Теорема является следствием равенства
\ShowEq{gs=sum sfss}
и определения
\RefDefinition{skew symmetric polylinear map}.
\end{proof}

\begin{theorem}
\labelTheorem{fx1n=0, xi=xi1}
Полилинейное отображение
\ShowEq{f in L(A->B)}{A^n}B{}
косо симметрично тогда и только тогда, когда
\ShowEq{fx1n=0}
при условии
$x_i=x_{i+1}$
хотя бы для одного\footnote{
В книге
\citeBib{Cartan differential form},
страница 192,
Анри Картан рассматривает теорему
\RefTheorem{fx1n=0, xi=xi1}
как определение косо симметричного отображения.
}
\ShowEq{1<=i<n}
\end{theorem}
\begin{proof}
Для заданного $i$ рассмотрим перестановку
\ShowEq{sigma i}
Очевидно, что
\ShowEq{|sigma i|}

Пусть
\ShowEq{f in L(A->B)}{A^n}B{}
- косо симметричное отображение.
Согласно определению
\RefDefinition{skew symmetric polylinear map},
из равенств
\EqRef{sigma i},
\EqRef{|sigma i|}
следует, что
\ShowEq{fxii}

Пусть
\ShowEq{f in L(A->B)}{A^n}B.
Пусть
\ShowEq{fx1n=0}
при условии
$x_i=x_{i+1}$
хотя бы для одного
\ShowEq{1<=i<n}
Тогда
\ShowEq{0=f xi+xi1}
Из равенств
\EqRef{sigma i},
\EqRef{|sigma i|},
\EqRef{0=f xi+xi1}
следует, что
\ShowEq{fxii1=-fxi1i}
Поскольку любую перестановку можно представить
как произведение перестановок $\sigma_i$,
то из равенства
\EqRef{fxii1=-fxi1i}
и определения
\RefDefinition{skew symmetric polylinear map}
следует, что отображение $f$ косо симметрично.
\end{proof}

\begin{theorem}
\labelTheorem{module of skew symmetric polylinear maps}
Множество
\ShowEq{module of skew symmetric polylinear maps}
косо симметричных полилинейных отображений
является $D$\Hyph модулем.
\end{theorem}
\begin{proof}
Согласно теореме
\RefTheorem{L(An;B) is free D module},
линейная комбинация косо симметричных полилинейных отображений
является полилинейным отображением.
Согласно теореме
\RefTheorem{fx1n=0, xi=xi1},
линейная комбинация косо симметричных полилинейных отображений
является косо симметричным полилинейным отображением.
\end{proof}

Не нарушая общности, мы положим
\ShowEq{L(A1,A0,B)=}

\begin{theorem}
Пусть $A$, $B$ - банаховы $D$\Hyph алгебры.
$D$\Hyph модуль $\LAnAB$ замкнут в $D$\Hyph модуле
\ShowEq{L(A;B)}D{A^n}B.
\end{theorem}
\begin{proof}
Теорема является следствием теорем
\RefTheorem{fx1n=0, xi=xi1},
\RefTheorem{module of skew symmetric polylinear maps},
так как равенство
\ShowEq{fxixi=0}
сохраняется в предельном переходе,
когда последовательность отображений $f_k$ сходится к отображению $f$.
\end{proof}

\Section{Произведение косо симметричных полилинейных отображениий}

\begin{definition}
\labelDefinition{product of symmetric polylinear maps}
{\it
Пусть $A$, $B_2$ - свободные алгебры над коммутативным кольцом $D$.\,\footnote{
Я дал определение произведения косо симметричных полилинейных отображениий
согласно определению в разделе
\citeBib{Cartan differential form}-1.4 главы 3,
страницы 195 - 198.
}
Пусть
\ShowEq{h:B1->*B2}
левостороннее представление
свободной ассоциативной $D$\Hyph алгебры $B_1$ в $D$\Hyph модуле $B_2$.
Отображение
\ShowEq{hpq:Lpq->Lp+q}
определено равенством
\ShowEq{hpq(fg)=}
где в правой части равенства
\EqRef{hpq(fg)=}
мы предполагаем левостороннее произведение
$B_2$\Hyph числа
\EqParm{g()}{=z}
на $B_1$\Hyph число
\EqParm{f()}{=.}
}
\qed
\end{definition}

Если $B_1=B_2$, то в правой части равенства
\EqRef{hpq(fg)=}
мы предполагаем произведение $B_1$\Hyph чисел
\EqParm{f()}{=c}
\EqParm{g()}{=.}
Согласно теореме
\RefTheorem{Free Algebra over Ring},
это определение совместимо с определением
\RefDefinition{product of symmetric polylinear maps}.

Пусть $f$, $g$ - косо симметричные полилинейные отображения.
Вообще говоря, отображение
\ShowEq{hpq(fg)}
не является косо симметричным полилинейным отображением.

\begin{definition}
\labelDefinition{exterior product polylinear map}
{\it
Косо симметричное полилинейное отображение
\ShowEq{exterior product}
\ShowEq{exterior product =}
называется
\AddIndex{внешним произведением}{exterior product}.
}
\qed
\end{definition}

\begin{theorem}
Внешнее произведение удовлетворяет следующему равенству
\ShowEq{exterior product = skew symmetric}
\end{theorem}
\begin{proof}
Равенство
\EqRef{exterior product = skew symmetric}
является следствием равенств
\EqRef{alternation of polylinear map =},
\EqRef{exterior product =}.
\end{proof}

\begin{theorem}
\labelTheorem{fAf ne 0}
Пусть $B$ - некоммутативная $D$\Hyph алгебра и
\ShowEq{f:A->B}fAB
линейное отображение. Тогда, вообще говоря,\,\footnote{
Смотри также равенство
(\citeBib{Sudbery Quaternionic Analysis}\Hyph (2.25).
}
\ShowEq{fAf ne 0}
\end{theorem}
\begin{proof}
Согласно равенству
\EqRef{exterior product = skew symmetric},
\ShowEq{fAf=}
Выражение
\EqRef{fAf=},
вообще говоря, отлично от $0$.
\end{proof}

Из доказательства теоремы
\RefTheorem{fAf ne 0}
следует, что
\ShowEq{fAf=0}
только при условии, что образ отображения $f$ является
подмножеством центра алгебры $B$.

\begin{convention}
\labelConvention{IJK=()}
Пусть
\ShowEq{IJK=()}
Порядок индекса в множествах $J$, $K$ тот же, что в множестве $I$.
Пусть
\ShowEq{RJI}
является множеством инъекций
\ShowEq{J->I}
Для произвольного отображения
\EqParm{l in RJI}{=c}
пусть
\ShowEq{D(l)}
- множество значений отображения $\lambda$ и
\ShowEq{D1=I-D}
Отображение
\ShowEq{K->D1}
определено равенством
\ShowEq{mu(l)()=}
Пусть
\ShowEq{S1(l)}
- множество перестановок множества
\ShowEq{D1(l)}
\qed
\end{convention}

Пусть множество $I_{m.n}$ определено равенством
\ShowEq{Imn=}

\begin{lemma}
\labelLemma{sigma=lambda,tau}
{\it
Для любой перестановки
\EqParm{s in S}{=c}
существует единственное отображение
\EqParm{l in RJI}{=z}
и единственная перестановка
\EqParm{t in S1l}{=z}
такие, что
\DrawEq{sigma=lambda,tau}{->}
}
\end{lemma}
\begin{proof}
Пусть
\EqParm{s in S}{=.}
Мы определим отображение
\EqParm{l in RJI}{=z}
с помощью таблицы
\ShowEq{lambda=}
Мы определим отображение
\ShowEq{t:D1->D1}
равенством
\ShowEq{t(l)=s(a)}
Равенство
\ShowEq{t(m(a))=s(a)}
является следствием равенств
\EqRef{mu(l)()=},
\EqRef{t(l)=s(a)}.
Поскольку отображения $\sigma$, $\mu(\lambda)$
являются биекциями, то отображение $\tau$ является биекцией.
Следовательно, отображение $\tau$ является перестановкой множества
\ShowEq{D1(l)}
Равенство
\eqRef{sigma=lambda,tau}{->}
является следствием равенств
\EqRef{lambda=},
\EqRef{t(m(a))=s(a)}.
\end{proof}

\begin{lemma}
\labelLemma{lambda,tau=sigma}
{\it
Для любого отображения
\EqParm{l in RJI}{=z}
и любой перестановки
\EqParm{t in S1l}{=c}
существует единственная перестановка
\EqParm{s in S}{=z}
такая, что
\DrawEq{sigma=lambda,tau}{<-}
}
\end{lemma}
\begin{proof}
Согласно
\EqRef{D1=I-D},
\ShowEq{D1+D=I}
Так как отображения
\ShowEq{l m(l) t}
инъективны, то
отображение $\sigma$ является перестановкой.
\end{proof}

%\ePrints{4975-6381}
%\ifx\Semafor\ValueOn
%\newpage
%\fi
Согласно леммам
\RefLemma{sigma=lambda,tau},
\RefLemma{lambda,tau=sigma},
существует биекция множества $S$ в множество кортежей
\ShowEq{(lambda,tau)}
где
\EqParm{l in RJI}{=c}
\EqParm{t in S1l}{=.}
Мы выражаем эту биекцию равенством
\ShowEq{s=(lambda,tau)}

\begin{lemma}
\labelLemma{sign of the map l}
{\it
Мы определим знак отображения
\EqParm{l in RJI}{=z}
равенством
\ShowEq{|l|=|l,d|}
где $\delta$ - тождественная перестановка множества
\ShowEq{D1(l)}
Тогда
\ShowEq{|lt|=|l||t|}
}
\end{lemma}
\begin{proof}
Так как
\ShowEq{|d|=1}
то теорема верна для перестановки
\EqParm{(l,d)}{=.}

Пусть перестановка $\tau$ является транспозицией.
Тогда перестановка
\ShowEq{(lambda,tau)}
отличается от перестановки
\EqParm{(l,d)}{=z}
на транспозицию.
Следовательно, в этом случае, равенство
\EqRef{|lt|=|l||t|}
верно.

Пусть перестановка $\tau$ имеет разложение в произведение $n$ транспозиций.
Тогда перестановка
\ShowEq{(lambda,tau)}
отличается от перестановки
\EqParm{(l,d)}{=z}
на произведение $n$ транспозиций.
Следовательно, в общем случае, равенство
\EqRef{|lt|=|l||t|}
верно.
\end{proof}

\begin{theorem}
\labelTheorem{f1 f2 = sum l in Rp}
Пусть
\ShowEq{f in LAAB}1p1
\ShowEq{f in LAAB}2q2
Пусть $R_0$ является множеством инъекций
\ShowEq{I1p->I1pq}
которые сохраняют порядок индекса в множестве $I_{1.p+q}$.
Пусть
\ShowEq{R1=I1p->I1pq}
Внешнее произведение косо симметричных полилинейных отображений удовлетворяет равенству\,\footnote{
В книге
\citeBib{Cartan differential form}, страницы 195 - 197,
равенство
\EqRef{f1 f2 = sum l in R0p}
является определением внешнего произведения косо симметричных полилинейных отображений,
поскольку отображение
\ShowEq{apq->l}
является перестановкой, удовлетворяющей требованию (1.4.3) на странице
\citeBib{Cartan differential form}\Hyph 196.
}
\ShowEq{f1 f2 = sum l in R1p}
\ShowEq{f1 f2 = sum l in R0p}
\end{theorem}
\begin{proof}
Пусть $S$ - множество перестановок множества
\ShowEq{I1pq}
Согласно определению
\EqRef{exterior product = skew symmetric},
\ShowEq{f1 A f2 =}
Согласно леммам
\RefLemma{sigma=lambda,tau},
\RefLemma{lambda,tau=sigma},
\RefLemma{sign of the map l},
\ShowEq{f1 A f2 = 1}
Поскольку отображение $f_2$ - косо симметрично, то, согласно определению
\RefDefinition{skew symmetric polylinear map},
\ShowEq{f2 l = |s| f2 sl}
Равенство
\ShowEq{f1 A f2 = 2}
является следствием равенств
\EqRef{f1 A f2 = 1},
\EqRef{f2 l = |s| f2 sl}.
Равенство
\EqRef{f1 f2 = sum l in R1p}
является следствием равенства
\EqRef{f1 A f2 = 2}.

Для произвольного
\EqParm{l in R0}{=c}
рассмотрим множество
\ShowEq{R2(l)=...}
Отображение
\ShowEq{m in R2}
отличается от отображения
\EqParm{l in R0}{=z}
на перестановку множества $D(\lambda)$ и
\ShowEq{|l|f1=|m|f1}
При этом
\ShowEq{R1=U R2}
Равенство
\ShowEq{f1 A f2 = 3}
является следствием равенств
\EqRef{f1 f2 = sum l in R1p},
\EqRef{|l|f1=|m|f1},
\EqRef{R1=U R2}.
Равенство
\EqRef{f1 f2 = sum l in R0p}
является следствием равенств
\EqRef{f1 A f2 = 3}.
\end{proof}

\begin{theorem}
Пусть
\ShowEq{f in LAAB}1p1
\ShowEq{f in LAAB}2q2
Пусть $R_0$ является множеством инъекций
\ShowEq{Ip1q->I1pq}
которые сохраняют порядок индекса в множестве $I_{1.p+q}$.
Пусть
\ShowEq{R1=Ip1q->I1pq}
Внешнее произведение косо симметричных полилинейных отображенй удовлетворяет равенству
\ShowEq{f1 f2 = sum l in R1q}
\ShowEq{f1 f2 = sum l in R0q}
\end{theorem}
\begin{proof}
Доказательство теоремы аналогично доказательству теоремы
\RefTheorem{f1 f2 = sum l in Rp}.
\end{proof}

\begin{theorem}
Внешнее произведение косо симметричных полилинейных отображенй ассоциативно.
Пусть
\ShowEq{f in LAAB}1p1
\ShowEq{f in LAAB}2q1
\ShowEq{f in LAAB}3r2
Тогда
\ShowEq{f1(f2f3)=(f1f2)f3 wedge}
\end{theorem}
\begin{proof}
Пусть представление $D$\Hyph алгебры $B_1$ в $D$\Hyph модуле $B_2$
определено отображением $h$ и произведение в $D$\Hyph алгебре $B_1$
определено отображением $g$.

Пусть $S$ - множество перестановок множества
\ShowEq{I1pqr}

Согласно определению
\RefDefinition[0912.3315]{left-side representation of group},
следующее равенство
\ShowEq{f1(f2f3)=(f1f2)f3}
верно для любых $B_1$\Hyph чисел
\ShowEq{f1()f2()}
и для любого $B_2$\Hyph числа
\ShowEq{f3()}
Согласно определению
\RefDefinition{product of symmetric polylinear maps},
мы можем записать равенство
\EqRef{f1(f2f3)=(f1f2)f3}
в виде
\ShowEq{f1(f2f3)=(f1f2)f3 1}
Равенство
\EqRef{f1(f2f3)=(f1f2)f3 1}
остаётся верным, если мы применим перестановку
\ShowEq{s in SI}
Поэтому равенство
\ShowEq{f1(f2f3)=(f1f2)f3 2}
является следствием равенства
\EqRef{f1(f2f3)=(f1f2)f3 1}.

Пусть
\ShowEq{R1=I1p->I1pqr}
Согласно леммам
\RefLemma{sigma=lambda,tau},
\RefLemma{lambda,tau=sigma},
\RefLemma{sign of the map l},
мы перепишем левую часть равенства
\EqRef{f1(f2f3)=(f1f2)f3 2}
следующим образом
\ShowEq{f1(f2f3)}
Согласно определениям
\EqRef{alternation of polylinear map =},
\EqRef{exterior product =},
равенство
\ShowEq{f1(f2f3) 2}
является следствием равенства
\EqRef{f1(f2f3)}.
Согласно леммам
\RefLemma{sigma=lambda,tau},
\RefLemma{lambda,tau=sigma},
\RefLemma{sign of the map l},
равенство
\ShowEq{f1(f2f3) 3}
является следствием равенств
\EqRef{exterior product = skew symmetric},
\EqRef{f1(f2f3) 2}.
Согласно определению
\RefDefinition{product of symmetric polylinear maps},
мы можем записать равенство
\EqRef{f1(f2f3) 3}
в виде
\ShowEq{f1(f2f3) 4}
Согласно определениям
\EqRef{alternation of polylinear map =},
\EqRef{exterior product =},
равенство
\ShowEq{f1(f2f3) 5}
является следствием равенства
\EqRef{f1(f2f3) 4}.

Пусть
\ShowEq{R2=Ipqpqr->I1pqr}
Согласно леммам
\RefLemma{sigma=lambda,tau},
\RefLemma{lambda,tau=sigma},
\RefLemma{sign of the map l},
мы перепишем правую часть равенства
\EqRef{f1(f2f3)=(f1f2)f3 2}
следующим образом
\ShowEq{(f1f2)f3}
Согласно определениям
\EqRef{alternation of polylinear map =},
\EqRef{exterior product =},
равенство
\ShowEq{(f1f2)f3 2}
является следствием равенства
\EqRef{(f1f2)f3}.
Согласно леммам
\RefLemma{sigma=lambda,tau},
\RefLemma{lambda,tau=sigma},
\RefLemma{sign of the map l},
равенство
\ShowEq{(f1f2)f3 3}
является следствием равенств
\EqRef{exterior product = skew symmetric},
\EqRef{(f1f2)f3 2}.
Согласно определению
\RefDefinition{product of symmetric polylinear maps},
мы можем записать равенство
\EqRef{(f1f2)f3 3}
в виде
\ShowEq{(f1f2)f3 4}
Согласно определениям
\EqRef{alternation of polylinear map =},
\EqRef{exterior product =},
равенство
\ShowEq{(f1f2)f3 5}
является следствием равенства
\EqRef{(f1f2)f3 4}.

Равенство
\EqRef{f1(f2f3)=(f1f2)f3 wedge}
является следствием равенств
\EqRef{f1(f2f3)=(f1f2)f3 1},
\EqRef{f1(f2f3) 5},
\EqRef{(f1f2)f3 5}.
\end{proof}

\Section{Дифференциальная форма}

\begin{definition}
\labelDefinition{map of class Cn}
{\it
Отображение принадлежит к классу $C^n$,
если отображение имеет непрерывную производную порядка $n$.
Отображение принадлежит к классу $C^{\infty}$,
если отображение имеет непрерывную производную любого порядка.
}
\qed
\end{definition}

\begin{definition}
{\it
Пусть $A$, $B$ - банаховы $D$\Hyph алгебры.
Пусть
\ShowEq{U subset A}
является открытым множеством.
Отображение
\ShowEq{o:U->LAAB}
называется
\AddIndex{дифференциальной формой степени $p$}{differential form of degree p},
определённой на $U$, со значениями в $B$
или $B$\Hyph значной
\AddIndex{дифференциальной $p$\Hyph формой}{differential p form},
определённой на $U$.
Говорят, что дифференциальная $p$\Hyph форма $\omega$
принадлежит к классу
\ShowEq{class Cn},
если отображение $\omega$ принадлежит к классу $C^n$.
Множество
\ShowEq{set of differential p forms}
$B$\Hyph значных дифференциальных $p$\Hyph форм
класса $C^n$, определённых на $U$
является $D$\Hyph модулем.
}
\qed
\end{definition}

\begin{theorem}
Пусть $A$, $B_2$ - свободные банаховые алгебры над коммутативным кольцом $D$.\,\footnote{
Я дал определение произведения дифференциальных форм
согласно определению в разделе
\citeBib{Cartan differential form}-2.2 главы 3,
страницы 204 - 205.
}
Пусть
\ShowEq{h:B1->*B2}
левостороннее представление
свободной ассоциативной банаховой $D$\Hyph алгебры $B_1$ в банаховом $D$\Hyph модуле $B_2$.
Пусть
\ShowEq{diff form in U}{\alpha}np{B_1},
\ShowEq{diff form in U}{\beta}nq{B_2}.
\AddIndex{Внешнее произведение}{exterior product}
\ShowEq{exterior product, differential forms}
дифференциальных форм $\alpha$, $\beta$,
определённое равенством
\ShowEq{a wedge b x =}
является дифференциальной формой класса $C^n$.
\end{theorem}
\begin{proof}
Для любого $x\in U$,
\EqParm{form x in LA}{form=alpha,A=AB,=c}
\EqParm{form x in LA}{form=beta,A=AB,=.}
Согласно определениям
\RefDefinition{product of symmetric polylinear maps},
\RefDefinition{exterior product polylinear map},
\ShowEq{a(x) wedge b(x) in}
Отображение
\ShowEq{x->a(x) wedge b(x)}
является отображением класса $C^n$,
так как оно является композицией отображения
\ShowEq{x->(a(x),b(x))}
класса $C^n$ и непрерывного билинейного отображения
\ShowEq{LA1xLA2->LA}
порождённого представлением $h$.
\end{proof}

\begin{corollary}
\labelCorollary{Exterior product generates bilinear map}
{\it
Внешнее произведение дифференциальных форм
порождает билинейное отображение
\EqParm{O(B1)xO(B2)->O(B2)}{A=B2}
}
\qed
\end{corollary}

\begin{theorem}
Пусть $A$, $B_2$ - свободные банаховые алгебры над коммутативным кольцом $D$.
Пусть
\ShowEq{h:B1->*B2}
левостороннее представление
свободной ассоциативной банаховой $D$\Hyph алгебры $B_1$ в банаховом $D$\Hyph модуле $B_2$.
Пусть
\ShowEq{diff form in U}{\alpha}np{B_1},
\ShowEq{diff form in U}{\beta}nq{B_2}.
Тогда
\ShowEq{(a wedge b)(x)()=}
\end{theorem}
\begin{proof}
Теорема является следствием равенств
\EqRef{alternation of polylinear map =},
\EqRef{hpq(fg)=},
\EqRef{exterior product =}.
\end{proof}

Для даного целого числа $n$
рассмотрим $D$\Hyph модуль
\ShowEq{OnB=...}
который является прямой суммой $D$\Hyph модулей
\ShowEq{OnB1}
$D$\Hyph модуль
\EqParm{OnB}{=c}
оснащённый внешним произведением
\EqParm{O(B1)xO(B2)->O(B2)}{A=B1}
является градуированной алгеброй.

\begin{theorem}
\labelTheorem{1 form in finite dimensional Banach algebra}
Пусть $\Basis e_A$ - базис
конечномерной банаховой алгебры $A$ над коммутативным кольцом $D$.
Пусть $\Basis e_B$ - базис
конечномерной банаховой алгебры $B$ над коммутативным кольцом $D$.
Пусть
\ShowEq{o1p x}
- координаты полилинейного отображения
\ShowEq{o(x) in L(An;B)}
относительно базисов $\Basis e_A$, $\Basis e_B$.
Тогда дифференциальная $p$\Hyph форма $\omega$ имеет вид
\ShowEq{w(a1p)=...}
где
\ShowEq{a1p=...}
\ShowEq{w1p=...}
\end{theorem}
\begin{proof}
Так как
\EqParm{a1p}{n=1,=z}
- произвольные $A$\Hyph числа, то равенства
\EqRef{w(a1p)=...},
\EqRef{w1p=...}
являются следствием равенства
\EqRef{a1p=...}
и равенства
\ShowEq{w(a1n)=a1n...}
\end{proof}

Отображение
\ShowEq{f:A->B}fAB
это пример $B$\Hyph значной дифференциальной $0$\Hyph формы.

Производная отображения
\ShowEq{f:A->B}fAB
это пример $B$\Hyph значной дифференциальной $1$\Hyph формы.

\begin{theorem}
\labelTheorem{derivative in finite dimensional Banach algebra}
Пусть $\Basis e$ - базис
конечномерной банаховой алгебры $A$ над полем $D$.
Мы можем рассматривать отображение
\ShowEq{f:A->B}fAA
как отображение
\ShowEq{f(x)=f(x1n)}
где
\ShowEq{x=x1n}
Если отображение $f$ дифференцируемо,
то существуют частные производные
\ShowEq{df/dxi 1n}
и верно следующее равенство
\DrawEq{df/dxi=}{theorem}
\end{theorem}
\begin{proof}
Согласно определению
\RefDefinition{differential of map},
дифференциал отображения $f$ имеет вид
\ShowEq{df=df/dx o dx}
Поскольку отображение $f$ является отображением
$D$\Hyph векторного пространства,
то мы можем записать дифференциалы в виде
\DrawEq{dx=dx e}{differential}
\ShowEq{df=df/dxi dxi}
Равенство
\ShowEq{df/dx o dx=df/dxi dxi}
является следствием равенств
\EqRef{df=df/dx o dx},
\eqRef{dx=dx e}{differential},
\EqRef{df=df/dxi dxi}.
Равенство
\eqRef{df/dxi=}{theorem}
является следствием равенства
\EqRef{df/dx o dx=df/dxi dxi}.
\end{proof}

Нетрудно видеть, что частная производная
\EqParm{df/dxi}{=c}
представленная в виде
\eqRef{df/dxi=}{theorem},
является отображением $D$\Hyph алгебры $A$.
Если это отображение дифференцируемо,
то мы можем рассмотреть частные производные второго порядка
\ShowEq{d/dxj df/dxi=}

\begin{theorem}
\labelTheorem{second derivative is symmetric bilinear map}
Пусть $A$ - свободный банаховый $D$\Hyph модуль.
Пусть производная второго порядка отображения
\ShowEq{f:A->B}fAB
непрерывна.
Тогда вторая производная является симметричным билинейным отображением
\ShowEq{df/dx2 ab=ba}
\end{theorem}
\begin{proof}
Поскольку отображение
\ShowEq{d2f/dx2}
непрерывно,
то непрерывность
отображения
\ShowEq{d2f/dxij}
следует из равенства
\EqRef{d/dxj df/dxi=}.
Согласно теореме
\citeBib{Fikhtengolts: Calculus volume 1}
(страницы 405, 406),
\ShowEq{df/dxij=df/dxji}
Равенство
\ShowEq{df/dx2 ij=ji}
является следствием равенств
\EqRef{d/dxj df/dxi=},
\EqRef{df/dxij=df/dxji}.
Равенство
\EqRef{df/dx2 ab=ba}
является следствием равенств
\ShowEq{a= b= e}
и равенства
\EqRef{df/dx2 ij=ji}.
\end{proof}

\Section{Внешнее дифференцирование}

Пусть $A$, $B$ - банаховы $D$\Hyph алгебры.
Пусть
\ShowEq{U subset A}
является открытым множеством.
Пусть отображение
\ShowEq{o:U->LAAB}
является дифференциальной $p$\Hyph формой,
класса $C_n$, $n>0$.
Согласно определению
\RefDefinition{map of class Cn},
в каждой точке $x\in U$
изменение отображения
$\omega$ может быть представлено в виде
\ShowEq{derivative of omega}
где
\ShowEq{d omega in Cn-1}
Согласно определению
\EqRef{derivative of omega},
отображение
\ShowEq{d omega a0p}
является косо симметричным полилинейным отображением
по переменным
\EqParm{a1p}{n=1,=z}
и является линейным отображением по переменной $a_0$.
Однако отображение
\EqRef{d omega a0p}
не является косо симметричным полилинейным отображением
по переменным
\ShowEq{a0p}

\begin{definition}
\labelDefinition{exterior differential}
{\it
Пусть $A$, $B$ - банаховы $D$\Hyph алгебры.
Пусть
\ShowEq{U subset A}
является открытым множеством.
Пусть отображение
\ShowEq{o:U->LAAB}
является дифференциальной $p$\Hyph формой,
класса $C_n$, $n>0$.
Отображение
\ShowEq{exterior differential}
\ShowEq{exterior differential def}
называется
\AddIndex{внешним дифференциалом}{exterior differential}.
}
\qed
\end{definition}

\begin{theorem}
Внешний дифференциал удовлетворяет равенству
\ShowEq{do=...sum}
\end{theorem}
\begin{proof}
Равенство
\EqRef{do=...sum}
является следствием равенств
\EqRef{alternation of polylinear map =},
\EqRef{exterior differential def}.
\end{proof}

\ifx\texFuture\Defined
\begin{convention}
Пусть, в соглашении
\RefConvention{IJK=()},
\ShowEq{I=a0p,J=a0}
Тогда мы можем отождествить любое отображение
\EqParm{l in RJI}{=z}
с перестановкой
\ShowEq{ti in S p+1}
определенной кортежем
\ShowEq{ti a0p}
Из равенства
\EqRef{ti a0p}
следует, что
\qed
\end{convention}
\fi

\begin{lemma}
\labelLemma{s->(ti mu)}
{\it
Пусть $S_1$ - множество перестановок множества $A$\Hyph чисел
\EqParm{a1p}{n=0,=.}
Пусть $S$ - множество перестановок множества $A$\Hyph чисел
\EqParm{a1p}{n=1,=.}
Пусть перестановка
\ShowEq{ti in S1}
определена кортежем
\ShowEq{ti a0p}
Для любой перестановки
\ShowEq{s in S1}
существуют перестановки
\ShowEq{ti in S1, s1 in S}
такие, что
\DrawEq{s=(ti mu)}{->}
}
\end{lemma}
\begin{proof}
Перестановка $\tau_i$ определена равенством
\ShowEq{ti 0 = s 0}
Перестановка $\mu$ определена равенством
\ShowEq{mu=()}
Равенство
\eqRef{s=(ti mu)}{->}
является следствием равенств
\EqRef{ti 0 = s 0},
\EqRef{mu=()}.
\end{proof}

\begin{lemma}
\labelLemma{(ti mu)->s}
{\it
Для любой перестановки $\mu$ множества $A$\Hyph чисел
\ShowEq{a0p - ai}
существует перестановка $\sigma$ множества $A$\Hyph чисел
\EqParm{a1p}{n=0,=z}
такая, что
\DrawEq{s=(ti mu)}{<-}
\ShowEq{|s|=(-1)i|mu|}
}
\end{lemma}
\begin{proof}
Перестановка $\sigma$ имеет вид
\ShowEq{s=mu i ne 0}
Равенство
\eqRef{s=(ti mu)}{<-}
является следствием равенства
\EqRef{s=mu i ne 0}.
Равенство
\ShowEq{|s|=|t mu|}
является следствием равенства
\EqRef{s=mu i ne 0}.
Так как перестановку $\tau_i$ можно представить
как произведение $i$ транспозиций, то
\ShowEq{|ti|=(-1)i}
Равенство
\EqRef{|s|=(-1)i|mu|}
является следствием равенств
\EqRef{|s|=|t mu|},
\EqRef{|ti|=(-1)i}.
\end{proof}

\begin{lemma}
\labelLemma{sum s1 =sum +-s}
{\it
Пусть $S_1$ - множество перестановок множества $A$\Hyph чисел
\EqParm{a1p}{n=0,=.}
Пусть $S$ - множество перестановок множества $A$\Hyph чисел
\EqParm{a1p}{n=1,=.}
Для любого полилинейного отображения $f$
\ShowEq{sum s1 =sum +-s}
}
\end{lemma}
\begin{proof}
Лемма является следствием лемм
\RefLemma{s->(ti mu)},
\RefLemma{(ti mu)->s}.
\end{proof}

\begin{theorem}
\labelTheorem{exterior differential of differential form}
Внешний дифференциал дифференциальной $p$\Hyph формы имеет вид\,\footnote{
Согласно определению
\EqRef{ti a0p},
равенство
\EqRef{d omega = sum tau}
можно записать в виде
\ShowEq{d omega = sum}
}
\ShowEq{d omega = sum tau}
\end{theorem}
\begin{proof}
Равенство
\ShowEq{d omega = sum 1}
является следствием равенств
\EqRef{alternation of polylinear map =},
\EqRef{exterior differential def}.
Согласно лемме
\RefLemma{sum s1 =sum +-s},
равенство
\ShowEq{d omega = sum 2}
является следствием равенства
\EqRef{d omega = sum 1}.
Равенство
\EqRef{d omega = sum tau}
является следствием равенства
\EqRef{d omega = sum 2},
так как отображение
\ShowEq{dx omega}
косо симметрично по переменным
\EqParm{a1p}{n=1,=z}
и мы вместо суммы по перестановкам $\mu$
можем записать слагаемое, соответствующее тождественной перестановке $\mu$.
\end{proof}

\begin{example}
Пусть
\ShowEq{diff form in U}{\omega}n2B.
Тогда
\ShowEq{d omega2=}
\qed
\end{example}

\begin{theorem}
Пусть $A$, $B_2$ - свободные банаховые алгебры над коммутативным кольцом $D$.\,\footnote{
Теорема аналогична теореме
\citeBib{Cartan differential form}-2.4.2,
страница 209.
Однако доказательство Картана меня не устраивает,
так как он пользуется коммутативностью произведения в поле действительных чисел.
}
Пусть
\ShowEq{h:B1->*B2}
левостороннее представление
свободной ассоциативной банаховой $D$\Hyph алгебры $B_1$ в банаховом $D$\Hyph модуле $B_2$.
Пусть
\ShowEq{diff form in U}{\alpha}np{B_1},
\ShowEq{diff form in U}{\beta}nq{B_2}.
Тогда
\ShowEq{d(a wedge b)=}
\end{theorem}
\begin{proof}
Согласно теореме
\RefTheorem{bilinear map and differential}
и следствию
\RefCorollary{Exterior product generates bilinear map},
\ShowEq{d(a A b)/dx=...}
Равенство
\ShowEq{d(a A b)/dx=..., 1}
является следствием равенства
\EqRef{d(a A b)/dx=...}.
%Пусть $S$ - множество перестановок множества $A$\Hyph чисел
%\ShowEq{a0p+q}
Равенство
\ShowEq{d(a A b)/dx=..., 2}
является следствием равенств
\EqRef{d omega = sum tau},
\EqRef{d(a A b)/dx=..., 1}.

Пусть $S_1$ - множество перестановок множества $A$\Hyph чисел
\EqParm{a1p+q}{n=0}
Пусть $S$ - множество перестановок множества $A$\Hyph чисел
\EqParm{a1p+q}{n=1}

Согласно определениям
\EqRef{alternation of polylinear map =},
\EqRef{exterior product =},
\ShowEq{d(a A b)/dx=..., 2 1.1}
Согласно лемме
\RefLemma{sum s1 =sum +-s},
равенство
\ShowEq{d(a A b)/dx=..., 2 1.2}
является следствием равенства
\EqRef{d(a A b)/dx=..., 2 1.1}.
Пусть
\ShowEq{R1=Ip+1q>I0p+q}
Согласно леммам
\RefLemma{sigma=lambda,tau},
\RefLemma{lambda,tau=sigma},
\RefLemma{sign of the map l},
равенство
\ShowEq{d(a A b)/dx=..., 2 1.3}
является следствием равенства
\EqRef{d(a A b)/dx=..., 2 1.2}.
Согласно определениям
\EqRef{alternation of polylinear map =},
\EqRef{exterior differential def},
равенство
\ShowEq{d(a A b)/dx=..., 2 1.4}
является следствием равенств
\EqRef{do=...sum},
\EqRef{d(a A b)/dx=..., 2 1.3}.
Равенство
\ShowEq{d(a A b)/dx=..., 2 1.5}
является следствием равенства
\EqRef{f1 f2 = sum l in R1q},
\EqRef{d(a A b)/dx=..., 2 1.4}.

Согласно определениям
\EqRef{alternation of polylinear map =},
\EqRef{exterior product =},
\ShowEq{d(a A b)/dx=..., 2 2.1}
Согласно лемме
\RefLemma{sum s1 =sum +-s},
равенство
\ShowEq{d(a A b)/dx=..., 2 2.2}
является следствием равенства
\EqRef{d(a A b)/dx=..., 2 2.1}.
Пусть
\ShowEq{R1=I1p->I0p+q}
Согласно леммам
\RefLemma{sigma=lambda,tau},
\RefLemma{lambda,tau=sigma},
\RefLemma{sign of the map l},
равенство
\ShowEq{d(a A b)/dx=..., 2 2.3}
является следствием равенства
\EqRef{d(a A b)/dx=..., 2 2.2}.
Согласно определениям
\EqRef{alternation of polylinear map =},
\EqRef{exterior differential def},
равенство
\ShowEq{d(a A b)/dx=..., 2 2.4}
является следствием равенств
\EqRef{do=...sum},
\EqRef{d(a A b)/dx=..., 2 2.3}.
Равенство
\ShowEq{d(a A b)/dx=..., 2 2.5}
является следствием равенств
\EqRef{f1 f2 = sum l in R1p},
\EqRef{d(a A b)/dx=..., 2 2.4}.
Поскольку
\ShowEq{|a1p a0 apq|=}
то равенство
\ShowEq{d(a A b)/dx=..., 2 2.6}
является следствием равенства
\EqRef{d(a A b)/dx=..., 2 2.5}.

Равенство
\ShowEq{d(a A b)/dx=..., 3}
является следствием равенств
\EqRef{d(a A b)/dx=..., 2},
\EqRef{d(a A b)/dx=..., 2 1.5},
\EqRef{d(a A b)/dx=..., 2 2.6}.
Равенство
\EqRef{d(a wedge b)=}
является следствием равенства
\EqRef{d(a A b)/dx=..., 3}.
\end{proof}

\begin{theorem}
\labelTheorem{d2omega=0}
Пусть $A$ - свободный банаховый $D$\Hyph модуль.
Если
\ShowEq{diff form in U}{\omega}npB,
$n\ge 2$, тогда\,\footnote{
Смотри также теорему
\citeBib{Cartan differential form}-2.5.1
на странице 210.
}
\ShowEq{d2omega=0}
\end{theorem}
\begin{proof}
Согласно определению
\RefDefinition{exterior differential},
\ShowEq{d2o=d/dx do/dx}
Пусть $S$ является множеством перестановок множества
\ShowEq{b12I1p}
Согласно определению
\EqRef{alternation of polylinear map =},
равенство
\ShowEq{d2o=d/dx do/dx 1}
является следствием равенства
\EqRef{d2o=d/dx do/dx}.
Согласно теореме
\RefTheorem{second derivative is symmetric bilinear map},
отображение
\ShowEq{d2o/dx2}
симметрично по $A$\Hyph числам $b_1$, $b_2$.
Равенство
\EqRef{d2omega=0}
является следствием определений
\RefDefinition{symmetric polylinear map},
\RefDefinition{skew symmetric polylinear map}.
\end{proof}

\Section{Теорема Пуанкаре}

\begin{definition}
{\it
Подмножество $U$ $D$\Hyph алгебры $B$ называется
\AddIndex{звёздным}{starlike set}
относительно $B$\Hyph числа
\EqParm{a in U}{=c}
если
\EqParm{t'a+tx in U}{=z}
для любого $B$\Hyph числа
\ShowEq{x in U}
и действительного числа
\EqParm{0<t<1}{=.}
}
\qed
\end{definition}

\begin{definition}
\labelDefinition{integrable form}
{\it
Пусть $A$, $B$ - банаховы алгебры.
Пусть
\ShowEq{U subset A}
- открытое множество.
Дифференциальная форма
\ShowEq{diff form in U}{\omega}npB{}
называется
\AddIndex{интегрируемой}{integrable form},
если существует дифференциальная форма
\ShowEq{diff form in U}{\alpha}n{p-1}B{}
такая, что
\DrawEq{da=o}{}
Тогда мы пользуемся записью
\ShowEq{indefinite integral form}
\ShowEq{a=int o}
и дифференциальная форма $\alpha$ называется
\AddIndex{неопределённым интегралом}{indefinite integral}
дифференциальной формы $\omega$.
}
\qed
\end{definition}

\begin{theorem}
\labelTheorem{map int continuous is continuous}
Пусть $A$, $B$ - банаховы алгебры.\,\footnote{
Утверждение аналогично лемме
\citeBib{Cartan differential form}\Hyph 2.12.2
на странице 223.
}
Пусть
\ShowEq{[01]}
- подмножество поля действительных чисел.
Пусть
\ShowEq{phi:UxI->B}
непрерывное отображение.
Тогда отображение
\ShowEq{psi:U->B}
определённое равенством
\DrawEq{psi=int phi}{}
непрерывно.
\end{theorem}
\begin{proof}
Пусть задано
\EqParm{eps>0}{=.}
\StartLabelItem
\begin{enumerate}
\item
Для каждой точки
\ShowEq{x,t in U I}
существует
\ShowEq{eta xt}
такое, что из утверждения
\ShowEq{|dx|<,|dt|<}
следует
\ShowEq{|d phi|< 1}
\labelItem{|d phi|< 1}
\item
В частности, из утверждения
\ShowEq{|dt|<}
следует
\ShowEq{|d phi|< 2}
\labelItem{|d phi|< 2}
\end{enumerate}
Из утверждений
\RefItem{|d phi|< 1},
\RefItem{|d phi|< 2}
следует, что из утверждения
\ShowEq{|dx|<,|dt|<}
следует
\DrawEq{|d phi|< 3}{}
Пусть
\ShowEq{I(t)=}
Поскольку множество $I$ компактно,
то для данного $x$
конечное множество интервалов $I(x,t)$,
которые покрывают множество $I$,
например
\ShowEq{I(x,ti)}
Пусть $\eta(x)$ - наименьшее из чисел $\eta(x,t_i)$.
Так как для любого $t'\in I$ существует $t_i$ такое, что
\ShowEq{|dti|<}
то из утверждения
\ShowEq{|dx|<}
следует
\DrawEq{|d phi|< 3}{1}
для любого $t'\in I$.
Следовательно, отображение $\varphi$ непрерывно в $x$
равномерно по $t$.

Так как
\ShowEq{d psi=}
то, согласно теореме
\RefTheorem{|int f|<int|f|},
\ShowEq{|d psi|<}
Из неравенств
\eqRef{|d phi|< 3}{1},
\EqRef{|d psi|<}
и теоремы
\RefTheorem{int |f|<M mu},
из утверждения
\ShowEq{|dx|<}
следует
\ShowEq{|d psi|< 1}
Следовательно, отображение $\psi$ непрерывно.
\end{proof}

\begin{lemma}
\labelLemma{o1=int o, |o1h/h|->0}
{\it
Пусть
\ShowEq{o:AxI->B}
такое непрерывное отображение, что
\DrawEq{|oh/h|->0}{lemma}
Тогда
\DrawEq{o1=int o}{}
отображение
\ShowEq{f:A->B}{o_1}AB
такое, что
\DrawEq{|o1h/h|->0}{lemma}
}
\end{lemma}
\begin{proof}
Из равенства
\eqRef{|oh/h|->0}{lemma}
следует, что
мы можем записать отображение $o$ как произведение
\ShowEq{o=o2 h}
где
\ShowEq{lim o2=0}
Из непрерывности отображения $o$ следует непрерывность отображения $o_2$.
Так как множество $I$ компактно, то существует отображение
\ShowEq{o3:A->R}
определённое равенством
\ShowEq{o3=max o2}

\begin{lemma}
\labelLemma{o3(h)->0}
{\it
\ShowEq{o3(h)->0}
}
\end{lemma}

{\sc Доказательство.}
Пусть
\ShowEq{o3(h) ne 0}
Тогда существует
\ShowEq{eps>0}
такое, что
\ShowEq{o3>e}
для любого
\EqParm{delta>0}{=z}
и для любого
\ShowEq{h<d}
Так как множество $I$ компактно, то существует $t=t(h)$
такое, что
\ShowEq{o2>e}
для любого
\ShowEq{h<d}
Это утверждение противоречит равенству
\EqRef{lim o2=0}.
Следовательно, утверждение
\EqRef{o3(h) ne 0}
неверно.
\hfill\(\odot\)

Согласно теореме
\RefTheorem{|int h|<int|omega||f1n|},
\ShowEq{|o1|<}
Утверждение
\eqRef{|o1h/h|->0}{lemma}
является следствием утверждения
\EqRef{|o1|<}
и леммы
\RefLemma{o3(h)->0}.
\end{proof}

\begin{theorem}
\labelTheorem{differentiation under integral}
Пусть $A$, $B$ - банаховы алгебры.\,\footnote{
Утверждение аналогично лемме
\citeBib{Cartan differential form}\Hyph 2.12.2
на странице 223.
}
Пусть
\ShowEq{[01]}
- подмножество поля действительных чисел.
Пусть
\ShowEq{phi:UxI->B}
непрерывное отображение.
Пусть отображение
\ShowEq{psi:U->B}
определённо равенством
\DrawEq{psi=int phi}{1}
Если производная
\ShowEq{d phi/dx}
существует во всех точках
\EqParm{x,t in U I}{=c}
то отображение $\psi$ дифференцируемо и
\ShowEq{d psi/dx}
\end{theorem}
\begin{proof}
Пусть производная
\ShowEq{d phi/dx}
существует и является непрерывным отображением
\ShowEq{d phi:UxI->LAB}
Согласно теореме
\RefTheorem{map int continuous is continuous},
отображение
\ShowEq{l=int d phi}
линейно и непрерывно.
Согласно теореме
\RefTheorem{h=fX g1 g2 representation},
равенство
\ShowEq{l=int d phi h}
является следствием равенства
\EqRef{l=int d phi}.

Согласно определению
\RefDefinition{differentiable map, algebra},
\ShowEq{phi x+h - x}
где
\DrawEq{|oh/h|->0}{integral}
Согласно теореме
\RefTheorem{int f+g X},
равенство
\ShowEq{phi x+h - x int}
является следствием равенства
\EqRef{phi x+h - x}.
Положим
\DrawEq{o1=int o}{integral}
Согласно лемме
\RefLemma{o1=int o, |o1h/h|->0},
равенство
\DrawEq{|o1h/h|->0}{integral}
является следствием равенств
\eqRef{|oh/h|->0}{integral},
\eqRef{o1=int o}{integral}.
Равенство
\ShowEq{phi x+h - x int 1}
является следствием равенств
\ShowEq{phi x+h - x int 2}
Равенство
\EqRef{d psi/dx}
является следствием равенств
\EqRef{l=int d phi},
\eqRef{|o1h/h|->0}{integral},
\EqRef{phi x+h - x int 1}
и определения
\RefDefinition{differentiable map, algebra}.
\end{proof}

\begin{theorem}
\labelTheorem{differentiation order n under integral}
Пусть $A$, $B$ - банаховы алгебры.\,\footnote{
Утверждение аналогично следствию
\citeBib{Cartan differential form}\Hyph 2.12.3
на странице 225.
}
Пусть
\ShowEq{[01]}
- подмножество поля действительных чисел.
Пусть
\ShowEq{phi:UxI->B}
отображение класса $C^n$.
Пусть отображение
\ShowEq{psi:U->B}
определённо равенством
\DrawEq{psi=int phi}{}
то отображение $\psi$ является отображением класса $C^n$ и
\ShowEq{d psi/dxn}
\end{theorem}
\begin{proof}
Теорема доказывается по индукции по $n$, так как является следствием теоремы
\RefTheorem{differentiation under integral}
и определения
\EqRef{derivative of Order n, algebra}.
\end{proof}

\begin{theorem}[Теорема Пуанкаре]
\labelTheorem{Poincare Theorem p=1}
Пусть $A$, $B$ - банаховы алгебры.\,\footnote{
Я следую теореме
\citeBib{Cartan differential form}\Hyph 2.12.1
на странице 222.
}
Пусть
\ShowEq{U subset A}
- открытое множество, звёздное относительно $A$\Hyph числа
\EqParm{a in U}{=.}
Если дифференциальная форма
\ShowEq{diff form in U}{\omega}n1B{}
удовлетворяет уравнению
\DrawEq{do=0}{}
то дифференциальная форма $\omega$ интегрируема.
\end{theorem}
\begin{proof}
Мы будем полагать, что $a=0$. В общем случае, за счёт сдвига
мы можем прийти к этому случаю.

Пусть 
\ShowEq{diff form in U}{\omega}n1B.
Положим
\ShowEq{f=int o(tx,x)}
Отображение
\ShowEq{phi(x,t)=o(tx,x)}
является композицией следующих отображений

\begin{itemize}
\item
отображение
\ShowEq{phi1:UxI->UxA}
определенно корректно, так как множество $U$
звёздно относительно $A$\Hyph числа $0$,
и является отображением класса $C^{\infty}$;
\item
отображение
\ShowEq{phi2:UxA->LxA}
является отображением класса $C^n$;
\item
билинейное отображение
\ShowEq{phi3:LxA->B}
является отображением класса $C^{\infty}$.
\end{itemize}
Следовательно, отображение $\varphi$ является отображением класса $C^n$.
Согласно теоремам
\RefTheorem{map int continuous is continuous},
\RefTheorem{differentiation order n under integral},
отображение $f$ является отображением класса $C^n$.

Согласно теореме
\RefTheorem{differentiation under integral},
\ShowEq{df/dx=int...}
Согласно теореме
\RefTheorem{bilinear map and differential},
равенство
\ShowEq{d phi(x,t)/dt=}
является следствием равенства
\EqRef{phi(x,t)=o(tx,x)}.
Утверждение
\DrawEq{do=0}{-}
означает, что
\ShowEq{dw a1 a2}
является билинейным симметричным отображением от $a_1$ и $a_2$.
Следовательно,
\ShowEq{dw a1 a2=dw a2 a1}
Равенство
\ShowEq{d phi(x,t)/dt= 1}
является следствием равенств
\EqRef{d phi(x,t)/dt=},
\EqRef{dw a1 a2=dw a2 a1}.
Равенство
\ShowEq{d phi(x,t)/dt= 2}
является следствием равенства
\EqRef{d phi(x,t)/dt= 1}.
В то же время
\ShowEq{d tw/dt=}
Равенство
\ShowEq{df/dx=int... 1}
является следствием равенств
\EqRef{df/dx=int...},
\EqRef{d phi(x,t)/dt= 2},
\EqRef{d phi(x,t)/dt= 1}.
Положим
\ShowEq{g=t omega}
Равенство
\ShowEq{df/dx=int... 2}
является следствием равенств
\EqRef{df/dx=int... 1},
\EqRef{g=t omega}.
Следовательно, $\omega$ совпадает с дифференциальной формой $df$.
\end{proof}

\begin{theorem}[Теорема Пуанкаре]
Пусть $A$, $B$ - банаховы алгебры.\,\footnote{
Я следую теореме
\citeBib{Cartan differential form}\Hyph 2.12.1
на странице 222.
}
Пусть
\ShowEq{U subset A}
- открытое множество, звёздное относительно $A$\Hyph числа
\EqParm{a in U}{=.}
Если дифференциальная форма
\ShowEq{diff form in U}{\omega}npB{}
удовлетворяет уравнению
\DrawEq{do=0}{}
то дифференциальная форма $\omega$ интегрируема.
\end{theorem}
\begin{proof}
Определим для данного $p$ линейное отображение
\ShowEq{k:Onp->Onp-1}
следующим образом.

\StartLabelItem
\begin{enumerate}
\item
Если
\ShowEq{f in O0n}
положим $k(f)=0$.
\labelItem{map k p=0}
\item
Для $p\ge 1$,
\ShowEq{diff form in U}{\omega}npB,
положим
\DrawEq{k(o)=a}{item}
где
\ShowEq{alpha=int dt omega}
\end{enumerate}

\begin{lemma}
{\it
Отображение $k$ определено корректно.
}
\end{lemma}

{\sc Доказательство.}
Для $p=0$ определение
\RefItem{map k p=0}
равносильно соглашению,
что $D$\Hyph модуль
\ShowEq{On,-1}
сводится к $0$.

Для $p>0$,
рассмотрим косо симметричное полилинейное отображение
\ShowEq{w(tx,x):}
Тогда мы можем записать равенство
\EqRef{alpha=int dt omega}
в следующем виде
\ShowEq{alpha=int dt omega 1}
Из
\EqRef{alpha=int dt omega 1}
следует, что
\ShowEq{alpha in LA}

Отображение
\ShowEq{x,t->w}
является композицией следующих отображений

\begin{itemize}
\item
отображение
\ShowEq{a1:UxI->UxIxA}
определенно корректно, так как множество $U$
звёздно относительно $A$\Hyph числа $0$,
и является отображением класса $C^{\infty}$;
\item
отображение
\ShowEq{a2:UxIxA->LxA}
является отображением класса $C^n$;
\item
отображение
\ShowEq{a3:LxA->L}
является отображением класса $C^{\infty}$.
\end{itemize}
Следовательно, $\alpha$ является дифференциальной $(p-1)$\Hyph формой класса $C^n$.
\hfill\(\odot\)

\begin{lemma}
{\it
Если
\ShowEq{f in O0n}
$n\ge 1$, то
\ShowEq{k df=f-f0}
где $f_0$ - постоянное отображение
\ShowEq{f0:U->B}
}
\end{lemma}

{\sc Доказательство.}
Дифференциальная форма $k(df)$ является отображением
\ShowEq{x->int01}
\hfill\(\odot\)

\begin{lemma}
{\it
Если
\ShowEq{diff form in U}{\omega}npB{}
$n\ge 1$, $p\ge 1$, то
\ShowEq{d(k w)...}
}
\end{lemma}

{\sc Доказательство.}
Равенство
\ShowEq{dw(tx)=}
является следствием равенства
\EqRef{d omega = sum}.
Из равенств
\EqRef{alpha=int dt omega},
\EqRef{dw(tx)=}
следует, что дифференциальная форма
\ShowEq{kdw=b}
определена равенством
\ShowEq{kdw=int}
Согласно теореме
\RefTheorem{differentiation under integral},
равенство
\ShowEq{alpha'=int dt omega'}
является следствием равенства
\EqRef{alpha=int dt omega}.
Равенство
\ShowEq{d alpha=int dt omega'}
является следствием равенств
\EqRef{d omega = sum},
\EqRef{alpha'=int dt omega'}.
Поскольку $\omega$ - косо симметричное отображение,
то верно равенство
\ShowEq{p int tw}
Равенство
\ShowEq{dk+kd=}
является следствием равенств
\ShowEq{dk+kd= ref}
Равенство
\ShowEq{dk+kd= 1}
является следствием равенства
\EqRef{dk+kd=}
В то же время
\ShowEq{d tpw/dt=}
Равенство
\ShowEq{dk+kd= 2}
является следствием равенств
\EqRef{dk+kd= 1},
\EqRef{d tpw/dt=}.
Равенство
\EqRef{d(k w)...}
является следствием равенства
\EqRef{dk+kd= 2}.
\hfill\(\odot\)

Если 
\DrawEq{do=0}{-},
то равенство
\ShowEq{w=d(k w)}
является следствием равенства
\EqRef{d(k w)...}.\
Следовательно, отображение $k$ порождает дифференциальную форму
\DrawEq{k(o)=a}{-}
такую, что
\DrawEq{da=o}{-}.
\end{proof}



==> Diff.Form.2.Russian.tex <==
%auto-ignore

\input{Diff.Form.2.Eq}

\Chapter{Структура дифференциальной формы}

\Section{Полилинейное отображение в ассоциативную \texorpdfstring{$D$}{D}-алгебру}

\begin{theorem}
Пусть $\Basis F$ - базис левого \BoxB{B}модуля
\ShowEq{L(A;B)}DAB.
Мы можем отождествить полилинейное отображение
\ShowEq{f in L(A->B)}{A^n}B{}
и тензор
\ShowEq{b in Bon}
посредством равенства
\ShowEq{f circ=b circ n}
\end{theorem}
\begin{proof}
Доказательство теоремы аналогично доказательству теоремы
\RefTheorem{representation of algebra An in LAnA}.
\end{proof}

\begin{theorem}
Пусть
\ShowEq{f=(b sigma)oI s}
полилинейное отображение. Тогда
\ShowEq{[f]=(b sigma)oI s}
\end{theorem}
\begin{proof}
Равенство
\ShowEq{[f]=(b sigma)oI s 1}
является следствием равенств
\EqRef{alternation of polylinear map =},
\EqRef{f=(b sigma)oI s}.
Равенство
\EqRef{[f]=(b sigma)oI s}
является следствием равенства
\EqRef{[f]=(b sigma)oI s 1}
так как для любого $s$ мы можем заменить сумму по
\EqParm{s2 in S}{=z}
на сумму по
\EqParm{s in S}{=c}
\EqParm{s=s2 o ss}{=.}
При этом
\ShowEq{|s2|=|s||ss|}
\end{proof}

Тензорное представление косо симметричного полилинейного отображения громоздко.
Поэтому, когда возможно, мы будем пользоваться выражением
\ShowEq{b o I}
для представления косо симметричного полилинейного отображения.

\ePrints{1610.309618526,CACAA.06}
\ifx\Semafor\ValueOn
\ShowDefinition{otimes -}

Смотри также определение
\Ref[1302.7204]{definition: otimes -}
и теорему
\RefTheorem[1302.7204]{Am->A(n+m)}
как мы используем операцию
\EqParm{otimes -=}{=c}
чтобы определить произведение многочленов.
\fi

\begin{theorem}
Пусть
\EquationParm{f in LAAB =}{nn=1}
\EquationParm{f in LAAB =}{nn=2}
Тогда
\ShowEq{b1 A b2}
\end{theorem}
\begin{proof}
Равенство
\ShowEq{f1of2o}
является следствием равенств
\EqRefParm{f in LAAB =}{nn=1},
\EqRefParm{f in LAAB =}{nn=2}.
Для любых $s$, $t$,
отображение
\ShowEq{sigma st}
является перестановкой.
Равенство
\ShowEq{f1of2o 1}
является следствием равенств
\EqRef{f1of2o},
\EqRef{sigma st}.
Равенство
\ShowEq{f1of2o 2}
является следствием равенств
\EqRef{otimes -, 1},
\EqRef{f1of2o 1}.
Равенство
\EqRef{b1 A b2}
является следствием равенств
\EqRef{exterior product =},
\EqRef{b o I},
\EqRef{f1of2o 2}.
\end{proof}

\begin{theorem}
Пусть $\Basis e$ - базис конечно мерной $D$\Hyph алгебры $B$.
Пусть
\EquationParm{f in LAAB =}{nn=}
Пусть
\ShowEq{b=b...e}
стандартное представление тензора $b_s$.
Тогда
\ShowEq{f=b...e}
\end{theorem}
\begin{proof}
Равенство
\EqRef{f=b...e}
является следствием равенств\newline
\EqRefParm{f in LAAB =}{nn=},
\EqRef{b=b...e}.
\end{proof}

\Section{Дифференциальная форма со значениями в ассоциативной \texorpdfstring{$D$}{D}-алгебре}

\begin{theorem}
\labelTheorem{tensor is continuous iff}
Пусть $A$, $B$ - ассоциативные конечно мерные банаховы $D$\Hyph алгебры.
Пусть
\ShowEq{U in A}
- открытое множество.
Отображение
\DrawEq{f:U->Bp}{continuous}
непрерывно тогда и только тогда, когда
мы можем представить отображение $f$ в виде
\ShowEq{f=sum f}
где отображения
\ShowEq{fis:U->B}
непрерывны.
\end{theorem}
\begin{proof}
Непосредственное доказательство теоремы сложно.
Например, пусть
\ShowEq{f01:U->B}
непрерывные отображения.
Тогда тензор
\ShowEq{f=f0of1}
является непрерывным отображением
\ShowEq{f:U->B2}
Однако в представлении тензора $f(x)$
\ShowEq{f=f0of1 1}
каждое из слагаемых не
является непрерывным отображением.

Следовательно, не каждое представление непрерывного отображения
\eqRef{f:U->Bp}{continuous}
имеет непрерывные слагаемые.
Однако в нашем распоряжении есть инструмент,
который поможет нам доказать теорему.

Пусть $\Basis e_B$ - базис конечно мерной $D$\Hyph алгебры $B$.
Тогда стандартное представление тензора $f(x)$ имеет вид\,\footnote{
Мы полагаем, что базис $\Basis e_B$ не зависит от $x$.
Однако это утверждение может быть ослаблено,
если мы будем рассматривать расслоенную $D$\Hyph алгебру $B$
над $D$\Hyph алгеброй $A$
(определение расслоенной универсальной алгебры рассмотрено в
\citeBib{0702.561}).
Я рассмотрел возможность построения объекта связности
многообразия над банаховой алгеброй
в разделе
\RefSection[0906.0135]{Manifolds with D-Affine Connections}.
Эта конструкция несущественна для доказательства теоремы
\RefTheorem{tensor is continuous iff}
и будет рассмотрена в последующих статьях.
}
\ShowEq{f(x)=...xe}

\begin{lemma}
\labelLemma{standard components of tensor are continuous maps}
{\it
Отображение $f$ непрерывно тогда и только тогда, когда
все стандартные компоненты тензора $f(x)$
\ShowEq{fi:U->D}
являются непрерывными отображениями.
}
\end{lemma}

{\sc Доказательство.}
Так как все отображения
\ShowEq{fi1p}
непрерывны,
то для произвольного
\EqParm{e>0}{=z}
существует
\ShowEq{d>0}
такое, что из утверждения
\ShowEq{|x-x1|<d}
следует
\ShowEq{|fix-fix1|<e}
для любого отображения
\ShowEq{fi1p}
(это утверждение возможно, так как множество отображений
\ShowEq{fi1p}
конечно).
Равенство
\ShowEq{|fx-fx1|<e 1}
является следствием равенства
\EqRef{|fix-fix1|<e}.

Мы определим норму тензорного произведения
\ShowEq{xei}
согласно определению
\RefDefinition{norm of polylinear map}
\ShowEq{|xei|}
Так как множество тензорных произведений
\ShowEq{xei}
конечно,
то мы положим
\ShowEq{E=max|xei|}
Неравенство
\ShowEq{|fx-fx1|<e 2}
где $k$ число слагаемых в сумме
\EqRef{|fx-fx1|<e 1},
является следствием
\EqRef{|fx-fx1|<e 1},
\EqRef{E=max|xei|}.

Из неравенства
\EqRef{|fx-fx1|<e 2}
следует, что норма
\ShowEq{|fx-fx1|}
может быть сделана сколь угодно малой
при соответствующем выборе $\epsilon$.
Следовательно отображение $f$ непрерывно.

Если мы предложим, что по крайней мере одно из отображений
\ShowEq{fi1p}
не является непрерывным,
то из рассуждений в доказательстве следует, что
отображение $f$ не является непрерывным.
\hfill\(\odot\)

Теорема является следствием леммы
\RefLemma{standard components of tensor are continuous maps}
так как стандартное представление тензора
является частным случаем представления тензора.
\end{proof}

\begin{theorem}
\labelLemma{standard components of tensor are differentiable maps}
Пусть $A$, $B$ - ассоциативные конечно мерные банаховы $D$\Hyph алгебры.
Пусть
\ShowEq{U in A}
- открытое множество.
Отображение
\DrawEq{f:U->Bp}{standard differentiable}
дифференцируемо тогда и только тогда, когда
стандартные компоненты тензора $f(x)$ дифференцируемы.
В этом случае\,\footnote{
Напомню, что отображение
\ShowEq{standard df/dx}
отображает $A$\Hyph число $a$ в $D$\Hyph число
\ShowEq{standard df/dx a}
}
\ShowEq{derivative of standard components of tensor}
\end{theorem}
\begin{proof}
Теорема является следствием теорем
\RefTheorem{bilinear map and differential},
\RefTheorem{definition of module over commutative ring}.
\end{proof}

\begin{theorem}
\labelTheorem{components of tensor are differentiable maps}
Пусть $A$, $B$ - ассоциативные конечно мерные банаховы $D$\Hyph алгебры.
Пусть
\ShowEq{U in A}
- открытое множество.
Отображение
\DrawEq{f:U->Bp}{differentiable}
дифференцируемо тогда и только тогда, когда
мы можем представить отображение $f$ в виде
\ShowEq{f=sum f}
где отображения
\ShowEq{fis:U->B}
дифференцируемы.
В этом случае
\ShowEq{derivative of components of tensor}
\end{theorem}
\begin{proof}
Теорема является следствием теоремы
\RefTheorem{derivative of tensor product}.
\end{proof}

\begin{theorem}
Пусть $A$, $B$ - ассоциативные конечно мерные банаховы $D$\Hyph алгебры.
Пусть
\ShowEq{U in A}
- открытое множество.
Форма
\ShowEq{diff form in U}{\omega}npB{}
тогда и только тогда, когда
мы можем представить форму $\omega$ в виде
\ShowEq{o=sum o}
где
\ShowEq{diff form in U}{\omega_{s\cdot i}}n0B.
\end{theorem}
\begin{proof}
Согласно теоремам
\RefTheorem[\RefCalculus]{|f(a)|<|f||a| 1n},
\RefTheorem[\RefCalculus]{|on|->0 ona1p->0},
отображение
\ShowEq{os Is}
непрерывно, если отображение
\ShowEq{os}
непрерывно.
Утверждение теоремы для $n=0$ является следствием теорем
\RefTheorem{exterior differential of differential form},
\RefTheorem{tensor is continuous iff}.

Пусть теорема верна для $n=k$. Пусть
\ShowEq{diff form in U}{\omega}{k+1}pB.
Следовательно
\ShowEq{diff form in U}{\omega}kpB,
и мы можем представить дифференциальную форму $\omega$ в виде
\ShowEq{o=sum o}
где
\ShowEq{diff form in U}{\omega_{s\cdot i}}k0B.
Мы можем представить дифференциальную форму
\ShowEq{diff form in U}{d^k\omega}1pB{}
в виде
\ShowEq{o=sum o dk}
где
\ShowEq{okis=}
где индекс $s$ зависит от индекса $t$ и $0\le j\le k$.
Согласно теореме
\RefTheorem{components of tensor are differentiable maps},
отображения
\ShowEq{okis}
дифференцируемы
и для любого индекса $s$ существует индекс $t$ такой, что
\ShowEq{okis=k}
Следовательно,
\ShowEq{diff form in U}{\omega_{s\cdot i}}{k+1}0B.
Мы доказали теорему для $n=k+1$.

Следовательно, мы доказали теорему для любого значения $n$.
\end{proof}

\Section{Дифференциальная \texorpdfstring{$1$}{1}-форма}

\begin{theorem}
Пусть $A$, $B$ - свободные банаховые $D$\Hyph алгебры.
Пусть
\ShowEq{U subset A}
- открытое звёздное множество.
Дифференциальная $1$\Hyph форма
\ShowEq{diff form in U}{\omega}n1B{}
интегрируема тогда и только тогда, когда
\ShowEq{d omega=0}
\end{theorem}
\begin{proof}
Если дифференциальная $1$\Hyph форма $\omega$
интегрируема,
то, согласно определению
\RefDefinition{integrable form},
существует отображения $f$ такое, что
\ShowEq{o=df}
Согласно теореме
\RefTheorem{d2omega=0},
\ShowEq{do=d2f}
В тоже время, если
\DrawEq{do=0}{}
то, согласно теореме
\RefTheorem{Poincare Theorem p=1},
дифференциальная $1$\Hyph форма $\omega$ интегрируема.
\end{proof}

\begin{definition}
{\it
Пусть $A$, $B$ - свободные банаховые $D$\Hyph алгебры.
Пусть
\ShowEq{U subset A}
- открытое множество.
Пусть
\ShowEq{g:ab->U}
путь класса $C^1$ в $U$.
\AddIndex{Интеграл дифференциальной $1$\Hyph формы $\omega$ вдоль пути}
{integral of differential 1 form along path}
$\gamma$ определён
равенством
\ShowEq{integral of differential 1 form along path}
\ShowEq{integral of differential 1 form along path =}
}
\qed
\end{definition}

\begin{theorem}
\labelTheorem{int o=sum int a=...<t<...=b}
Пусть
\ShowEq{a=...<t<...=b}
разбиение отрезка $[a,b]$.
Пусть $\gamma_i$ обозначает путь, соответствующий отрезку
\ShowEq{[ti]}
Тогда
\ShowEq{int o=sum int}
\end{theorem}
\begin{proof}
Равенство
\EqRef{int o=sum int}
является следствием равенства
\ShowEq{int ac=int ab+int bc}
и индукции по числу слагаемых.
\end{proof}

\begin{theorem}
\labelTheorem{int df=fb-fa}
Пусть $A$, $B$ - свободные банаховые $D$\Hyph алгебры.
Пусть
\ShowEq{U subset A}
- открытое множество.
Пусть
\ShowEq{g:ab->U}
путь класса $C^1$ в $U$.
Пусть
\ShowEq{f:A->B}fAB
дифференцируемое отображение.
Тогда
\ShowEq{int df=fb-fa}
\end{theorem}
\begin{proof}
Теорема является следствием теоремы
\RefTheorem{Lebesgue Integral along Path}.\,\footnote{
Смотри также теорему
\citeBib{Cartan differential form}\Hyph 3.4.1
на странице 43.
}
\end{proof}

\begin{theorem}
\labelTheorem{integral depends only on origin and extremity}
Пусть $A$, $B$ - свободные банаховые $D$\Hyph алгебры.
Пусть
\ShowEq{U subset A}
- открытое множество.
Пусть
\ShowEq{f:A->B}fAB
дифференцируемое отображение.
Интеграл
\ShowEq{int df}
зависит только от начала $\gamma(a)$ и конца $\gamma(b)$
кусочно гладкого пути $\gamma$.
\end{theorem}
\begin{proof}
Теорема является следствием теорем
\RefTheorem{int o=sum int a=...<t<...=b},
\RefTheorem{int df=fb-fa}.
\end{proof}

\begin{theorem}
Пусть $A$, $B$ - свободные банаховые $D$\Hyph алгебры.
Пусть
\ShowEq{U subset A}
- открытое связное множество.
Следующие свойства дифференциальной формы
\ShowEq{diff form in U}{\omega}n1B{}
эквивалентны
\StartLabelItem
\begin{enumerate}
\item
$\omega$ интегрируемо в $U$
\labelItem{omega is integrable}
\item
\DrawEq{int g o=0}{-}
для любого кусочно гладкого цикла $\gamma$ в $U$ класса $C^1$
\labelItem{int g o=0}
\end{enumerate}
\end{theorem}
\begin{proof}
Утверждение
\RefItem{int g o=0}
является следствием утверждения
\RefItem{omega is integrable}
согласно теоремам
\RefTheorem{int o=sum int a=...<t<...=b},
\RefTheorem{integral depends only on origin and extremity}.

Пусть утверждение
\RefItem{int g o=0}
верно.
Пусть
\ShowEq{x0 x in U}
Так как множество $U$ связно,
то существуют кусочно гладкий путь
\ShowEq{g1:[ab]->U}
и кусочно гладкий путь
\ShowEq{g2:[bc]->U}
Кусочно гладкий путь
\ShowEq{g:[ac]->U}
определённый равенством
\ShowEq{g:[ac]->U =}
является циклом.
Согласно утверждению
\RefItem{int g o=0}
\DrawEq{int g o=0}{proof}
Согласно теореме
\RefTheorem{int o=sum int a=...<t<...=b},
\ShowEq{int g o=1+2}
Из равенств
\eqRef{int g o=0}{proof},
\EqRef{int g o=1+2}
следует, что интеграл
\ShowEq{int g1 o=int g o-int g2 o}
не зависит от пути.
Положим
\ShowEq{fx=int g1 o}

Так как множество $U$ открыто, то существует
\ShowEq{eta1>0}
такое, что линейный путь
\ShowEq{g:[01]->U x+th}
содержится в $U$, если
\ShowEq{|h|<eta1}
Согласно теореме
\RefTheorem{int o=sum int a=...<t<...=b},
равенство
\ShowEq{fx+h=fx+int o}
является следствием равенства
\EqRef{fx=int g1 o}.
Равенство
\ShowEq{fx+h-fx=int o}
является следствием равенств
\EqRef{g:[01]->U x+th},
\EqRef{fx+h=fx+int o}.
Равенство
\ShowEq{fx+h-fx-oh=int o}
является следствием равенства
\EqRef{fx+h-fx=int o}.

Поскольку отображение
\ShowEq{o:U->LAB}
непрерывно, то для любого
\EqParm{eps>0}{=z}
существует
\ShowEq{0<eta<eta1}
такое, что
\ShowEq{oh+t-oh<e}
Утверждение
\ShowEq{(oh+t-oh)h<eh}
является следствием утверждения
\EqRef{oh+t-oh<e}.
Утверждение
\ShowEq{|fx+h-fx-oh|<eh}
является следствием утверждения
\EqRef{(oh+t-oh)h<eh}
и равенства
\EqRef{fx+h-fx-oh=int o}.
Утверждение
\ShowEq{|fx+h-fx-oh|<o(h)}
является следствием утверждения
\EqRef{|fx+h-fx-oh|<eh}.
Из утверждения
\EqRef{|fx+h-fx-oh|<o(h)}
и определения
\RefDefinition{differentiable map, algebra}
следует, что дифференциальная форма $\omega$
является производной отображения $f$.
Следовательно, утверждение
\RefItem{omega is integrable}
является следствием утверждения
\RefItem{int g o=0}.
\end{proof}

\begin{definition}
{\it
Пусть $A$, $B$ - свободные банаховые $D$\Hyph алгебры.
Пусть
\ShowEq{U subset A}
- открытое связное множество.
Пусть дифференциальная форма
\ShowEq{diff form in U}{\omega}n1B{}
интегрируема.
%Если интеграл
%\ShowEq{int h omega}
%не зависит от пути $\gamma$ из $a$ в $b$,
Для любых $A$\Hyph чисел $a$, $b$,
мы определим
\AddIndex{определённый интеграл}{definite integral}
с помощью равенства
\ShowEq{definite integral}
\ShowEq{definite integral ab}
для любого пути $\gamma$ из $a$ в $b$.
}
\qed
\end{definition}

%\section{Дифференциальная \texorpdfstring{$2$}{2}-форма}

%В этом разделе мы рассмотрим дифференциальную $2$\Hyph форму
%\ShowEq{omega=a012}
%Согласно теореме
%\RefTheorem{derivative of tensor product},
%\ShowEq{d omega/dx=a012}
%\ShowEq{d omega/dx=a012o}

\Section{Комплексное поле}

Мы можем рассматривать поле комплексных чисел
либо как $C$\Hyph алгебру, либо как $R$\Hyph алгебру.

\begin{itemize}
\item
$C$\Hyph векторное пространство
\ShowEq{L(A;B)}CCC{}
порождёно отображением $I_0=E$.
Если производная отображения $f$ поля комплексных чисел
принадлежит множеству $CE$,
то отображение $f$ называется
\AddIndex{голоморфным}{holomorphic map}.
Согласно теоремам
\RefTheorem{L(CCC)=CE},
\RefTheorem{Cauchy Riemann equations linear},
голоморфное отображение удовлетворяет дифференциальному уравнению
(уравнения Коши\Hyph Римана)
\ShowEq{Cauchy Riemann equations, complex field, 1}
\item
Согласно теореме
\RefTheorem{linear map of complex field},
$C$\Hyph векторное пространство
\ShowEq{L(A;B)}RCC{}
имеет базис, состоящий из
тождественного отображения $E$
и сопряжения $I$.
Если производная отображения $f$ поля комплексных чисел
принадлежит множеству $CI$,
то отображение $f$ называется
\AddIndex{сопряжённо голоморфным}{conjugate holomorphic map}.
Согласно теоремам
\RefTheorem{L(CCC)=CE},
\RefTheorem{matrix of linear map f in CI},
сопряжённо голоморфное отображение удовлетворяет дифференциальному уравнению
\ShowEq{conjugate holomorphic map}
В этом разделе мы рассмотрим как это сказывается на производной отображения
\ShowEq{f:A->B}fCC
\end{itemize}

\begin{example}
Рассмотрим производную отображения
\ShowEq{y=x*n}
Равенство
\ShowEq{dx*n}
является следствием равенства
\EqRef{y=x*n}.
Согласно определению
\RefDefinition{differentiable map, algebra},
равенство
\ShowEq{dx*n/dx}
является следствием равенства
\EqRef{dx*n}.
Следовательно, ряд Тейлора для отображения
\EqRef{y=x*n}
имеет следующий вид
\ShowEq{y=(Ix)n}
\qed
\end{example}

Теперь мы готовы рассмотреть более сложный пример.

\begin{example}
Рассмотрим производную отображения
\ShowEq{y=xx*2}
Равенство
\ShowEq{xx*2 h1}
является следствием равенства
\EqRef{y=xx*2}.
Согласно определению
\RefDefinition{differentiable map, algebra},
равенство
\ShowEq{dxx*2/dx}
является следствием равенства
\EqRef{xx*2 h1}.
Равенство
\ShowEq{xx*2 h1h2}
является следствием равенства
\EqRef{dxx*2/dx}.
Согласно определению
\RefDefinition{derivative of Second Order, algebra},
равенство\,\footnote{
Когда я увидел симметрию в равенстве
\EqRef{d2xx*2/dx2},
это для меня было неожиданостью.
Первоначальным замыслом этого примера было ожидание
дифференциальной формы подобной дифференциальной форме
\ShowEq{o=3 dx x2},
рассмотренной в замечании
\ref{remark: differential equation 3x^2 does not possess a solution}.
Но потом я понял, что равенство
\EqRef{d2xx*2/dx2}
является следствием теоремы
\RefTheorem{d2omega=0}.
}
\ShowEq{d2xx*2/dx2}
является следствием равенства
\EqRef{xx*2 h1h2}.
Равенство
\ShowEq{d3xx*2/dx3}
\ePrints{1610.309618526,CACAA.06}
\ifx\Semafor\ValueOn
является следствием определения
\RefDefinition{derivative of Order n, algebra}.
\else
является следствием определения
\RefDefinition{derivative of Order n, algebra}
и теоремы
\RefTheorem{derivative, fx=axb, algebra}.
\fi
Следовательно, ряд Тейлора для отображения
\EqRef{y=xx*2}
имеет следующий вид
\ShowEq{y=(Ex)(Ix)2}
\qed
\end{example}

Немедленно возникает следующий вопрос.
Если верно
равенство
\ShowEq{dx*/dx}
то какое отношение это имеет к теории функций комплексного переменного
(\citeBib{Shabat: Complex Analysis})?
Ответ на этот вопрос прост.
Теория функций комплексного переменного рассматривает
$C$\Hyph векторное пространство
\ShowEq{L(A;B)}CCC.
В этом случае не существует линейного отображения,
аппроксимирующего отображение $y=x^*$.
Это утверждение выражено равенством
\ShowEq{dx*/dx=0}
которое означает независимость $x$ и $x^*$.

Поскольку $C$\Hyph векторное пространство $C$
одномерно,
то не существует
косо симметричного полилинейного отображения
\EqParm{f in LA}{f=f,p=2,A=CC,=.}
Однако $R$\Hyph векторное пространство $C$
имеет размерность $2$.
Поэтому существует
косо симметричное полилинейное отображение
\EqParm{f in LA}{f=f,p=2,A=C,=.}

Например, отображение
\ShowEq{fa12=a11 a22-a12 a21}
является косо симметричным полилинейным отображением.
Поскольку
\ShowEq{a11= a12=}
где
\ShowEq{Ia=a*}
отображение сопряжения,
то равенство
\ShowEq{fa12=re im-im re}
является следствием равенства
\EqRef{fa12=a11 a22-a12 a21}.
Мы можем записать полилинейное отображение в примере
\EqRef{fa12=re im-im re}
в виде
\ShowEq{f a1 a2=(I,E)}

\begin{theorem}
\labelTheorem{df/dx= complex field}
Если отображение поля комплексных чисел
\ShowEq{f:A->B}fCC
рассматривать как функцию переменных
\ShowEq{x=x0+ix1}
то
\ShowEq{df/dx= complex field}
\end{theorem}
\begin{proof}
Согласно теореме
\RefTheorem{linear map of complex field},
производная отображения $f$ имеет вид
\ShowEq{df/dx=a0E+a1I}
где
\ShowEq{a01= df/dx}
Равенство
\EqRef{df/dx= complex field}
является следствием равенств
\EqRef{df/dx=a0E+a1I},
\EqRef{a01= df/dx}.
\end{proof}

Согласно теореме
\RefTheorem{linear map of complex field},
дифференциальная $1$\Hyph форма
\EqParm{form x in LA}{form=omega p2,A=C,=z}
имеет вид
\DrawEq{omega=aE+bI}{}
где $a$, $b$ - комплексно значные отображения.
Для любого $C$\Hyph числа $c_1$
\ShowEq{omega c1}

\begin{theorem}
\labelTheorem{omega=aE+bI is integrable}
Дифференциальная форма
\DrawEq{omega=aE+bI}{theorem}
интегрируема тогда и только тогда, когда
\DrawEq{d omega=0 condition}{theorem}
\end{theorem}
\begin{proof}
Производная дифференциальной формы
\eqRef{omega=aE+bI}{theorem}
имеет вид
\ShowEq{do/dx=da/dx+db/dx}
Согласно теореме
\RefTheorem{df/dx= complex field},
\ShowEq{da db /dx}
Равенство
\ShowEq{d omega/dx c1 c2}
является следствием равенств
\EqRef{do/dx=da/dx+db/dx},
\EqRef{d omega/dx c1 c2}.
Внешний дифференциал дифференциальной формы $\omega$ имеет вид
\ShowEq{d omega a12}
Согласно теореме
\RefTheorem{Poincare Theorem p=1},
равенство
\eqRef{d omega=0 condition}{theorem}
является следствием равенства
\EqRef{d omega a12}.
\end{proof}

Пусть
\ShowEq{f=int o}
Мы имеем два различных случая.

\begin{itemize}
\item
Если равенство
\ShowEq{df dx01 =0}
верно, то мы можем представить отображение $f$
как сумму голоморфного отображения
и сопряжённо голоморфного отображения.
\item
Если равенство
\EqRef{df dx01 =0}
не верно, то мы не можем представить отображение $f$
как сумму голоморфного отображения
и сопряжённо голоморфного отображения.
В разделе
\RefSection{differential form in complex field},
мы рассматриваем такую форму.
\end{itemize}


==> Indefinite.Integral.Russian.tex <==
%auto-ignore

\input{Indefinite.Integral.Eq}

\Chapter{Метод последовательного дифференцирования}

\Section{Неопределённый интеграл}
\labelSection{indefinite integral}

\ShowDefinition{indefinite integral}

В этом разделе мы рассмотрим
интегрирование, как операцию, обратную дифференцированию.
По сути дела, мы рассмотрим процедуру решения обыкновенного дифференциального
уравнения
\ShowEq{df=g}

\ShowExample{differential equation y=xx, real number}

\ShowTheorem{int=x3 algebra}
\ShowProof{int=x3 algebra}

\ShowRemark{int=x3 algebra}

\ShowRemark{notation int=x3 algebra}

\ShowRemark{differential equation 3x^2 does not possess a solution}

\Section{Экспонента}

В поле мы можем определить экспоненту как решение
дифференциального уравнения
\ShowEq{exponent over field}
Очевидно, что мы не можем записать подобное уравнения для тела.
Однако мы можем уравнение
\EqRef{exponent over field}
записать в виде
\ShowEq{exponent derivative over field}
Это уравнение уже ближе к нашей цели,
однако остаётся открытым вопрос в каком порядке
мы должны перемножать $y$ и $h$.
Что бы ответить на этот вопрос, мы изменим запись уравнения
\EqRef{exponent derivative over field}
\ShowEq{exponent derivative over division ring}
Следовательно, наша задача - решить дифференциальное уравнение
\EqRef{exponent derivative over division ring}
при начальном условии \[y(0)=1\]

\begin{definition}
\labelDefinition{set of permutations in derivative}
{\it
Для $n\ge 0$, пусть
\ShowEq{set of permutations}
- множество перестановок
\EqParm{derivative, permutation}{K=n,J=}
таких, что каждая перестановка $\sigma$ обладает следующими свойствами
\ifx\setCACAA\undefined
\StartLabelItem
\else
\StartLabelItem[definition]
\fi
\begin{enumerate}
\item Если существуют $i$, $j$, $i\ne j$, такие, что
$\sigma(h_i)$ располагается в произведении
\ShowEq{sigma yh1n}
левее $\sigma(h_j)$ и $\sigma(h_j)$ располагается
левее $\sigma(y)$, то $i<j$.
\labelItem{derivative, permutation n, left}
\item Если существуют $i$, $j$, $i\ne j$, такие, что
$\sigma(h_i)$ располагается в произведении
\ShowEq{sigma yh1n}
правее $\sigma(h_j)$ и $\sigma(h_j)$ располагается
правее $\sigma(y)$, то $i>j$.
\labelItem{derivative, permutation n, right}
\end{enumerate}
}
\qed
\end{definition}

\begin{lemma}
\labelLemma{permutation n+1 generated by permutation n}
{\it
Для $n\ge 0$,
для любой перестановки
\ShowEq{t in Sn+1}
существует единственная перестановка
\ShowEq{s in Sn}
такая, что
\DrawEq{tau yh1...=sigma yh... 1}{->}
или
\DrawEq{tau yh1...=sigma yh... 2}{->}
}
\end{lemma}
\begin{proof}
Рассмотрим произведение
\DrawEq{tau yh...}{->}
Так как $n+1$ - самый большой индекс, то, согласно условиям
\RefItem{derivative, permutation n, left},
\RefItem{derivative, permutation n, right},
$\tau(h_{n+1})$
записано непосредственно перед или непосредственно после $\tau(y)$.
Следовательно, произведение
\eqRef{tau yh...}{->}
имеет либо вид
\eqRef{tau yh1...=sigma yh... 1}{->},
либо вид
\eqRef{tau yh1...=sigma yh... 2}{->}.
Следовательно, для любой перестановки
\ShowEq{t in Sn+1}
существует соответствующая
перестановка
\ShowEq{s in Sn}.
\end{proof}

\begin{lemma}
\labelLemma{permutation n generates permutation n+1, 1}
{\it
Для $n\ge 0$,
для любой перестановки
\ShowEq{s in Sn}.
существует единственная перестановка
\ShowEq{t in Sn+1}
такая, что
\DrawEq{tau yh1...=sigma yh... 1}{<-}
}
\end{lemma}
\begin{proof}
Рассмотрим перестановку
\ShowEq{sigma yh... 1}
Чтобы записать перестановку
\EqParm{derivative, permutation}{K=n+1,J=}
которая удовлетворяет
\eqRef{tau yh1...=sigma yh... 1}{<-},
мы вместо верхнего кортежа
\ShowEq{sigma yh... 1 top}
запишем кортеж
\ShowEq{tau yh1... top}
и вместо нижнего кортежа
\ShowEq{sigma yh... 1 down}
запишем кортеж
\ShowEq{tau yh1... 1 down}
В выражении
\DrawEq{tau yh...}{}
$h_{n+1}$ записано непосредственно перед $y$.
Так как $n+1$ - самое большое значение индекса,
то перестановка $\tau\in S(n+1)$.
\end{proof}

\begin{lemma}
\labelLemma{permutation n generates permutation n+1, 2}
{\it
Для $n\ge 0$,
для любой перестановки
\ShowEq{s in Sn}.
существует единственная перестановка
\ShowEq{t in Sn+1}
такая, что
\DrawEq{tau yh1...=sigma yh... 2}{<-}
}
\end{lemma}
\begin{proof}
Рассмотрим перестановку
\ShowEq{sigma yh... 2}
Чтобы записать перестановку
\EqParm{derivative, permutation}{K=n+1,J=}
которая удовлетворяет
\eqRef{tau yh1...=sigma yh... 2}{<-},
мы вместо верхнего кортежа
\ShowEq{sigma yh... 2 top}
запишем кортеж
\ShowEq{tau yh1... top}
и вместо нижнего кортежа
\ShowEq{sigma yh... 2 down}
запишем кортеж
\ShowEq{tau yh1... 2 down}
В выражении
\DrawEq{tau yh...}{}
$h_{n+1}$ записано непосредственно после $y$.
Так как $n+1$ - самое большое значение индекса,
то перестановка $\tau\in S(n+1)$.
\end{proof}

\begin{theorem}
\labelTheorem{permutation sigma generates permutation tau, n=2k}
\ShowEq{tau yh1...=sigma yh... +}
\end{theorem}
\begin{proof}
Теорема является следствием лемм
\RefLemma{permutation n+1 generated by permutation n},
\RefLemma{permutation n generates permutation n+1, 1},
\RefLemma{permutation n generates permutation n+1, 2}.
\end{proof}

\begin{theorem}
\labelTheorem{exponent derivative n over division ring}
Производная порядка $n$ отображения $y$,
удовлетворяющего дифференциальному уравнению
\EqRef{exponent derivative over division ring}
имеет вид
\ShowEq{exponent derivative n over division ring}
\end{theorem}
\begin{proof}
Мы докажем это утверждение индукцией.
Для $n=0$ утверждение верно, так как это утверждение $y=y$.
Для $n=1$ утверждение верно, так как это дифференциальное уравнение
\EqRef{exponent derivative over division ring}.
Пусть утверждение верно для $n=k-1$.
Следовательно
\ShowEq{exponent derivative n=k-1}
Согласно определению
\ShowEq{ref derivative of Order n, algebra}
производная порядка $k$ имеет вид
\ShowEq{exponent derivative n=k, 1}
Из равенств
\EqRef{exponent derivative over division ring},
\EqRef{exponent derivative n=k, 1}
следует
\ShowEq{exponent derivative n=k, 2}
Из равенств
\EqRef{tau yh1...=sigma yh... +},
\EqRef{exponent derivative n=k, 2}
следует, что
утверждение теоремы верно для $n=k$.
Теорема доказана.
\end{proof}

\begin{theorem}
\labelTheorem{exponent}
Решением дифференциального уравнения
\EqRef{exponent derivative over division ring}
при начальном условии $y(0)=1$ является
\AddIndex{экспонента}{exponent}
\ShowEq{exponent over division ring}
которая имеет следующее разложение в ряд Тейлора
\ShowEq{exponent Taylor series}
\end{theorem}
\begin{proof}
Производная порядка $n$ содержит $2^n$ слагаемых.
Действительно, производная порядка $1$ содержит $2$ слагаемых,
и каждое дифференцирование увеличивает число слагаемых вдвое.
Из начального условия $y(0)=1$ и теоремы
\RefTheorem{exponent derivative n over division ring}
следует, что производная порядка $n$
искомого решения имеет вид
\ShowEq{exponent derivative n, x=0}
Из
\EqRef{exponent derivative n, x=0}
следует разложение
\EqRef{exponent Taylor series}
в ряд Тейлора.
\end{proof}

\begin{theorem}
\labelTheorem{exponent of sum}
Равенство
\ShowEq{exponent of sum}
справедливо тогда и только тогда, когда
\ShowEq{exponent of sum, 1}
\end{theorem}
\begin{proof}
Для доказательства теоремы достаточно рассмотреть ряды Тейлора
\ShowEq{exponent a b a+b}
Перемножим выражения
\EqRef{exponent a} и \EqRef{exponent b}.
Сумма одночленов порядка $3$ имеет вид
\ShowEq{exponent ab 3}
и не совпадает, вообще говоря, с выражением
\ShowEq{exponent a+b 3}
Доказательство утверждения, что
\EqRef{exponent of sum} следует из \EqRef{exponent of sum, 1}
тривиально.
\end{proof}

\Section{Гиперболическая тригонометрия}

Чтобы определить гиперболический синус
\ShowEq{y1=sh}
и гиперболический косинус
\ShowEq{y2=ch}
мы рассмотрим систему дифференциальных уравнений в поле действительных чисел
\ShowEq{d sh ch R}
и начальные условия
\DrawEq{d sh ch init}{real}
Система дифференциальных уравнений
\EqRef{d sh ch R},
\eqRef{d sh ch init}{real}
эквивалентна дифференциальным уравнениям
\ShowEq{d2 sh}
\ShowEq{d2 ch}

В банаховой $D$\Hyph алгебре $A$
мы запишем систему дифференциальных уравнений
\EqRef{d sh ch R},
\eqRef{d sh ch init}{real}
в форме аналогичной дифференциальному уравнению
\EqRef{exponent derivative over division ring}
\ShowEq{d sh ch A}
\DrawEq{d sh ch init}{}

\begin{theorem}
Производная порядка $n$ отображений $y_1$, $y_2$,
удовлетворяющих системе дифференциальных уравнений
\EqRef{d sh ch A}
имеет вид
\ShowEq{sh ch derivative n}
\end{theorem}
\begin{proof}
Мы докажем это утверждение индукцией.
Для $n=0$ утверждение верно, так как это утверждение $y_1=y_1$, $y_2=y_2$.
Для $n=1$ утверждение верно, так как это система дифференциальных уравнений
\EqRef{d sh ch A}.
Пусть утверждение верно для $n=k-1$.
Следовательно
\ShowEq{sh ch derivative n=k-1}
где
$i=1$, $2$ и
\ShowEq{j=i,2-i}
$j=i$, если $k-1=2m$; в противном случае $j=2-i$.
Согласно определению
\ShowEq{ref derivative of Order n, algebra}
производная порядка $k$ имеет вид
\ShowEq{sh ch derivative n=k, 1}
Из
\EqRef{d sh ch A},
\EqRef{sh ch derivative n=k, 1}
следует
\ShowEq{sh ch derivative n=k, 2}
где
\ShowEq{l=2-j}
Из
\EqRef{j=i,2-i},
\EqRef{l=2-j},
следует, что
\ShowEq{l=i,2-i}
Из
\EqRef{tau yh1...=sigma yh... +},
\EqRef{sh ch derivative n=k, 2}
следует, что
утверждение теоремы верно для $n=k$.
Теорема доказана.
\end{proof}

\begin{theorem}
\labelTheorem{sh ch}
Решением системы дифференциальных уравнений
\EqRef{d sh ch A}
при начальном условии
\DrawEq{d sh ch init}{Taylor}
является пара отображений
\begin{itemize}
\item
\AddIndex{гиперболический синус}{hyperbolic sine}
\ShowEq{hyperbolic sine}
который имеет следующее разложение в ряд Тейлора
\ShowEq{hyperbolic sine Taylor series}
\item
\AddIndex{гиперболический косинус}{hyperbolic cosine}
\ShowEq{hyperbolic cosine}
который имеет следующее разложение в ряд Тейлора
\ShowEq{hyperbolic cosine Taylor series}
\end{itemize}
\end{theorem}
\begin{proof}
Производная порядка $n$ содержит $2^n$ слагаемых.
Действительно, производная порядка $1$ содержит $2$ слагаемых,
и каждое дифференцирование увеличивает число слагаемых вдвое.
Из начального условия
\eqRef{d sh ch init}{Taylor}
и равенства
\EqRef{sh ch derivative n}
следует, что производная порядка $n$ искомого решения имеет вид
\ShowEq{sh ch derivative n, x=0}
Из
\EqRef{sh ch derivative n, x=0}
следуют разложения
\EqRef{hyperbolic sine Taylor series},
\EqRef{hyperbolic cosine Taylor series}
в ряд Тейлора.
\end{proof}

\begin{theorem}
Система дифференциальных уравнений
\DrawEq{d sh A}{sinh}
\ShowEq{d ch A}
эквивалентна дифференциальному уравнению
\ShowEq{d2 sh A}
\end{theorem}
\begin{proof}
Из дифференциального уравнения
\eqRef{d sh A}{sinh}
следует, что
\DrawEq{d2 sh A 1}{sinh}
Из
\EqRef{d ch A},
\eqRef{d2 sh A 1}{sinh}
следует, что
\ShowEq{d2 sh A 2}
Дифференциальное уравнение
\EqRef{d2 sh A}
следует из
\EqRef{d2 sh A 2}.
\end{proof}

\Section{Эллиптическая тригонометрия}

Чтобы определить синус
\ShowEq{y1=sin}
и косинус
\ShowEq{y2=cos}
мы рассмотрим систему дифференциальных уравнений в поле действительных чисел
\ShowEq{d sin cos R}
и начальные условия
\DrawEq{d sh ch init}{real sin}
Система дифференциальных уравнений
\EqRef{d sin cos R},
\eqRef{d sh ch init}{real sin}
эквивалентна дифференциальным уравнениям
\ShowEq{d2 sin}
\ShowEq{d2 cos}

В банаховой $D$\Hyph алгебре $A$
мы запишем систему дифференциальных уравнений
\EqRef{d sin cos R},
\eqRef{d sh ch init}{real sin}
в форме аналогичной дифференциальному уравнению
\EqRef{exponent derivative over division ring}
\ShowEq{d sin cos A}
\DrawEq{d sh ch init}{}

\begin{theorem}
Производная порядка $n$ функции $y_1$, $y_2$,
удовлетворяющих системе дифференциальных уравнений
\EqRef{d sin cos A}
имеет вид
\begin{itemize}
\item $n=2k$
\ShowEq{sin cos derivative n=2k}
\item $n=2k+1$
\ShowEq{sin cos derivative n=2k+1}
\end{itemize}
\end{theorem}
\begin{proof}
Мы докажем это утверждение индукцией.
Для $k=0$ утверждение верно:
\begin{itemize}
\item
Если $n=2k$,
то это утверждение $y_1=y_1$, $y_2=y_2$.
\item
Если $n=2k+1$,
то утверждение следует из системы дифференциальных уравнений
\EqRef{d sin cos A}.
\end{itemize}
Пусть утверждение верно для $k=l-1$.
Следовательно, для $n=2k+1$,
\ShowEq{sin derivative n=2k+1 k=l-1}
\ShowEq{cos derivative n=2k+1 k=l-1}
Согласно определению
\ShowEq{ref derivative of Order n, algebra},
из
\EqRef{sin derivative n=2k+1 k=l-1},
\EqRef{cos derivative n=2k+1 k=l-1}
следует, что
производные порядка $m=n+1$ имеют вид
\ShowEq{sin derivative m=2k+2 k=l-1, 1}
\ShowEq{cos derivative m=2k+2 k=l-1, 1}
Из
\EqRef{d sin cos A},
\EqRef{sin derivative m=2k+2 k=l-1, 1},
\EqRef{cos derivative m=2k+2 k=l-1, 1}
следует, что
\ShowEq{sin derivative m=2k+2 k=l-1, 2}
\ShowEq{cos derivative m=2k+2 k=l-1, 2}
Из
\EqRef{tau yh1...=sigma yh... +},
\EqRef{sin derivative m=2k+2 k=l-1, 2},
\EqRef{cos derivative m=2k+2 k=l-1, 2}
следует, что
\ShowEq{sin cos derivative m=2k+2 k=l-1, 2}
Так как
\ShowEq{m=2l}
то равенства
\EqRef{sin cos derivative n=2k}
верны для $k=l$, $n=2k$.

Согласно определению
\ShowEq{ref derivative of Order n, algebra}
из
\EqRef{sin cos derivative n=2k}
следует, что
производные порядка $m=n+1$ имеют вид
\ShowEq{sin derivative m=2k+1 k=l, 1}
\ShowEq{cos derivative m=2k+1 k=l, 1}
Из
\EqRef{d sin cos A},
\EqRef{sin derivative m=2k+1 k=l, 1},
\EqRef{cos derivative m=2k+1 k=l, 1}
следует, что
\ShowEq{sin derivative m=2k+1 k=l, 2}
\ShowEq{cos derivative m=2k+1 k=l, 2}
Так как
\ShowEq{m=2k+1}
то равенства
\EqRef{sin cos derivative n=2k+1}
являются следствием
\EqRef{tau yh1...=sigma yh... +},
\EqRef{sin derivative m=2k+1 k=l, 2},
\EqRef{cos derivative m=2k+1 k=l, 2}.
\EqRef{sin cos derivative n=2k}
для $k=l$, $n=2k+1$.

Теорема доказана.
\end{proof}

\begin{theorem}
\labelTheorem{sin cos}
Решением системы дифференциальных уравнений
\EqRef{d sin cos A}
при начальном условии
\DrawEq{d sh ch init}{Taylor syn}
является пара отображений
\begin{itemize}
\item
\AddIndex{синус}{sine}
\ShowEq{sine}
который имеет следующее разложение в ряд Тейлора
\ShowEq{sine Taylor series}
\item
\AddIndex{косинус}{cosine}
\ShowEq{cosine}
который имеет следующее разложение в ряд Тейлора
\ShowEq{cosine Taylor series}
\end{itemize}
\end{theorem}
\begin{proof}
Производная порядка $n$ содержит $2^n$ слагаемых.
Действительно, производная порядка $1$ содержит $2$ слагаемых,
и каждое дифференцирование увеличивает число слагаемых вдвое.
Из начального условия
\eqRef{d sh ch init}{Taylor syn}
и равенств
\EqRef{sin cos derivative n=2k},
\EqRef{sin cos derivative n=2k+1}
следует, что производная порядка $n$
искомого решения имеет вид
\begin{itemize}
\item $n=2k$
\ShowEq{sin cos derivative n=2k, x=0}
\item $n=2k+1$
\ShowEq{sin cos derivative n=2k+1, x=0}
\end{itemize}
Из
\EqRef{sin cos derivative n=2k, x=0},
\EqRef{sin cos derivative n=2k+1, x=0}
следуют разложения
\EqRef{sine Taylor series},
\EqRef{cosine Taylor series}
в ряд Тейлора.
\end{proof}

\begin{theorem}
Система дифференциальных уравнений
\DrawEq{d sh A}{sine}
\ShowEq{d cos A}
эквивалентна дифференциальному уравнению
\ShowEq{d2 sin A}
\end{theorem}
\begin{proof}
Из дифференциального уравнения
\eqRef{d sh A}{sine}
следует, что
\DrawEq{d2 sh A 1}{sine}
Из
\EqRef{d cos A},
\eqRef{d2 sh A 1}{sine}
следует, что
\ShowEq{d2 sin A 2}
Дифференциальное уравнение
\EqRef{d2 sin A}
следует из
\EqRef{d2 sin A 2}.
\end{proof}



==> Index.Russian.tex <==
%auto-ignore
\OpenIndex
\SetIndexSpace%
\Index%192%*%*A-векторное пространство
   {$*A$\Hyph векторное пространство}%
   {*A-vector space}%
\Index%202%*%*D вектор строка
   {$*D$\Hyph вектор строка}%
   {row *D vector}%
\Index%9%*%CR произведение
   {\CR произведение}%
   {cr-product}%
\Index%66%*%RC произведение
   {\RC произведение}%
   {rc-product}%
\SetIndexSpace%
\Index%1%1%1-форма
   {$1$\Hyph форма}%
   {1-form}%
\SetIndexSpace%
\Index%2%2%2- арное расслоенное отношение
   {$2$\Hyph арное расслоенное отношение}%
   {2 ary fibered relation}%
\SetIndexSpace%
\Index%819%A%A алгебра многочленов над D алгеброй
   {$A$\Hyph алгебра многочленов над $D$\Hyph алгеброй $A$}%
   {algebra of polynomials over algebra}%
\Index%5%A%A- значная функция
   {$A$\Hyph значная функция}%
   {A valued function}%
\Index%685%A%A- модуль
   {$A$\Hyph модуль}%
   {module over algebra}%
\Index%818%A%A число
   {$A$\Hyph число}%
   {A number}%
\Index%603%A%A(A) отображение
   {$\mathcal A(A)$\Hyph отображение}%
   {A(A) map}%
\Index%660%A%A*- модуль
   {$A*$\Hyph модуль}%
   {A*-module}%
\Index%575%A%A*-векторное пространство
   {$A*$\Hyph векторное пространство}%
   {A*-vector space}%
\Index%582%A%Arc базис в векторном пространстве
   {$A\RCstar$\Hyph базис в векторном пространстве}%
   {Arc basis, vector space}%
\Index%864%A%A-представление в Omega алгебре
   {$A$\Hyph представление в $\Omega$\Hyph алгебре}%
   {A representation of algebra}%
\Index%3%A%j i-CR квазидетерминант
   {$(^j_i)$\hyph \CR квазидетерминант}%
   {j i cr-quasideterminant}%
\SetIndexSpace%
\Index%799%B%b множество
   {$B$\Hyph множество}%
   {B set}%
\SetIndexSpace%
\Index%6%C%c строка матрицы
   {\subs строка матрицы}%
   {c row}%
\Index%7%C%CR матричная группа
   {\CR матричная группа}%
   {cr-matrix group}%
\Index%8%C%CR обратный элемент бикольца
   {\CR обратный элемент бикольца}%
   {cr-inverse element}%
\Index%589%C%cr произведение матриц отображений
   {$\CRcirc$\Hyph произведение матриц отображений}%
   {cr product of matrices of maps}%
\Index%10%C%CR степень
   {\CR степень}%
   {cr power}%
\Index%304%C%crd вектор
   {\crd вектор}%
   {crd vector}%
\Index%11%C%crd векторное пространство
   {\crd векторное пространство}%
   {crd vector space}%
\Index%768%C%Cstar-алгебра
   {$C^*$\Hyph алгебра}%
   {Cstar-algebra}%
\Index%12%C%c-строка матрицы
   {$c$\hyph строка матрицы}%
   {c-row}%
\SetIndexSpace%
\Index%251%D%D- алгебра
   {$D$\Hyph алгебра}%
   {D algebra}%
\Index%549%D%D- аффинная связность на многообразии аффинной связности
   {$D$\Hyph аффинная связность на многообразии аффинной связности}%
   {D affine connection, affine manifold}%
\Index%14%D%D- вектор- функция
   {$D$\Hyph вектор\Hyph функция}%
   {d vector function}%
\Index%48%D%D- значная переменная
   {$D$\Hyph значная переменная}%
   {D valued variable}%
\Index%581%D%D линейный функционал
   {$D$\Hyph линейный функционал}%
   {D linear functional}%
\Index%584%D%D- модуль
   {$D$\Hyph модуль}%
   {D module}%
\Index%71%D%D- модуль
   {$D$\Hyph модуль}%
   {D-module}%
\Index%92%D%D* вектор столбец
   {$D*$\Hyph вектор столбец}%
   {column D* vector}%
\Index%93%D%D* вектор строка
   {$D*$\Hyph вектор строка}%
   {row D* vector}%
\Index%87%D%D*- векторное пространство матриц
   {$D*$\hyph векторное пространство матриц}%
   {matrices vector space}%
\Index%40%D%D*-векторное пространство
   {$D*$\hyph векторное пространство}%
   {D* vector space}%
\Index%156%D%D*-модуль
   {$D*$\Hyph модуль}%
   {D*-module}%
\Index%18%D%dcr векторное пространство
   {\dcr векторное пространство}%
   {dcr vector space}%
\Index%38%D%dcr производная Гато отображения f D- векторного пространства V в D- векторное пространство W
   {\dcr производная Гато отображения $\Vector f$ $D$\Hyph векторного пространства $V$ в $D$\Hyph векторное пространство $W$}%
   {Gateaux dcr derivative of map, D vector space}%
\Index%17%D%drc вектор
   {\drc вектор}%
   {drc vector}%
\Index%200%D%drc вектор
   {\dcr вектор}%
   {dcr vector}%
\Index%28%D%drc векторное пространство
   {\drc векторное пространство}%
   {drc vector space}%
\Index%36%D%Drc линейное отображение векторных расслоений
   {\Drc линейное отображение векторных расслоений}%
   {drc linear map of vector bundles}%
\Index%771%D%Dstar антилинейный гомоморфизм
   {$D\star$\Hyph антилинейный гомоморфизм}%
   {Dstar antilinear homomorphism}%
\Index%39%D%Dstar- векторное поле
   {$\mathcal D\star$\Hyph векторное поле}%
   {Dstar vector field}%
\Index%41%D%Dstar- векторное расслоение
   {$\mathcal D\star$\Hyph векторное расслоение}%
   {Dstar vector bundle}%
\Index%46%D%Dstar производная Гато функции f тела D
   {\Ds производная Гато функции $f$ тела $D$}%
   {Gateaux Dstar derivative of map, division ring}%
\Index%47%D%Dstar производная Фреше отображения f тела D в точке x
   {\Ds производная Фреше отображения $f$ тела $D$ в точке $x$}%
   {Frechet Dstar derivative of map, division ring}%
\Index%43%D%Dstar-линейная комбинация векторных полей
   {$\mathcal D\star$\hyph линейная комбинация векторных полей}%
   {linear composition of vector fields}%
\Index%45%D%Dstar-произведение векторного поля на скаляр
   {$\mathcal D\star$\hyph произведение векторного поля на скаляр}%
   {Dstar product of vector field over scalar, vector space}%
\Index%15%D%D-векторное пространство
   {$D$\hyph векторное пространство}%
   {D vector space}%
\SetIndexSpace%
\Index%50%E%enhanced Lie group
   {enhanced Lie group}%
   {enhanced Lie group}%
\SetIndexSpace%
\Index%55%G%$G$\Hyph пространство
   {$G$\Hyph пространство}%
   {GSpace}%
\Index%52%G%G- система отсчёта
   {$G$\Hyph система отсчёта}%
   {G reference frame}%
\Index%53%G%G-basis векторного пространства
   {$G$\Hyph базис векторного пространства}%
   {G-basis}%
\Index%54%G%G-координаты базиса
   {$G$\Hyph координаты базиса}%
   {G-coordinates}%
\SetIndexSpace%
\Index%596%J%j i RCcirc квазидетерминант
   {$(^j_i)$\hyph $\RCcirc$\Hyph квазидетерминант}%
   {j i RCcirc-quasideterminant}%
\Index%678%J%ji- квазидетерминант
   {$(ji)$\hyph квазидетерминант}%
   {j i quasideterminant}%
\SetIndexSpace%
\Index%57%M%m- вектор
   {$m$\Hyph вектор}%
   {m-vector}%
\Index%56%M%m- мерный параллепипед
   {$m$\Hyph мерный параллепипед}%
   {m dimensional parallelepiped}%
\SetIndexSpace%
\Index%58%N%n- арное расслоенное отношение
   {$n$\Hyph арное расслоенное отношение}%
   {fibered relation}%
\Index%845%N%n-арная операция на множестве
   {$n$\Hyph арная операция на множестве}%
   {n-ary operation on set}%
\SetIndexSpace%
\Index%4%R%j i-RC квазидетерминант
   {$(^j_i)$\hyph \RC квазидетерминант}%
   {j i RC-quasideterminant}%
\Index%728%R%R- модуль
   {$R$\Hyph модуль}%
   {R- module}%
\Index%59%R%r строка матрицы
   {\sups строка матрицы}%
   {r row}%
\Index%60%R%RC вырожденная матрица
   {\RC вырожденная матрица}%
   {RC singular matrix}%
\Index%61%R%RC главная минорная матрица
   {\RC главная минорная матрица}%
   {RC-major minor}%
\Index%62%R%RC квазидетерминант
   {\RC квазидетерминант}%
   {RC-quasideterminant}%
\Index%63%R%RC матричная группа
   {\RC матричная группа}%
   {rc-matrix group}%
\Index%64%R%RC невырожденная матрица
   {\RC невырожденная матрица}%
   {RC nonsingular matrix}%
\Index%65%R%RC обратный элемент бикольца
   {\RC обратный элемент бикольца}%
   {rc-inverse element}%
\Index%590%R%rc произведение матриц отображений
   {$\RCcirc$\Hyph произведение матриц отображений}%
   {rc product of matrices of maps}%
\Index%67%R%RC ранг матрицы
   {\RC ранг матрицы}%
   {rc-rank of matrix}%
\Index%68%R%RC степень
   {\RC степень}%
   {rc power}%
\Index%600%R%RCcirc вырожденная матрица
   {$\RCcirc$\Hyph вырожденная матрица}%
   {RCcirc singular matrix}%
\Index%597%R%RCcirc квазидетерминант
   {$\RCcirc$\Hyph квазидетерминант}%
   {RCcirc-quasideterminant definition}%
\Index%601%R%RCcirc невырожденная матрица
   {$\RCcirc$\Hyph невырожденная матрица}%
   {RCcirc nonsingular matrix}%
\Index%602%R%RCcirc невырожденная система аддитивных уравнений
   {$\RCcirc$\Hyph невырожденная система аддитивных уравнений}%
   {RCcirc nonsingular system of additive equations}%
\Index%759%R%rcd аффинная плоскость
   {\rcd аффинная плоскость}%
   {rcd affine plane}%
\Index%736%R%rcd аффинное пространство
   {\rcd аффинное пространство}%
   {rcd affine space}%
\Index%27%R%rcd вектор
   {\rcd вектор}%
   {rcd vector}%
\Index%69%R%rcd векторное пространство
   {\rcd векторное пространство}%
   {rcd vector space}%
\Index%13%R%rcd производная Гато отображения f D-векторного пространства V в D-векторное пространство W
   {\rcd производная Гато отображения $f$ $D$\hyph векторного пространства $V$ в $D$\hyph векторное пространство $W$}%
   {Gateaux rcd derivative of map, D vector space}%
\Index%72%R%r-строка матрицы
   {$r$\hyph строка матрицы}%
   {r-row}%
\Index%510%R%частная rcd производная Гато отображения fb по переменной xa
   {частная \rcd производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial rcd derivative of map with respect to variable, D vector space}%
\SetIndexSpace%
\Index%74%S%SRCstar,TRCstar- линейное отображение векторных расслоений
   {$(\mathcal S\RCstar,\mathcal T\RCstar)$\Hyph линейное отображение векторных расслоений}%
   {src trc linear map of vector bundles}%
\Index%112%S%Sstar, star T-бимодуль
   {($S\star$, $\star T$)\hyph бимодуль}%
   {(Sstar,starT)-bimodule}%
\Index%669%S%star A- модуль
   {$\star A$\Hyph модуль}%
   {starA-module}%
\Index%79%S%star R-модуль
   {$\star R$\hyph модуль}%
   {starR-module}%
\Index%76%S%starD производная Гато функции f тела D
   {\sD производная Гато функции $f$ тела $D$}%
   {Gateaux starD derivative of map, division ring}%
\Index%198%S%starD-произведение вектора на скаляр
   {$\star D$\hyph произведение вектора на скаляр}%
   {starD product of vector over scalar, vector space}%
\Index%83%S%starT- представление расслоенной Omega- алгебры
   {\sT представление расслоенной $\Omega$\Hyph алгебры}%
   {starT representation of fibered Omega-algebra}%
\Index%84%S%starT- представление расслоенной группы
   {\sT представление расслоенной группы}%
   {starT representation of fibered group}%
\Index%185%S%starT- представление расслоенной группы
   {\sT представление расслоенной группы}%
   {starT representation of fibered group}%
\Index%86%S%starT- преобразование расслоения
   {\sT преобразование расслоения}%
   {starT transformation of bundle}%
\Index%81%S%starT- сдвиг на расслоении групп
   {\sT сдвиг на расслоении групп}%
   {starT shift, fibered group}%
\SetIndexSpace%
\Index%823%T%T_1 пространство
   {$T_1$\Hyph пространство}%
   {T1 space}%
\Index%91%T%Tstar- представление расслоенной Omega- алгебры
   {\Ts представление расслоенной $\Omega$\Hyph алгебры}%
   {Tstar representation of fibered Omega-algebra}%
\Index%187%T%Tstar- представление расслоенной группы
   {\Ts представление расслоенной группы}%
   {Tstar representation of fibered group}%
\SetIndexSpace%
\Index%645%А%абелевая Omega группа
   {абелевая $\Omega$\Hyph группа}%
   {Abelian Omega group}%
\Index%830%А%абелевая мультипликативная Omega группа
   {абелевая мультипликативная $\Omega$\Hyph группа}%
   {Abelian multiplicative Omega group}%
\Index%869%А%абелевая полугруппа
   {абелевая полугруппа}%
   {Abelian semigroup}%
\Index%284%А%абсолютная величина
   {абсолютная величина}%
   {absolute value}%
\Index%859%А%автоморфизм
   {автоморфизм}%
   {automorphism}%
\Index%560%А%автоморфизм башни представлений
   {автоморфизм башни представлений}%
   {automorphism of tower of representations}%
\Index%22%А%автоморфизм векторного пространства
   {автоморфизм векторного пространства}%
   {automorphism of vector space}%
\Index%94%А%автоморфизм представления Omega алгебры
   {автоморфизм представления $\Omega$\Hyph алгебры}%
   {automorphism of representation}%
\Index%95%А%автопараллельная кривая
   {автопараллельная кривая}%
   {auto parallel line}%
\Index%805%А%аддитивное отображение
   {аддитивное отображение}%
   {additive map}%
\Index%99%А%активное *G представление
   {активное \sT{G}представление}%
   {active representation, vector space}%
\Index%100%А%активное представление
   {активное представление}%
   {active representation}%
\Index%716%А%активное представление группы в многообразии базисов башни представлений
   {активное представление группы $G(\Vector  f)$ в многообразии базисов  башни представлений}%
   {active representation in basis manifold, tower of representations}%
\Index%569%А%активное представление группы в многообразии базисов представления
   {активное представление группы $G(f)$ в многообразии базисов представления}%
   {active representation in basis manifold}%
\Index%715%А%активное преобразование многообразия базисов башни представлений
   {активное преобразование многообразия базисов башни представлений}%
   {active transformation of basis, tower of representations}%
\Index%326%А%активное преобразование многообразия базисов представления
   {активное преобразование многообразия базисов представления}%
   {active transformation of basis, representation}%
\Index%101%А%активное преобразование на многообразии базисов
   {активное преобразование на многообразии базисов}%
   {active transformation}%
\Index%102%А%активное преобразование на множестве rcd базисов
   {активное преобразование на множестве \rcd базисов}%
   {active transformation, vector space}%
\Index%103%А%алгебра E кватернионов над полем F
   {алгебра $E$ кватернионов над полем $F$}%
   {quaternion algebra over the field}%
\Index%808%А%алгебра Бореля
   {алгебра Бореля}%
   {Borel algebra}%
\Index%741%А%алгебра кватернионов
   {алгебра кватернионов}%
   {quaternion algebra}%
\Index%104%А%алгебра Ли группы Ли
   {алгебра Ли группы Ли}%
   {algebra Lie group Lie}%
\Index%487%А%алгебра многочленов над D алгеброй
   {алгебра многочленов над $D$\Hyph алгеброй}%
   {algebra of polynomials over D algebra}%
\Index%797%А%алгебра множеств
   {алгебра множеств}%
   {algebra of sets}%
\Index%607%А%алгебра над кольцом
   {алгебра над кольцом}%
   {algebra over ring}%
\Index%639%А%алгебра октонионов
   {алгебра октонионов}%
   {octonion algebra}%
\Index%618%А%алгебра рациональных отображений алгебры
   {алгебра рациональных отображений алгебры}%
   {algebra of rational mappings of algebra}%
\Index%167%А%алгебра с делением
   {алгебра с делением}%
   {division algebra}%
\Index%780%А%алгебра с сопряжением
   {алгебра с сопряжением}%
   {algebra with conjugation}%
\Index%786%А%алгебра скаляров алгебры
   {алгебра скаляров алгебры}%
   {scalar algebra of algebra}%
\Index%775%А%алгебра скаляров кольца
   {алгебра скаляров кольца}%
   {scalar algebra of ring}%
\Index%400%А%алгебра частных алгебры с сопряжением
   {алгебра частных алгебры с сопряжением}%
   {algebra of fractions of algebra with conjugation}%
\Index%623%А%алгебра, противоположная алгебре
   {алгебра, противоположная алгебре $P$}%
   {opposite algebra}%
\Index%105%А%альтернативное представление матрицы
   {альтернативное представление матрицы}%
   {Alternative representation}%
\Index%907%А%альтернация полилинейного отображения
   {альтернация полилинейного отображения}%
   {alternation of polylinear map}%
\Index%779%А%антилинейное отображение
   {антилинейное отображение}%
   {antilinear map}%
\Index%107%А%антисимметричное 2- арное расслоенное отношение
   {антисимметричное $2$\Hyph арное расслоенное отношение}%
   {antisymmetric 2 ary fibered relation}%
\Index%849%А%арность
   {арность}%
   {arity}%
\Index%108%А%арность операции
   {арность операции}%
   {arity of operation}%
\Index%617%А%ассоциативная D алгебра
   {ассоциативная $D$\Hyph алгебра}%
   {associative D algebra}%
\Index%89%А%ассоциативная Omega группа
   {ассоциативная $\Omega$\Hyph группа}%
   {associative Omega group}%
\Index%866%А%ассоциативная операция
   {ассоциативная операция}%
   {associative operation}%
\Index%616%А%ассоциатор D алгебры
   {ассоциатор $D$\Hyph алгебры}%
   {associator of algebra}%
\Index%733%А%аффинная структура на множестве
   {аффинная структура на множестве}%
   {affine structure on set}%
\Index%682%А%аффинное представление группы Ли
   {аффинное представление группы Ли}%
   {affine representation of Lie group}%
\Index%758%А%аффинное преобразование
   {аффинное преобразование}%
   {affine transformation}%
\Index%109%А%аффинное преобразование на многообразии базисов
   {аффинное преобразование на многообразии базисов}%
   {affine transformation}%
\Index%734%А%аффинное пространство
   {аффинное пространство}%
   {affine space}%
\Index%110%А%аффинный базис
   {аффинный базис}%
   {Affine Basis}%
\Index%579%А%аффинный функционал
   {аффинный функционал}%
   {affine functional}%
\SetIndexSpace%
\Index%113%Б%база отображения
   {база отображения}%
   {base of map}%
\Index%114%Б%база расслоенного соответствия
   {база расслоенного соответствия}%
   {base of fibered correspondence}%
\Index%115%Б%базис
   {базис}%
   {Basis}%
\Index%203%Б%базис crd векторного пространства
   {базис \crd векторного пространства}%
   {basis, crd vector space}%
\Index%106%Б%базис dcr векторного пространства
   {базис \dcr векторного пространства}%
   {basis, dcr vector space}%
\Index%16%Б%базис drc векторного пространства
   {базис \drc векторного пространства}%
   {basis, drc vector space}%
\Index%24%Б%базис rcd векторного пространства
   {базис \rcd векторного пространства}%
   {basis, rcd vector space}%
\Index%913%Б%базис абелевой группы
   {базис абелевой группы}%
   {basis of Abelian group}%
\Index%653%Б%базис алгебры L(A;A)
   {базис алгебры $\mathcal L(A;A)$}%
   {basis of algebra L(A,A)}%
\Index%567%Б%базис башни представлений
   {базис башни представлений}%
   {basis of tower of representations}%
\Index%26%Б%базис в векторном расслоении
   {базис в векторном расслоении}%
   {basis, vector bundle}%
\Index%197%Б%базис векторного пространства
   {базис векторного пространства}%
   {basis, vector space}%
\Index%783%Б%базис Гамеля
   {базис Гамеля}%
   {Hamel basis}%
\Index%659%Б%базис модуля
   {базис модуля}%
   {basis, module}%
\Index%329%Б%базис представления
   {базис представления}%
   {basis of representation}%
\Index%791%Б%базис Шаудера
   {базис Шаудера}%
   {Schauder basis}%
\Index%223%Б%базис, двойственный базису
   {базис, двойственный базису}%
   {dual basis}%
\Index%49%Б%базис, дуальный базису
   {базис, дуальный базису}%
   {basis dual to basis}%
\Index%116%Б%базовый вектор представления группы Ли над алгеброй A
   {базовый вектор представления группы Ли над алгеброй $A$}%
   {basis vector of representation of Lie group over algebra A}%
\Index%118%Б%базовый оператор группы Ли
   {базовый оператор группы Ли}%
   {Lie group basic operators}%
\Index%503%Б%банахова D- алгебра
   {банахова $D$\Hyph алгебра}%
   {Banach algebra}%
\Index%313%Б%банаховый D- модуль
   {банаховый $D$\Hyph модуль}%
   {Banach module}%
\Index%531%Б%башня подпредставлений
   {башня подпредставлений}%
   {tower of subrepresentations}%
\Index%532%Б%башня подпредставлений башни представлений, порождённая кортежем множеств
   {башня подпредставлений башни представлений $\Vector f$, порождённая кортежем множеств $\VX X$}%
   {subrepresentation generated by tuple of sets}%
\Index%119%Б%башня представлений Omega алгебр
   {башня представлений $\Vector{\Omega}$\Hyph алгебр}%
   {tower of representations of algebras}%
\Index%120%Б%башня расслоений
   {башня расслоений}%
   {tower of bundles}%
\Index%324%Б%башня эффективных представлений
   {башня эффективных представлений}%
   {tower of effective representations}%
\Index%121%Б%бесконечно малый генератор представления
   {бесконечно малый генератор представления}%
   {infinitesimal generator}%
\Index%122%Б%бикольцо
   {бикольцо}%
   {biring}%
\Index%798%Б%борелевское множество
   {борелевское множество}%
   {Borel set}%
\Index%803%Б%борелевское отображение
   {борелевское отображение}%
   {Borel-measurable map}%
\SetIndexSpace%
\Index%901%В%вектор
   {вектор}%
   {vector}%
\Index%123%В%вектор Киллинга второго рода
   {вектор Киллинга второго рода}%
   {Killing vector second type}%
\Index%785%В%вектор элемента алгебры
   {вектор элемента алгебры}%
   {vector of algebra}%
\Index%774%В%вектор элемента кольца
   {вектор элемента кольца}%
   {vector of ring}%
\Index%727%В%векторное пространство
   {векторное пространство}%
   {vector space}%
\Index%125%В%векторное расслоение
   {векторное расслоение}%
   {vector bundle}%
\Index%126%В%векторный потенциал
   {векторный потенциал}%
   {vector potential}%
\Index%124%В%вектор-столбец
   {вектор\hyph столбец}%
   {column vector}%
\Index%127%В%вектор-строка
   {вектор\hyph строка}%
   {row vector}%
\Index%398%В%вертикальная компонента вектора
   {вертикальная компонента вектора}%
   {vertical component of vector}%
\Index%687%В%вертикальное подпространство
   {вертикальное подпространство}%
   {vertical subspace}%
\Index%33%В%вертикальный вектор
   {вертикальный вектор}%
   {vertical vector}%
\Index%481%В%взаимно простые  A числа
   {взаимно простые  $A$\Hyph числа}%
   {relatively prime A numbers}%
\Index%908%В%внешнее произведение
   {внешнее произведение}%
   {exterior product}%
\Index%508%В%внешний дифференциал
   {внешний дифференциал}%
   {exterior differential}%
\Index%163%В%внешняя мера
   {внешняя мера}%
   {outer measure}%
\Index%128%В%вполне интегрируемая система
   {вполне интегрируемая система}%
   {completely integrable system}%
\Index%651%В%времениподобный вектор
   {времениподобный вектор}%
   {timelike vector}%
\Index%231%В%всюду плотное множество
   {всюду плотное множество}%
   {everywhere dense subset}%
\Index%70%В%вторая аксиома счётности
   {вторая аксиома счётности}%
   {second axiom of countability}%
\Index%129%В%второй закон Ньютона
   {второй закон Ньютона}%
   {Second Newton law}%
\Index%781%В%выпуклое множество
   {выпуклое множество}%
   {convex set}%
\Index%130%В%вырожденное линейное отображение
   {вырожденное линейное отображение}%
   {singular linear map}%
\SetIndexSpace%
\Index%871%Г%геодезический эффект
   {геодезический эффект}%
   {geodetic effect}%
\Index%132%Г%геометрический объект в векторном пространстве
   {геометрический объект в векторном пространстве}%
   {geometric object, vector space}%
\Index%133%Г%геометрический объект в координатном представлении
   {геометрический объект в координатном представлении}%
   {geometric object, coordinate vector space}%
\Index%698%Г%геометрический объект в координатном представлении, определённом в Omega_2- алгебре
   {геометрический объект в координатном представлении, определённом в $\Omega_2$\Hyph алгебре $M$}%
   {geometric object, coordinate representation g}%
\Index%134%Г%геометрический объект в координатном представлении, определённом в rcd векторном пространстве
   {геометрический объект в координатном представлении, определённом в \rcd векторном пространстве}%
   {geometric object, coordinate rcd vector space}%
\Index%719%Г%геометрический объект в координатном представлении, определённом в кортеже Omega- алгебр
   {геометрический объект в координатном представлении, определённом в кортеже $\VX\Omega$\Hyph алгебр $\VX A$}%
   {geometric object, coordinate tower of representations g}%
\Index%704%Г%геометрический объект типа
   {геометрический объект типа $H$}%
   {geometric object of type H, representation g}%
\Index%135%Г%геометрический объект типа A
   {геометрический объект типа $A$ в векторном пространстве}%
   {geometric object of type A, vector space}%
\Index%700%Г%геометрический объект, определённый в Omega_2- алгбре
   {геометрический объект, определённый в $\Omega_2$\Hyph алгбре $M$}%
   {geometric object, representation g}%
\Index%136%Г%геометрический объект, определённый в rcd векторном пространстве
   {геометрический объект, определённый в \rcd векторном пространстве}%
   {geometric object, rcd vector space}%
\Index%722%Г%геометрический объект, определённый в кортеже Omega- алгебр
   {геометрический объект, определённый в кортеже $\VX\Omega$\Hyph алгебр $\VX A$}%
   {geometric object, tower of representations g}%
\Index%838%Г%гиперболический косинус
   {гиперболический косинус}%
   {hyperbolic cosine}%
\Index%837%Г%гиперболический синус
   {гиперболический синус}%
   {hyperbolic sine}%
\Index%767%Г%главный идеал
   {главный идеал}%
   {principal ideal}%
\Index%885%Г%голоморфное отображение
   {голоморфное отображение}%
   {holomorphic map}%
\Index%137%Г%голономные координаты вектора
   {голономные координаты вектора}%
   {vector holonomic coordinates}%
\Index%138%Г%голономные координаты связности
   {голономные координаты связности}%
   {holonomic coordinates of connection}%
\Index%854%Г%гомоморфизм
   {гомоморфизм}%
   {homomorphism}%
\Index%140%Г%гомоморфизм расслоенных групп
   {гомоморфизм расслоенных групп}%
   {homomorphism of fibered groups}%
\Index%139%Г%гомоморфизм расслоенных универсальных алгебр
   {гомоморфизм расслоенных универсальных алгебр}%
   {homomorphism of fibered universal algebras}%
\Index%861%Г%гомоморфный образ
   {гомоморфный образ}%
   {homomorphic image}%
\Index%73%Г%горизонтальная компонента вектора
   {горизонтальная компонента вектора}%
   {horizontal component of vector}%
\Index%686%Г%горизонтальное подпространство
   {горизонтальное подпространство}%
   {horizontal subspace}%
\Index%765%Г%горизонтальный вектор
   {горизонтальный вектор}%
   {horizontal vector}%
\Index%568%Г%группа автоморфизмов представления
   {группа автоморфизмов представления}%
   {group of automorphisms of representation}%
\Index%141%Г%группа аффинных преобразований
   {группа аффинных преобразований}%
   {affine transformation group}%
\Index%142%Г%группа аффинных преобразований
   {группа аффинных преобразований}%
   {affine transformation group}%
\Index%613%Г%группа линейных преобразований
   {группа линейных преобразований}%
   {linear transformation group}%
\Index%143%Г%группа симметрии
   {группа симметрии}%
   {symmetry group}%
\Index%144%Г%группа симметрии
   {группа симметрии}%
   {SymmetryGroup}%
\Index%145%Г%группа стабилизации
   {группа стабилизации}%
   {stability group}%
\Index%146%Г%групповая алгебра
   {групповая алгебра}%
   {group algebra}%
\SetIndexSpace%
\Index%147%Д%движение на многообразии базисов
   {движение на многообразии базисов}%
   {movement transformation}%
\Index%586%Д%движение пространства Минковского
   {движение пространства Минковского}%
   {motion, Minkowski space}%
\Index%755%Д%двойной определитель
   {двойной определитель}%
   {double determinant}%
\Index%865%Д%декартова степень
   {декартова степень}%
   {Cartesian power}%
\Index%148%Д%декартова степень A множества B
   {декартова степень $A$ множества $B$}%
   {Cartesian power of set}%
\Index%149%Д%декартова степень A расслоения B
   {декартова степень $\Bundle A$ расслоения $\Bundle B$}%
   {Cartesian power A of bundle B}%
\Index%594%Д%декартова степень n H алгебры
   {декартова степень $n$ $\mathfrak{H}$\Hyph алгебры}%
   {Cartesian power of algebra}%
\Index%150%Д%декартова степень n расслоения E
   {декартова степень $n$ расслоения $\Bundle E$}%
   {Cartesian power n of bundle E}%
\Index%655%Д%декартова степень систем подмножеств
   {декартова степень систем подмножеств}%
   {Cartesian power of systems of subsets}%
\Index%390%Д%декартово произведение групп
   {декартово произведение групп}%
   {Cartesian product of groups}%
\Index%199%Д%декартово произведение мер
   {декартово произведение мер}%
   {Cartesian product of measures}%
\Index%151%Д%декартово произведение расслоений
   {декартово произведение расслоений}%
   {Cartesian product of bundles}%
\Index%152%Д%декартово произведение расслоенных пространств
   {декартово произведение расслоенных пространств}%
   {Cartesian product of total spaces}%
\Index%625%Д%декартово произведение систем подмножеств
   {декартово произведение систем подмножеств}%
   {Cartesian product of systems of subsets}%
\Index%825%Д%декартово произведением Omega алгебр
   {декартово произведением \(\Omega\)\Hyph алгебр}%
   {Cartesian product of Omega algebras}%
\Index%598%Д%деление без остатка
   {деление без остатка}%
   {division without remainder}%
\Index%573%Д%деление с остатком
   {деление с остатком}%
   {division with remainder}%
\Index%820%Д%делитель многочлена
   {делитель многочлена}%
   {divisor of polynomial}%
\Index%814%Д%делитель нуля
   {делитель нуля}%
   {zero divisor}%
\Index%153%Д%диагональ в расслоении
   {диагональ в расслоении}%
   {diagonal in bundle}%
\Index%725%Д%диаграмма представлений
   {диаграмма представлений}%
   {diagram of representations}%
\Index%154%Д%диаграмма соответствий
   {диаграмма соответствий}%
   {diagram of correspondences}%
\Index%661%Д%дифференциал независимой переменной
   {дифференциал независимой переменной}%
   {differential of independent variable}%
\Index%157%Д%дифференциал отображения
   {дифференциал отображения}%
   {differential of map}%
\Index%902%Д%дифференциальная p форма
   {дифференциальная $p$\Hyph форма}%
   {differential p form}%
\Index%737%Д%дифференциальная форма степени p
   {дифференциальная форма степени $p$}%
   {differential form of degree p}%
\Index%877%Д%дифференцируемое отображение
   {дифференцируемое отображение}%
   {differentiable map}%
\Index%78%Д%долгота
   {долгота}%
   {longitude}%
\Index%159%Д%дуальное пространство к rcd векторному пространству
   {дуальное пространство к \rcd векторному пространству}%
   {dual space of rcd vector space}%
\SetIndexSpace%
\Index%796%Е%единица кольца множеств
   {единица кольца множеств}%
   {unit of ring of sets}%
\Index%315%Е%единичная сфера в алгебре
   {единичная сфера в $D$\Hyph алгебре}%
   {unit sphere in algebra}%
\Index%160%Е%единичная сфера в теле
   {единичная сфера в теле}%
   {unit sphere in division ring}%
\Index%523%Е%единичный вектор
   {единичный вектор}%
   {unit vector}%
\Index%44%Е%единичный интервал
   {единичный интервал}%
   {unit interval}%
\Index%875%Е%естественный гомоморфизм
   {естественный гомоморфизм}%
   {natural homomorphism}%
\SetIndexSpace%
\Index%662%З%закон ассоциативности
   {закон ассоциативности}%
   {associative law}%
\Index%672%З%закон дистрибутивности
   {закон дистрибутивности}%
   {distributive law}%
\Index%673%З%закон унитарности
   {закон унитарности}%
   {unitarity law}%
\Index%807%З%замкнутый шар
   {замкнутый шар}%
   {closed ball}%
\Index%80%З%замыкание множества
   {замыкание множества}%
   {closure of set}%
\Index%261%З%звёздное множество
   {звёздное множество}%
   {starlike set}%
\SetIndexSpace%
\Index%459%И%идеал алгебры
   {идеал алгебры}%
   {ideal of algebra}%
\Index%800%И%измеримое отображение
   {измеримое отображение}%
   {measurable map}%
\Index%164%И%измеримое по Лебегу множество
   {измеримое по Лебегу множество}%
   {Lebesgue measurable}%
\Index%855%И%изоморфизм
   {изоморфизм}%
   {isomorphism}%
\Index%31%И%изоморфизм векторных пространств
   {изоморфизм векторных пространств}%
   {isomorphism of vector spaces}%
\Index%266%И%изоморфизм представлений Omega- алгебры
   {изоморфизм представлений $\Omega$\Hyph алгебры}%
   {isomorphism of repesentations of Omega algebra}%
\Index%173%И%изоморфизм расслоенных Omega- алгебр
   {изоморфизм расслоенных $\Omega$\Hyph алгебр}%
   {isomorphism of fibered Omega-algebras}%
\Index%648%И%изотропный вектор
   {изотропный вектор}%
   {isotropic vector}%
\Index%745%И%инволюция в кватернионной алгебре
   {инволюция в кватернионной алгебре}%
   {involution, quaternion algebra}%
\Index%257%И%интеграл дифференциальной 1 формы вдоль пути
   {интеграл дифференциальной $1$\Hyph формы вдоль пути}%
   {integral of differential 1 form along path}%
\Index%680%И%интеграл Лебега
   {интеграл Лебега}%
   {Lebesgue integral}%
\Index%111%И%интегрируемая форма
   {интегрируемая форма}%
   {integrable form}%
\Index%693%И%интегрируемое отображение
   {интегрируемое отображение}%
   {integrable map}%
\Index%174%И%инфинитезимальные образующие группы Ли
   {инфинитезимальные образующие группы Ли}%
   {infinitesimal generators of group Lie}%
\SetIndexSpace%
\Index%599%К%каноническое представление деления с остатком
   {каноническое представление деления с остатком}%
   {canonical representation of division with remainder}%
\Index%726%К%каноническое частное от деления
   {каноническое частное от деления}%
   {canonical remainder of the division}%
\Index%175%К%категория drc векторных пространств
   {категория \drc векторных пространств}%
   {category of drc vector spaces}%
\Index%177%К%категория левосторонних представлений
   {категория левосторонних представлений}%
   {category of left-side representations}%
\Index%176%К%категория левосторонних представлений Omega1 алгебры A
   {категория левосторонних представлений $\Omega$\Hyph алгебры $A$}%
   {category of left-side representations of Omega1 algebra}%
\Index%887%К%категория представлений
   {категория представлений}%
   {category of representations}%
\Index%178%К%категория приведенных расслоенных соответствий
   {категория приведенных расслоенных соответствий}%
   {category of reduced fibered correspondences}%
\Index%179%К%категория расслоенных соответствий над диагональю
   {категория расслоенных соответствий над диагональю}%
   {category of fibered correspondences over diagonal}%
\Index%555%К%квадратичная форма на теле
   {квадратичная форма на теле}%
   {quadratic form, division ring}%
\Index%551%К%квадратичное отображение тела
   {квадратичное отображение тела}%
   {Quadratic Map of Division Ring}%
\Index%842%К%квадратное уравнение
   {квадратное уравнение}%
   {quadratic equation}%
\Index%841%К%квадратный корень
   {квадратный корень}%
   {square root}%
\Index%180%К%квазиаффинное преобразование на многообразии базисов
   {квазиаффинное преобразование на многообразии базисов}%
   {quasi affine transformation}%
\Index%181%К%квазиаффинное преобразование на многообразии базисов
   {квазиаффинное преобразование на многообразии базисов}%
   {quasi affine drc transformation}%
\Index%182%К%квазидвижение на многообразии базисов
   {квазидвижение на многообразии базисов}%
   {quasi movement, division ring}%
\Index%183%К%квазидвижение на многообразии базисов
   {квазидвижение на многообразии базисов}%
   {quasi movement}%
\Index%75%К%квазидвижение пространства Минковского
   {квазидвижение пространства Минковского}%
   {Quasimotion, Minkowski space}%
\Index%679%К%квазидетерминант
   {квазидетерминант}%
   {quasideterminant definition}%
\Index%604%К%квазизамкнутое кольцо отображений
   {квазизамкнутое кольцо отображений}%
   {quasiclosed ring of maps}%
\Index%746%К%кватернион, сопряженный к кватерниону
   {кватернион, сопряженный к кватерниону $x$}%
   {conjugate of quaternion}%
\Index%188%К%кольцо имеет характеристику 0
   {кольцо имеет характеристику $0$}%
   {ring has characteristic 0}%
\Index%189%К%кольцо имеет характеристику p
   {кольцо имеет характеристику $p$}%
   {ring has characteristic p}%
\Index%794%К%кольцо множеств
   {кольцо множеств}%
   {ring of sets}%
\Index%577%К%кольцо множеств, порождённое полукольцом множеств
   {кольцо множеств, порождённое полукольцом множеств}%
   {ring of sets generated by semiring}%
\Index%778%К%кольцо с сопряжением
   {кольцо с сопряжением}%
   {ring with conjugation}%
\Index%615%К%коммутативная D алгебра
   {коммутативная $D$\Hyph алгебра}%
   {commutative D algebra}%
\Index%190%К%коммутативная диаграмма соответствий
   {коммутативная диаграмма соответствий}%
   {commutative diagram of correspondences}%
\Index%867%К%коммутативная операция
   {коммутативная операция}%
   {commutative operation}%
\Index%832%К%коммутативность представлений
   {коммутативность представлений}%
   {commutativity of representations}%
\Index%614%К%коммутатор D алгебры
   {коммутатор $D$\Hyph алгебры}%
   {commutator of algebra}%
\Index%815%К%компактное множество
   {компактное множество}%
   {compact set}%
\Index%191%К%компактно-открытая топология
   {компактно\hyph открытая топология}%
   {compact open topology}%
\Index%193%К%компонента линейного отображения
   {компонента линейного отображения}%
   {component of linear map}%
\Index%647%К%компонента полилинейного отображения
   {компонента полилинейного отображения}%
   {component of polylinear map}%
\Index%879%К%компонента производной
   {компонента производной}%
   {component of derivative}%
\Index%883%К%компонента производной второго порядка
   {компонента производной второго порядка}%
   {component of derivative of Second Order}%
\Index%629%К%компонента производной Гато
   {компонента производной Гато}%
   {component of Gateaux derivative}%
\Index%633%К%компонента производной Гато второго порядка
   {компонента производной Гато второго порядка}%
   {component of Gateaux derivative of Second Order}%
\Index%873%К%конгруенция
   {конгруенция}%
   {congruence}%
\Index%170%К%конечное разложение множества
   {конечное разложение множества}%
   {finite expansion of set}%
\Index%691%К%координатная матрица вектора
   {координатная матрица вектора}%
   {coordinate matrix of vector}%
\Index%205%К%координатная матрица векторного поля в Drc базисе
   {координатная матрица векторного поля в \Drc базисе}%
   {coordinate matrix of vector field in drc basis}%
\Index%206%К%координатная матрица множества векторов
   {координатная матрица множества векторов}%
   {coordinate matrix of set of vectors}%
\Index%208%К%координатная система отсчёта
   {координатная система отсчёта}%
   {coordinate reference frame}%
\Index%209%К%координатное rcd векторное пространство
   {координатное \rcd векторное пространство}%
   {coordinate rcd vector space}%
\Index%211%К%координатное векторное пространство
   {координатное векторное пространство}%
   {coordinate vector space}%
\Index%210%К%координатное векторное расслоение
   {координатное векторное расслоение}%
   {coordinate vector bundle}%
\Index%697%К%координатное представление в Omega_2- алгебре
   {координатное представление в $\Omega_2$\Hyph алгебре}%
   {coordinate representation, Omega_2 algebra}%
\Index%212%К%координатное представление в rcd векторном пространстве
   {координатное представление в \rcd векторном пространстве}%
   {coordinate representation, rcd vector space}%
\Index%720%К%координатное представление в кортеже Omega- алгебр
   {координатное представление в кортеже $\VX\Omega$\Hyph алгебр}%
   {coordinate tower of representations, Omega algebra}%
\Index%664%К%координатное представление вектора
   {координатное представление вектора}%
   {coordinate representation of vector}%
\Index%213%К%координатное представление группы в векторном пространстве
   {координатное представление группы в векторном пространстве}%
   {coordinate representation, vector space}%
\Index%215%К%координатный изоморфизм
   {координатный изоморфизм}%
   {coordinate isomorphism}%
\Index%738%К%координаты
   {координаты}%
   {coordinates}%
\Index%25%К%координаты базиса
   {координаты базиса}%
   {coordinates of basis}%
\Index%325%К%координаты базиса представления
   {координаты базиса представления}%
   {coordinates of basis relative to basis, representation}%
\Index%216%К%координаты вектора
   {координаты вектора}%
   {coordinates of vector}%
\Index%286%К%координаты вектора относительно базиса Гамеля
   {координаты вектора относительно базиса Гамеля}%
   {coordinates of vector, Hamel basis}%
\Index%676%К%координаты вектора относительно базиса Шаудера
   {координаты вектора относительно базиса Шаудера}%
   {coordinates of vector, Schauder basis}%
\Index%217%К%координаты векторного поля в Drc базисе
   {координаты векторного поля в \Drc базисе}%
   {coordinates of vector field in drc basis}%
\Index%218%К%координаты геометрического объекта
   {координаты геометрического объекта}%
   {coordinates of geometric object, vector space}%
\Index%701%К%координаты геометрического объекта в Omega_2- алгбре
   {координаты геометрического объекта в $\Omega_2$\Hyph алгбре $M$}%
   {coordinates of geometric object, representation g}%
\Index%219%К%координаты геометрического объекта в rcd векторном пространстве
   {координаты геометрического объекта в \rcd векторном пространстве}%
   {coordinates of geometric object, rcd vector space}%
\Index%220%К%координаты геометрического объекта в координатном rcd векторном пространстве
   {координаты геометрического объекта в координатном \rcd векторном пространстве}%
   {coordinates of geometric object, coordinate rcd vector space}%
\Index%221%К%координаты геометрического объекта в координатном представлении
   {координаты геометрического объекта в координатном представлении}%
   {coordinates of geometric object, coordinate vector space}%
\Index%721%К%координаты геометрического объекта в координатном пространстве башни представлений
   {координаты геометрического объекта в координатном пространстве башни представлений}%
   {coordinates of geometric object, coordinate tower of representations}%
\Index%699%К%координаты геометрического объекта в координатном пространстве представления
   {координаты геометрического объекта в координатном пространстве представления}%
   {coordinates of geometric object, coordinate representation}%
\Index%723%К%координаты геометрического объекта в кортеже Omega- алгебр
   {координаты геометрического объекта в кортеже $\VX\Omega$\Hyph алгебр}%
   {coordinates of geometric object, tower of representations g}%
\Index%222%К%координаты множества векторов
   {координаты множества векторов}%
   {coordinates of set of vectors}%
\Index%224%К%координаты представления
   {координаты представления}%
   {coordinates of representation, drc vector space}%
\Index%225%К%координаты представления
   {координаты представления}%
   {coordinates of representation}%
\Index%730%К%координаты точки аффинного пространства относительно базиса
   {координаты точки $A$ аффинного пространства $\overset{\circ}{A}$ относительно базиса $(O,\Basis e)$}%
   {coordinates in affine space}%
\Index%558%К%координаты элемента представления относительно множества
   {координаты элемента $m$ представления $f$ относительно множества $X$}%
   {coordinates of element relative to set, representation}%
\Index%711%К%координаты эндоморфизма башни представлений
   {координаты эндоморфизма башни представлений}%
   {coordinates of endomorphism, tower of representations}%
\Index%696%К%координаты эндоморфизма представления
   {координаты эндоморфизма представления}%
   {coordinates of endomorphism, representation}%
\Index%910%К%копроизведение в категории
   {копроизведение в категории}%
   {coproduct in category}%
\Index%634%К%корень полинома
   {корень полинома}%
   {root of polynomial}%
\Index%708%К%кортеж Omega слов элементов башни представления относительно кортежа множеств образующих
   {кортеж $\Vector{\Omega}$\Hyph слов элемента башни представления относительно кортежа множеств образующих}%
   {tuple of words relative to tuple of generating sets, tower of representations}%
\Index%535%К%кортеж координат элемента относительно кортежа множеств
   {кортеж координат элемента $\Vector a$ относительно кортежа множеств $\VX X$}%
   {coordinates of element, tower of representations}%
\Index%533%К%кортеж множеств образующих башни подпредставлений
   {кортеж множеств образующих башни подпредставлений}%
   {tuple of generating sets of tower subrepresentations}%
\Index%534%К%кортеж множеств образующих башни представлений
   {кортеж множеств образующих башни представлений}%
   {tuple of generating sets of tower of representations}%
\Index%713%К%кортеж отношений эквивалентности, порождённых башней представлений
   {кортеж отношений эквивалентности, порождённых башней представлений $\Vector f$}%
   {tuple of equivalence of tower of representations}%
\Index%530%К%кортеж стабильных множеств башни представлений
   {кортеж стабильных множеств башни представлений}%
   {tuple of stable sets of tower of representations}%
\Index%840%К%косинус
   {косинус}%
   {cosine}%
\Index%904%К%косо симметричное полилинейное отображение
   {косо симметричное полилинейное отображение}%
   {skew symmetric polylinear map}%
\Index%226%К%косое произведение векторов
   {косое произведение векторов}%
   {skew product of vectors}%
\Index%821%К%коэффициент многочлена
   {коэффициент многочлена}%
   {coefficient of polynomial}%
\Index%550%К%коэффициенты D- аффинной связности на многообразии
   {коэффициенты $D$\Hyph аффинной связности на многообразии}%
   {D affine connection coefficients, manifold}%
\Index%538%К%коэффициенты связности в D аффинном пространстве
   {коэффициенты связности в аффинном пространстве}%
   {connection coefficients, affine space}%
\Index%227%К%кривизна Картана
   {кривизна Картана}%
   {Cartan curvature}%
\Index%537%К%криволинейные координаты точки аффинного пространства
   {криволинейные координаты точки аффинного пространства}%
   {curvilinear coordinates of point in affine space}%
\SetIndexSpace%
\Index%166%Л%лебегово продолжение меры
   {лебегово продолжение меры}%
   {Lebesgue extension of measure}%
\Index%158%Л%левая дробь
   {левая дробь}%
   {left fraction}%
\Index%896%Л%левое A векторное пространство
   {левое $A$\Hyph векторное пространство}%
   {left A vector space}%
\Index%585%Л%левое D векторное пространство столбцов
   {левое $D$\hyph векторное пространство столбцов}%
   {left vector space of columns}%
\Index%576%Л%левое D векторное пространство строк
   {левое $D$\hyph векторное пространство строк}%
   {left vector space of rows}%
\Index%754%Л%левое алгебраическое дополнение элемента матрицы
   {левое алгебраическое дополнение элемента матрицы}%
   {left cofactor, matrix}%
\Index%228%Л%левое векторное пространство
   {левое векторное пространство}%
   {left vector space}%
\Index%756%Л%левое двойное алгебраическое дополнение элемента матрицы
   {левое двойное алгебраическое дополнение элемента матрицы}%
   {left double cofactor}%
\Index%229%Л%левоинвариантное векторное поле
   {левоинвариантное векторное поле}%
   {left invariant vector}%
\Index%899%Л%левостороннее A представление
   {левостороннее $A_1$\Hyph представление}%
   {left-side A representation}%
\Index%184%Л%левостороннее представление
   {левостороннее представление}%
   {left-side representation}%
\Index%232%Л%левостороннее представление Omega1 алгебры A в Omega2 алгебре M
   {левостороннее представление $\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре $M$}%
   {left-side representation of algebra}%
\Index%233%Л%левостороннее представление расслоенной Omega- алгебры
   {левостороннее представление расслоенной $\Omega$\Hyph алгебры}%
   {left-side representation of fibered Omega-algebra}%
\Index%234%Л%левостороннее преобразование
   {левостороннее преобразование}%
   {left-side transformation}%
\Index%235%Л%левостороннее преобразование расслоения
   {левостороннее преобразование расслоения}%
   {left-side transformation of bundle}%
\Index%892%Л%левостороннее произведение
   {левостороннее произведение}%
   {left-side product}%
\Index%665%Л%левостороннее произведение вектора на скаляр
   {левостороннее произведение вектора на скаляр}%
   {left-side product of vector over scalar}%
\Index%271%Л%левостороннее произведение отображения на скаляр
   {левостороннее произведение отображения на скаляр}%
   {left-side product of map over scalar}%
\Index%236%Л%левые структурные константы алгебры Ли
   {левые структурные константы алгебры Ли}%
   {left structural constant of Lie algebra}%
\Index%895%Л%левый A модуль
   {левый $A$\Hyph модуль}%
   {left A module}%
\Index%513%Л%левый главный идеал
   {левый главный идеал}%
   {left principal ideal}%
\Index%812%Л%левый делитель нуля
   {левый делитель нуля}%
   {left zero divisor}%
\Index%681%Л%левый идеал алгебры
   {левый идеал алгебры}%
   {left ideal of algebra}%
\Index%237%Л%левый модуль
   {левый модуль}%
   {left module}%
\Index%731%Л%левый сдвиг модуля
   {левый сдвиг модуля}%
   {left shift of module}%
\Index%238%Л%левый сдвиг на группе
   {левый сдвиг на группе}%
   {left shift}%
\Index%239%Л%левый сдвиг на группе
   {левый сдвиг на группе}%
   {left shift, group}%
\Index%240%Л%левый сдвиг на расслоении групп
   {левый сдвиг на расслоении групп}%
   {left shift, fibered group}%
\Index%88%Л%линейная комбинация
   {линейная комбинация}%
   {linear combination}%
\Index%32%Л%линейная оболочка в векторном пространстве
   {линейная оболочка в векторном пространстве}%
   {linear span, vector space}%
\Index%98%Л%линейнное отображение, порождённое отображением
   {линейное отображение, порождённое отображением}%
   {linear map generated by map}%
\Index%21%Л%линейно зависимое множество
   {линейно зависимое множество}%
   {linearly dependent set}%
\Index%20%Л%линейно зависимые векторные поля
   {линейно зависимые векторные поля}%
   {linearly dependent vector fields}%
\Index%833%Л%линейно зависимый
   {линейно зависимый}%
   {linearly dependent}%
\Index%34%Л%линейно независимое множество
   {линейно независимое множество}%
   {linearly independent set}%
\Index%37%Л%линейное G* представление
   {линейное \Ts{G}представление}%
   {linear G* representation}%
\Index%35%Л%линейное отображение
   {линейное отображение}%
   {linear map}%
\Index%97%Л%линейное отображение тела
   {линейное отображение тела}%
   {linear map of division ring}%
\Index%244%Л%линейное представление группы
   {линейное представление группы}%
   {linear representation of group}%
\Index%608%Л%линейное представление группы Ли
   {линейное представление группы Ли}%
   {linear representation of Lie group}%
\Index%735%Л%линейное преобразование аффинного пространства
   {линейное преобразование аффинного пространства}%
   {linear transformation, affine space}%
\Index%630%Л%линейный геометрический объект
   {линейный геометрический объект}%
   {linear geometric object}%
\Index%769%Л%линейный гомоморфизм
   {линейный гомоморфизм}%
   {linear homomorphism}%
\Index%397%Л%линейный функционал
   {линейный функционал}%
   {linear functional}%
\Index%245%Л%лифт отображения
   {лифт отображения}%
   {lift of map}%
\Index%246%Л%лифт соответствия
   {лифт соответствия}%
   {lift of correspondence}%
\Index%247%Л%локальная система отсчёта
   {локальная система отсчёта}%
   {local reference frame}%
\Index%248%Л%локально компактное в точке p пространство
   {локально компактное в точке $p$ пространство}%
   {locally compact at point space}%
\Index%249%Л%локально компактное пространство
   {локально компактное пространство}%
   {locally compact space}%
\SetIndexSpace%
\Index%250%М%малая группа
   {малая группа}%
   {little group}%
\Index%894%М%матрица
   {матрица}%
   {matrix}%
\Index%772%М%матрица антилинейного гомоморфизма
   {матрица антилинейного гомоморфизма}%
   {matrix of antilinear homomorphism}%
\Index%252%М%матрица билинейной функции
   {матрица билинейной функции}%
   {matrix of bilinear function}%
\Index%552%М%матрица квадратичного отображения
   {матрица квадратичного отображения}%
   {matrix of quadratic map, division ring}%
\Index%770%М%матрица линейного гомоморфизма
   {матрица линейного гомоморфизма}%
   {matrix of linear homomorphism}%
\Index%194%М%матрица линейного отображения
   {матрица линейного отображения}%
   {matrix of linear map}%
\Index%591%М%матрица линейных отображений
   {матрица линейных отображений}%
   {matrix of linear maps}%
\Index%588%М%матрица отображений
   {матрица отображений}%
   {matrix of maps}%
\Index%253%М%матрица расслоенного Drc линейного отображения
   {матрица расслоенного \Drc линейного отображения}%
   {matrix of fibered drc linear map}%
\Index%595%М%матрица эндоморфизмов Omega алгебры
   {матрица эндоморфизмов $\Omega$\Hyph алгебры}%
   {matrix of endomorphisms of Omega algebra}%
\Index%527%М%матрица Якоби Гато отображения
   {матрица Якоби\Hyph Гато отображения}%
   {Jacobi Gateaux matrix of map}%
\Index%890%М%матрица Якоби отображения
   {матрица Якоби отображения}%
   {Jacobi matrix of map}%
\Index%161%М%мера
   {мера}%
   {measure}%
\Index%165%М%мера Лебега
   {мера Лебега}%
   {Lebesgue measure}%
\Index%835%М%метод последовательного дифференцирования
   {метод последовательного дифференцирования}%
   {method of successive differentiation}%
\Index%254%М%метрико-аффинное многообразие
   {метрико-аффинное многообразие}%
   {metric-affine manifold}%
\Index%96%М%метрический тензор в пространстве Минковского
   {метрический тензор в пространстве Минковского}%
   {metric tensor, Minkowski space}%
\Index%642%М%минорная матрица
   {минорная матрица}%
   {minor matrix}%
\Index%556%М%многообразие D- аффинной связности
   {многообразие $D$\Hyph аффинной связности}%
   {manifold with D- affine connections}%
\Index%255%М%многообразие базисов rcd векторного пространства
   {многообразие базисов \rcd векторного пространства}%
   {basis manifold of rcd vector space}%
\Index%256%М%многообразие базисов аффинного пространства
   {многообразие базисов аффинного пространства}%
   {Basis Manifold, Affine Space}%
\Index%714%М%многообразие базисов башни представлений
   {многообразие базисов башни представлений}%
   {basis manifold tower of representations}%
\Index%258%М%многообразие базисов векторного пространства
   {многообразие базисов векторного пространства}%
   {basis manifold of vector space}%
\Index%259%М%многообразие базисов евклидова пространства
   {многообразие базисов евклидова пространства}%
   {Basis Manifold, Euclid Space}%
\Index%260%М%многообразие базисов евклидова пространства
   {многообразие базисов евклидова пространства}%
   {Basis Manifold, Euclid Space, division ring}%
\Index%536%М%многообразие базисов представления
   {многообразие базисов представления}%
   {basis manifold representation F algebra}%
\Index%262%М%многообразие базисов центро-аффинного пространства
   {многообразие базисов центро-аффинного пространства}%
   {Basis Manifold, Central Affine Space}%
\Index%263%М%многообразие систем отсчёта
   {многообразие систем отсчёта}%
   {reference frame manifold}%
\Index%804%М%многочлен
   {многочлен}%
   {polynomial}%
\Index%571%М%множество Omega_2- слов представления
   {множество $\Omega_2$\Hyph слов представления}%
   {word set of representation}%
\Index%847%М%множество допускает операцию
   {множество допускает операцию}%
   {set admits operation}%
\Index%846%М%множество замкнуто относительно операции
   {множество замкнуто относительно операции}%
   {set is closed with respect to operation}%
\Index%562%М%множество координат представления
   {множество координат представления}%
   {coordinate set of representation}%
\Index%709%М%множество кортежей Omega- слов башни представлений
   {множество кортежей $\Vector\Omega$\Hyph слов башни представлений}%
   {word set of tower of representations}%
\Index%563%М%множество кортежей координат башни представлений
   {множество кортежей координат башни представлений}%
   {coordinate set of tower of representations}%
\Index%626%М%множество нулей алгебры
   {множество нулей алгебры}%
   {set of zeros of algebra}%
\Index%332%М%множество образующих
   {множество образующих}%
   {generating set}%
\Index%628%М%множество обратимых элементов алгебры
   {множество обратимых элементов алгебры}%
   {set of invertible elements of algebra}%
\Index%356%М%множество, плотное в множестве
   {множество, плотное в множестве}%
   {dense in set}%
\Index%787%М%модуль векторов алгебры
   {модуль векторов алгебры}%
   {vector module of algebra}%
\Index%776%М%модуль векторов кольца
   {модуль векторов кольца}%
   {vector module of ring}%
\Index%611%М%модуль над кольцом
   {модуль над кольцом}%
   {module over ring}%
\Index%860%М%может быть вложена
   {может быть вложена}%
   {can be embeded}%
\Index%856%М%мономорфизм
   {мономорфизм}%
   {monomorphism}%
\Index%264%М%морфизм Tstar- представлений расслоенной Omega- алгебры
   {морфизм \Ts представлений расслоенной $\Omega$\Hyph алгебры}%
   {morphism of representations of fibered Omega algebra}%
\Index%265%М%морфизм из башни представлений в башню представлений
   {морфизм из башни представлений в башню представлений}%
   {morphism from tower of representations into tower of representations}%
\Index%267%М%морфизм представлений Omega1 алгебры в Omega2 алгебре
   {морфизм представлений $\Omega_1$\Hyph алгебры в $\Omega_2$\Hyph алгебре}%
   {morphism of representations of Omega1 algebra in Omega2 algebra}%
\Index%268%М%морфизм представлений из f в g
   {морфизм представлений из $f$ в $g$}%
   {morphism of representations from f into g}%
\Index%732%М%морфизм представления f
   {морфизм представления $f$}%
   {morphism of representation f}%
\Index%269%М%морфизм расслоенных Tstar- представлений из F в G
   {морфизм расслоенных \Ts представлений из $\Bundle F$ в $\Bundle G$}%
   {morphism of fibered representations from f into g}%
\Index%828%М%мультипликативная Omega группа
   {мультипликативная $\Omega$\Hyph группа}%
   {multiplicative Omega group}%
\Index%829%М%мультипликативное отображение
   {мультипликативное отображение}%
   {multiplicative map}%
\Index%85%М%открытое множество
   {открытое множество}%
   {open set}%
\SetIndexSpace%
\Index%207%Н%наибольший общий делитель
   {наибольший общий делитель}%
   {highest common factor}%
\Index%763%Н%направление над коммутативным кольцом
   {направление над коммутативным кольцом}%
   {direction over commutative ring}%
\Index%729%Н%начало системы координат аффинного пространства
   {начало системы координат аффинного пространства}%
   {origin of coordinate system of affine space}%
\Index%649%Н%не полная Omega алгебра
   {не полная $\Omega$\Hyph алгебра}%
   {not complete Omega algebra}%
\Index%632%Н%не полная группа
   {не полная группа}%
   {not complete group}%
\Index%272%Н%невырожденная билинейная функция
   {невырожденная билинейная функция}%
   {nonsingular bilinear function}%
\Index%273%Н%невырожденная система drc линейных уравнений
   {невырожденная система \rcd линейных уравнений}%
   {nonsingular system of linear equations}%
\Index%553%Н%невырожденное квадратичное отображение тела
   {невырожденное квадратичное отображение тела}%
   {regular quadratic map, division ring}%
\Index%274%Н%невырожденное преобразование
   {невырожденное преобразование}%
   {nonsingular transformation}%
\Index%643%Н%невырожденный тензор
   {невырожденный тензор}%
   {nonsingular tensor}%
\Index%330%Н%невырожденный эндоморфизм представления
   {невырожденный эндоморфизм представления}%
   {regular endomorphism of representation}%
\Index%275%Н%неголономная координата
   {неголономная координата}%
   {anholonomic coordinate}%
\Index%276%Н%неголономные координаты вектора
   {неголономные координаты вектора}%
   {vector anholonomic coordinates}%
\Index%277%Н%неголономные координаты на многообразии
   {неголономные координаты на многообразии}%
   {anholonomic coordinates on manifold}%
\Index%278%Н%неголономные координаты связности
   {неголономные координаты связности}%
   {anholonomic coordinates of connection}%
\Index%29%Н%независимые точки
   {независимые точки}%
   {independent points}%
\Index%870%Н%нейтральный элемент операции
   {нейтральный элемент операции}%
   {neutral element of operation}%
\Index%279%Н%неметричность
   {неметричность}%
   {nonmetricity}%
\Index%834%Н%неопределённый интеграл
   {неопределённый интеграл}%
   {indefinite integral}%
\Index%280%Н%непрерывное отображение
   {непрерывное отображение}%
   {continuous map}%
\Index%610%Н%непрерывное отображение нескольких переменных
   {непрерывное отображение нескольких переменных}%
   {continuous multivariable map}%
\Index%281%Н%непрерывное соответствие
   {непрерывное соответствие}%
   {continuous correspondence}%
\Index%668%Н%непрерывный базис
   {непрерывный базис}%
   {continues basis}%
\Index%346%Н%норма в D- алгебре
   {норма в $D$\Hyph алгебре}%
   {norm on D algebra}%
\Index%460%Н%норма в D-модуле
   {норма в $D$\Hyph модуле}%
   {norm on D module}%
\Index%742%Н%норма в кватернионной алгебре
   {норма в кватернионной алгебре}%
   {norm, quaternion algebra}%
\Index%282%Н%норма кватерниона
   {норма кватерниона}%
   {norm of quaternion}%
\Index%283%Н%норма на D- векторном пространстве
   {норма на $D$\Hyph векторном пространстве}%
   {norm on D vector space}%
\Index%675%Н%норма на Omega группе
   {норма на $\Omega$\Hyph группе}%
   {norm on Omega group}%
\Index%641%Н%норма на кольце
   {норма на кольце}%
   {norm on ring}%
\Index%657%Н%норма операции
   {норма операции}%
   {norm of operation}%
\Index%314%Н%норма отображения
   {норма отображения}%
   {norm of map}%
\Index%285%Н%норма полилинейного отображения
   {норма полилинейного отображения}%
   {norm of polymap}%
\Index%801%Н%норма представления
   {норма представления}%
   {norm of representation}%
\Index%196%Н%норма функционала
   {норма функционала}%
   {norm of functional}%
\Index%343%Н%нормированная D-алгебра
   {нормированная $D$\Hyph алгебра}%
   {normed D algebra}%
\Index%792%Н%нормированная Omega группа
   {нормированная $\Omega$\Hyph группа}%
   {normed Omega group}%
\Index%287%Н%нормированное D-векторное пространство
   {нормированное $D$\Hyph векторное пространство}%
   {normed D vector space}%
\Index%640%Н%нормированное кольцо
   {нормированное кольцо}%
   {normed ring}%
\Index%288%Н%нормированное тело
   {нормированное тело}%
   {valued division ring}%
\Index%364%Н%нормированный D-модуль
   {нормированный $D$\Hyph модуль}%
   {normed D module}%
\Index%692%Н%нормированный базис
   {нормированный базис}%
   {normal basis}%
\Index%852%Н%носитель Omega-алгебры
   {носитель $\Omega$\Hyph алгебры}%
   {carrier of Omega-algebra}%
\SetIndexSpace%
\Index%848%О%область операторов
   {область операторов}%
   {operator domain}%
\Index%289%О%образующая линейного отображения
   {образующая линейного отображения}%
   {generator of linear map}%
\Index%290%О%обратное приведенное расслоенное соответствие
   {обратное приведенное расслоенное соответствие}%
   {inverse reduced fibered correspondence}%
\Index%291%О%обратное расслоенное соответствие
   {обратное расслоенное соответствие}%
   {inverse fibered correspondence}%
\Index%292%О%обращение Адамара матрицы
   {обращение Адамара матрицы}%
   {Hadamard inverse of matrix}%
\Index%482%О%общий делитель
   {общий делитель}%
   {common factor}%
\Index%293%О%объект неголономности
   {объект неголономности}%
   {anholonomity object}%
\Index%294%О%однородное отображение степени k над полем F
   {однородное отображение степени $k$ над полем $F$}%
   {homogeneous map of degree over field, D vector space}%
\Index%295%О%однородное пространство
   {однородное пространство}%
   {homogeneous space}%
\Index%296%О%однородное расслоение расслоенной группы
   {однородное расслоение расслоенной группы}%
   {homogeneous bundle of fibered group}%
\Index%631%О%однородный линейный геометрический объект
   {однородный линейный геометрический объект}%
   {homogeneous linear geometric object}%
\Index%689%О%однородный многочлен степени
   {однородный многочлен степени $n$}%
   {homogeneous polynomial of power}%
\Index%297%О%однотранзитивное представление Omega- алгебры A
   {однотранзитивное представление $\Omega$\Hyph алгебры $A$}%
   {single transitive representation of algebra}%
\Index%298%О%однотранзитивное представление группы
   {однотранзитивное представление группы}%
   {single transitive representation of group}%
\Index%299%О%однотранзитивное представление расслоенной Omega- алгебры
   {однотранзитивное представление расслоенной $\Omega$\Hyph алгебры}%
   {single transitive representation of fibered Omega-algebra}%
\Index%766%О%одночлен степени
   {одночлен степени $k$}%
   {monomial of power}%
\Index%844%О%операция на множестве
   {операция на множестве}%
   {operation on set}%
\Index%300%О%операция на расслоении
   {операция на расслоении}%
   {operation on bundle}%
\Index%301%О%определённая слева алгебра Ли группы Ли
   {определённая слева алгебра Ли группы Ли}%
   {left defined Lie algebra}%
\Index%302%О%определённая справа алгебра Ли группы Ли
   {определённая справа алгебра Ли группы Ли}%
   {right defined Lie algebra}%
\Index%740%О%определённый интеграл
   {определённый интеграл}%
   {definite integral}%
\Index%303%О%определитель матрицы
   {определитель матрицы}%
   {determinant}%
\Index%624%О%орбита линейного отображения
   {орбита линейного отображения}%
   {orbit of linear map}%
\Index%893%О%орбита представления
   {орбита представления}%
   {orbit of representation}%
\Index%305%О%орбита представления группы
   {орбита представления группы}%
   {orbit of representation of group}%
\Index%306%О%орбита представления расслоенной группы
   {орбита представления расслоенной группы}%
   {orbit of representation of fibered group}%
\Index%636%О%ортогональность в пространстве Минковского
   {ортогональность в пространстве Минковского}%
   {Minkowski orthogonality}%
\Index%637%О%ортогональный базис в пространстве Минковского
   {ортогональный базис в пространстве Минковского}%
   {orthogonal basis, Minkowski space}%
\Index%307%О%ортонормированный базис
   {ортонормированный базис}%
   {Orthonornal Basis}%
\Index%308%О%ортонормированный базис
   {ортонормированный базис}%
   {Orthonormal Basis, division ring}%
\Index%638%О%ортонормированный базис в пространстве Минковского
   {ортонормированный базис в пространстве Минковского}%
   {orthonormal basis, Minkowski space}%
\Index%484%О%остаток от деления
   {остаток от деления}%
   {remainder of the division}%
\Index%309%О%отклонение траекторий
   {отклонение траекторий}%
   {deviation of trajectories}%
\Index%793%О%открытый шар
   {открытый шар}%
   {open ball}%
\Index%706%О%отношение эквивалентности порождённое представлением
   {отношение эквивалентности, порождённое представлением $f$}%
   {equivalence of representation}%
\Index%502%О%отображение n D- значных переменных
   {отображение $\gi n$ $D$\Hyph значных переменных}%
   {map of n D valued variables}%
\Index%312%О%отображение колец полилинейное над коммутативным кольцом
   {отображение колец полилинейное над коммутативным кольцом}%
   {map polylinear over commutative ring, ring}%
\Index%886%О%отображение согласовано с операцией
   {отображение согласовано с операцией}%
   {map is compatible with operation}%
\Index%876%О%отображение сопряжения
   {отображение сопряжения}%
   {map of conjugation}%
\Index%316%О%отображение типа G на многообразии
   {отображение типа $G$ на многообразии}%
   {map of type G on manifold}%
\Index%505%О%отображение, дифференцируемое по Гато
   {отображение, дифференцируемое по Гато}%
   {map differentiable in Gateaux sense}%
\Index%506%О%отображение, непрерывное по совокупности аргументов
   {отображение, непрерывное по совокупности аргументов}%
   {map continuous with respect to set of arguments}%
\Index%572%О%отображение, полилинейное над конечномерными алгебрами
   {отображение, полилинейное над конечномерными алгебрами}%
   {map polylinear over finite dimensional algebras}%
\Index%677%О%отображение, проективное над коммутативным кольцом
   {отображение, проективное над коммутативным кольцом}%
   {map projective over commutative ring}%
\SetIndexSpace%
\Index%317%П%параллелограмм
   {параллелограмм}%
   {parallelogram}%
\Index%739%П%параллельный сдвиг аффинного пространства
   {параллельный сдвиг аффинного пространства}%
   {parallel shift, affine space}%
\Index%587%П%парные представления
   {парные представления}%
   {twin representations}%
\Index%318%П%парные представления группы
   {парные представления группы}%
   {twin representations of group}%
\Index%319%П%парные представления расслоенной группы
   {парные представления расслоенной группы}%
   {twin representations of fibered group}%
\Index%320%П%парные представления тела
   {парные представления тела}%
   {twin representations of division ring}%
\Index%321%П%пассивное *G представление
   {пассивное \sT{G}представление}%
   {passive *G representation}%
\Index%333%П%пассивное представление
   {пассивное представление}%
   {passive representation}%
\Index%718%П%пассивное представление группы в многообразии базисов башни представлений
   {пассивное представление группы $G(\Vector f)$ в многообразии базисов башни представлений}%
   {passive representation in basis manifold, tower of representations}%
\Index%695%П%пассивное представление группы в многообразии базисов представления
   {пассивное представление группы $G(f)$ в многообразии базисов представления}%
   {passive representation in basis manifold}%
\Index%717%П%пассивное преобразование многообразия базисов башни представлений
   {пассивное преобразование многообразия базисов башни представлений}%
   {passive transformation of basis, tower of representations}%
\Index%570%П%пассивное преобразование многообразия базисов представления
   {пассивное преобразование многообразия базисов представления}%
   {passive transformation of basis, representation}%
\Index%335%П%пассивное преобразование на многообразии базисов
   {пассивное преобразование на многообразии базисов}%
   {passive transformation}%
\Index%336%П%пассивное преобразование на множестве rcd базисов
   {пассивное преобразование на множестве \rcd базисов}%
   {passive transformation, vector space}%
\Index%337%П%первый закон Ньютона
   {первый закон Ньютона}%
   {First Newton law}%
\Index%338%П%перенос Картана
   {перенос Картана}%
   {Cartan transport}%
\Index%339%П%перенос Френе
   {перенос Френе}%
   {Frenet transport}%
\Index%863%П%перестановка
   {перестановка}%
   {permutation}%
\Index%853%П%подалгебра Omega-алгебры
   {подалгебра $\Omega$\Hyph алгебры}%
   {subalgebra of Omega-algebra}%
\Index%230%П%подгруппа Omega группы
   {подгруппа $\Omega$\Hyph группы}%
   {subgroup of Omega group}%
\Index%909%П%подмодуль
   {подмодуль}%
   {submodule}%
\Index%912%П%подмодуль, порождённым множеством
   {подмодуль, порождённым множеством}%
   {submodule generated by set}%
\Index%334%П%подпредставление представления
   {подпредставление представления}%
   {subrepresentation of representation}%
\Index%322%П%подпредставление, порождённое множеством X
   {подпредставление, порождённое множеством $X$}%
   {subrepresentation generated by set}%
\Index%340%П%подрасслоение
   {подрасслоение}%
   {subbundle}%
\Index%341%П%подрасслоение Dstar-векторного расслоения
   {подрасслоение $\mathcal D\star$\hyph векторного расслоения}%
   {subbundle of Dstar vector bundle}%
\Index%806%П%полиаддитивное отображение
   {полиаддитивное отображение}%
   {polyadditive map}%
\Index%344%П%поливектор
   {поливектор}%
   {polyvector}%
\Index%345%П%полилинейное косо симметричное отображение
   {полилинейное косо симметричное отображение}%
   {polylinear map skew symmetric}%
\Index%609%П%полилинейное отображение
   {полилинейное отображение}%
   {polylinear map}%
\Index%347%П%полилинейное симметричное отображение
   {полилинейное симметричное отображение}%
   {polylinear map symmetric}%
\Index%760%П%полиморфизм представлений
   {полиморфизм представлений}%
   {polymorphism of representations}%
\Index%764%П%полная мера
   {полная мера}%
   {complete measure}%
\Index%811%П%полная нормированная Omega группа
   {полная нормированная $\Omega$\Hyph группа}%
   {complete Omega group}%
\Index%348%П%полная система линейных дифференциальных уравнений в частных производны
   {полная система линейных дифференциальных уравнений в частных производны}%
   {Complete System of Linear Partial Differential Equations}%
\Index%270%П%полное кольцо
   {полное кольцо}%
   {complete ring}%
\Index%349%П%полное тело
   {полное тело}%
   {complete division ring}%
\Index%868%П%полугруппа
   {полугруппа}%
   {semigroup}%
\Index%169%П%полукольцо множеств
   {полукольцо множеств}%
   {semiring of sets}%
\Index%186%П%пополнение нормированной Omegaгруппы
   {пополнение нормированной $\Omega$\Hyph группы}%
   {completion of normed Omega group}%
\Index%19%П%пополнение представления
   {пополнение представления}%
   {completion of representation}%
\Index%241%П%последовательность Коши
   {последовательность Коши}%
   {Cauchy sequence}%
\Index%816%П%последовательность сходится
   {последовательность сходится}%
   {sequence converges}%
\Index%578%П%последовательность сходится почти всюду
   {последовательность сходится почти всюду}%
   {converges almost everywhere}%
\Index%817%П%последовательность сходится равномерно
   {последовательность сходится равномерно}%
   {sequence converges uniformly}%
\Index%352%П%потенциальная энергия
   {потенциальная энергия}%
   {potential energy}%
\Index%30%П%правая дробь
   {правая дробь}%
   {right fraction}%
\Index%898%П%правое A векторное пространство
   {правое $A$\Hyph векторное пространство}%
   {right A vector space}%
\Index%671%П%правое D векторное пространство столбцов
   {правое $D$\hyph векторное пространство столбцов}%
   {right vector space of columns}%
\Index%654%П%правое D векторное пространство строк
   {правое $D$\hyph векторное пространство строк}%
   {right vector space of rows}%
\Index%753%П%правое алгебраическое дополнение элемента матрицы
   {правое алгебраическое дополнение элемента матрицы}%
   {right cofactor, matrix}%
\Index%353%П%правое векторное пространство
   {правое векторное пространство}%
   {right vector space}%
\Index%757%П%правое двойное алгебраическое дополнение элемента матрицы
   {правое двойное алгебраическое дополнение элемента матрицы}%
   {right double cofactor}%
\Index%354%П%правоинвариантное векторное поле
   {правоинвариантное векторное поле}%
   {right invariant vector}%
\Index%900%П%правостороннее A представление
   {правостороннее $A_1$\Hyph представление}%
   {right-side A representation}%
\Index%355%П%правостороннее представление
   {правостороннее представление}%
   {right-side representation}%
\Index%357%П%правостороннее представление Omega1 алгебры A в Omega2 алгебре M
   {правостороннее представление $\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре $M$}%
   {right-side representation of algebra}%
\Index%358%П%правостороннее представление расслоенной Omega- алгебры
   {правостороннее представление расслоенной $\Omega$\Hyph алгебры}%
   {right-side representation of fibered Omega-algebra}%
\Index%359%П%правостороннее преобразование
   {правостороннее преобразование}%
   {right-side transformation}%
\Index%891%П%правостороннее произведение
   {правостороннее произведение}%
   {right-side product}%
\Index%674%П%правостороннее произведение вектора на скаляр
   {правостороннее произведение вектора на скаляр}%
   {right-side product of vector over scalar}%
\Index%360%П%правые структурные константы алгебры Ли
   {правые структурные константы алгебры Ли}%
   {right structural constant of Lie algebra}%
\Index%897%П%правый D модуль
   {правый $D$\Hyph модуль}%
   {right D module}%
\Index%242%П%правый главный идеал
   {правый главный идеал}%
   {right principal ideal}%
\Index%813%П%правый делитель нуля
   {правый делитель нуля}%
   {right zero divisor}%
\Index%42%П%правый идеал алгебры
   {правый идеал алгебры}%
   {right ideal of algebra}%
\Index%361%П%правый модуль
   {правый модуль}%
   {right module}%
\Index%362%П%правый сдвиг на группе
   {правый сдвиг на группе}%
   {right shift}%
\Index%363%П%правый сдвиг на группе
   {правый сдвиг на группе}%
   {right shift, group}%
\Index%670%П%праый модуль над D- алгеброй A
   {правый модуль над $D$\Hyph алгеброй $A$}%
   {right module over algebra}%
\Index%467%П%предел последовательности
   {предел последовательности}%
   {limit of sequence}%
\Index%365%П%предел соответствия по фильтру
   {предел соответствия по фильтру}%
   {limit of correspondence with respect to the filter}%
\Index%366%П%предел фильтра
   {предел фильтра}%
   {limit of filter}%
\Index%367%П%предельное множество фильтра
   {предельное множество фильтра}%
   {limit set of filter}%
\Index%702%П%представитель геометрического объекта в drc векторном пространстве
   {представитель геометрического объекта в \drc векторном пространстве}%
   {representative of geometric object, drc vector space}%
\Index%703%П%представитель геометрического объекта в Omega_2- алгбре
   {представитель геометрического объекта в $\Omega_2$\Hyph алгбре}%
   {representative of geometric object, representation g}%
\Index%368%П%представитель геометрического объекта в rcd векторном пространстве
   {представитель геометрического объекта в \rcd векторном пространстве}%
   {representative of geometric object, rcd vector space}%
\Index%369%П%представитель геометрического объекта в векторном пространстве
   {представитель геометрического объекта в векторном пространстве}%
   {representative of geometric object, vector space}%
\Index%724%П%представитель геометрического объекта в кортеже Omega- алгебр
   {представитель геометрического объекта в кортеже $\VX\Omega$\Hyph алгебр}%
   {representative of geometric object, tower of representations g}%
\Index%370%П%представление Omega- алгебры A в категории B
   {представление $\Omega$\Hyph алгебры $A$ в категории $\mathcal B$}%
   {representation of Omega algebra in category}%
\Index%529%П%представление Omega алгебры в башне представлений
   {представление $\Omega$\Hyph алгебры в башне представлений}%
   {representation of Omega algebra in tower of representations}%
\Index%528%П%представление Omega алгебры в представлении
   {представление $\Omega$\Hyph алгебры в представлении}%
   {representation of Omega algebra in representation}%
\Index%82%П%представление Omega1 алгебры A в Omega2 алгебре *A
   {\sT{A}представление $\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре}%
   {*A representation of algebra}%
\Index%371%П%представление Omega1 алгебры A в Omega2 алгебре M
   {представление $\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре $M$}%
   {representation of algebra}%
\Index%90%П%представление в Omega2- алгебре A*
   {\Ts{A}представление в $\Omega_2$\Hyph алгебре}%
   {A* representation of algebra}%
\Index%372%П%представление группы
   {представление группы}%
   {representation of group}%
\Index%117%П%представление, сопряжённое представлению
   {представление, сопряжённое представлению}%
   {representation conjugated to representation}%
\Index%373%П%преобразование Лоренца
   {преобразование Лоренца}%
   {Lorentz transformation}%
\Index%375%П%преобразование расслоения
   {преобразование расслоения}%
   {transformation of bundle}%
\Index%23%П%преобразование сопряжения
   {преобразование сопряжения}%
   {conjugation transformation}%
\Index%374%П%преобразование универсальной алгебры
   {преобразование универсальной алгебры}%
   {transformation of universal algebra}%
\Index%376%П%преобразование, согласованное с эквивалентностью 
   {преобразование, согласованное с эквивалентностью }%
   {transformation coordinated with equivalence}%
\Index%377%П%приведенное декартово произведение расслоений
   {приведенное декартово произведение расслоений}%
   {reduced Cartesian product of bundles}%
\Index%378%П%приведенное декартово произведение расслоенных пространств
   {приведенное декартово произведение расслоенных пространств}%
   {reduced Cartesian product of total spaces}%
\Index%843%П%приведенное квадратное уравнение
   {приведенное квадратное уравнение}%
   {reduced quadratic equation}%
\Index%380%П%приведенное расслоенное соответствие в A
   {приведенное расслоенное соответствие в $\Bundle{A}$}%
   {reduced fibered correspondence in A}%
\Index%379%П%приведенное расслоенное соответствие из A в B
   {приведенное расслоенное соответствие из $\mathcal{A}$ в $\Bundle{B}$}%
   {reduced fibered correspondence from A to B}%
\Index%831%П%приведенный морфизм представлений
   {приведенный морфизм представлений}%
   {reduced morphism of representations}%
\Index%761%П%приведенный полиморфизм представлений
   {приведенный полиморфизм представлений}%
   {reduced polymorphism of representations}%
\Index%381%П%приводимое бикольцо
   {приводимое бикольцо}%
   {reducible biring}%
\Index%382%П%принцип двойственности для бикольца
   {принцип двойственности для бикольца}%
   {duality principle for biring}%
\Index%383%П%принцип двойственности для бикольца матриц
   {принцип двойственности для бикольца матриц}%
   {duality principle for biring of matrices}%
\Index%705%П%принцип инвариантности в \drc векторном пространстве
   {принцип инвариантности в \drc векторном пространстве}%
   {invariance principle}%
\Index%710%П%принцип инвариантности в башне представлений универсальных алгебр
   {принцип инвариантности в башне представлений универсальных алгебр}%
   {invariance principle, tower of representations g}%
\Index%385%П%принцип инвариантности в векторном пространстве
   {принцип инвариантности в векторном пространстве}%
   {invariance principle, vector space}%
\Index%384%П%принцип инвариантности в представлении универсальной алгебры
   {принцип инвариантности в представлении универсальной алгебры}%
   {invariance principle, representation g}%
\Index%162%П%продолжение меры
   {продолжение меры}%
   {extension of measure}%
\Index%386%П%продолжение соответствия
   {продолжение соответствия}%
   {extension of correspondence}%
\Index%195%П%проективное отображение непрерывно по направлению над полем
   {проективное отображение непрерывно по направлению над полем}%
   {projective map is continuous in direction over field}%
\Index%387%П%проекция расслоения E вдоль слоя E
   {проекция расслоения $\Bundle E$ вдоль слоя $E$}%
   {projection of bundle along fiber}%
\Index%395%П%произведение в категории
   {произведение в категории}%
   {product in category}%
\Index%388%П%произведение геометрического объекта и константы
   {произведение геометрического объекта и константы}%
   {product of geometric object and constant}%
\Index%389%П%произведение геометрического объекта и константы в векторном пространстве
   {произведение геометрического объекта и константы в векторном пространстве}%
   {product of geometric object and constant, vector space}%
\Index%663%П%произведение колец множеств
   {произведение колец множеств}%
   {product of rings of sets}%
\Index%172%П%произведение мер
   {произведение мер}%
   {product of measures}%
\Index%666%П%произведение многочленов
   {произведение многочленов}%
   {product of polynomials}%
\Index%392%П%произведение морфизмов Tstar- представлений расслоенной Omega- алгебры
   {произведение морфизмов \Ts представлений расслоенной $\Omega$\Hyph алгебры}%
   {product of morphisms of representations of fibered Omega algebra}%
\Index%561%П%произведение морфизмов башни представлений
   {произведение морфизмов башни представлений}%
   {product of morphisms of tower of representations}%
\Index%391%П%произведение морфизмов представлений универсальной алгебры
   {произведение морфизмов представлений универсальной алгебры}%
   {product of morphisms of representations of universal algebra}%
\Index%393%П%произведение приведенных расслоенных соответствий
   {произведение приведенных расслоенных соответствий}%
   {composition of reduced fibered correspondences}%
\Index%394%П%произведение расслоенных соответствий
   {произведение расслоенных соответствий}%
   {composition of fibered correspondences}%
\Index%396%П%производная Гато второго порядка
   {производная Гато второго порядка}%
   {Gateaux derivative of Second Order}%
\Index%882%П%производная Гато второго порядка
   {производная второго порядка}%
   {derivative of Second Order}%
\Index%627%П%производная Гато отображения
   {производная Гато отображения}%
   {Gateaux derivative of map}%
\Index%399%П%производная Гато порядка n
   {производная Гато порядка $n$}%
   {Gateaux derivative of Order n}%
\Index%401%П%производная Картана
   {производная Картана}%
   {Cartan derivative}%
\Index%402%П%производная Ли
   {производная Ли}%
   {Lie derivative}%
\Index%403%П%производная Ли метрики
   {производная Ли метрики}%
   {Lie derivative of metric}%
\Index%404%П%производная Ли связности
   {производная Ли связности}%
   {Lie derivative of connection}%
\Index%878%П%производная отображения
   {производная отображения}%
   {derivative of map}%
\Index%884%П%производная порядка n
   {производная порядка $n$}%
   {derivative of Order n}%
\Index%483%П%простое A число
   {простое $A$\Hyph число}%
   {prime A number}%
\Index%810%П%простое отображение
   {простое отображение}%
   {simple map}%
\Index%405%П%простой поливектор
   {простой поливектор}%
   {simple polyvector}%
\Index%342%П%пространственноподобный вектор
   {пространственноподобный вектор}%
   {spacelike vector}%
\Index%635%П%пространство Минковского
   {пространство Минковского}%
   {Minkowski space, Finsler}%
\Index%406%П%пространство орбит G* представления
   {пространство орбит \Ts{G}представления}%
   {space of orbits of G* representation}%
\Index%684%П%пространство орбит левостороннего представления
   {пространство орбит левостороннего представления}%
   {space of orbits of left side representation}%
\Index%407%П%пространство отображений
   {пространство отображений}%
   {mapping space}%
\Index%408%П%противоположная расслоенная предупорядоченность
   {противоположная расслоенная предупорядоченность}%
   {opposite fibered preordering}%
\Index%911%П%прямая сумма
   {прямая сумма}%
   {direct sum}%
\Index%409%П%прямая сумма представлений
   {прямая сумма представлений}%
   {direct sum of representations}%
\Index%410%П%прямое произведение D- векторных пространств
   {прямое произведение $D$\Hyph векторных пространств}%
   {direct product of D vector spaces}%
\Index%412%П%прямое произведение G* представлений
   {прямое произведение \Ts{G}представлений}%
   {direct product of G* representations}%
\Index%411%П%прямое произведение rcd векторных пространств
   {прямое произведение \rcd векторных пространств}%
   {direct product, rcd vector space}%
\Index%413%П%прямое произведение представлений группы
   {прямое произведение представлений группы}%
   {direct product of representations of group}%
\Index%414%П%прямое произведение представлений расслоенной группы
   {прямое произведение представлений расслоенной группы}%
   {direct product of representations of fibered group}%
\Index%415%П%прямое произведение тел
   {прямое произведение тел}%
   {direct product of division rings}%
\Index%826%П%прямое произведением Omega алгебр
   {прямое произведением \(\Omega\)\Hyph алгебр}%
   {direct product of Omega algebras}%
\Index%540%П%псевдоэвклидова метрика на теле
   {псевдоэвклидова метрика на теле}%
   {pseudo-Euclidean metric on division ring}%
\Index%548%П%псевдоэвклидово скалярное произведение в D- векторном пространстве
   {псевдоэвклидово скалярное произведение в $D$\Hyph векторном пространстве}%
   {pseudo-Euclidean scalar product, vector space}%
\Index%543%П%псевдоэвклидово скалярное произведение на теле
   {псевдоэвклидово скалярное произведение на теле}%
   {pseudo-Euclidean scalar product on division ring}%
\Index%416%П%пфаффова производная
   {пфаффова производная}%
   {pfaffian derivative}%
\SetIndexSpace%
\Index%204%Р%разложение вектора относительно базиса сходится
   {разложение вектора относительно базиса сходится}%
   {expansion converges}%
\Index%621%Р%разложение вектора относительно базиса сходится нормально
   {разложение вектора относительно базиса сходится нормально}%
   {expansion converges normally}%
\Index%417%Р%размерность rcd векторного пространства
   {размерность \rcd векторного пространства}%
   {dimension of vector space}%
\Index%554%Р%ранг квадратичного отображения тела
   {ранг квадратичного отображения тела}%
   {rank of quadratic map, division ring}%
\Index%749%Р%ранг эрмитовой матрицы по главным минорам
   {ранг эрмитовой матрицы по главным минорам}%
   {rank of Hermitian matrix by principal minors}%
\Index%419%Р%расслоение уровня 2
   {расслоение уровня $2$}%
   {bundle of level 2}%
\Index%418%Р%расслоение уровня n
   {расслоение уровня $n$}%
   {bundle of level n}%
\Index%420%Р%расслоенная Omega- алгебра
   {расслоенная $\Omega$\Hyph алгебра}%
   {fibered Omega-algebra}%
\Index%421%Р%расслоенная Omega- подалгебра
   {расслоенная $\Omega$\Hyph подалгебра}%
   {fibered Omega-subalgebra}%
\Index%422%Р%расслоенная группа
   {расслоенная группа}%
   {fibered group}%
\Index%423%Р%расслоенная группа стабилизации
   {расслоенная группа стабилизации}%
   {fibered stability group}%
\Index%424%Р%расслоенная малая группа
   {расслоенная малая группа}%
   {fibered little group}%
\Index%425%Р%расслоенная предупорядоченность
   {расслоенная предупорядоченность}%
   {fibered preordering}%
\Index%426%Р%расслоенная упорядоченность
   {расслоенная упорядоченность}%
   {fibered ordering}%
\Index%427%Р%расслоенная эквивалентность
   {расслоенная эквивалентность}%
   {fibered equivalence}%
\Index%428%Р%расслоенное кольцо
   {расслоенное кольцо}%
   {fibered ring}%
\Index%429%Р%расслоенное подмножество
   {расслоенное подмножество}%
   {fibered subset}%
\Index%430%Р%расслоенное соответствие в A
   {расслоенное соответствие в $\Bundle{A}$}%
   {fibered correspondence in A}%
\Index%431%Р%расслоенное соответствие гомоморфизма
   {расслоенное соответствие гомоморфизма}%
   {fibered correspondence of homomorphism}%
\Index%432%Р%расслоенное соответствие из A в B
   {расслоенное соответствие из $\Bundle A$ в $\Bundle B$}%
   {fibered correspondence from A to B}%
\Index%433%Р%расслоенный естественный морфизм
   {расслоенный естественный морфизм}%
   {fibered natural morphism}%
\Index%434%Р%расслоенный координатный Drc изоморфизм
   {расслоенный координатный изоморфизм}%
   {fibered coordinate isomorphism}%
\Index%435%Р%расслоенный морфизм из расслоения A в B
   {расслоенный морфизм из расслоения $\Bundle A$ в $\Bundle B$}%
   {fibered morphism from A into B}%
\Index%436%Р%расслоенный морфизм отождествления
   {расслоенный морфизм отождествления}%
   {fibered identification morphism}%
\Index%437%Р%расширенная матрица drc линейных уравнений
   {расширенная матрица \drc линейных уравнений}%
   {extended matrix, system of drc linear equations}%
\Index%438%Р%расширенная матрица rcd линейных уравнений
   {расширенная матрица \rcd линейных уравнений}%
   {extended matrix, system of rcd linear equations}%
\Index%439%Р%рефлексивное 2- арное расслоенное отношение
   {рефлексивное $2$\Hyph арное расслоенное отношение}%
   {reflexive 2 ary fibered relation}%
\Index%782%Р%ряд сходится нормально
   {ряд сходится нормально}%
   {series converges normally}%
\Index%440%Р%ряд Тейлора
   {ряд Тейлора}%
   {Taylor series, division ring}%
\SetIndexSpace%
\Index%331%С%свободная абелевая группа
   {свободная абелевая группа}%
   {free Abelian group}%
\Index%606%С%свободная алгебра над кольцом
   {свободная алгебра над кольцом}%
   {free algebra over ring}%
\Index%442%С%свободное Tstar- представление расслоенной группы
   {свободное \Ts представление расслоенной группы}%
   {free representation of fibered group}%
\Index%862%С%свободное представление
   {свободное представление}%
   {free representation}%
\Index%441%С%свободное представление группы
   {свободное представление группы}%
   {free representation of group}%
\Index%690%С%свободный A- модуль
   {свободный $A$\Hyph модуль}%
   {free A module}%
\Index%612%С%свободный модуль
   {свободный модуль}%
   {free module}%
\Index%517%С%связное множество
   {связное множество}%
   {connected set}%
\Index%583%С%связность в главном расслоении
   {связность в главном расслоении}%
   {connection in principal bundle}%
\Index%443%С%связность Картана
   {связность Картана}%
   {Cartan connection}%
\Index%694%С%сечение расслоения
   {сечение расслоения}%
   {section of bundle}%
\Index%444%С%символ Картана
   {символ Картана}%
   {Cartan symbol}%
\Index%445%С%символ Кронекерa
   {символ Кронекерa}%
   {Kronecker symbol}%
\Index%906%С%симметрирование полилинейного отображения
   {симметрирование полилинейного отображения}%
   {symmetrization of polylinear map}%
\Index%446%С%симметричное 2- арное расслоенное отношение
   {симметричное $2$\Hyph арное расслоенное отношение}%
   {symmetric 2 ary fibered relation}%
\Index%447%С%симметричное билинейное отображение D- векторного пространства в тело
   {симметричное билинейное отображение $D$\Hyph векторного пространства в тело}%
   {symmetric bilinear map, vector space to division ring}%
\Index%903%С%симметричное полилинейное отображение
   {симметричное полилинейное отображение}%
   {symmetric polylinear map}%
\Index%650%С%симметричное полилинейное отображение в ассоциативную алгебру
   {симметричное полилинейное отображение в ассоциативную алгебру}%
   {polylinear map symmetric, associative algebra}%
\Index%214%С%симплекс
   {симплекс}%
   {simplex}%
\Index%839%С%синус
   {синус}%
   {sine}%
\Index%448%С%синхронизация системы отсчёта
   {синхронизация системы отсчёта}%
   {synchronization of reference frame}%
\Index%449%С%система drc линейных уравнений
   {система \drc линейных уравнений}%
   {system of drc linear equations}%
\Index%311%С%система rcd линейных уравнений
   {система \rcd линейных уравнений}%
   {system of rcd linear equations}%
\Index%605%С%система аддитивных уравнений
   {система аддитивных уравнений}%
   {system of additive equations}%
\Index%201%С%система линейных уравнений
   {система линейных уравнений}%
   {system of linear equations}%
\Index%450%С%система отсчёта в пространстве событий
   {система отсчёта в пространстве событий}%
   {reference frame in event space}%
\Index%784%С%скаляр элемента алгебры
   {скаляр элемента алгебры}%
   {scalar of algebra}%
\Index%773%С%скаляр элемента кольца
   {скаляр элемента кольца}%
   {scalar of ring}%
\Index%451%С%скалярный потенциал
   {скалярный потенциал}%
   {scalar potential}%
\Index%452%С%скорость отклонения
   {скорость отклонения}%
   {speed of deviation}%
\Index%743%С%след кватерниона
   {след кватерниона}%
   {trace, quaternion algebra}%
\Index%453%С%смешанная частная производная Гато
   {смешанная частная производная Гато}%
   {Gateaux partial derivative of Second Order}%
\Index%454%С%соответствие гомоморфизма
   {соответствие гомоморфизма}%
   {correspondence of homomorphism}%
\Index%455%С%соответствие, непрерывное на множестве
   {соответствие, непрерывное на множестве}%
   {correspondence continuous on the set}%
\Index%788%С%сопряжение в алгебре
   {сопряжение в алгебре}%
   {conjugation in algebra}%
\Index%777%С%сопряжение в кольце
   {сопряжение в кольце}%
   {conjugation in ring}%
\Index%683%С%сопряжённое аффинное пространство
   {сопряжённое аффинное пространство}%
   {conjugated affine space}%
\Index%789%С%сопряжённое векторное пространство
   {сопряжённое векторное пространство}%
   {conjugated vector space}%
\Index%580%С%сопряжённый D  модуль
   {сопряжённый $D$\Hyph  модуль}%
   {conjugated D module}%
\Index%457%С%стабильное множество представления
   {стабильное множество представления}%
   {stable set of representation}%
\Index%458%С%стандартная компонента дифференциала Гато
   {стандартная компонента производной Гато}%
   {standard component of Gateaux derivative}%
\Index%456%С%стандартная компонента линейного отображения
   {стандартная компонента линейного отображения}%
   {standard component of linear map}%
\Index%461%С%стандартная компонента над полем F билинейного отображения f
   {стандартная компонента над полем $F$ билинейного отображения $f$}%
   {standard component of bilinear map, division ring}%
\Index%462%С%стандартная компонента полилинейного отображения
   {стандартная компонента полилинейного отображения}%
   {standard component of polylinear map}%
\Index%881%С%стандартная компонента производной
   {стандартная компонента производной}%
   {standard component of derivative}%
\Index%463%С%стандартная компонента тензора
   {стандартная компонента тензора}%
   {standard component of tensor}%
\Index%466%С%стандартное представление квадратичного отображения тела над полем F
   {стандартное представление квадратичного отображения тела над полем $F$}%
   {quadratic map, standard representation, division ring}%
\Index%464%С%стандартное представление линейного отображения
   {стандартное представление линейного отображения}%
   {linear map, standard representation}%
\Index%468%С%стандартное представление матрицы
   {стандартное представление матрицы}%
   {Standard representation}%
\Index%469%С%стандартное представление над полем F билинейного отображения тела
   {стандартное представление над полем $F$ билинейного отображения тела}%
   {bilinear map, standard representation, division ring}%
\Index%470%С%стандартное представление полилинейного отображения
   {стандартное представление полилинейного отображения}%
   {polylinear map, standard representation}%
\Index%880%С%стандартное представление производной
   {стандартное представление производной}%
   {derivative, standard representation}%
\Index%465%С%стандартное представление производной Гато
   {стандартное представление производной Гато}%
   {Gateaux derivative, standard representation}%
\Index%471%С%стандартные координаты базиса
   {стандартные координаты базиса}%
   {standard coordinates of basis}%
\Index%472%С%стандартные координаты базиса
   {стандартные координаты базиса}%
   {standard coordinates of basis}%
\Index%822%С%старший коэффициент многочлена
   {старший коэффициент многочлена}%
   {leading coefficient of polynomial}%
\Index%171%С%степень меры
   {степень меры}%
   {power of measure}%
\Index%750%С%столбцовый определитель
   {столбцовый определитель}%
   {column determinant}%
\Index%748%С%строчный определитель
   {строчный определитель}%
   {row determinant}%
\Index%473%С%структурные константы
   {структурные константы}%
   {structural constants}%
\Index%474%С%сужение соответствия \Phi на множество C
   {сужение соответствия $\Phi$ на множество $C$}%
   {restriction of correspondence}%
\Index%476%С%сумма геометрических объектов
   {сумма геометрических объектов}%
   {sum of geometric objects}%
\Index%477%С%сумма геометрических объектов в векторном пространстве
   {сумма геометрических объектов в векторном пространстве}%
   {sum of geometric objects, vector space}%
\Index%667%С%сумма многочленов
   {сумма многочленов}%
   {sum of polynomials}%
\Index%351%С%сумма отображений
   {сумма отображений}%
   {sum of maps}%
\Index%712%С%суперпозиция координат эндоморфизма башни представлений и элемента
   {суперпозиция координат эндоморфизма башни представлений $\Vector f$ и элемента $\VX a$}%
   {superposition of coordinates, tower of representations}%
\Index%323%С%суперпозиция координат эндоморфизма представления и элемента
   {суперпозиция координат эндоморфизма представления $f$ и элемента $m$}%
   {superposition of coordinates, representation}%
\Index%51%С%существенные параметры  семейства функций
   {существенные параметры  семейства функций}%
   {essential parameters}%
\Index%168%С%сферические координаты
   {сферические координаты}%
   {spherical coordinates}%
\SetIndexSpace%
\Index%478%Т%тензор кручения
   {тензор кручения}%
   {torsion tensor}%
\Index%479%Т%тензор напряжённости поля
   {тензор напряжённости поля}%
   {field-strength tensor}%
\Index%802%Т%тензор, обратный тензору
   {тензор, обратный тензору}%
   {inverse tensor}%
\Index%652%Т%тензорная степень
   {тензорная степень}%
   {tensor power}%
\Index%480%Т%тензорное произведение
   {тензорное произведение}%
   {tensor product}%
\Index%485%Т%тип векторного пространства
   {тип векторного пространства}%
   {vector space type}%
\Index%310%Т%топологическая D-алгебра
   {топологическая $D$\Hyph алгебра}%
   {topological D algebra}%
\Index%486%Т%топологическое D- векторное пространство
   {топологическое $D$\Hyph векторное пространство}%
   {topological D vector space}%
\Index%790%Т%топологическое кольцо
   {топологическое кольцо}%
   {topological ring}%
\Index%488%Т%топологическое тело
   {топологическое тело}%
   {topological division ring}%
\Index%824%Т%точка прикосновения множества
   {точка прикосновения множества}%
   {contact point of set}%
\Index%489%Т%транзитивное 2- арное расслоенное отношение
   {транзитивное $2$\Hyph арное расслоенное отношение}%
   {transitive 2 ary fibered relation}%
\Index%490%Т%транзитивное представление Omega- алгебры A
   {транзитивное представление $\Omega$\Hyph алгебры $A$}%
   {transitive representation of algebra}%
\Index%491%Т%транзитивное представление группы
   {транзитивное представление группы}%
   {transitive representation of group}%
\Index%492%Т%транзитивное представление расслоенной Omega- алгебры
   {транзитивное представление расслоенной $\Omega$\Hyph алгебры}%
   {transitive representation of fibered Omega-algebra}%
\SetIndexSpace%
\Index%851%У%универсальная алгебра
   {универсальная алгебра}%
   {universal algebra}%
\Index%688%У%универсально отталкивающий  объект категории
   {универсально отталкивающий  объект категории}%
   {universally repelling}%
\Index%914%У%универсально притягивающий объект категории
   {универсально притягивающий объект категории}%
   {universally attracting}%
\Index%915%У%унитальное кольцо
   {унитальное кольцо}%
   {unital ring}%
\Index%916%У%унитальное расширение
   {унитальное расширение}%
   {unital extension}%
\Index%751%У%упорядоченное слева представление подстановки произведением циклов
   {упорядоченное слева представление подстановки произведением циклов}%
   {left-ordered cycle notation of permutation}%
\Index%752%У%упорядоченное справа представление подстановки произведением циклов
   {упорядоченное справа представление подстановки произведением циклов}%
   {right-ordered cycle notation of permutation}%
\Index%493%У%уравнение Киллинга
   {уравнение Киллинга}%
   {Killing equation}%
\Index%494%У%уравнение Киллинга второго рода
   {уравнение Киллинга второго рода}%
   {Killing equation second type}%
\Index%744%У%условие перестановочности следа
   {условие перестановочности следа}%
   {permutability property of trace}%
\Index%495%У%условие приводимости произведений
   {условие приводимости произведений}%
   {condition of reducibility of products}%
\SetIndexSpace%
\Index%496%Ф%фактор расслоение
   {фактор расслоение}%
   {quotient bundle}%
\Index%497%Ф%фильтр F сходится к A
   {фильтр $\mathfrak{F}$ сходится к $A$}%
   {filter converges}%
\Index%131%Ф%финслерова метрика
   {финслерова метрика}%
   {Finsler metric}%
\Index%574%Ф%финслерова структура
   {финслерова структура}%
   {Finsler structure}%
\Index%77%Ф%финслерово пространство
   {финслерово пространство}%
   {Finsler space}%
\Index%498%Ф%форма кручение
   {форма кручение}%
   {torsion form}%
\Index%499%Ф%формула Тейлора для многочлена
   {формула Тейлора для многочлена}%
   {Taylor polynomial, division ring}%
\Index%243%Ф%фундаментальная последовательность
   {фундаментальная последовательность}%
   {fundamental sequence}%
\Index%504%Ф%функция тела, Dstar дифференцируемая по Фреше
   {функция тела, \Ds дифференцируемая по Фреше}%
   {function Dstar differentiable in Frechet sense, division ring}%
\Index%155%Ф%функция, однородная степени
   {функция, однородная степени $k$}%
   {function homogeneous}%
\SetIndexSpace%
\Index%620%Ц%центр алгебры
   {центр $D$\Hyph алгебры $A$}%
   {center of algebra}%
\Index%507%Ц%центр кольца D
   {центр кольца $D$}%
   {center of ring}%
\Index%509%Ц%центро-аффинный базис
   {центро-аффинный базис}%
   {Central Affine Basis}%
\SetIndexSpace%
\Index%511%Ч%частная dcr производная Гато отображения f^b по переменной x^a
   {частная \dcr производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial dcr derivative of map with respect to variable, D vector space}%
\Index%888%Ч%частная производная
   {частная производная}%
   {partial derivative}%
\Index%889%Ч%частная производная второго порядка
   {частная производная второго порядка}%
   {partial derivative of second order}%
\Index%512%Ч%частная производная Гато
   {частная производная Гато}%
   {Gateaux partial derivative}%
\Index%475%Ч%частное линейное отображение
   {частное линейное отображение}%
   {partial linear map}%
\Index%827%Ч%частное от деления
   {частное от деления}%
   {quotient divided by}%
\Index%905%Ч%чётность перестановки
   {чётность перестановки}%
   {parity of permutation}%
\SetIndexSpace%
\Index%501%Ш%широта
   {широта}%
   {latitude}%
\SetIndexSpace%
\Index%566%Э%невырожденный эндоморфизм башни представлений
   {невырожденный эндоморфизм башни представлений}%
   {regular endomorphism of tower of representations}%
\Index%539%Э%эвклидова метрика на теле
   {эвклидова метрика на теле}%
   {Euclidean metric on division ring}%
\Index%547%Э%эвклидово скалярное произведение в D- векторном пространстве
   {эвклидово скалярное произведение в $D$\Hyph векторном пространстве}%
   {Euclidean scalar product, vector space}%
\Index%542%Э%эвклидово скалярное произведение на теле
   {эвклидово скалярное произведение на теле}%
   {Euclidean scalar product on division ring}%
\Index%917%Э%эквивалентные нормы
   {эквивалентные нормы}%
   {equivalent norms}%
\Index%836%Э%экспонента
   {экспонента}%
   {exponent}%
\Index%515%Э%экстремальная кривая
   {экстремальная кривая}%
   {extreme line}%
\Index%858%Э%эндоморфизм
   {эндоморфизм}%
   {endomorphism}%
\Index%559%Э%эндоморфизм башни представлений
   {эндоморфизм башни представлений}%
   {endomorphism of tower of representations}%
\Index%565%Э%эндоморфизм башни представлений, вырожденный на кортеже множеств образующих
   {эндоморфизм башни представлений, вырожденный на кортеже множеств образующих}%
   {endomorphism of representation, singular on tuple}%
\Index%564%Э%эндоморфизм башни представлений, невырожденный на кортеже множеств образующих
   {эндоморфизм башни представлений, невырожденный на кортеже множеств образующих}%
   {endomorphism of representation, regular on tuple}%
\Index%557%Э%эндоморфизм представления Omega алгебры
   {эндоморфизм представления $\Omega$\Hyph алгебры}%
   {endomorphism of representation}%
\Index%328%Э%эндоморфизм представления, вырожденный на множестве образующих X
   {эндоморфизм представления, вырожденный на множестве образующих $X$}%
   {endomorphism of representation, singular on set}%
\Index%327%Э%эндоморфизм представления, невырожденный на множестве образующих X
   {эндоморфизм представления, невырожденный на множестве образующих $X$}%
   {endomorphism of representation, regular on set}%
\Index%857%Э%эпиморфизм
   {эпиморфизм}%
   {epimorphism}%
\Index%747%Э%эрмитова матрица
   {эрмитова матрица}%
   {hermitian matrix}%
\Index%544%Э%эрмитова метрика на теле
   {эрмитова метрика на теле}%
   {hermitian metric on division ring}%
\Index%350%Э%эрмитово скалярное произведение в D- векторном пространстве
   {эрмитово скалярное произведение в $D$\Hyph векторном пространстве}%
   {hermitian scalar product, vector space}%
\Index%545%Э%эрмитово скалярное произведение на теле
   {эрмитово скалярное произведение на теле}%
   {hermitian scalar product on division ring}%
\Index%541%Э%эрмитово сопряжение в теле
   {эрмитово сопряжение в теле}%
   {hermitian conjugation, division ring}%
\Index%546%Э%эрмитово сопряжённый вектор
   {эрмитово сопряжённый вектор}%
   {hermitian conjugated vector}%
\Index%872%Э%эффект увлечения системы отсчёта
   {эффект увлечения системы отсчёта}%
   {frame dragging effect}%
\Index%516%Э%эффективное G* представление
   {эффективное \Ts{G}представление}%
   {effective G* representation}%
\Index%514%Э%эффективное Tstar- представление расслоенного тела
   {эффективное \Ts представление расслоенного тела}%
   {effective representation of fibered division ring}%
\Index%520%Э%эффективное Tstar- представление расслоенной группы
   {эффективное \Ts представление расслоенной группы}%
   {effective representation of fibered group}%
\Index%500%Э%эффективное представление
   {эффективное представление}%
   {effective representation}%
\Index%518%Э%эффективное представление группы
   {эффективное представление группы}%
   {effective representation of group}%
\Index%622%Э%эффективное представление кольца
   {эффективное представление кольца}%
   {effective representation of ring}%
\Index%519%Э%эффективное представление расслоенной Omega- алгебры
   {эффективное представление расслоенной $\Omega$\Hyph алгебры}%
   {effective representation of fibered Omega-algebra}%
\Index%521%Э%эффективное представление тела
   {эффективное представление тела}%
   {effective representation of division ring}%
\SetIndexSpace%
\Index%619%Я%ядро алгебры
   {ядро $D$\Hyph алгебры $A$}%
   {nucleus of algebra}%
\Index%874%Я%ядро гомоморфизма
   {ядро гомоморфизма}%
   {kernel of homomorphism}%
\Index%522%Я%ядро линейного отображения
   {ядро линейного отображения}%
   {kernel of linear map}%
\Index%524%Я%ядро неэффективности G* представления
   {ядро неэффективности \Ts{G}представления}%
   {kernel of inefficiency of G* representation}%
\Index%525%Я%ядро неэффективности представления группы
   {ядро неэффективности представления группы}%
   {kernel of inefficiency of representation of group}%
\Index%526%Я%ядро неэффективности представления расслоенной группы
   {ядро неэффективности представления расслоенной группы}%
   {kernel of inefficiency of representation of fibered group}%
\Index%593%Я%якобиевая полная система drc дифференциальных уравнений
   {якобиевая полная система \drc дифференциальных уравнений}%
   {Jacobian complete system of drc differential equations}%
\Index%592%Я%якобиевая полная система дифференциальных уравнений
   {якобиевая полная система дифференциальных уравнений}%
   {Jacobian complete system of differential equations}%
\SetIndexSpace%
\Index%809%M%mu измеримое отображение
   {$\mu$\Hyph измеримое отображение}%
   {mu measurable map}%
\SetIndexSpace%
\Index%644%O%Omega группа
   {$\Omega$\Hyph группа}%
   {Omega group}%
\Index%656%O%Omega кольцо
   {\(\Omega\)\Hyph кольцо}%
   {Omega ring}%
\Index%646%O%Omega линейное отображение
   {$\Omega$\Hyph линейное отображение}%
   {Omega linear map}%
\Index%707%O%Omega_2- слово элемента представления относительно множества образующих
   {$\Omega_2$\Hyph слово элемента представления относительно множества образующих}%
   {word of element relative to generating set, representation}%
\Index%850%O%Omega-алгебра
   {$\Omega$\Hyph алгебра}%
   {Omega-algebra}%
\SetIndexSpace%
\Index%658%S%sigma алгебра множеств
   {$\sigma$\Hyph алгебра множеств}%
   {sigma algebra of sets}%
\Index%795%S%sigma кольцо множеств
   {$\sigma$\Hyph кольцо множеств}%
   {sigma ring of sets}%
\Index%762%S%sigma-аддитивная мера
   {\(\sigma\)\Hyph аддитивная мера}%
   {sigma-additive measure}%

\CloseIndex


==> Preface.1601.03259.English.tex <==
%auto-ignore
\input{Preface.\BookNumber.Eq}

\chapter{Preface}

\section{Preface to Version 1}

\epigraph
{
The way of charms and disappointments.
//
However, I would put it another way.
When you understand that the reason for
your disappointments is in your expectations,
you start to examine surrounding landscape.
You found yourself on the path
where nobody went before.
New impressions are stronger
than impressions from travel along well known and trodden road.
}
{Author is unknown. The Adventures of an Explorer.}

The possibility of linear approximation of a map
is at the heart of calculus and
main constructions of calculus have their roots in linear
algebra.
Since the product in the field is
commutative, then linear algebra over a field is relatively simple.
When we explore algebra over commutative ring,
we still see some familiar statements of linear
algebra; however, we meet new statements, which
change the landscape of linear algebra.

Here I want to draw attention to the evolution of the concept
of the derivative from the time of Newton.
When we study functions of single variable, the derivative in selected point
is a number
\ShowEq{derivative single variable}
When we study function of multiple variables, we realize
that it is not enough to use number. The derivative becomes vector or gradient
\ShowEq{derivative multiple variables}
When we study maps of vector spaces, this is a first time that we tell about derivative
as operator
\ShowEq{derivative vector variables}
However since this operator is linear, then we can represent
derivative as matrix.
Again we express a vector of increment of a map
as product of a matrix of derivative (Jacobian matrix) over
vector of increment of argument
\ShowEq{derivative vector variables 1}

To understand the structure of derivative of a map of Banach algebra,
consider the map $y=x^2$ of quaternion algebra.
Since the argument $x$ has the increment $dx$,
then the increment $dy$ of the function $y$ has form
\ShowEq{dy of x2}
Since $dx$ is infinitesimal,
then we can ignore the value of $(dx)^2$
and, from the equality
\EqRef{dy of x2},
it follows that
\ShowEq{dy of x2 =}

If we assume that we can separate
left or right factor in the expression
\EqRef{dy of x2 =}
\ShowEq{dy of x2 = a dx}
like in the equality
\EqRef{derivative single variable},
then we see that the value $a$ depends on direction
of the differential $dx$.
It is reason to assume that the derivative in
quaternion algebra is directional derivative
or the G\^ateaux derivative
(\citeBib{Vadim Komkov}, page 322).
In such case, we consider the differential
\EqRef{dy of x2 =}
as additive map, namely, the map which satisfies the equality
\ShowEq{f(a+b)=fa+fb}

Already in the process of working on the paper
\citeBib{0812.4763},
I realized that I need to consider both left and right factors
instead of the expression
\EqRef{dy of x2 = a dx}
\ShowEq{dy of x2 = a dx b}
However, I continued to consider the expression
\EqRef{dy of x2 = a dx b}
as an additive map of the differential $dx$.

During exploring of the representation theory of universal algebra
(\citeBib{0912.3315,1502.04063}),
I realized that the expression
\EqRef{dy of x2 = a dx b}
is linear map of the differential $dx$.
So, the expression
\EqRef{dy of x2 =}
is the definition of the derivative of the map $y=x^2$.
This new concept is the basis of this paper.

\begin{flushright}
January, 2016
\end{flushright}

%\counterwithin{equation}{section}



==> Preface.1601.03259.Eq.tex <==
%auto-ignore

%\counterwithout{equation}{section}

\DefEquation
{
dx^2=\textcolor{red}{2x}\ dx
}
{derivative single variable}

\DefEquation
{
dy=(x+dx)^2-x^2=x^2+x\,dx+dx\,x+(dx)^2-x^2
=x\,dx+dx\,x+(dx)^2
}
{dy of x2}

\DefEquation
{
dy=x\,dx+dx\,x
}
{dy of x2 =}

\DefEquation
{
x\,dx+dx\,x=a\,dx
}
{dy of x2 = a dx}

\DefEquation
{
x\,dx+dx\,x=a\,dx\,b
}
{dy of x2 = a dx b}

\DefEq
{
f(a+b)=f(a)+f(b)
}
{f(a+b)=fa+fb}

\DefEq
{
\begin{align*}
z&=x^2+y^3
\\
dz&=\textcolor{red}{2x}\ dx+\textcolor{red}{3y^2}\ dy
\end{align*}
}
{derivative multiple variables}

\DefEq
{
\[
\begin{pmatrix}
dx\\dy\\dz
\end{pmatrix}
=
\textcolor{red}{\begin{pmatrix}
\sin v&u\cos v\\
\cos v&-u\sin v\\
1&0
\end{pmatrix}}
\begin{pmatrix}
du\\dv
\end{pmatrix}
\]
}
{derivative vector variables 1}

\DefEq
{
\[
\begin{matrix}
x=u\sin v&y=u\cos v&z=u
\\
dx=\textcolor{red}{\sin v}\ du+\textcolor{red}{u\cos v}\ dv&
dy=\textcolor{red}{\cos v}\ du-\textcolor{red}{u\sin v}\ dv&
dz=\textcolor{red}{1}\ du+\textcolor{red}{0}\ dv
\end{matrix}
\]
}
{derivative vector variables}



==> Preface.1601.03259.Russian.tex <==
%auto-ignore
\input{Preface.\BookNumber.Eq}

\chapter{Предисловие}

\section{Предисловие к изданию 1}

\epigraph
{Дорога очарований и разочарований.
//
Но я бы сказал наоборот.
Когда ты понимаешь, что причина
твоих разочарований - в твоих ожиданиях,
ты начинаешь присматриваться к окружающему ландшафту.
Ты оказался на тропе,
по которой до тебя никто не ходил.
И новые впечатления куда сильнее,
чем если бы ты шёл по дороге многократно протоптанной
и хорошо изученной.}
{Автор неизвестен. Записки путешественника.}

В основе математического
анализа лежит возможность линейного приближения к отображению,
и основные построения математического анализа уходят корнями в линейную
алгебру.
Так как произведение в поле
коммутативно, то линейная алгебра над полем относительно проста.
При переходе к алгебре над коммутативным кольцом, некоторые утверждения линейной
алгебры сохраняются, но появляются и новые утверждения, которые
меняют ландшафт линейной алгебры.

Здесь я хочу обратить внимание на эволюцию,
которую претерпело понятие производной со времён Ньютона.
Когда мы изучаем функции одной переменной, то производная в заданной точке
является числом
\ShowEq{derivative single variable}
Когда мы изучаем функцию нескольких переменных, выясняется,
что числа недостаточно. Производная становится вектором или градиентом
\ShowEq{derivative multiple variables}
При изучении отображений векторных пространств мы впервые говорим о производной
как об операторе
\ShowEq{derivative vector variables}
Но так как этот оператор линеен, то мы можем представить
производную как матрицу.
И в этом случае мы можем представить вектор приращения отображения
как произведение матрицы производной (матрицы Якоби) на
вектор приращения аргумента
\ShowEq{derivative vector variables 1}

Чтобы понять структуру производной отображения банаховой алгебры,
рассмотрим отображение $y=x^2$ алгебры кватернионов.
Если аргумент $x$ имеет приращение $dx$,
то приращение $dy$ функции $y$ имеет вид
\ShowEq{dy of x2}
Так как $dx$ является бесконечно малой,
то мы можем пренебречь значением величины $(dx)^2$
и из равенства
\EqRef{dy of x2}
следует, что
\ShowEq{dy of x2 =}

Если мы предположим, что в выражении
\EqRef{dy of x2 =}
можно выделить левый или правый множитель
\ShowEq{dy of x2 = a dx}
подобно равенству
\EqRef{derivative single variable},
то мы видим, что величина $a$ зависит от направления
дифференциала $dx$.
Это даёт основание предположить, что производная в
алгебре кватернионов является производной по направлению
или производной Гато
(\citeBib{Vadim Komkov}, страница 322).
При этом мы рассматриваем дифференциал
\EqRef{dy of x2 =}
как аддитивное отображение, т. е. отображение удовлетворяющее равенству
\ShowEq{f(a+b)=fa+fb}

Уже в процессе работы над статьёй
\citeBib{0812.4763}
я понял, что вместо выражения
\EqRef{dy of x2 = a dx}
я должен рассматривать оба левый и правый множители
\ShowEq{dy of x2 = a dx b}
Тем не менее, я продолжал рассматривать выражение
\EqRef{dy of x2 = a dx b}
как аддитивное отображение дифференциала $dx$.

В процессе изучения теории представлений универсальной алгебры
(\citeBib{0912.3315,1502.04063})
я понял, что выражение
\EqRef{dy of x2 = a dx b}
является линейным отображение дифференциала $dx$.
Следовательно, выражение
\EqRef{dy of x2 =}
является определением производной отображения $y=x^2$.
Эта новая концепция является основой данной статьи.

\begin{flushright}
Январь, 2016
\end{flushright}

%\counterwithin{equation}{section}



==> Preface.1610.01.English.tex <==
%auto-ignore

\ePrints{1610.01}%
\ifx\Semafor\ValueOn%
\input{Preface.\BookNumber.Eq}
\chapter{Preface}
\else
\input{Preface.1610.01.Eq}
\fi

\section{Integration in \texorpdfstring{$D$}{D}-algebra}

When professor Svetlin asked me if I can solve differential equations
over quaternion algebra my first answer was that I am not ready.
Diversity of differential equations of first order and
identification of the derivative of any order with function
of real field make this task extremely difficult.

However later I recalled that, in the paper
\citeBib{0812.4763},
I considered the operation inverse to differentiation.
I considered the indefinite integral
\ShowEq{f=indefinite integral g}
as solution of differential equation
\ShowEq{partial f=g}
and I represented this solution as Taylor series.
So, when I was writing the paper
\citeBib{CACAA.05.001},
I decided explicitly use integral notation.

If this had happened in 2012,
I would have stopped at this point and would start to study another subject.
\ePrints{4975-6381}
\ifx\Semafor\ValueOff
But in 2013 I had published the paper
\citeBib{1310.5591}.
\else
But in 2013 I started to write the book
\citeBib{5410-9916}.
\fi
And I had seen a serious problem.

I have two definitions of integral:
namely Lebesgue integral and indefinite integral.
And they have different formats of integrand.
In an indefinite integral,
we consider the representation of $D$\Hyph module
\ShowEq{AoA}
in $D$\Hyph algebra $A$
and integrand is an action of a tensor
\ShowEq{a in AA}
over differential.
In Lebesgue integral,
we consider the representation of algebra with measure
in $D$\Hyph algebra $A$.
What is the relation between
Lebesgue integral and indefinite integral?

At first sight, there is no answer to this question.
In the calculus over real field,
we use the same map in both cases.
And the relation between
Lebesgue integral and indefinite integral
can be expressed by either of following statements.

\begin{itemize}
\item
\ShowEq{int f=int 0x f}
\item
If
\ShowEq{g=int f}
then
\ShowEq{int ab f=g(b)-g(a)}
\end{itemize}

If we consider Lebesgue integral in $D$\Hyph algebra,
what does it mean to get an integral from $a$ to $b$?
The simplest solution is to use a path from $a$ to $b$.
In the paper
\citeBib{CACAA.05.001},
I considered the simplest path
\ShowEq{path abt}
However, the question remained open for arbitrary path.
If Lebesgue integral depends on the path,
then we need to study a dependence of Lebesgue integral from the path
instead of the relation between
Lebesgue integral and indefinite integral.
But this is absolutely different theory.

There exist maps which have
Lebesgue integral dependent on the path.
It follows from the remark
\ref{remark: differential equation 3x^2 does not possess a solution}.
%However, I was looking for maps which have Lebesgue integral.
However, I had great interest in the study of maps which have indefinite integral.

When I discussed this question with the professor Sudbery,
I suddenly found simple proof
of the statement that Lebesgue integral
of the derivative of the map does not depend on path (the theorem
\RefTheorem{Lebesgue Integral along Path}).
However I was not satisfied by this statement.
I knew that new adventure is waiting for me.

\section{Differential Form}

The question about possibility to solve differential equation
\ShowEq{df=g partial}
remained opened.
If solution does not exist,
then we can assume that Lebesgue integral of the map $g$
depends on the path.
In the differential geometry,
the map $f$ is called anholonomic.
Anholonomic maps are important in general relativity.
And I could not ignore this problem.

However if the Lebesgue integral depends on path,
then, of course, the question about integral over a closed circuit arises.
At this point, I realized that the map $g$ is differential form.

The study of differential forms demanded from me to expand the scope of my research.
In the definition
\xRef{1601.03259}{definition: differentiable map, algebra},
I considered differentiable map into Banach $D$\Hyph algebra.
However this definition is still true in case of Banach $D$\Hyph module.
To write the derivative of the map into Banach $D$\Hyph module,
we need a basis of the module and we write the Jacobian matrix of this map.
However, we can write the derivative of the map $f$ into Banach $D$\Hyph algebra $A$ analytically
using tensor
\ShowEq{df/dx in AxA}
I considered relation between two forms of representation of linear map
in the theorem
\ref{theorem: coordinates of map A1 A2, algebra}.

Moreover, we have the opportunity to write analytically a map into Banach $D$\Hyph module
when we consider $D$\Hyph module of polylinear maps
into $D$\Hyph algebra $B$
(the theorem
\RefTheorem{dfa1p/dx=df/dx a1p}).
In this case we can use
product in $D$\Hyph algebra $B$
to represent linear map in $D$\Hyph module
\ShowEq{L(AnB)}

\ePrints{1610.01}%
\ifx\Semafor\ValueOn%
When I started my research in July of 2008,
it was a blind search.
My research was based on the definition of linear map
which I learned in
\citeBib{0701.238}.
I wanted to clarify some details;
and I chose calculus because
this subject was interesting for me,
as well I knew that I need calculus
to study differential geometry.
At that time, I knew only map linear from left
and map linear from right.
Left and right derivatives looked like a layered cake;
the increment of the argument was its stuffing.

Without a doubt, it was Gateaux derivative.
And I used symbol $\partial$
to distinguish this derivative.
But I was not satisfied with this definition;
starting from 2010, I started to consider linear map
of $D$\Hyph algebra $A$ as representation of algebra $A\otimes A$
in algebra $A$. However, I still used old notation.

From the definition
\ref{definition: linear map from A1 to A2, algebra},
it follows that the definition
\ref{definition: differentiable map, algebra}
of derivative of map into Banach algebra
is not different from standard definition
of derivative of map into Banach module.
So I decided (starting from this paper)
to use standard notation for derivative.
\fi

%\section{General remarks}

\ePrints{1601.03259}%
\ifx\Semafor\ValueOn%
\begin{flushright}
January, 2017
\end{flushright}
\fi%


==> Preface.1610.01.Eq.tex <==
%auto-ignore

\DefEq
{
\[
\frac{d f(x)}{d x}=g(x)
\]
}
{df=g partial}

\AddEq{df/dx in AxA}
{
$\displaystyle\frac{df(x)}{dx}\in A\otimes A$.
}

\DefEq
{
\[
f(x)=\int g(x)\circ dx
\]
}
{f=indefinite integral g}

\DefEq
{
$a\in A\otimes A$
}
{a in AA}

\DefEq
{
$\mathcal L(D;A^n\rightarrow B)$.
}
{L(AnB)}

\DefEq
{
$\displaystyle \int_a^bf(x)dx=g(b)-g(a)$\,.
}
{int ab f=g(b)-g(a)}

\DefEq
{
$\displaystyle g(x)=\int f(x)dx$\,,
}
{g=int f}

\DefEq
{
\[x=a+t(b-a)\]
}
{path abt}

\DefEq
{
$\displaystyle\int f(x)dx=\int_a^x f(x)dx$
}
{int f=int 0x f}

\DefEq
{
$A\otimes A$
}
{AoA}

\DefEq
{
\[
\frac{d f(x)}{d x}\circ dx=g(x)\circ dx
\]
}
{partial f=g}


==> Preface.1610.01.Russian.tex <==
%auto-ignore

\ePrints{1610.01}%
\ifx\Semafor\ValueOn%
\input{Preface.\BookNumber.Eq}
\chapter{Предисловие}
\else
\input{Preface.1610.01.Eq}
\fi

\section{Интегрирование в \texorpdfstring{$D$}{D}-алгебре}

Когда профессор Светлин спросил меня, умею ли я решать дифференциальные уравнения
над алгеброй кватернионов, мой первый ответ был, что я ещё не готов.
Разнообразие дифференциальных уравнений первого порядка и
отождествление производной любого порядка с отображением
поля действительных чисел делают эту задачу невероятно сложной.

Однако позже я вспомнил, что в статье
\citeBib{0812.4763}
я рассматривал операцию обратную дифференцированию.
Я рассматривал неопределённый интеграл
\ShowEq{f=indefinite integral g}
как решение дифференциального уравнения
\ShowEq{partial f=g}
записанное в форме ряда Тейлора.
Поэтому, когда я писал статью
\citeBib{CACAA.05.001},
я решил явно писать интеграл.

Если бы это произошло в 2012,
на этом месте я бы остановился и начал бы изучать другую тему.
\ePrints{4975-6381}
\ifx\Semafor\ValueOff
Но в 2013 я опубликовал статью
\citeBib{1310.5591}.
\else
Но в 2013 я начал работать над книгой
\citeBib{5410-9916}.
\fi
И я увидел серьёзную проблему.

Я имею два определения интеграла:
интеграл Лебега и неопределённый интеграл.
И они имеют разный формат подынтегрального выражения.
В неопределённом интеграле,
мы рассматриваем представление $D$\Hyph модуля
\ShowEq{AoA}
в $D$\Hyph алгебре $A$,
и подынтегральное выражение равно действию тензора
\ShowEq{a in AA}
на дифференциал.
В интеграле Лебега,
мы рассматриваем представление алгебры, в которой определена мера,
в $D$\Hyph алгебре $A$.
Какова связь между
интегралом Лебега и неопределённым интегралом.

На первый взгляд, вопрос кажется неразрешимым.
В математическом анализе над полем действительных чисел,
в обоих случаях мы имеем дело с одним и тем же отображением.
И связь между
интегралом Лебега и неопределённым интегралом
может быть выражена любым из следующих утверждений.

\begin{itemize}
\item
\ShowEq{int f=int 0x f}
\item
Если
\ShowEq{g=int f}
то
\ShowEq{int ab f=g(b)-g(a)}
\end{itemize}

Если мы рассматриваем интеграл Лебега в $D$\Hyph алгебре,
что значит интегрировать от $a$ до $b$.
Самое простое решение - это рассмотреть путь из $a$ в $b$.
В статье
\citeBib{CACAA.05.001},
я рассмотрел самый простой путь
\ShowEq{path abt}
Однако вопрос оставался открытым для произвольного пути.
Если интеграл Лебега зависит от пути,
то вместо связи между
интегралом Лебега и неопределённым интегралом
мы должны изучать зависимость интеграла Лебега от пути.
Но это совершено другая теория.

Существуют отображения, для которых интеграл Лебега
зависит от пути интегрирования.
Это следует из замечания
\ref{remark: differential equation 3x^2 does not possess a solution}.
Но меня в первую очередь интересовали отображения, для
которых неопределённый интеграл существует.

Обсуждая этот вопрос с профессором Садбери,
я неожиданно нашёл простое доказательство
утверждения, что интеграл Лебега
производной отображения не зависит от пути (теорема
\RefTheorem{Lebesgue Integral along Path}).
Но я не был удовлетворён этим результатом.
Я знал, что меня ждёт новое приключение.

\section{Дифференциальная форма}

Вопрос о возможности решить дифференциальное уравнение
\ShowEq{df=g partial}
оставался открытым.
Если решения не существует,
то можно предположить, что интеграл Лебега отображения $g$
зависит от пути.
В дифференциальной геометрии,
отображение $f$ называется неголономным.
Неголономные отображения важны в общей теории относительности.
И я не мог пройти мимо этой задачи.

Но если интеграл Лебега зависит от пути,
то естественно возникает вопрос об интеграле по замкнутому контуру.
В эту минуту я осознал, что отображение $g$ является дифференциальной формой.

Изучение дифференциальных форм потребовало от меня расширить рамки моего исследования.
В определении
\xRef{1601.03259}{definition: differentiable map, algebra},
я рассматривал дифференцируемое отображение в банаховую $D$\Hyph алгебру.
Однако это определение верно также в случае банахового $D$\Hyph модуля.
Чтобы записать производную отображения в банаховый $D$\Hyph модуль,
нам нужен базис этого модуля, и мы записываем матрицу Якоби этого отображения.
Однако мы можем записать производную отображения $f$ в банаховую $D$\Hyph алгебру $A$ аналитически
с помощью тензора
\ShowEq{df/dx in AxA}
Я рассмотрел связь между двумя формами представления линейного отображения
в теореме
\ref{theorem: coordinates of map A1 A2, algebra}.

Более того, возможность записать аналитически отображение в банаховый $D$\Hyph модуль
появляется, если мы рассматриваем $D$\Hyph модуль полилинейных отображений
в $D$\Hyph алгебру $B$
(теорема
\RefTheorem{dfa1p/dx=df/dx a1p}).
В этом случае мы можем воспользоваться
произведением в $D$\Hyph алгебре $B$
для представления линейного отображения в $D$\Hyph модуль
\ShowEq{L(AnB)}

\ePrints{1610.01}%
\ifx\Semafor\ValueOn%
Когда я начал мой поиск в июле 2008,
это был поиск вслепую.
Я опирался на конструкцию линейного отображения,
которую я изучал в
\citeBib{0701.238}.
Мне нужно было прояснить некоторые детали,
и я выбрал математический анализ как наиболее
близкую для меня тему.
Кроме того, я понимал, что мне необходим математический анализ
для изучения дифференциальной геометрии.
В тот период я знал только отображение, линейное слева,
и отображение, линейное справа.
Левая и правая производные напоминали слоённый пирог,
начинка которого было приращение аргумента.

Без сомнения, это была производная Гато.
И я воспользовался символом $\partial$,
чтобы отличать эту производную.
Но я не был удовлетворён этим определением,
и начиная с 2010 я стал рассматривать линейное отображение
$D$\Hyph алгебры $A$ как представление алгебры $A\otimes A$
в алгебре $A$. А старое обозначение осталось.

Из определения
\ref{definition: linear map from A1 to A2, algebra}
следует, что определение
\ref{definition: differentiable map, algebra}
производной отображения в банаховую алгебру
не отличается от стандартного определения производной
отображения в банаховый модуль.
Поэтому я решил, начиная с этой статьи,
пользоваться стандартным обозначением производной.
\fi

%\section{Общие замечания}


\ePrints{1601.03259}%
\ifx\Semafor\ValueOn%
\begin{flushright}
Январь, 2017
\end{flushright}
\fi%


==> Preface.1610.309618526.Russian.tex <==
%auto-ignore
\input{Preface.1610.309618526.Eq}

\ePrints{1610.309618526,CACAA.06}%
\ifx\Semafor\ValueOn%
\Chapter{Предисловие}
\fi

\Section{Интегрирование в \texorpdfstring{$D$}{D}-алгебре}

Когда профессор Светлин спросил меня, умею ли я решать дифференциальные уравнения
над алгеброй кватернионов, мой первый ответ был, что я ещё не готов.
Разнообразие дифференциальных уравнений первого порядка и
отождествление производной любого порядка с отображением
поля действительных чисел делают эту задачу невероятно сложной.

Однако позже я вспомнил, что в статье
\citeBib{0812.4763}
я рассматривал операцию обратную дифференцированию.
Я рассматривал неопределённый интеграл
\ShowEq{f=indefinite integral g}
как решение дифференциального уравнения
\ShowEq{partial f=g}
записанное в форме ряда Тейлора.
Поэтому, когда я писал статью
\citeBib{CACAA.05.001},
я решил явно писать интеграл.

Если бы это произошло в 2012,
на этом месте я бы остановился и начал бы изучать другую тему.
\ePrints{4975-6381}
\ifx\Semafor\ValueOff
Но в 2013 я опубликовал статью
\ePrints{CACAA.06}
\ifx\Semafor\ValueOff
\citeBib{1310.5591}.
\else
\citeBib{CACAA.04.001}.
\fi
\else
Но в 2013 я начал работать над книгой
\citeBib{5410-9916}.
\fi
И я увидел серьёзную проблему.

Я имею два определения интеграла:
интеграл Лебега и неопределённый интеграл.
И они имеют разный формат подынтегрального выражения.
В неопределённом интеграле,
мы рассматриваем представление $D$\Hyph модуля
\ShowEq{AoA}
в $D$\Hyph алгебре $A$,
и подынтегральное выражение равно действию тензора
\ShowEq{a in AA}
на дифференциал.
В интеграле Лебега,
мы рассматриваем представление алгебры, в которой определена мера,
в $D$\Hyph алгебре $A$.
Какова связь между
интегралом Лебега и неопределённым интегралом.

На первый взгляд, вопрос кажется неразрешимым.
В математическом анализе над полем действительных чисел,
в обоих случаях мы имеем дело с одним и тем же отображением.
И связь между
интегралом Лебега и неопределённым интегралом
может быть выражена любым из следующих утверждений.

\begin{itemize}
\item
\ShowEq{int f=int 0x f}
\item
Если
\ShowEq{g=int f}
то
\ShowEq{int ab f=g(b)-g(a)}
\end{itemize}

Если мы рассматриваем интеграл Лебега в $D$\Hyph алгебре,
что значит интегрировать от $a$ до $b$.
Самое простое решение - это рассмотреть путь из $a$ в $b$.
В статье
\citeBib{CACAA.05.001},
я рассмотрел самый простой путь
\ShowEq{path abt}
Однако вопрос оставался открытым для произвольного пути.
Если интеграл Лебега зависит от пути,
то вместо связи между
интегралом Лебега и неопределённым интегралом
мы должны изучать зависимость интеграла Лебега от пути.
Но это совершено другая теория.

Существуют отображения, для которых интеграл Лебега
зависит от пути интегрирования.
Это следует из замечания
\ref{remark: differential equation 3x^2 does not possess a solution}.
Но меня в первую очередь интересовали отображения, для
которых неопределённый интеграл существует.

Обсуждая этот вопрос с профессором Садбери,
я неожиданно нашёл простое доказательство
утверждения, что интеграл Лебега
производной отображения не зависит от пути (теорема
\RefTheorem{Lebesgue Integral along Path}).
Но я не был удовлетворён этим результатом.
Я знал, что меня ждёт новое приключение.

\Section{Дифференциальная форма}

Вопрос о возможности решить дифференциальное уравнение
\ShowEq{df=g partial}
оставался открытым.
Если решения не существует,
то можно предположить, что интеграл Лебега отображения $g$
зависит от пути.
В дифференциальной геометрии,
отображение $f$ называется неголономным.
Неголономные отображения важны в общей теории относительности.
И я не мог пройти мимо этой задачи.

Но если интеграл Лебега зависит от пути,
то естественно возникает вопрос об интеграле по замкнутому контуру.
В эту минуту я осознал, что отображение $g$ является дифференциальной формой.

Изучение дифференциальных форм потребовало от меня расширить рамки моего исследования.
В определении
\RefDefinition[1601.03259]{differentiable map, algebra},
я рассматривал дифференцируемое отображение в банаховую $D$\Hyph алгебру.
Однако это определение верно также в случае банахового $D$\Hyph модуля.
Чтобы записать производную отображения в банаховый $D$\Hyph модуль,
нам нужен базис этого модуля, и мы записываем матрицу Якоби этого отображения.
Однако мы можем записать производную отображения $f$ в банаховую $D$\Hyph алгебру $A$ аналитически
с помощью тензора
\ShowEq{df/dx in AxA}
Я рассмотрел связь между двумя формами представления линейного отображения
в теореме
\RefTheorem{coordinates of map A1 A2, algebra}.

Более того, возможность записать аналитически отображение в банаховый $D$\Hyph модуль
появляется, если мы рассматриваем $D$\Hyph модуль полилинейных отображений
в $D$\Hyph алгебру $B$
(теорема
\RefTheorem{dfa1p/dx=df/dx a1p}).
В этом случае мы можем воспользоваться
произведением в $D$\Hyph алгебре $B$
для представления линейного отображения в $D$\Hyph модуль
\ShowEq{L(AnB)}

\ePrints{1610.309618526,CACAA.06}%
\ifx\Semafor\ValueOn%
Когда я начал мой поиск в июле 2008,
это был поиск вслепую.
Я опирался на конструкцию линейного отображения,
которую я изучал в
\citeBib{0701.238}.
Мне нужно было прояснить некоторые детали,
и я выбрал математический анализ как наиболее
близкую для меня тему.
Кроме того, я понимал, что мне необходим математический анализ
для изучения дифференциальной геометрии.
В тот период я знал только отображение, линейное слева,
и отображение, линейное справа.
Левая и правая производные напоминали слоённый пирог,
начинка которого было приращение аргумента.

Без сомнения, это была производная Гато.
И я воспользовался символом $\partial$,
чтобы отличать эту производную.
Но я не был удовлетворён этим определением,
и начиная с 2010 я стал рассматривать линейное отображение
$D$\Hyph алгебры $A$ как представление алгебры $A\otimes A$
в алгебре $A$. А старое обозначение осталось.

Из определения
\RefDefinition{linear map from A1 to A2, algebra}
следует, что определение
\RefDefinition{differentiable map, algebra}
производной отображения в банаховую алгебру
не отличается от стандартного определения производной
отображения в банаховый модуль.
Поэтому я решил, начиная с этой статьи,
пользоваться стандартным обозначением производной.
\fi

%\section{Общие замечания}


\ePrints{1601.03259}%
\ifx\Semafor\ValueOn%
\begin{flushright}
Январь, 2017
\end{flushright}
\fi%


==> Preliminary.Omega.Russian.tex <==
%auto-ignore
\input{Preliminary.Omega.Eq}

\ePrints{4975-6381,1601.03259,1610.309618526,CACAA.06}
\ifx\Semafor\ValueOn
\def\Preliminary{on}
\ShowEq{SetupRefMeasure}
\Chapter{Интеграл Лебега в абелевой \texorpdfstring{$\Omega$}{Omega}-группе}
\fi

\ePrints{5148-4632,MVector,5410-9916,4975-6381,1601.03259,1610.309618526,CACAA.06}
\ifx\Semafor\ValueOn
\Section{\texorpdfstring{$\Omega$}{Omega}-группа}

\begin{definition}
\labelDefinition{additive map}
Пусть в $\Omega$\Hyph алгебре
$A$ определена операция сложения.
Отображение
\ShowEq{f:A->B}fAA
$\Omega_1$\Hyph алгебры $A$
называется
\AddIndex{аддитивным отображением}{additive map},
если
\ShowEq{f(a+b)=}
\qed
\end{definition}

\ShowDefinition{polyadditive map}

\ShowDefinition{Omega group}

\ShowTheorem{operation is distributive over addition}
\begin{proof}
Теорема является следствием определений
\RefDefinition{polyadditive map},
\RefDefinition{Omega group}.
\end{proof}

\ShowEq{contents: norm on Omega group}

\ePrints{5410-9916,4975-6381,1601.03259}
\ifx\Semafor\ValueOff
\ShowDefinition{multiplicative Omega group}
\fi

\ifx\texFuture\Defined
\begin{definition}
\labelDefinition{multiplicative map}
{\it
Пусть $A$, $B$ -
мультипликативные $\Omega$\Hyph группы.
Отображение
\ShowEq{f:A->B}fAB
называется
\AddIndex{мультипликативным}{multiplicative map},
если
\DrawEq{f(ab)=f(a)f(b)}{}
}
\qed
\end{definition}
\fi

\ePrints{5148-4632,MVector}
\ifx\Semafor\ValueOn
\ShowDefinition{Abelian multiplicative Omega group}

\ShowDefinition{Omega ring}

\ShowTheorem{product in Omega ring is distributive over addition}
\ShowProof{product in Omega ring is distributive over addition}

\ShowDefinition{matrix over Omega ring}

\ShowEq{convention: Einstein summation}

\ShowDefinition{matrix operations}

\ShowEq{remark: pronunciation of product}

\ShowTheorem{rcstar transpose}
\ProofTheorem{\RefRepresentation}{rcstar transpose}

\ShowDefinition{biring}

\ShowTheorem{duality principle for biring}

\ShowTheorem{duality principle for biring of matrices}

\ShowEq{remark: reducible biring}
\fi
\fi

\ePrints{aaa}
\ifx\Semafor\ValueOn
\begin{definition}
\labelDefinition{orbit of left-side representation}
{\it
Пусть отображение
\ShowEq{f:A->*B}g{A_1}{A_2}
является левосторонним представлением
мультипликативной $\Omega$\Hyph группы $A_1$
в $\Omega_2$\Hyph алгебре $A_2$.
Для любого
\EqParm{a in A}{=z,n=2}
мы определим
\AddIndex{орбиту представления}{orbit of representation}
мультипликативной $\Omega$\Hyph группы $A_1$ как множество
\ShowEq{orbit of representation}
}
\qed
\end{definition}
\fi

\ePrints{5148-4632,MVector}
\ifx\Semafor\ValueOn
\Section{Представление мультипликативной \texorpdfstring{$\Omega$}{Omega}-Group}

Мы предполагаем, что преобразования представления
\ShowEq{f:A->*B}g{A_1}{A_2}
мультипликативной $\Omega$\Hyph группы $A_1$
в $\Omega_2$\Hyph алгебре $A_2$
могут действовать на $A_2$\Hyph числа либо слева, либо справа.
Мы должны рассматривать эндоморфизм $\Omega_2$\Hyph алгебры $A_2$ как оператор.
При этом должны быть выполнены следующие условия.

\ShowDefinition{representation of group}

\ShowTheorem{left right shift}
\ProofTheorem{\RefRepresentation}{left right shift}

\EqParm{remark: notation for effective representation}{=left}

\EqParm{remark: notation for effective representation}{=right}

\ShowTheorem{duality principle, algebra representation}
\fi

\ePrints{Mpolym,5148-4632}
\ifx\Semafor\ValueOn

\Section{Тензорное произведение представлений}

\ShowDefinition{reduced polymorphism of representations}

\ShowDefinition{tensor product of representations}

\ShowTheorem{tensor product of representations}
\ProofTheorem{\RefRepresentation}{tensor product of representations}

\ShowTheorem{representation, tensor product}
\ProofTheorem{\RefRepresentation}{representation, tensor product}

\ShowTheorem{tensor product and polymorphism}
\ProofTheorem{\RefRepresentation}{tensor product and polymorphism}

\ShowTheorem{B times->B otimes}
\ProofTheorem{\RefRepresentation}{B times->B otimes}
\fi

\ePrints{4975-6381,1601.03259,1610.309618526,CACAA.06}
\ifx\Semafor\ValueOn

\Section{Алгебра множеств}

\ShowEq{contents: Algebra of Sets}

\Section{Интеграл Лебега}

\ShowEq{contents: Lebesgue Integral}
\fi


==> Preliminary.Russian.tex <==
%auto-ignore
\def\Preliminary{on}
\input{Preliminary.Eq}

\Chapter{Предварительные определения}

\ifx\PrintBook\undefined
В этом разделе
\else
В этой главе
\fi
собраны определения и теоремы,
которые необходимы для понимания текста предлагаемой
\ifx\PrintBook\undefined
статьи.
\else
книги.
\fi
Поэтому читатель может обращаться к утвердениям из
\ifx\PrintBook\undefined
этого раздела
\else
этой главы
\fi
по мере чтения основного текста
\ifx\PrintBook\undefined
статьи.
\else
книги.
\fi

\ePrints{4975-6381,1506.00061,MQuater,5148-4632,MRepro,BRepro}%,MVector
\Items{1601.03259,5410-9916}
\ifx\Semafor\ValueOn
\Section{Универсальная алгебра}

\ePrints{5410-9916}
\ifx\Semafor\ValueOff
\begin{theorem}
\labelTheorem{maps and kernel equivalence}
Пусть $N$ - отношение эквивалентности
на множестве $A$.
Рассмотрим категорию $\mathcal A$ объектами которой являются
отображения\,\footnote{
Утверждение леммы аналогично утверждению 
на с. \citeBib{Serge Lang}-94.}
\ShowEq{maps category}
Мы определим морфизм $f_1\rightarrow f_2$
как отображение $h:S_1\rightarrow S_2$,
для которого коммутативна диаграмма
\ShowEq{maps category, diagram}
Отображение
\ShowEq{maps category, universal}
является универсально отталкивающим в категории $\mathcal A$.\,\footnote{Определение
универсального объекта смотри в определении
на с. \citeBib{Serge Lang}-47.}
\end{theorem}
\begin{proof}
Рассмотрим диаграмму
\ShowEq{maps category, universal, diagram}
\ShowEq{maps category, universal, ker}
Из утверждения
\EqRef{maps category, universal, ker}
и равенства
\ShowEq{maps category 1}
следует
\ShowEq{maps category 2}
Следовательно, мы можем однозначно определить отображение $h$
с помощью равенства
\ShowEq{maps category, h}
\end{proof}
\fi

\begin{definition}
\labelDefinition{Cartesian power}
{\it
Для любых множеств\,\footnote{
Я следую определению из примера (iV),
\citeBib{Cohn: Universal Algebra}, страницы 17, 18.
}
$A$, $B$,
\AddIndex{декартова степень}{Cartesian power}
\ShowEq{Cartesian power}
- это множество отображений
\ShowEq{f:A->B}fAB
}
\qed
\end{definition}

\begin{definition}
\labelDefinition{operation on set}
{\it
Пусть дано множество $A$ и целое число $n\ge 0$. Отображение\,\footnote{
\ePrints{MVector,5148-4632,MRepro,BRepro}
\ifx\Semafor\ValueOn
Определения
\RefDefinition{operation on set},
\RefDefinition{set is closed with respect to operation}
опираются
\else
Определение
\RefDefinition{operation on set}
опирается
\fi
на определение в примере (vi),
страница \citeBib{Cohn: Universal Algebra}\Hyph 26.
}
\ShowEq{o:An->A}
называется
\AddIndex{$n$\Hyph арной операцией на множестве}{n-ary operation on set}
$A$ или просто
\AddIndex{операцией на множестве}{operation on set}
$A$.
Для любых
\EqParm{b1n in B}{B=A}
мы пользуемся любой из форм записи
\ShowEq{a1no=oa1n}
для обозначения образа отображения $\omega$.
}
\qed
\end{definition}

\begin{remark}
\labelRemark{o in AAn}
Согласно определениям
\RefDefinition{Cartesian power},
\RefDefinition{operation on set},
$n$\Hyph арная операция
\ShowEq{o in AAn}
\qed
\end{remark}

\begin{definition}
{\it
\AddIndex{Область операторов}{operator domain}
- это множество операторов\,\footnote{
Я следую определению 1,
страница \citeBib{Cohn: Universal Algebra}\Hyph 62.
}
\ShowEq{operator domain}
вместе с отображением
\ShowEq{a:O->N}
Если
\ShowEq{o in O},
то $a(\omega)$ называется
\AddIndex{арностью}{arity}
оператора $\omega$. Если
\ShowEq{a(o)=n}
то оператор $\omega$ называется $n$\Hyph арным.
\ShowEq{set of n-ary operators}
Мы пользуемся обозначением
\ShowEq{set of n-ary operators =}
для множества $n$\Hyph арных операторов.
}
\qed
\end{definition}

\begin{definition}
\labelDefinition{Omega-algebra}
{\it
Пусть $A$ - множество, а $\Omega$ - область операторов.\,\footnote{
Я следую определению 2,
страница \citeBib{Cohn: Universal Algebra}\Hyph 62.
}
Семейство отображений
\ShowEq{O(n)->AAn}
называется структурой $\Omega$\Hyph алгебры на $A$.
Множество $A$ со структурой $\Omega$\Hyph алгебры называется
\AddIndex{$\Omega$\Hyph алгеброй}{Omega-algebra}
\ShowEq{Omega-algebra}
или
\AddIndex{универсальной алгеброй}{universal algebra}.
Множество $A$ называется
\AddIndex{носителем $\Omega$\Hyph алгебры}{carrier of Omega-algebra}.
}
\qed
\end{definition}

Область операторов $\Omega$ описывает множество $\Omega$\Hyph алгебр.
Элемент множества $\Omega$ называется оператором,
так как операция предполагает некоторое множество.
Согласно замечанию
\ref{remark: o in AAn}
и определению
\RefDefinition{Omega-algebra},
каждому оператору
\EqParm{omega n ari}{=z}
сопоставляется $n$\Hyph арная операция $\omega$ на $A$.

\ePrints{MVector,5148-4632,MRepro,BRepro}
\ifx\Semafor\ValueOn

\begin{theorem}
\labelTheorem{Cartesian power is universal algebra}
Пусть множество $B$ является $\Omega$\Hyph алгеброй.
Тогда множество $B^A$ отображений
\ShowEq{f:A->B}fAB
также является $\Omega$\Hyph алгеброй.
\end{theorem}
\begin{proof}
Пусть
\EqParm{omega n ari}{=.}
Для отображений
\ShowEq{f1n in B**A}
мы определим операцию $\omega$ равенством
\DrawEq{f1n omega=}{}
\end{proof}
\fi

\ePrints{MVector,5148-4632,MRepro,BRepro}
\ifx\Semafor\ValueOn
\begin{definition}
\labelDefinition{set is closed with respect to operation}
{\it
Пусть
\ShowEq{B subset A}.
Если для любых
\EqParm{b1n in B}{B=B}
\ShowEq{b1no in B}
то мы говорим, что $B$
\AddIndex{замкнуто относительно}{set is closed with respect to operation}
$\omega$ или что $B$
\AddIndex{допускает операцию}{set admits operation}
$\omega$.
}
\qed
\end{definition}

\begin{definition}
$\Omega$\Hyph алгебра $B_{\Omega}$ является
\AddIndex{подалгеброй}{subalgebra of Omega-algebra}
$\Omega$\Hyph алгебры $A_{\Omega}$,
если верны следующие утверждения\,\footnote{
Я следую определению на
странице \citeBib{Cohn: Universal Algebra}\Hyph 62.
}
\StartLabelItem
\begin{enumerate}
\item
\ShowEq{B subset A}.
\item
Если оператор
\ShowEq{o in O}
определяет операции $\omega_A$ на $A$ и $\omega_B$ на $B$, то
\ShowEq{oAB=oB}
\end{enumerate}
\qed
\end{definition}
\fi

\begin{definition}
\labelDefinition{homomorphism}
{\it
Пусть $A$, $B$ - $\Omega$\Hyph алгебры и
\EqParm{omega n ari}{=.}
Отображение\,\footnote{
Я следую определению на
странице \citeBib{Cohn: Universal Algebra}\Hyph 63.
}
\ShowEq{f:A->B}fAB
\AddIndex{согласовано с операцией}{map is compatible with operation}
$\omega$, если, для любых
\EqParm{b1n in B}{B=A}
\ShowEq{afo=aof}
Отображение $f$ называется
\AddIndex{гомоморфизмом}{homomorphism}
$\Omega$\Hyph алгебры $A$ в $\Omega$\Hyph алгебру $B$,
если $f$ согласовано с каждым
\ShowEq{o in O}.
\ePrints{MRepro,BRepro}%
\ifx\Semafor\ValueOn%
Мы обозначим
\ShowEq{set of homomorphisms}
множество гомоморфизмов
$\Omega$\Hyph алгебры $A$ в $\Omega$\Hyph алгебру $B$.
\fi
}
\qed
\end{definition}

\ePrints{MRepro,BRepro}
\ifx\Semafor\ValueOn
\begin{theorem}
\labelTheorem{Hom empty A B=B**A}
Если область операторов пуста,
то гомоморфизм
$\Omega$\Hyph алгебры $A$ в $\Omega$\Hyph алгебру $B$
- это отображение
\ShowEq{f:A->B}fAB
Следовательно,
\ShowEq{Hom empty A B=B**A}
\end{theorem}
\begin{proof}
Теорема является следствием определений
\RefDefinition{Cartesian power},
\RefDefinition{homomorphism}.
\end{proof}
\fi

\ePrints{MVector,5148-4632,MRepro,BRepro}
\ifx\Semafor\ValueOn
\begin{definition}
\labelDefinition{isomorphism}
{\it
Гомоморфизм $f$ назывется\,\footnote{
Я следую определению на
странице \citeBib{Cohn: Universal Algebra}\Hyph 63.
}
\AddIndex{изоморфизмом}{isomorphism}
между $A$ и $B$, если соответствие $f^{-1}$ является гомоморфизмом.
Если существует изоморфизм между $A$ и $B$, то говорят,
что $A$ и $B$ изоморфны, и пишут
\ShowEq{isomorphic}
Инъективный гомоморфизм называется
\AddIndex{мономорфизмом}{monomorphism}.
Суръективный гомоморфизм называется
\AddIndex{эпиморфизмом}{epimorphism}.
}
\qed
\end{definition}
\fi

\begin{definition}
\labelDefinition{endomorphism}
{\it
Гомоморфизм, источником и целью которого является одна и таже алгебра, называется
\AddIndex{эндоморфизмом}{endomorphism}.
%\ePrints{MRepro,BRepro}%
%\ifx\Semafor\ValueOn%
Мы обозначим
\ShowEq{set of endomorphisms}
множество эндоморфизмов
$\Omega$\Hyph алгебры $A$.
%\fi
\ePrints{4975-6381,1506.00061,MQuater,1601.03259,MVector,5148-4632}%
\ifx\Semafor\ValueOff%
Эндоморфизм, который является изоморфизмом, называется
\AddIndex{автоморфизмом}{automorphism}.
\fi
}
\qed
\end{definition}

\ePrints{MRepro,BRepro}
\ifx\Semafor\ValueOn

\begin{theorem}
\labelTheorem{End A=Hom AA}
\ShowEq{End A=Hom AA}
\end{theorem}
\begin{proof}
Теорема является следствием определений
\RefDefinition{homomorphism},
\RefDefinition{endomorphism}.
\end{proof}

\begin{theorem}
\labelTheorem{End empty A=A**A}
Если область операторов пуста,
то эндоморфизм множества $A$
- это отображение
\ShowEq{t:A->A}
Следовательно,
\ShowEq{End empty A=A**A}
\end{theorem}
\begin{proof}
Теорема является следствием теорем
\RefTheorem{Hom empty A B=B**A},
\RefTheorem{End A=Hom AA}.
\end{proof}
\fi

\ePrints{4975-6381,1506.00061,MQuater,1601.03259,MVector,5148-4632,5410-9916}%
\ifx\Semafor\ValueOff%
\begin{definition}
{\it
Если существует мономорфизм $\Omega$\Hyph алгебры $A$
в $\Omega$\Hyph алгебру $B$, то говорят, что
\AddIndex{$A$ может быть вложена в $B$}{can be embeded}.
}
\qed
\end{definition}

\begin{definition}
{\it
Если существует эпиморфизм из $A$ в $B$, то $B$ называется
\AddIndex{гомоморфным образом}{homomorphic image} алгебры $A$.
}
\qed
\end{definition}
\fi
\fi

\ePrints{MVector,5148-4632,5410-9916}
\ifx\Semafor\ValueOn
\begin{convention}
Элемент
$\Omega$\Hyph алгебры
$A$ называется
\AddIndex{$A$\Hyph числом}{A number}.
Например, комплексное число также называется
$C$\Hyph числом, а кватернион называется $H$\Hyph числом.
\qed
\end{convention}
\fi

\ePrints{MRepro,BRepro}
\ifx\Semafor\ValueOn

\Section{Декартово произведение универсальных алгебр}

\ShowDefinition{product in category}

\begin{example}
Пусть \(\mathcal S\) - категория множеств.\,\footnote{
Смотри также пример в
\citeBib{Serge Lang},
страница 45.
}
Согласно определению
\RefDefinition{product in category},
декартово произведение
\ShowEq{Cartesian product of sets}
семейства множеств
\ShowEq{Ai iI}
и семейство проекций на \(i\)\Hyph й множитель
\ShowEq{projection on i factor}
являются произведением в категории \(\mathcal S\).
\qed
\end{example}

\begin{theorem}
\labelTheorem{product exists in category of Omega algebras}
Произведение существует в категории \(\mathcal A\) \(\Omega\)\Hyph алгебр.
Пусть \(\Omega\)\Hyph алгебра \(A\)
и семейство морфизмов
\ShowEq{p:A->Ai i in I}
является произведением в категории \(\mathcal A\).
%семейства \(\Omega\)\Hyph алгебр
Тогда
\StartLabelItem
\begin{enumerate}
\item
Множество \(A\) является декартовым произведением
семейства множеств
\ShowEq{Ai iI}
\item
Гомоморфизм \(\Omega\)\Hyph алгебры
\ShowEq{projection on i factor}
является проекцией на \(i\)\Hyph й множитель.
\item
Любое \(A\)\Hyph число $a$ может быть однозначно представлено
в виде кортежа
\ShowEq{tuple represent A number}
\(A_i\)\Hyph чисел.
\labelItem{tuple represent A number}
\item
Пусть
\ShowEq{omega in Omega}{}{}
- n\Hyph арная операция.
Тогда операция $\omega$ определена покомпонентно
\ShowEq{operation is defined componentwise}
где
\ShowEq{a=ai 1n}.
\labelItem{operation is defined componentwise}
\end{enumerate}
\end{theorem}
\begin{proof}
Пусть
\ShowEq{Cartesian product of sets}
декартово произведение
семейства множеств
\ShowEq{Ai iI}
и, для каждого \iI, отображение 
\ShowEq{projection on i factor}
является проекцией на \(i\)\Hyph й множитель.
Рассмотрим диаграмму морфизмов в категории множеств $\mathcal S$
\ShowEq{operation is defined componentwise, diagram}
где отображение $g_i$ определено равенством
\ShowEq{gi()=}
Согласно определению
\RefDefinition{product in category},
отображение $\omega$ определено однозначно из множества диаграмм
\EqRef{operation is defined componentwise, diagram}
\ShowEq{omega(ai)=(omega ai)}
Равенство
\EqRef{operation is defined componentwise}
является следствием равенства
\EqRef{omega(ai)=(omega ai)}.
\ifx\texFuture\Defined

\begin{lemma}
\labelLemma{tuple represent A number}
{\it
Пусть \(\Omega\)\Hyph алгебра \(A\)
и семейство морфизмов
\ShowEq{projection on i factor}
является произведением в категории \(\mathcal A\).
Любое \(A\)\Hyph число $a$ может быть однозначно представлено
в виде кортежа
\ShowEq{tuple represent A number}
\(A_i\)\Hyph чисел.
}
\end{lemma}

{\sc Доказательство.}
Пусть
\ShowEq{a ne b}
- такие \(A\)\Hyph числа, что для любого \iI
\ShowEq{p(a)=p(b)}
Если предположить, что неравные \(A\)\Hyph числа
имеют равные разложения в виде кортежа,
то мы можем определить отношение эквивалентности,
фактор по которому скорее кандидат на произведение.
\hfill\(\odot\)

Из равенства
\ShowEq{pj(a)=aj}
следует, что отображение \(p_j\) является проекцией.
\fi
\end{proof}

\begin{definition}
Если \(\Omega\)\Hyph алгебра \(A\)
и семейство морфизмов
\ShowEq{p:A->Ai i in I}
является произведением в категории \(\mathcal A\),
то \(\Omega\)\Hyph алгебра \(A\) называется
\AddIndex{прямым}{direct product of Omega algebras}
или
\AddIndex{декартовым произведением \(\Omega\)\Hyph алгебр}
{Cartesian product of Omega algebras}
\ShowEq{Ai iI}.
\qed
\end{definition}

\begin{theorem}
\labelTheorem{map from product into product}
Пусть множество \(A\) является
декартовым произведением множеств
\ShowEq{Ai iI}
и множество \(B\) является
декартовым произведением множеств
\ShowEq{Bi iI}.
Для каждого \iI, пусть
\ShowEq{f:A->B i}
является отображением множества $A_i$ в множество $B_i$.
Для каждого \iI, рассмотрим коммутативную диаграмму
\ShowEq{homomorphism of Cartesian product of Omega algebras diagram}
где отображения
\ShowEq{pi p'i}
являются проекцией на \(i\)\Hyph й множитель.
Множество коммутативных диаграмм
\EqRef{homomorphism of Cartesian product of Omega algebras diagram}
однозначно определяет отображение
\ShowEq{f:A->B}fAB
\DrawEq{f:A->B=}{}
\end{theorem}
\begin{proof}
Для каждого \iI, рассмотрим коммутативную диаграмму
\ShowEq{homomorphism of Cartesian product of Omega algebras}
Пусть \(a\in A\).
Согласно утверждению
\RefItem{tuple represent A number},
\(A\)\Hyph число \(a\)
может быть представлено в виде кортежа \(A_i\)\Hyph чисел
\ShowEq{a=p(a)i}
Пусть
\ShowEq{b=f(a)}
Согласно утверждению
\RefItem{tuple represent A number},
\(B\)\Hyph число \(b\)
может быть представлено в виде кортежа \(B_i\)\Hyph чисел
\ShowEq{b=p(b)i}
Из коммутативности диаграммы $(1)$
и из равенств
\EqRef{b=f(a)},
\EqRef{b=p(b)i}
следует, что
\ShowEq{b=g(a)i}
Из коммутативности диаграммы $(2)$
и из равенства
\EqRef{a=p(a)i}
следует, что
\ShowEq{b=f(a)i}
\end{proof}

\begin{theorem}
\labelTheorem{homomorphism of Cartesian product of Omega algebras}
Пусть \(\Omega\)\Hyph алгебра \(A\) является
декартовым произведением \(\Omega\)\Hyph алгебр
\ShowEq{Ai iI}
и \(\Omega\)\Hyph алгебра \(B\) является
декартовым произведением \(\Omega\)\Hyph алгебр
\ShowEq{Bi iI}.
Для каждого \iI,
пусть отображение
\ShowEq{f:A->B i}
является гомоморфизмом \(\Omega\)\Hyph алгебры.
Тогда отображение
\ShowEq{f:A->B}fAB
определённое равенством
\DrawEq{f:A->B=}{homomorphism}
является гомоморфизмом \(\Omega\)\Hyph алгебры.
\end{theorem}
\begin{proof}
Пусть
\ShowEq{omega in Omega}{}{}
- n\Hyph арная операция.
Пусть
\ShowEq{a=ai 1n} и
\ShowEq{b=bi 1n}.
Из равенств
\EqRef{operation is defined componentwise},
\eqRef{f:A->B=}{homomorphism}
следует, что
\ShowEq{f:A->B omega}
\end{proof}

\begin{definition}
{\it
Эквивалентность на $\Omega$\Hyph алгебре $A$,
которая является подалгеброй $\Omega$\Hyph алгебры $A^2$,
называется
\AddIndex{конгруенцией}{}\,\footnote{
Я следую определению на
странице \citeBib{Cohn: Universal Algebra}\Hyph 71.
}
на $A$.
}
\qed
\end{definition}

\begin{theorem}[первая теорема об изоморфизмах]
\labelTheorem{first isomorphism theorem}
Пусть
\ShowEq{f:A->B}fAB
гомоморфизм $\Omega$\Hyph алгебр с ядром $s$.
Тогда отображение $f$ имеет разложение
\ShowEq{decomposition of map f}
\StartLabelItem
\begin{enumerate}
\item
\AddIndex{Ядро гомоморфизма}{kernel of homomorphism}
\ShowEq{kernel of homomorphism}
является конгруэнцией на $\Omega$\Hyph алгебре $A$.
\labelItem{kernel of homomorphism}
\item
Множество
\ShowEq{A/ker f}
является $\Omega$\Hyph алгеброй.
\labelItem{A/ker f is Omega-algebra}
\item
Отображение
\ShowEq{p:A->/ker}
является эпиморфизмом и называется
\AddIndex{естественным гомоморфизмом}{natural homomorphism}.
\labelItem{natural homomorphism}
\item
Отображение
\ShowEq{q:A/ker->f(A)}
является изоморфизмом.
\labelItem{q:A/ker->f(A) isomorphism}
\item
Отображение
\ShowEq{r:f(A)->B}
является мономорфизмом.
\labelItem{r:f(A)->B monomorphism}
\end{enumerate}
\end{theorem}
\begin{proof}
Утверждение
\RefItem{kernel of homomorphism}
является следствием предложения II.3.4
(\citeBib{Cohn: Universal Algebra}, страница 72).
Утверждения
\RefItem{A/ker f is Omega-algebra},
\RefItem{natural homomorphism}
являются следствием теоремы II.3.5
(\citeBib{Cohn: Universal Algebra}, страница 72)
и последующего определения.
Утверждения
\RefItem{q:A/ker->f(A) isomorphism},
\RefItem{r:f(A)->B monomorphism}
являются следствием теоремы II.3.7
(\citeBib{Cohn: Universal Algebra}, страница 74).
\end{proof}
\fi

\ePrints{MRepro,BRepro}
\ifx\Semafor\ValueOn
\Section{Полугруппа}

Обычно операция
\ShowEq{omega 2 ari}
называется произведением
\ShowEq{abo=ab}
либо суммой
\ShowEq{abo=a+b}

\begin{definition}
{\it
Пусть $A$ является $\Omega$\Hyph алгеброй и
\ShowEq{omega 2 ari.}
$A$\Hyph число $e$ называется
\AddIndex{нейтральным элементом операции}{neutral element of operation}
$\omega$, если для любого $A$\Hyph числа $a$ верны равенства
\ShowEq{left neutral element}
\ShowEq{right neutral element}
}
\qed
\end{definition}

\begin{definition}
{\it
Пусть $A$ является $\Omega$\Hyph алгеброй.
Операция
\ShowEq{omega 2 ari}
называется
\AddIndex{ассоциативной}{associative operation},
если верно равенство
\ShowEq{associative operation}
}
\qed
\end{definition}

\begin{definition}
{\it
Пусть $A$ является $\Omega$\Hyph алгеброй.
Операция
\ShowEq{omega 2 ari}
называется
\AddIndex{коммутативной}{commutative operation},
если верно равенство
\ShowEq{commutative operation}
}
\qed
\end{definition}

\begin{definition}
\labelDefinition{semigroup}
{\it
Пусть
\ShowEq{Omega=omega}
Если операция
\ShowEq{omega 2 ari}
ассоциативна, то $\Omega$\Hyph алгебра называется
\AddIndex{полугруппой}{semigroup}.
Если операция в полугруппе коммутативна,
то полугруппа называется
\AddIndex{абелевой полугруппой}{Abelian semigroup}.
}
\qed
\end{definition}
\fi

\ePrints{4975-6381,1506.00061,MQuater,1601.03259,5148-4632}
\Items{MVector,5410-9916}
\ifx\Semafor\ValueOn
\Section{Представление универсальной алгебры}
\labelSection{Representation of Universal Algebra}

\begin{definition}
\labelDefinition{representation of algebra} 
Пусть множество $A_2$ является $\Omega_2$\Hyph алгеброй.
Пусть
на множестве преобразований
\ShowEq{End O2}{A_2}{}
определена структура $\Omega_1$\Hyph алгебры.
Гомоморфизм
\ShowEq{representation of algebra}
$\Omega_1$\Hyph алгебры $A_1$ в
$\Omega_1$\Hyph алгебру
\ShowEq{End O2}{A_2}{}
называется
\AddIndex{представлением $\Omega_1$\Hyph алгебры}
{representation of algebra}
или
\AddIndex{$A_1$\Hyph представлением}{A representation of algebra}
в $\Omega_2$\Hyph алгебре $A_2$.
\qed
\end{definition}

Мы будем также пользоваться записью
\ShowEq{f:A->*B}f{A_1}{A_2}
для обозначения представления $\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $A_2$.

\begin{definition}
\labelDefinition{effective representation of algebra}
Мы будем называть представление
\ShowEq{f:A->*B}f{A_1}{A_2}
$\Omega_1$\Hyph алгебры $A_1$
\AddIndex{эффективным}{effective representation},\,\footnote{
Аналогичное определение эффективного представления группы смотри в
\citeBib{Postnikov: Differential Geometry}, страница 16,
\citeBib{Basic Concepts of Differential Geometry}, страница 111,
\citeBib{Cohn: Algebra 1}, страница 51
(Кон называет такое представление точным).
}
если отображение
\ShowEq{representation of algebra}
является изоморфизмом $\Omega_1$\Hyph алгебры $A_1$ в
\ShowEq{End O2}{A_2}.
\qed
\end{definition}

\ePrints{MVector,5148-4632}
\ifx\Semafor\ValueOn

\begin{theorem}
\labelTheorem{representation is effective}
Представление
\ShowEq{f:A->*B}g{A_1}{A_2}
эффективно тогда и только, когда из утверждения
\ShowEq{a1 ne b1}
следует существование
\EqParm{a in A}{n=2,=z}
такого, что\,\footnote{
Для группы теорема
\RefTheorem{representation is effective}
имеет следующий вид.
{\it
Представление
\ShowEq{f:A->*B}g{A_1}{A_2}
эффективно тогда и только тогда, когда для любого $A_1$\Hyph числа $a\ne e$
существует
\EqParm{a in A}{n=2,=z}
такое, что
\ShowEq{fam ne m}
}
}
\ShowEq{fam ne fbm}
\end{theorem}
\ProofTheorem{\RefRepresentation}{representation is effective}

\begin{theorem}
\labelTheorem{effective representation of the ring}
Пусть кольцо $D$ имеет единицу $e$.
Представление
\ShowEq{f:A->*B}fDA
кольца $D$
в абелевой группе $A$
\AddIndex{эффективно}{effective representation of ring}
тогда и только тогда, когда
из равенства $f(a)=0$ следует $a=0$.
\end{theorem}
\begin{proof}
Сумма преобразований $f$ и $g$ абелевой группы определяется согласно
правилу
\ShowEq{(f+g)(a)=}
Поэтому, рассматривая представление кольца $D$ в
абелевой группе $A$, мы полагаем
\ShowEq{sum of transformations of Abelian group, 1}

Если $a$, $b\in R$
порождают одно и то же преобразование, то
\ShowEq{representation of ring, 1}
для любого $m\in A$.
Из равенства
\EqRef{representation of ring, 1}
следует, что $a-b$ порождает нулевое преобразование
\ShowEq{representation of ring, 2}
Элемент $e+a-b$ порождает тождественное преобразование.
Следовательно, представление $f$ эффективно тогда и только тогда,
когда $a=b$.
\end{proof}
\fi

\ePrints{1506.00061}
\ifx\Semafor\ValueOn
\begin{definition}
\labelDefinition{free representation of algebra}
{\it
Мы будем называть представление
\ShowEq{f:A->*B}g{A_1}{A_2}
$\Omega_1$\Hyph алгебры $A_1$
\AddIndex{свободным}{free representation},\,\footnote{
Аналогичное определение свободного представления группы смотри в
\citeBib{Postnikov: Differential Geometry}, страница 16.
}
если из утверждения
\ShowEq{faa=fba}
для любого
\EqParm{a in A}{n=2,=z}
следует, что $a=b$.
}
\qed
\end{definition}

\begin{theorem}
\labelTheorem{Free representation is effective}
Свободное представление эффективно.
\end{theorem}
\ProofTheorem{\RefRepresentation}{Free representation is effective}

\begin{remark}
Представление группы вращений в аффинном пространстве эффективно,
но не свободно, так как начало координат
является неподвижной точкой любого преобразования.
\qed
\end{remark}

\begin{definition}
\labelDefinition{transitive representation of algebra}
Мы будем называть представление
\ShowEq{f:A->*B}g{A_1}{A_2}
$\Omega_1$\Hyph алгебры
\AddIndex{транзитивным}{transitive representation of algebra},\,\footnote{
Аналогичное определение транзитивного представления группы смотри в
\citeBib{Basic Concepts of Differential Geometry}, страница 110,
\citeBib{Cohn: Algebra 1}, страница 51.
}
если для любых
\EqParm{ab in A}{A=2,=z}
существует такое $g$, что
\[a=f(g)(b)\]
Мы будем называть представление $\Omega_1$\Hyph алгебры
\AddIndex{однотранзитивным}{single transitive representation of algebra},
если оно транзитивно и свободно.
\qed
\end{definition}

\begin{theorem}%однотранзитивное
\labelTheorem{Representation is single transitive iff}
Представление однотранзитивно тогда и только тогда, когда для любых $a, b \in A_2$
существует одно и только одно $g\in A_1$ такое, что $a=f(g)(b)$
\end{theorem}
\begin{proof}
Следствие определений \RefDefinition{free representation of algebra}
и \RefDefinition{transitive representation of algebra}.
\end{proof}

\begin{theorem}
\labelTheorem{single transitive representation generates algebra}
Пусть
\ShowEq{f:A->*B}g{A_1}{A_2}
однотранзитивное представление
$\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $A_2$.
Существует структура $\Omega_1$\Hyph алгебры на множестве $A_2$.
\end{theorem}
\ProofTheorem{\RefRepresentation}{single transitive representation generates algebra}
\fi

\begin{definition}
\labelDefinition{morphism of representations of universal algebra}
Пусть
\ShowEq{f:A->*B}f{A_1}{A_2}
представление $\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $A_2$ и 
\ShowEq{f:A->*B}g{B_1}{B_2}
представление $\Omega_1$\Hyph алгебры $B_1$
в $\Omega_2$\Hyph алгебре $B_2$.
Для
\EqParm{i=1,2}{=c}
пусть отображение
\ShowEq{ri:A->B}
является гомоморфизмом $\Omega_i$\Hyph алгебры.
Матрица отображений
\ShowEq{map r,R}{r_1}{r_2}{}
таких, что
\ShowEq{morphism of representations of universal algebra, definition, 2}
называется
\AddIndex{морфизмом представлений из $f$ в $g$}
{morphism of representations from f into g}.
Мы также будем говорить, что определён
\AddIndex{морфизм представлений $\Omega_1$\Hyph алгебры
в $\Omega_2$\Hyph алгебре}
{morphism of representations of Omega1 algebra in Omega2 algebra}.
\qed
\end{definition}

\begin{remark}
Мы можем рассматривать пару отображений $r_1$, $r_2$ как отображение
\ShowEq{F:A1+A2->B1+B2}
такое, что
\ShowEq{F:A1+A2->B1+B2 1}
Поэтому в дальнейшем матрицу отображений
\ShowEq{map r,R}{r_1}{r_2}{}
мы будем также называть отображением.
\qed
\end{remark}

\ePrints{5148-4632,MVector}
\ifx\Semafor\ValueOn

\begin{remark}
Рассмотрим морфизм представлений
\ShowEq{r12:A->B}rAB
Мы можем обозначать элементы множества $B$, пользуясь буквой по образцу $b\in B$.
Но если мы хотим показать, что $b$ является образом элемента
\EqParm{a in A1}{=c}
мы будем пользоваться обозначением $\RedText{r_1(a)}$.
Таким образом, равенство
\ShowEq{r1(a)=r1(a)}
означает, что $\RedText{r_1(a)}$ (в левой части равенства)
является образом
\EqParm{a in A1}{=z}
(в правой части равенства).
Пользуясь подобными соображениями, мы будем обозначать
элемент множества $B_2$ в виде $\BlueText{r_2(m)}$.
Мы будем следовать этому соглашению, изучая соотношения
между гомоморфизмами $\Omega_1$\Hyph алгебр
и отображениями между множествами,
где определены соответствующие представления.
\qed
\end{remark}

\begin{theorem}
\labelTheorem{Tuple of maps is morphism of representations iff}
Пусть
\ShowEq{f:A->*B}g{A_1}{A_2}
представление $\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $A_2$ и 
\ShowEq{f:A->*B}g{B_1}{B_2}
представление $\Omega_1$\Hyph алгебры $B_1$
в $\Omega_2$\Hyph алгебре $B_2$.
Отображение
\ShowEq{r12:A->B}rAB
является морфизмом представлений тогда и только тогда, когда
\DrawEq{morphism of representations of universal algebra, 2m}{definition}
\end{theorem}
\ProofTheorem{\RefRepresentation}{Tuple of maps is morphism of representations iff}

\begin{remark}
\labelRemark{morphism of representations of universal algebra}
Мы можем интерпретировать
\eqRef{morphism of representations of universal algebra, 2m}{definition}
двумя способами
\begin{itemize}
\item Пусть преобразование $\BlueText{f(a)}$ отображает $m\in A_2$
в $\BlueText{f(a)}(m)$.
Тогда преобразование
\ShowEq{g(r1(a))}
отображает
\ShowEq{r2(m)in B2}
в
\ShowEq{r2(f(a,m))}
\item Мы можем представить морфизм представлений из $f$ в $g$,
пользуясь диаграммой
\DrawEq{morphism of representations of universal algebra, 2m 1}{definition}
Из \EqRef{morphism of representations of universal algebra, definition, 2}
следует, что диаграмма $(1)$ коммутативна.
\end{itemize}
Мы будем также пользоваться диаграммой
\ShowEq{morphism of representations of universal algebra, definition, 2m 2}
вместо диаграммы
\eqRef{morphism of representations of universal algebra, 2m 1}{definition}.
\qed
\end{remark}
\fi

\begin{definition}
Если представления $f$ и $g$ совпадают, то морфизм представлений
\ShowEq{map r,R}{r_1}{r_2}{}
называется
\AddIndex{морфизмом представления $f$}{morphism of representation f}.
\qed
\end{definition}

\ePrints{aa}%MVector,5148-4632}
\ifx\Semafor\ValueOn

\begin{theorem}
\labelTheorem{unique morphism of representations of universal algebra}
Если представление
\ShowEq{f:A->*B}g{A_1}{A_2}
$\Omega_1$\Hyph алгебры $A_1$ однотранзитивно
и представление
\ShowEq{f:A->*B}g{B_1}{B_2}
$\Omega_1$\Hyph алгебры $B_1$ однотранзитивно,
то для заданного гомоморфизма $\Omega_1$\Hyph алгебры
\ShowEq{f:A->B}{r_1}{A_1}{B_1}
гомоморфизм $\Omega_2$\Hyph алгебры
\ShowEq{f:A->B}{r_2}{A_2}{B_2}
такой, что
\ShowEq{map r,R}{r_1}{r_2}{}
является морфизмом
представлений из $f$ в $g$,
определён однозначно
с точностью до выбора образа $n=H(m)\in N$
заданного элемента $m\in A_2$.
\end{theorem}
\ProofTheorem{\RefRepresentation}{unique morphism of representations of universal algebra}

\begin{definition}
\labelDefinition{transformation coordinated with equivalence}
Пусть на множестве $A_2$ определена эквивалентность $S$.
Преобразование $f$ называется
\AddIndex{согласованным с эквивалентностью}{transformation coordinated with equivalence} $S$,
если из условия
\ShowEq{m1 m2 modS}
следует
$f(m_1)\equiv f(m_2)(\mathrm{mod}\ S)$.
\qed
\end{definition}

\begin{theorem}
\labelTheorem{transformation correlated with equivalence}
Пусть на множестве $A_2$ определена эквивалентность $S$.
Пусть на множестве
\ShowEq{End O2}{A_2}{}
определена $\Omega_1$\Hyph алгебра.
Если любое преобразование $f\in{}^* A_2$ согласованно с эквивалентностью $S$,
то мы можем определить структуру $\Omega_1$\Hyph алгебры
на множестве ${}^*(A_2/S)$.
\end{theorem}
\ProofTheorem{\RefRepresentation}{transformation correlated with equivalence}

\begin{theorem}
\labelTheorem{decompositions of morphism of representations}
Пусть
\ShowEq{f:A->*B}g{A_1}{A_2}
представление $\Omega_1$\Hyph алгебры $A_1$,
\ShowEq{f:A->*B}g{B_1}{B_2}
представление $\Omega_1$\Hyph алгебры $B_1$.
Пусть
\ShowEq{r12:A->B}tAB
морфизм представлений из $f$ в $g$.
Тогда для отображений $t_1$, $t_2$ существуют разложения,
которые можно описать диаграммой
\ShowEq{decompositions of morphism of representations, diagram}
\StartLabelItem
\begin{enumerate}
\item
Ядро гомоморфизма
\ShowEq{kernel of homomorphism i}
является конгруэнцией на $\Omega_i$\Hyph алгебре $A_i$,
\EqParm{i=1,2}{=.}
\labelItem{kernel of homomorphism i}
\item
Существует разложение гомоморфизма $t_i$,
\EqParm{i=1,2}{=c}
\ShowEq{morphism of representations of algebra, homomorphism, 1}
\labelItem{exists decomposition of homomorphism}
\item
Отображения
\ShowEq{morphism of representations of algebra, p1=}
\ShowEq{morphism of representations of algebra, p2=}
являются естественными гомоморфизмами.
\labelItem{p12 are natural homomorphisms}
\item
Отображения
\ShowEq{morphism of representations of algebra, q1=}
\ShowEq{morphism of representations of algebra, q2=}
являются изоморфизмами.
\labelItem{q12 are isomorphisms}
\item
Отображения
\ShowEq{morphism of representations of algebra, r1=}
\ShowEq{morphism of representations of algebra, r2=}
являются мономорфизмами.
\labelItem{r12 are monomorphisms}
\item $F$ - представление $\Omega_1$\Hyph алгебры $A_1/s_1$ в $A_2/s_2$
\item $G$ - представление $\Omega_1$\Hyph алгебры $t_1A_1$ в $t_2A_2$
\item Отображение
\ShowEq{map r,R}{p_1}{p_2}{}
является морфизмом представлений $f$ и $F$
\labelItem{(p12) is morphism of representations}
\item Отображение
\ShowEq{map r,R}{q_1}{q_2}{}
является изоморфизмом представлений $F$ и $G$
\labelItem{(q12) is isomorphism of representations}
\item Отображение
\ShowEq{map r,R}{r_1}{r_2}{}
является морфизмом представлений $G$ и $g$
\labelItem{(r12) is morphism of representations}
\item Существует разложение морфизма представлений
\labelItem{exists decompositions of morphism of representations}
\ShowEq{decompositions of morphism of representations}
\end{enumerate} 
\end{theorem}
\ProofTheorem{\RefRepresentation}{decompositions of morphism of representations}
\fi

\ShowDefinition{reduced morphism of representations}
\fi

\ePrints{5148-4632,MVector,5410-9916}
\ifx\Semafor\ValueOn
\Input{Preliminary.Omega}
\fi

\ePrints{MVector,5148-4632}
\ifx\Semafor\ValueOn

\Section{Базис представления универсальной алгебры}

\begin{definition}
Пусть
\ShowEq{f:A->*B}g{A_1}{A_2}
представление $\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $A_2$.
Множество
\ShowEq{B2 subset A2}
называется
\AddIndex{стабильным множеством представления}
{stable set of representation} $f$,
если
\ShowEq{fam in B2}
для любых
\EqParm{a in A1}{=c}
$m\in B_2$.
\qed
\end{definition}

\begin{theorem}%
\labelTheorem{subrepresentation of representation}
Пусть
\ShowEq{f:A->*B}g{A_1}{A_2}
представление $\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $A_2$.
Пусть множество
\ShowEq{B2 subset A2}
является подалгеброй $\Omega_2$\Hyph алгебры $A_2$
и стабильным множеством представления $f$.
Тогда существует представление
\ShowEq{representation of algebra A in algebra B}
такое, что
\ShowEq{fB2(a)=}
Представление $f_{B_2}$ называется
\AddIndex{подпредставлением представления}
{subrepresentation of representation} $f$.
\end{theorem}
\ProofTheorem{\RefRepresentation}{subrepresentation of representation}

\begin{theorem}%
\labelTheorem{lattice of subrepresentations}
Множество\,\footnote{Это определение
аналогично определению структуры подалгебр
(\citeBib{Cohn: Universal Algebra}, стр. 93, 94)}
\ShowEq{lattice of subrepresentations}
всех подпредставлений представления $f$ порождает
систему замыканий на $\Omega_2$\Hyph алгебре $A_2$
и, следовательно, является полной структурой.
\end{theorem}
\ProofTheorem{\RefRepresentation}{lattice of subrepresentations}

Обозначим соответствующий оператор замыкания через
\ShowEq{closure operator, representation}
Таким образом,
\ShowEq{subrepresentation generated by set}
является пересечением всех подалгебр
$\Omega_2$\Hyph алгебры $A_2$,
содержащих $X$ и стабильных относительно представления $f$.

\begin{definition}
\labelDefinition{generating set of representation}
\ShowEq{show closure operator, representation}
называется
\AddIndex{подпредставлением, порождённым множеством $X$}
{subrepresentation generated by set},
а $X$ -
\AddIndex{множеством образующих подпредставления $J_f(X)$}
{generating set of subrepresentation}.
В частности,
\AddIndex{множеством образующих представления $f$}
{generating set of representation}
будет такое подмножество $X\subset A_2$, что
\ShowEq{generating set of representation}
\qed
\end{definition}

\ShowTheorem{structure of subrepresentations}
\ProofTheorem{\RefRepresentation}{structure of subrepresentations}

\begin{definition}
\labelDefinition{basis of representation}
Если множество $X\subset A_2$ является множеством образующих
представления $f$, то любое множество $Y$, $X\subset Y\subset A_2$
также является множеством образующих представления $f$.
Если существует минимальное множество $X$, порождающее
представление $f$, то такое множество $X$ называется
\AddIndex{базисом представления}{basis of representation} $f$.
\qed
\end{definition}

\begin{theorem}
\labelTheorem{X is basis of representation}
Множество образующих $X$ представления $f$ является базисом
тогда и только тогда, когда для любого $m\in X$
множество $X\setminus\{m\}$ не является
множеством образующих представления $f$.
\end{theorem}
\ProofTheorem{\RefRepresentation}{X is basis of representation}

\begin{remark}
\labelRemark{X is basis of representation}
Доказательство теоремы
\RefTheorem{X is basis of representation}
даёт нам эффективный метод построения базиса представления $f$.
Выбрав произвольное множество образующих, мы шаг за шагом
исключаем те элементы множества, которые имеют координаты
относительно остальных элементов множества.
Если множество образующих представления бесконечно,
то рассмотренная операция может не иметь последнего шага.
Если представление имеет конечное множество образующих,
то за конечное число шагов мы можем построить базис этого представления.

Как отметил Кон в 
\citeBib{Cohn: Universal Algebra}, cтр. 96, 97,
представление может иметь неэквивалентные базисы.
Например, циклическая группа шестого порядка имеет
базисы $\{a\}$ и $\{a^2,a^3\}$, которые нельзя отобразить
один в другой эндоморфизмом представления.
\qed
\end{remark}

\begin{theorem}
\labelTheorem{automorphism uniquely defined by image of basis}
Пусть $X$ - базис представления $f$.
Пусть
\ShowEq{R1 X->}
произвольное отображение множества $X$.
%Рассмотрим отображение $\Omega_2$\Hyph слов
%\ShowEq{map of words of representation, W}
%удовлетворяющее условиям
%\RefItem{map of words of representation, m in X},
%\RefItem{map of words of representation, omega},
%\RefItem{map of words of representation, am},
%и такое, что
%\ShowEq{map of words of representation, W in X}
Существует единственный эндоморфизм представления $f$\,\footnote{Это утверждение
похоже на теорему \citeBib{Serge Lang}-1, с. 104.}
\ShowEq{R:A2->A2}
определённый правилом
\ShowEq{Rm=R1m}
%\ShowEq{endomorphism based on map of words of representation}
\end{theorem}
\ProofTheorem{\RefRepresentation}{automorphism uniquely defined by image of basis}
\fi

\ePrints{MVector,5148-4632}
\ifx\Semafor\ValueOn

\Section{Башня представлений универсальных алгебр}

\begin{definition}
\labelDefinition{tower of representations}
Рассмотрим множество $\Omega_k$\Hyph алгебр $A_k$, \Kn1.
Положим $A=(A_1,...,A_n)$.
Положим $f=(f_{1,2},...,f_{n-1,n})$.
Множество представлений $f_{k,k+1}$, \Kn1, 
$\Omega_k$\Hyph алгебры $A_k$ в
$\Omega_{k+1}$\Hyph алгебре $A_{k+1}$
называется
\AddIndex{башней $(A,f)$ представлений $\Omega$\Hyph алгебр}
{tower of representations of algebras}.
\qed
\end{definition}

Мы можем проиллюстрировать определение \RefDefinition{tower of representations}
с помощью диаграммы
\ShowEq{Tower of Representations}
$f_{i,i+1}$ - представление $\Omega_i$\Hyph алгебры $A_i$
в $\Omega_{i+1}$\Hyph алгебре $A_{i+1}$.
$f_{i+1,i+2}$ - представление $\Omega_{i+1}$\Hyph алгебры $A_{i+1}$
в $\Omega_{i+2}$\Hyph алгебре $A_{i+2}$.

\begin{definition}
Рассмотрим множество $\Omega_k$\Hyph алгебр $A_k$, $B_k$, \Kn1.
Множество отображений
$(h_1,...,h_n)$ называется \AddIndex{морфизмом из башни представлений
$(A,f)$ в башню представлений $(B,g)$}
{morphism from tower of representations into tower of representations},
если для каждого $k$, $k=1$, ..., $n-1$,
пара отображений $(h_k,h_{k+1})$ является
морфизмом представлений из $f_{k,k+1}$ в $g_{k,k+1}$.
\qed
\end{definition}

Для любого $k$, $k=1$, ..., $n-1$, мы имеем диаграмму
\ShowEq{morphism of tower of representations of F algebra, level k, diagram}
Равенства
\ShowEq{morphism of tower of representations, level k}
\ShowEq{morphism of tower of representations, levels k k+1}
выражают коммутативность диаграммы (1).

\begin{definition}
{\it
Пусть
\ShowEq{Aij}
- множество
\ShowEq{Omegaij}%
алгебр.
}
\qed
\end{definition}
\fi

\ePrints{MVector,5148-4632,4975-6381,1601.03259,1610.309618526,CACAA.06}
\ifx\Semafor\ValueOn
\Section{Перестановка}

\begin{definition}
{\it
Инъективное отображение конечного множества в себя называется
\AddIndex{перестановкой}{permutation}.\,\footnote{
Смотри определение и свойства перестановки в
\citeBib{Kurosh: High Algebra}, страницы 28 - 32,
\citeBib{Cohn: Algebra 1}, страницы 58, 59.
}
}
\qed
\end{definition}

Обычно перестановку $\sigma$ мы записываем в виде матрицы
\ShowEq{permutation as matrix}
Запись
\EqRef{permutation as matrix}
перестановки эквивалентна утверждению
\ShowEq{a->sigma a}
Поэтому порядок столбцов в записи
\EqRef{permutation as matrix}
несущественен.

Если на множестве
\EqParm{set a1n}{=z}
задан некоторый порядок
(например, мы предполагаем, что $a_i$ предшествует $a_j$,
если $i<j$),
то мы можем подразумевать, что элементы первой строки
записаны согласно предполагаемому порядку
и будем отождествлять перестановку со второй строкой
\ShowEq{permutation as matrix 2}

\begin{definition}
{\it
Отображение
\ShowEq{sigma->+-}
определённое равенством
\def\permutation{перестановка }
\def\even{чётная}
\def\odd{не\even}
\ShowEq{parity of permutation}
называется
\AddIndex{чётностью перестановки}{parity of permutation}.
}
\qed
\end{definition}
\fi

\ePrints{4975-6381,1506.00061,MQuater,1601.03259,MVector,1610.309618526,CACAA.06}
\ifx\Semafor\ValueOn
\Section{Модуль над кольцом}

\ShowEq{=module}

\ShowDefinition{module over commutative ring}

\ShowTheorem{definition of module over commutative ring}
\ProofTheorem{\RefLinearMap}{definition of module over commutative ring}

\ShowDefinition{coordinates of vector 2016}

\ePrints{MVector}
\ifx\Semafor\ValueOn

\ShowEq{=left}
\ShowTheorem{set of vectors generated by set of vectors}
\ProofTheorem{\RefLinearMap}{set of vectors generated by set of vectors}

\ShowDefinition{vector linearly dependent on vectors}

\ShowEq{remark: scalars and vectors as matrix}

\ShowDefinition{linearly independent vectors}

\ShowTheorem{basis of module}
\ProofTheorem{\RefLinearMap}{basis of module}

\ShowDefinition{free module over ring}

\ShowTheorem{division algebra, basis}
\ProofTheorem{\RefLinearMap}{division algebra, basis}
\fi

\ShowDefinition{linear map from A1 to A2, commutative module}

\ShowTheorem{linear map from A1 to A2, commutative module}
\ProofTheorem{\RefLinearMap}{linear map from A1 to A2, commutative module}
\fi

\ePrints{4975-6381,MQuater,1601.03259}
\ifx\Semafor\ValueOn
\begin{theorem}
\labelTheorem{linear map, 0, D algebra}
Пусть отображение
\ShowEq{f:A->B}f{A_1}{A_2}
является линейным отображением $D$\Hyph модуля $A_1$ в $D$\Hyph модуль $A_2$.
Тогда
\ShowEq{linear map, 0, D algebra}
\end{theorem}
\ProofTheorem{\RefLinearMap}{linear map, 0, D algebra}
\fi

\ePrints{1601.03259,4975-6381}
\ifx\Semafor\ValueOn
%\ePrints{4975-6381}
%\ifx\Semafor\ValueOff
%\ShowTheorem{sum of linear maps, D module}
%\ProofTheorem{\RefLinearMap}{sum of linear maps, D module}
%\fi

\begin{definition}
\labelDefinition{polylinear map of modules}
Пусть $D$ - коммутативное кольцо.
Пусть $A_1$, ..., $A_n$, $S$ - $D$\Hyph модули.
Мы будем называть отображение
\ShowEq{polylinear map of algebras}
\AddIndex{полилинейным отображением}{polylinear map} модулей
$A_1$, ..., $A_n$
в модуль $S$,
если
\ShowEq{polylinear map of algebras, 1}
\qed
\end{definition}

\ShowTheorem{sum of polylinear maps, module}
\ProofTheorem{\RefLinearMap}{sum of polylinear maps, module}

\ShowEq{corollary: sum of linear maps, D module}
\fi

\ePrints{1601.03259,4975-6381}
\ifx\Semafor\ValueOn
\begin{definition}
\labelDefinition{tensor product of algebras}
Пусть $A_1$, ..., $A_n$ -
свободные модули над  коммутативным кольцом $D$.\,\footnote{
Я определяю
тензорное произведение $D$\Hyph модулей
по аналогии с определением в \citeBib{Serge Lang}, с. 456 - 458.
}
Рассмотрим категорию $\mathcal A_1$ объектами которой являются
полилинейные отображения
\ShowEq{polylinear maps category}
где $S_1$, $S_2$ - модули над кольцом $D$.
Мы определим морфизм
\ShowEq{f->g}
как линейное отображение
\ShowEq{f->g 1}
такое, что коммутативна диаграмма
\ShowEq{polylinear maps category, diagram}
Универсальный объект
\ShowEq{tensor product of algebras}
категории $\mathcal A_1$ называется
\AddIndex{тензорным произведением}{tensor product}
модулей $A_1$, ..., $A_n$.
\qed
\end{definition}

\begin{theorem}
\labelTheorem{Tensor product is distributive over sum}
Пусть $D$ - коммутативное кольцо.
Пусть $A_1$, ..., $A_n$ - $D$\Hyph модули.
Тензорное произведение дистрибутивно относительно сложения
\ShowEq{tensors 1, tensor product}
Представление кольца $D$
в тензорном произведении определено равенством
\ShowEq{tensors 2, tensor product}
\end{theorem}
\ProofTheorem{\RefLinearMap}{Tensor product is distributive over sum}

\begin{theorem}
\labelTheorem{tensor product and polylinear map}
Пусть $A_1$, ..., $A_n$ -
модули над коммутативным кольцом $D$.
Тензорное произведение
\ShowEq{f:xA->oxA}
существует и единственно.
Мы пользуемся обозначением
\ShowEq{fxa=oxa}
для образа отображения $f$.
Пусть
\ShowEq{map g, algebra, tensor product}
полилинейное отображение в $D$\Hyph модуль $V$.
Существует линейное отображение
\ShowEq{map h, algebra, tensor product}
такое, что диаграмма
\ShowEq{map gh, algebra, tensor product}
коммутативна.
Отображение \(h\) определено равенством
\ShowEq{g=h, algebra, tensor product}
\end{theorem}
\begin{proof}
Смотри доказательство теорем
\ShowEq{ref tensor product and polylinear map}
\end{proof}

\begin{convention}
\labelConvention{isomorphic representations S1=S2}
Алгебры $S_1$, $S_2$ могут быть различными множествами.
Однако они неразличимы для нас, если мы рассматриваем их
как изоморфные представления.
В этом случае мы будем писать $S_1=S_2$.
\qed
\end{convention}

\begin{theorem}
\labelTheorem{tensor product is associative}
\ShowEq{A1xA2xA3}
\end{theorem}
\ProofTheorem{\RefLinearMap}{tensor product is associative}

\begin{definition}
\labelDefinition{tensor power of algebra}
Тензорное произведение
\ShowEq{tensor power of algebra}
называется
\AddIndex{тензорной степенью}{tensor power} модуля $A_1$.
\qed
\end{definition}

\begin{theorem}
\labelTheorem{V times->V otimes}
Отображение
\ShowEq{V times->V otimes}
является полилинейным отображением.
\end{theorem}
\ProofTheorem{\RefLinearMap}{V times->V otimes}
\fi

\ePrints{4975-6381,MQuater,1601.03259}
\ifx\Semafor\ValueOn
\begin{theorem}
\labelTheorem{standard component of tensor, algebra}
Пусть
\ShowEq{tensor product of algebras, basis i}
- базис модуля $A_i$ над кольцом $D$.
Произвольный тензор $a\in\Tensor A$ можно представить в виде
\ShowEq{standard component of tensor}
\ShowEq{tensor canonical representation, algebra}
Мы будем
называть выражение
$\ShowSymbol{standard component of tensor}{}$
\AddIndex{стандартной компонентой тензора}{standard component of tensor}.
\end{theorem}
\ProofTheorem{\RefLinearMap}{standard component of tensor, algebra}
\fi

\ePrints{4975-6381,1506.00061,MQuater,1601.03259,MVector,1610.309618526,CACAA.06}
\ifx\Semafor\ValueOn
\Section{Алгебра над коммутативным кольцом}

\ShowDefinition{algebra over ring}

\ePrints{1601.03259}
\ifx\Semafor\ValueOff
\begin{theorem}
\labelTheorem{multiplication in algebra is distributive over addition}
Произведение в алгебре $A_1$ дистрибутивно по отношению к сложению.
\end{theorem}
\ProofTheorem{\RefLinearMap}{multiplication in algebra is distributive over addition}
\fi

\ePrints{1506.00061,MQuater,4975-6381,1601.03259,1610.309618526,CACAA.06}
\ifx\Semafor\ValueOn
\begin{convention}
Элемент
$D$\Hyph алгебры
$A$ называется
\AddIndex{$A$\Hyph числом}{A number}.
Например, комплексное число также называется
$C$\Hyph числом, а кватернион называется $H$\Hyph числом.
\qed
\end{convention}
\fi

Произведение в алгебре может быть ни коммутативным,
ни ассоциативным. Следующие определения основаны на
определениях, данных в \citeBib{Richard D. Schafer}, страница 13.

\ShowDefinition{commutator of algebra}

\ShowDefinition{associator of algebra}

\ShowDefinition{nucleus of algebra}

\ShowDefinition{center of algebra}

\ShowEq{convention: we use separate color for index of element}

\ShowEq{convention: unit of algebra in basis}

\ePrints{1610.309618526,CACAA.06,1601.03259}
\ifx\Semafor\ValueOff
\begin{theorem}
\labelTheorem{product in algebra}
Пусть $\Basis e$ - базис свободной алгебры $A_1$ над кольцом $D$.
Пусть
\ShowEq{a b in basis of algebra}
Произведение $a$, $b$ можно получить согласно правилу
\ShowEq{product in algebra}
где
\ShowEq{structural constants of algebra}
- \AddIndex{структурные константы}{structural constants}
алгебры $A_1$ над кольцом $D$.
Произведение базисных векторов в алгебре $A_1$ определено согласно правилу
\ShowEq{product of basis vectors, algebra}
\end{theorem}
\ProofTheorem{\RefLinearMap}{product in algebra}
\fi

\ePrints{4975-6381,1601.03259,1610.309618526,CACAA.06}
\ifx\Semafor\ValueOn
\begin{theorem}
\labelTheorem{Free Algebra over Ring}
\ShowEq{text: Free Algebra over Ring}
\end{theorem}
\begin{proof}
\TheoremFollows
\RefTheorem[\RefLinearMap]{Free Algebra over Ring}
и следствия
\RefCorollary[\RefLinearMap]{Free Algebra over Ring}.
\end{proof}
\fi

\ShowEq{=DD}

\ShowDefinition{linear map from A1 to A2, algebra}

\ePrints{1601.03259,4975-6381}
\ifx\Semafor\ValueOn

\begin{theorem}
\labelTheorem{module L(A;A) is algebra}
Пусть $A$ - алгебра над коммутативным кольцом $D$.
$D$\Hyph модуль $\mathcal L(D;A;A)$, оснащённый произведением
\ShowEq{module L(A;A) is algebra}
\ShowEq{product of linear map, algebra 1}
является алгеброй над $D$.
\end{theorem}
\ProofTheorem{\RefLinearMap}{module L(A;A) is algebra}
\fi

\begin{definition}
\labelDefinition{polylinear map of algebras}
Пусть $A_1$, ..., $A_n$, $S$ - $D$\Hyph алгебры.
Мы будем называть
полилинейное отображение
\ShowEq{polylinear map of algebras}
$D$\Hyph модулей
$A_1$, ..., $A_n$
в $D$\Hyph модуль $S$
\AddIndex{полилинейным отображением}{polylinear map}
$D$\Hyph алгебр
$A_1$, ..., $A_n$
в $D$\Hyph модуль $S$.
Обозначим
\ShowEq{set polylinear maps}
множество полилинейных отображений
$D$\Hyph алгебр
$A_1$, ..., $A_n$
в $D$\Hyph алгебру
$S$.
Обозначим
\ShowEq{set polylinear maps An}
множество $n$\hyph линейных отображений
$D$\Hyph алгебры $A_1$ ($A_1=...=A_n=A_1$)
в $D$\Hyph алгебру
$S$.
\qed
\end{definition}

\ShowTheorem{tensor product of D-algebras is D-algebra}
\ProofTheorem{\RefLinearMap}{tensor product of D-algebras is D-algebra}

\ShowTheorem{representation of algebra A2 in LA}
\ProofTheorem{\RefLinearMap}{representation of algebra A2 in LA}

\begin{convention}
В выражении вида
\ShowEq{Sum over repeated index}
предполагается сумма по индексу $i$.
\qed
\end{convention}

%\ShowTheorem{h generated by f, associative algebra}
%\ProofTheorem{\RefLinearMap}{h generated by f, associative algebra}

\ePrints{4975-6381,1506.00061,MQuater,1601.03259}
\ifx\Semafor\ValueOn
\ShowTheorem{standard representation of map A1 A2, associative algebra}
\ProofTheorem{\RefLinearMap}{standard representation of map A1 A2, associative algebra}

\ePrints{4975-6381}
\ifx\Semafor\ValueOff
\ShowDefinition{component of linear map}
\fi

\ShowTheorem{conjugation transformation}
\ProofTheorem{\RefLinearMap}{conjugation transformation}

\ShowTheorem{representation of composition of linear maps}
\ProofTheorem{\RefLinearMap}{representation of composition of linear maps}

\ShowTheorem{representation of composition of linear maps A->A}
\ProofTheorem{\RefLinearMap}{representation of composition of linear maps A->A}

%\ShowTheorem{linear map in L(A,A), associative algebra}
%\ProofTheorem{\RefLinearMap}{linear map in L(A,A), associative algebra}
\fi

\ePrints{1601.03259,4975-6381,1610.309618526,CACAA.06}
\ifx\Semafor\ValueOn
\ShowTheorem{coordinates of map A1 A2, algebra}
\ProofTheorem{\RefLinearMap}{coordinates of map A1 A2, algebra}

По определению
\ShowEq{Basis F=...}
Мы также рассматриваем множество
\ShowEq{F=...}
имея в виду, что возможно равенство
\ShowEq{Fi=Fj}
при условии $i\ne j$.
\fi

\ePrints{4975-6381,1506.00061}
\ifx\Semafor\ValueOn
\begin{convention}
В равенстве
\ShowEq{n linear map A LA}
также как и в других выражениях полилинейного отображения,
принято соглашение, что отображение $f_i$ имеет своим аргументом переменную $x_i$.
\qed
\end{convention}
\fi

\ePrints{1601.03259,4975-6381,1506.00061,1610.309618526,CACAA.06}
\ifx\Semafor\ValueOn

\ShowTheorem{L(An;B) is free D module}
\ProofTheorem{\RefLinearMap}{L(An;B) is free D module}

\begin{theorem}
\labelTheorem{polylinear map, algebra}
Пусть $A$ - ассоциативная $D$\Hyph алгебра.
Полилинейное отображение
\ShowEq{polylinear map, algebra}
порождённое отображениями
\ShowEq{I1n in L(A;A)},
имеет вид
\ShowEq{polylinear map, algebra, canonical morphism}
где $\sigma_s$ - перестановка множества переменных
\ShowEq{transposition of set of variables, algebra}
\end{theorem}
\ProofTheorem{\RefLinearMap}{polylinear map, algebra}

\ShowTheorem{representation of algebra An in LAnA}
\ProofTheorem{\RefLinearMap}{representation of algebra An in LAnA}

\begin{convention}
Если тензор
\EqParm{a in Aoxn+1}{=z}
имеет разложение
\ShowEq{a=oxi}
то множество перестановок
\ShowEq{si in Sn}
и тензор $a$
порождают отображение
\ShowEq{ox:An->A}
определённое равенством
\ShowEq{ox circ =}
\qed
\end{convention}
\fi
\fi

\ePrints{}
\ifx\Semafor\ValueOn
\Section{Модуль над алгеброй}

\ShowEq{=left}

\ShowDefinition{module over algebra}

\ShowTheorem{definition of A module}
\ProofTheorem{\RefLinearMap}{definition of left A module}

\ShowEq{=right}
\ShowDefinition{module over algebra}
\fi

\ePrints{1506.00061}
\ifx\Semafor\ValueOn
\Section{Алгебра с сопряжением}

Пусть $D$ - коммутативное кольцо.
Пусть $A$ - $D$\hyph алгебра с единицей $e$, $A\ne D$.

Пусть существует подалгебра $F$ алгебры $A$ такая, что
$F\ne A$, $D\subseteq F\subseteq Z(A)$, и алгебра $A$ является свободным
модулем над кольцом $F$.
Пусть $\Basis e$ - базис свободного модуля $A$ над кольцом $F$.
Мы будем полагать $e_{\gi 0}=1$.

\begin{theorem}
\labelTheorem{structural constant of algebra with unit}
Структурные константы
$D$\hyph алгебры с единицей $e$ удовлетворяют условию
\ShowEq{structural constant re algebra, 1}
\end{theorem}
\begin{proof}
\TheoremFollows
\ShowEq{ref structural constant of algebra with unit}
\end{proof}

Рассмотрим отображения
\ShowEq{Re Im A->A}
определенные равенством
\ShowEq{Re Im A->F 0}
\ShowEq{Re Im A->F 1}
Выражение
\ShowEq{Re Im A->F 2}
называется
\AddIndex{скаляром элемента}{scalar of algebra} $d$.
Выражение
\ShowEq{Re Im A->F 3}
называется
\AddIndex{вектором элемента}{vector of algebra} $d$.

Согласно
\EqRef{Re Im A->F 1}
\ShowEq{Re Im A->F 4}
Мы будем пользоваться записью
\ShowEq{scalar algebra of algebra}
для обозначения
\AddIndex{алгебры скаляров алгебры}{scalar algebra of algebra} $A$.

\begin{theorem}
\labelTheorem{Re Im A->F}
Множество
\ShowEq{vector module of algebra}
является $(\re A)$\Hyph модулем,
который мы называем
\AddIndex{модуль векторов алгебры}{vector module of algebra} $A$.
\ShowEq{A=re+im}
\end{theorem}
\begin{proof}
\TheoremFollows
\ShowEq{ref Re Im A->F}
\end{proof}

Согласно теореме \RefTheorem{Re Im A->F},
однозначно определенно представление
\ShowEq{d Re Im}

\begin{definition}
\labelDefinition{conjugation in algebra}
Отображение
\ShowEq{conjugation in algebra}
\ShowEq{conjugation in algebra, 0}
называется
\AddIndex{сопряжением в алгебре}{conjugation in algebra}
при условии, если это отображение удовлетворяет равенству
\ShowEq{conjugation in algebra, 1}
$(\re A)$\Hyph алгебра $A$,
в которой определено сопряжение, называется
\AddIndex{алгеброй с сопряжением}{algebra with conjugation}.
\qed
\end{definition}

\begin{theorem}
\labelTheorem{conjugation in algebra}
$(\re A)$\Hyph алгебра $A$ является
алгеброй с сопряжением
тогда и только тогда, когда структурные константы
$(\re A)$\Hyph алгебры $A$ удовлетворяют условию
\ShowEq{conjugation in algebra, 5}
\ShowEq{conjugation in algebra, 4}
\end{theorem}
\begin{proof}
\TheoremFollows
\ShowEq{ref conjugation in algebra}
\end{proof}
\fi

\ePrints{1601.03259,4975-6381,1506.00061}
\ifx\Semafor\ValueOn
\Section{Многочлен над ассоциативной \texorpdfstring{$D$}{D}-алгеброй}

Пусть $D$ - коммутативное кольцо и
$A$ - ассоциативная $D$\Hyph алгебра с единицей.
Пусть $\Basis F$ - базис алгебры
\ShowEq{L(A;B)}DAA.

\begin{theorem}
\labelTheorem{monomial of power k}
Пусть $p_k(x)$ -
\AddIndex{одночлен степени}{monomial of power} $k$
над $D$\Hyph алгеброй $A$.
Тогда
\StartLabelItem
\begin{enumerate}
\item
Одночлен степени $0$ имеет вид
\ShowEq{p0(x)=a0}
\item
Если $k>0$, то
\ShowEq{monomial of power k}
где $a_k\in A$ и  $F\in\Basis F$.
\end{enumerate}
\end{theorem}
\begin{proof}
\TheoremFollows
\ShowEq{ref monomial of power k}
\end{proof}

В частности, одночлен степени $1$ имеет вид
\ShowEq{p1(x)=aFxa}

\begin{definition}
\labelDefinition{Abelian group of homogeneous polynomials over algebra}
Обозначим
\ShowEq{module of homogeneous polynomials over algebra}
абелевую группу,
порождённую множеством одночленов степени $k$.
Элемент $p_k(x)$ абелевой группы $A_k[x]$ называется
\AddIndex{однородным многочленом степени}
{homogeneous polynomial of power} $k$.
\qed
\end{definition}

\begin{convention}
Пусть тензор
\EqParm{a in Aoxn+1}{=.}
Пусть
\ShowEq{F1n in F}
Если
\ShowEq{x1=xn=x}
то мы положим
\ShowEq{a xn=}
\qed
\end{convention}

\begin{convention}
Если мы имеем несколько кортежей отображений $F\in\Basis F$,
то мы будем пользоваться индексом вида $[k]$
для индексирования кортежа
\ShowEq{F[k]=...}
\qed
\end{convention}

\begin{theorem}
\labelTheorem{homogeneous polynomial a circ xk}
Однородный многочлен $p(x)$
может быть записан в виде
\ShowEq{p(x)=a circ xk}
\end{theorem}
\begin{proof}
\TheoremFollows
\ShowEq{ref map A(k+1)->pk otimes is polylinear map}
\end{proof}

\begin{definition}
\labelDefinition{Polynomial over algebra}
Обозначим
\ShowEq{algebra of polynomials over algebra}
прямую сумму\,\footnote{Смотри определение
прямой суммы модулей в
\citeBib{Serge Lang},
страница 98.
Согласно теореме 1 на той же странице, прямая сумма модулей существует.
}
$A$\Hyph модулей $A_n[x]$.
Элемент $p(x)$ $A$\Hyph модуля $A[x]$ называется
\AddIndex{многочленом}{polynomial}
над $D$\Hyph алгеброй $A$.
\qed
\end{definition}

\ePrints{4975-6381,1601.03259}
\ifx\Semafor\ValueOn
Следующее определение
\RefDefinition{otimes -}
опирается на определение
\Ref[1302.7204]{definition: otimes -}.

\ShowDefinition{otimes -}

\begin{definition}
\labelDefinition{product of homogeneous polynomials}
Произведение однородных многочленов
\ShowEq{polynomials p,r}
определено равенством\,\footnote{
Определение
\RefDefinition{product of homogeneous polynomials}
опирается на определение
\Ref[1302.7204]{definition: product of homogeneous polynomials}.
}
\ShowEq{pr=p circ r}
\qed
\end{definition}

\ePrints{}
\ifx\Semafor\ValueOn
\begin{theorem}
\labelTheorem{p(x)=a k-1 k}
Пусть
\ShowEq{p(x)=a circ xk}
одночлен степени $k>1$.
Тогда многочлен $p(x)$ может быть представлен в 
одной из следующих форм
\ShowEq{p(x)=a k-1 k 1}
\ShowEq{p(x)=a k-1 k 2}
где
\ShowEq{p(x)=a k-1 k 3}
\end{theorem}
\begin{proof}
Смотри доказательство теоремы
\RefTheorem[1302.7204]{p(x)=a k-1 k}.
\end{proof}
\fi
\fi

\ePrints{1506.00061}
\ifx\Semafor\ValueOn

\begin{definition}
\labelDefinition{divisor of polynomial}
Многочлен $p(x)$ называется
\AddIndex{делителем многочлена}{divisor of polynomial} $r(x)$,
если мы можем представить многочлен $r(x)$ в виде
\ShowEq{r=qpq(x)}
\qed
\end{definition}

\begin{theorem}
\labelTheorem{r=+q circ p}
Пусть
\ShowEq{p=p circ x}
- однородный многочлен степени $1$ и $p_1$ - невырожденный тензор.
Пусть
\ShowEq{r power k}
многочлен степени $k$.
Тогда
\ShowEq{r=+q circ p}
\end{theorem}
\begin{proof}
\TheoremFollows
\ShowEq{ref r=+q circ p}
\end{proof}

\begin{theorem}
\labelTheorem{r=+q circ p 1}
Пусть
\ShowEq{p=p+p circ x}
- многочлен степени $1$ и $p_1$ - невырожденный тензор.
Пусть
\ShowEq{r power k}
многочлен степени $k$.
Тогда
\ShowEq{r=+q circ p 1}
\end{theorem}
\begin{proof}
\TheoremFollows
\ShowEq{ref r=+q circ p 1}
\end{proof}
\fi
\fi

\ePrints{MQuater,1610.309618526,CACAA.06}
\ifx\Semafor\ValueOn
\Section{Производная отображения банаховой алгебры}

\begin{definition}
Нормированная $D$\Hyph алгебра $A_1$ называется 
\AddIndex{банаховой $D$\Hyph алгеброй}{Banach algebra}
если любая фундаментальная последовательность элементов
алгебры $A_1$ сходится, т. е.
имеет предел в алгебре $A_1$.
\qed
\end{definition}

\begin{definition}
\labelDefinition{continuous map, algebra}
Отображение
\ShowEq{f:A->B}f{A_1}{A_2}
банаховой $D_1$\Hyph алгебры $A_1$ с нормой $|x|_1$
в банаховую $D_2$\Hyph алгебру $A_2$ с нормой $|y|_2$
называется \AddIndex{непрерывным}{continuous map}, если
для любого сколь угодно малого $\epsilon>0$
существует такое $\delta>0$, что
\[
|x'-x|_1<\delta
\]
влечёт
\[
|f(x')-f(x)|_2<\epsilon
\]
\qed
\end{definition}

\ePrints{1610.309618526,CACAA.06}
\ifx\Semafor\ValueOff

\ShowTheorem{set of A->B is D module}
\begin{proof}
\TheoremFollows
ффф
\end{proof}

\else

\ShowDefinition{norm of polylinear map}

\ShowTheorem{|f(a)|<|f||a| 1n}
\ePrints{CACAA.06}
\ifx\Semafor\ValueOff
\ProofTheorem{\RefCalculus}{|f(a)|<|f||a| 1n}
\else
\ShowProof{|f(a)|<|f||a| 1n}
\fi

\ShowTheorem{|on|->0 ona1p->0}
\ePrints{CACAA.06}
\ifx\Semafor\ValueOff
\ProofTheorem{\RefCalculus}{|on|->0 ona1p->0}
\else
\ShowProof{|on|->0 ona1p->0}
\fi
\fi

\ShowDefinition{differentiable map}DAB{algebra}

\begin{definition}
\labelDefinition{differential of map}
{\it
Если, для данного $x$, приращение
\eqRef{derivative of map, def}{algebra}
отображения
\ShowEq{f:A->B}fAA
рассматривать как функцию дифференциала $dx$ переменной $x$,
то линейная часть этой функции
\ShowEq{differential of independent variable}
\ShowEq{differential of map}
\DrawEq{differential of map =}{}
называется
\AddIndex{дифференциалом отображения}{differential of map}
$f$.
}
\qed
\end{definition}

\ShowEq{remark: differential L(A,A)}

\ePrints{1610.309618526,CACAA.06}
\ifx\Semafor\ValueOff
\ShowTheorem{derivative, representation in algebra}
\begin{proof}
Смотри доказательство теоремы
\ShowEq{ref derivative, representation in algebra}
\end{proof}
\fi

\ShowTheorem{representation of derivative, algebra A->B}
\begin{proof}
\TheoremFollows
\ShowEq{ref differentiable map A->B}
\end{proof}

\ShowDefinition{coordinates of derivative, algebra A->B}

\ePrints{1610.309618526,CACAA.06}
\ifx\Semafor\ValueOn

\ShowTheorem{dfa1p/dx=df/dx a1p}
\ShowProof{dfa1p/dx=df/dx a1p}

\ShowTheorem{bilinear map and differential}

\ShowTheorem{derivative of tensor product}

%\ShowTheorem{map is continuous, derivative}
%\begin{proof}
%\TheoremFollows
%\ShowEq{ref map is continuous, derivative}
%\end{proof}
\fi

\ePrints{1610.309618526,CACAA.06}
\ifx\Semafor\ValueOn
\ShowDefinition{derivative of Second Order, algebra}

\ShowDefinition{derivative of Order n, algebra}
\fi
\fi

\ePrints{1601.03259,4975-6381,MQuater,1610.309618526,CACAA.06}
\ifx\Semafor\ValueOn

\Section{Комплексное поле}

\begin{theorem}
\labelTheorem{complex field over real field}
Рассмотрим поле комплексных чисел $C$ как двумерную алгебру над полем действительных чисел.
Положим
\ShowEq{basis of complex field}
базис алгебры $C$.
Тогда в этом базисе произведение имеет вид
\ShowEq{product of complex field}
и структурные константы имеют вид
\ShowEq{structural constants of complex field}
\end{theorem}
\ProofTheorem{1003.1544}{complex field over real field}

\begin{definition}
{\it
Поле комплексных чисел имеет следующие
\AddIndex{отображения сопряжения}{map of conjugation}
\ShowEq{Ex= C}
\ShowEq{Ix= C}
}
\qed
\end{definition}

\begin{theorem}
\labelTheorem{linear map of complex field}
Линейное отображение
\ShowEq{f:C->C y=}
поля комплексных чисел имеет вид
\ShowEq{linear map of complex field, structure}
где $C$\Hyph числа
\ShowEq{a01}
определены равенством
\ShowEq{a01=}
\end{theorem}
\ProofTheorem{1003.1544}{additive map of complex field, structure}

\begin{corollary}
\labelCorollary{basis of L(R;C;C)}
{\it
$C\otimes C$\Hyph модуль
\ShowEq{L(R;C;C)}
является $C$\Hyph векторным пространством
и имеет базис
\EqParm{e=(E,I)}{=.}
}
\qed
\end{corollary}

\begin{theorem}
\labelTheorem{CE is algebra isomorphic to complex field}
Множество
\ShowEq{CE set}
является $R$\Hyph алгеброй, изоморфной полю комплексных чисел.
\end{theorem}
\begin{proof}
Теорема является следствием равенств
\ShowEq{aE+bE=(a+b)E}
\ShowEq{aE o bE=(ab)E}
опирающихся на теорему
\RefTheorem{linear map of complex field}.
\end{proof}

\begin{theorem}
\labelTheorem{L(CCC)=CE}
\ShowEq{L(CCC)=CE}
\end{theorem}
\begin{proof}
Теорема является следствием равенства
\EqRef{linear map of complex field, structure, 2}
и коммутативности произведения комплексных чисел.
\end{proof}

\begin{theorem}[Уравнения Коши\Hyph Римана]
\labelTheorem{Cauchy Riemann equations linear}
Матрица линейного отображения $f\in CE$
\ShowEq{yi=xj fji}
удовлетворяет соотношению
\ShowEq{complex field over real field}
\end{theorem}
\ProofTheorem{1003.1544}{complex field over real field}

\begin{theorem}
\labelTheorem{matrix of linear map f in CI}
Матрица линейного отображения $f\in CI$
\ShowEq{yi=xj fji}
удовлетворяет соотношению\,\footnote{
Смотри также раздел
\Ref[1003.1544]{section: System of Additive Equations in Complex Field}.
}
\ShowEq{matrix of linear map f in CI}
\end{theorem}
\begin{proof}
Утверждение следует из равенств
\ShowEq{congugate map complex field, 3}
\end{proof}

\ePrints{4975-6381,MQuater}
\ifx\Semafor\ValueOn

\begin{theorem}
Множество
\ShowEq{CI set}
не является $R$\Hyph алгеброй.
\end{theorem}
\begin{proof}
Теорема является следствием равенства
\ShowEq{aI o bI=...E}
опирающегося на теорему
\RefTheorem{linear map of complex field}.
\end{proof}

\ePrints{MQuater}
\ifx\Semafor\ValueOn

\begin{definition}
\labelDefinition{differentiable map of complex field}
{\it
Отображение
\ShowEq{f:C->C}
поля комплексных чисел
называется
\AddIndex{дифференцируемым}{differentiable map}
на множестве $U\subset C$,
если в каждой точке $x\in U$
изменение отображения
$f$ может быть представлено в виде
\ShowEq{derivative of map}
\DrawEq{derivative of map, def}{}
где
\ShowEq{df:A->B}CC
- линейное отображение $C$\Hyph векторного пространства $C$ и
\ShowEq{o:A->B}oCC
- такое непрерывное отображение, что
\ShowEq{lim |o|/|a|}CC
Линейное отображение
$\displaystyle\ShowSymbol{derivative of map}{}$
называется
\AddIndex{производной отображения}{derivative of map}
$f$.
}
\qed
\end{definition}

\begin{theorem}
\labelTheorem{dx fx in CE}
Если отображение
\ShowEq{f:C->C}
поля комплексных чисел
дифференцируемо,
то
\ShowEq{dx fx in CE}
\end{theorem}
\begin{proof}
\TheoremFollows
\RefTheorem{CE is algebra isomorphic to complex field}
и определения
\RefDefinition{differentiable map of complex field}.
\end{proof}

\begin{definition}
{\it
Дифференцируемое отображение поля комплексных чисел называется
\AddIndex{голоморфным}{holomorphic map}.
}
\qed
\end{definition}

\begin{theorem}[Уравнения Коши\Hyph Римана]
Если матрица
\ShowEq{Jacobian of map of complex variable}
является матрицей Якоби функции комплексного переменного
\ShowEq{map of complex variable}
над полем действительных чисел,
то
\ShowEq{Cauchy Riemann equations, complex field, 1}
\end{theorem}
\begin{proof}
Теорема является следствием теорем
\RefTheorem{Cauchy Riemann equations linear},
\RefTheorem{dx fx in CE}.
\end{proof}

\begin{theorem}[Уравнение Коши\Hyph Римана]
\labelTheorem{Cauchy Riemann equations, complex field}
Производная отображения комплексного переменного удовлетворяет
уравнению Коши\Hyph Римана
\DrawEq{Cauchy Riemann equation, complex field}{theorem}
\end{theorem}
\begin{proof}
Равенство
\ShowEq{Cauchy Riemann equations, complex field, 2, 1}
следует из равенств
\EqRef{Cauchy Riemann equations, complex field, 1}.
Равенство
\eqRef{Cauchy Riemann equation, complex field}{theorem}
является следствием равенства
\EqRef{Cauchy Riemann equations, complex field, 2, 1}.
\end{proof}

\begin{definition}
\labelDefinition{projection maps, complex field}
{\it
Следующие отображения проекции определены в поле комплексных чисел
\ShowEq{projection maps, complex field}
}
\qed
\end{definition}

\begin{theorem}
\labelTheorem{Expansion of projection maps relative E,I}
Разложение отображений проекции относительно базиса
\EqParm{e=(E,I)}{=z}
имеет вид
\ShowEq{projection mappings 1, complex field}
\end{theorem}
\begin{proof}
Теорема является следствием теоремы
\RefTheorem{linear map of complex field}
и определения
\RefDefinition{projection maps, complex field}.
\end{proof}

\begin{theorem}
\labelTheorem{df=...dx= CE}
Производная отображения
\ShowEq{f:C->C}
поля комплексных чисел
имеет вид\,\footnote{
Теоремы в этом разделе
аналогичны теоремам в \citeBib{Shabat: Complex Analysis}, с. 31 - 33.}
\ShowEq{df=...dx= CE}
\end{theorem}
\begin{proof}
Согласно теореме
\RefTheorem{Expansion of projection maps relative E,I},
\ShowEq{dx01=}
является следствием равенства
\ShowEq{dx=dx0+dx1}
Равенство
\ShowEq{df=...dx}
является следствием равенств
\EqRef{dx01=}
и
\ShowEq{df=df/dx0+df/dx1}
Равенство
\DrawEq{df=...dx=}{theorem}
является следствием равенства
\EqRef{df=...dx}
и определения
\RefDefinition{differential of map}.
Равенство
\EqRef{df=...dx= CE}
является следствием равенства
\eqRef{df=...dx=}{theorem}
и теоремы
\RefTheorem{Cauchy Riemann equations, complex field}.
\end{proof}
\fi
\fi
\fi

\ePrints{1506.00061,MQuater,1610.309618526,CACAA.06}
\ifx\Semafor\ValueOn

\Section{Алгебра кватернионов}

\begin{definition}
Пусть $R$ - поле действительных чисел.
Расширение
\ShowEq{quaternion algebra}
поля $R$ называется
\AddIndex{алгеброй кватернионов}{quaternion algebra},
если произведение в алгебре $H$ определено согласно правилам
\ShowEq{product of quaternions}
\qed
\end{definition}

Элементы алгебры $H$ имеют вид
\ShowEq{quaternion algebra, element}
Кватернион
\ShowEq{conjugate to the quaternion}
называется сопряжённым кватерниону $x$.
Мы определим
\AddIndex{норму кватерниона}{norm of quaternion}
$x$ равенством
\ShowEq{norm of quaternion}
Из равенства
\EqRef{norm of quaternion}
следует, что обратный элемент имеет вид
\ShowEq{inverce quaternion}

\ePrints{MQuater}
\ifx\Semafor\ValueOn
\begin{theorem}
\labelTheorem{quaternion conjugation}
Сопряжение кватернионов удовлетворяет равенству
\ShowEq{quaternion conjugation}
\end{theorem}
\begin{proof}
Смотри доказательство теоремы
\ShowEq{ref quaternion conjugation}
\end{proof}
\fi

\ePrints{1610.309618526,CACAA.06}
\ifx\Semafor\ValueOff
\begin{theorem}
\labelTheorem{Quaternion over real field}
Положим
\DrawEq{basis of quaternion}{algebra}
базис алгебры кватернионов $H$.
Тогда в базисе \eqRef{basis of quaternion}{algebra} структурные константы имеют вид
\ShowEq{structural constants, quaternion}
\end{theorem}
\begin{proof}
Смотри доказательство теоремы
\ShowEq{ref Quaternion over real field}
\end{proof}
\fi

\ePrints{MQuater}
\ifx\Semafor\ValueOn
\begin{theorem}
\labelTheorem{Quaternion over real field, matrix}
Рассмотрим алгебру кватернионов $H$ с базисом
\eqRef{basis of quaternion}{algebra}.
Стандартные компоненты линейного отображения над полем $R$
и координаты этого отображения над полем $R$
удовлетворяют соотношениям
\EqParm{quaternion, 3, B->A}{f=f}
\EqParm{quaternion, 3, A->B}{f=f}
где
\ShowEq{quaternion, 3, 1}
\end{theorem}
\begin{proof}
Смотри доказательство теоремы
\ShowEq{ref Quaternion over real field, matrix}
\end{proof}
\fi

\ePrints{MQuater,1610.309618526,CACAA.06}
\ifx\Semafor\ValueOn

\begin{definition}
\labelDefinition{quaternion maps of conjugation}
{\it
Алгебра кватернионов имеет следующие
\AddIndex{отображения сопряжения}{map of conjugation}
\ShowEq{Ex= H}
\ShowEq{Ix= H}
\ShowEq{Jx= H}
\ShowEq{Kx= H}
}
\qed
\end{definition}

\ePrints{1610.309618526,CACAA.06}
\ifx\Semafor\ValueOff
\begin{theorem}
\labelTheorem{aE, quaternion, Jacobian matrix}
Мы можем отождествить отображение
\ShowEq{aE, quaternion}
и матрицу
\ShowEq{aE, quaternion, Jacobian matrix}
\ShowEq{aE, quaternion, matrix}
\end{theorem}
\begin{proof}
\TheoremFollows
\ShowEq{ref aE, quaternion, Jacobian matrix}
\end{proof}
\fi

\begin{theorem}
\labelTheorem{linear map of quaternion algebra}
Линейное отображение алгебры кватернионов
\ShowEq{f:H->H ij}
имеет вид
\ShowEq{linear map of quaternion algebra, structure}
где $H$\Hyph числа
\ShowEq{a0123}
определены равенством
\ShowEq{a0123=}
\end{theorem}
\begin{proof}
\TheoremFollows
\ShowEq{ref expand linear mapping, quaternion}
\end{proof}

\begin{corollary}
\labelCorollary{linear map of quaternion algebra}%basis of L(R;H;H)
{\it
$H\otimes H$\Hyph модуль
\ShowEq{L(R;H;H)}
является левым $H$\Hyph векторным пространством
и имеет базис
\EqParm{e=(E,I,J,K)}{=.}
\qed
}
\end{corollary}

\ePrints{1610.309618526,CACAA.06}
\ifx\Semafor\ValueOff
\begin{theorem}
\labelTheorem{HE is algebra isomorphic to quaternion algebra}
Множество
\ShowEq{HE set}
является $R$\Hyph алгеброй, изоморфной алгебре кватернионов.
\end{theorem}
\begin{proof}
Теорема является следствием равенств
\ShowEq{aE+bE=(a+b)E}
\ShowEq{aE o bE=(ab)E}
опирающихся на теорему
\RefTheorem{linear map of quaternion algebra}.
\end{proof}
\fi
\fi

\ePrints{1506.00061}
\ifx\Semafor\ValueOn
\begin{theorem}
\labelTheorem{ax-xa=1 quaternion algebra}
Уравнение
\ShowEq{ax-xa=1}
в алгебре кватернионов не имеет решений.
\end{theorem}
\begin{proof}
\TheoremFollows
\ShowEq{ref ax-xa=1 quaternion algebra}
\end{proof}
\fi
\fi

\def\Preliminary{off}
\ShowEq{SetupRef}


==> Second.Derivative.16.Russian.tex <==
%auto-ignore

\input{Second.Derivative.16.Eq}

\Chapter{Производная второго порядка отображения \texorpdfstring{$D$}{D}-алгебры}
\labelChapter{Derivative of Second Order of Map of Algebra}

\Section{Производная второго порядка отображения \texorpdfstring{$D$}{D}-алгебры}

Пусть $D$ - полное коммутативное кольцо характеристики $0$.
Пусть $A$, $B$ - банаховые $D$\Hyph модули.
Пусть
\ShowEq{f:A->B}fAB
дифференцируемое отображение.
Согласно замечанию \ref{remark: differential L(A,A)},
производная является отображением
\EqParm{x->df/dx in L(A,B)}{A=AB}
Согласно теореме
\RefTheorem{L(A;B) is Banach module},
множество
\ShowEq{L(A;B)}DAB{}
является банаховым $D$\Hyph модулем.
Следовательно, мы можем рассмотреть вопрос,
является ли отображение
\ShowEq{df/dx}
дифференцируемым.

Согласно определению
\RefDefinition{differentiable map, algebra}
и теореме
\RefTheorem{dfa1p/dx=df/dx a1p},
\ShowEq{derivative of map df, algebra}
где
\ShowEq{derivative of map df, algebra, o2}
- такое непрерывное отображение, что
\ShowEq{derivative of map df, algebra, o2 lim}
Согласно определению
\RefDefinition{differentiable map, algebra},
отображение
\ShowEq{increment of derivative, algebra}
линейно по переменной $a_2$. Из равенства
\EqRef{derivative of map df, algebra}
следует, что отображение
\ShowEq{increment of derivative, algebra}
линейно по переменной $a_1$.
Следовательно, отображение
\ShowEq{increment of derivative, algebra}
билинейно.

\ShowDefinition{derivative of Second Order, algebra}

\begin{remark}
Согласно определению
\RefDefinition{derivative of Second Order, algebra}
производная второго порядка отображения $f$ является отображением
\ShowEq{differential L(A,A;A)}
Согласно теореме
\ShowEq{ref theorem tensor product and polylinear map}
мы можем также рассматривать отображение
\ShowEq{differential AA A,A}
Тогда
\ShowEq{differential L(AA;A)}
Мы будем пользоваться одним и тем же символом
\ShowEq{differential D2A2}
для обозначения отображений
\EqRef{differential L(A,A;A)}
и
\EqRef{differential L(AA;A)},
так как по характеру аргумента ясно о каком отображении идёт речь.
\qed
\end{remark}

\ShowTheorem{Differential of Second Order, algebra, representation}
\begin{proof}
Следствие определения
\RefDefinition{derivative of Second Order, algebra}
и теоремы
\ShowEq{ref polylinear map}
\end{proof}

\ShowDefinition{derivative of Order n, algebra}

\Section{Ряд Тейлора}
\labelSection{Taylor Series}

Пусть $D$ - полное коммутативное кольцо характеристики $0$.
Пусть $A$ - ассоциативная $D$\Hyph алгебра.
%Пусть левый \BoxB{A}модуль
%\ShowEq{L(A;B)}DAA{}
%порождён тождественным отображением $I_0=\delta$.
Пусть $p_n(x)$ - одночлен степени $n$, $n>0$,
одной переменной над $D$\Hyph алгеброй $A$.
Пусть $\Basis F$ - базис алгебры
\ShowEq{L(A;B)}DAA.

\begin{theorem}
\labelTheorem{derivative of f(x)x, algebra}
Для произвольного $m>0$ справедливо равенство
\ShowEq{derivative of f(x)x, algebra}
где символ $\widehat{h^i}$ означает отсутствие переменной $h^i$ в списке.
\end{theorem}
\begin{proof}
Для $m=1$ - это следствие равенства
\EqRef{derivative of product, algebra}
и теоремы
\RefTheorem{derivative of linear map}
\ShowEq{derivative of f(x)x, 1, algebra}
Допустим, \EqRef{derivative of f(x)x, algebra} справедливо
для $m-1$. Тогда
\ShowEq{derivative of f(x)x, m-1, algebra}
Так как
\ShowEq{dhi=0}
то, пользуясь равенством
\EqRef{derivative of product, algebra},
получим
\ShowEq{derivative of f(x)x, m, algebra}
Равенства \EqRef{derivative of f(x)x, algebra} и
\EqRef{derivative of f(x)x, m, algebra}
отличаются только формой записи.
Теорема доказана.
\end{proof}

\begin{theorem}
\labelTheorem{derivative of pn = 0, algebra}
Для произвольного $n\ge 0$ справедливо равенство
\ShowEq{derivative n1 of pn, algebra}
\end{theorem}
\begin{proof}
Так как $p_0(x)=a_0$, $a_0\in D$, то при $n=0$ теорема является следствием
определения
\RefDefinition{differentiable map, algebra}.
Пусть утверждение теоремы верно для $n-1$. Согласно теореме
\RefTheorem{derivative of f(x)x, algebra},
при условии $f(x)=p_{n-1}(x)$ мы имеем
\ShowEq{d(p(n-1)xan)}
Согласно предположению индукции все одночлены равны $0$.
\end{proof}

\begin{theorem}
\labelTheorem{derivative of pn = 0, m < n, algebra}
Если $m<n$, то справедливо равенство
\ShowEq{m derivative of polinom pn, algebra}
\end{theorem}
\begin{proof}
Для $n=1$ справедливо равенство
\ShowEq{d0p1(0)=0}
Допустим, утверждение справедливо
для $n-1$. Тогда согласно теореме \RefTheorem{derivative of f(x)x, algebra}
\ShowEq{dm p(n-1)xan}
Первое слагаемое равно $0$ так как $x=0$.
Так как $m-1<n-1$, то
остальные слагаемые равны $0$ согласно предположению индукции.
Утверждение теоремы доказано.
\end{proof}

Если $h_1=...=h_n=h$, то мы положим
\ShowEq{dfxh}
Эта запись не будет приводить к неоднозначности, так как по числу аргументов
ясно, о какой функции идёт речь.

\begin{theorem}
\labelTheorem{n derivative of polinom pn, algebra}
Для произвольного $n>0$ справедливо равенство
\ShowEq{n derivative of polinom pn, algebra}
\end{theorem}
\begin{proof}
Для $n=1$ справедливо равенство
\ShowEq{n derivative of polinom pn, 2, algebra}
Допустим, утверждение справедливо
для $n-1$. Тогда согласно теореме \RefTheorem{derivative of f(x)x, algebra}
\ShowEq{n derivative of polinom pn, 1, algebra}
Первое слагаемое равно $0$ согласно теореме
\RefTheorem{derivative of pn = 0, algebra}.
Остальные $n$ слагаемых равны, и согласно предположению индукции
из равенства \EqRef{n derivative of polinom pn, 1, algebra}
следует
\ShowEq{n derivative of polinom pn, 3, algebra}
Следовательно, утверждение теоремы верно для любого $n$.
\end{proof}

Пусть $p(x)$ - многочлен степени $n$.\,\footnote{Я рассматриваю
формулу Тейлора для многочлена по аналогии с
построением формулы Тейлора в \citeBib{Fikhtengolts: Calculus volume 1}, с. 246.}
\[
p(x)=p_0+p_{1i_1}(x)+...+p_{ni_n}(x)
\]
Мы предполагаем сумму по индексу $i_k$, который нумерует слагаемые
степени $k$.
Согласно теоремам \RefTheorem{derivative of pn = 0, algebra},
\RefTheorem{derivative of pn = 0, m < n, algebra},
\RefTheorem{n derivative of polinom pn, algebra}
\ShowEq{Taylor polynomial 1, algebra}
Следовательно, мы можем записать
\ShowEq{Taylor polynomial 2, algebra}
Это представление многочлена называется
\AddIndex{формулой Тейлора для многочлена}{Taylor polynomial, algebra}.
Если рассмотреть замену переменных $x=y-y_0$, то рассмотренное построение
остаётся верным для многочлена
\[
p(y)=p_0+p_{1i_1}(y-y_0)+...+p_{ni_n}(y-y_0)
\]
откуда следует
\ShowEq{Taylor polynomial 3, algebra}

Предположим, что функция $f(x)$ в точке $x_0$ дифференцируема
до любого порядка.\,\footnote{Я рассматриваю
построение ряда Тейлора по аналогии с
построением ряда Тейлора в \citeBib{Fikhtengolts: Calculus volume 1}, с. 248, 249.}

\ShowTheorem{n derivative equal 0, algebra}
\begin{proof}
При $n=1$ это утверждение следует из равенства
\EqRef{differential of map, t, algebra}.

Пусть утверждение справедливо для $n-1$.
Для отображения
\ShowEq{n derivative equal 0, 1, algebra}
выполняется условие
\ShowEq{n derivative equal 0, 2, algebra}
Согласно предположению индукции
\[
f_1(x_0+th)=o(t^{n-1})
\]
Тогда равенство
\EqRef{derivative, linear path}
примет вид
\[
o(t^{n-1})=\lim_{t\rightarrow 0,\ t\in R}(t^{-1}f(x+th))
\]
Следовательно,
\[
f(x+th)=o(t^n)
\]
\end{proof}

\ShowEq{Taylor polynomial}

\ShowEq{Taylor series}


==> Stmt.Derivative.Russian.tex <==
%auto-ignore
\input{Stmt.Derivative.Eq}

\DefTheorem{bilinear map and differential}
{
Пусть $A$ - банаховый $D$\Hyph модуль.
Пусть $B_1$, $B_2$, $B$ - банаховые $D$\Hyph алгебры.
Пусть
\ShowEq{h:BxB->B}
непрерывное билинейное отображение.
Пусть $f$, $g$ - дифференцируемые отображения
\ShowEq{f,g:A->B12}
Отображение
\ShowEq{h(f,g):A->B}
дифференцируемо и
производная удовлетворяет соотношению
\ShowEq{bilinear map and derivative, 3}
\ShowEq{bilinear map and derivative, 5}
}

\DefTheorem{derivative of product, algebra}
{
Пусть $A$ - банаховый $D$\Hyph модуль.
Пусть $B$ - банаховая $D$\Hyph алгебра.
Пусть $f$, $g$ - дифференцируемые отображения
\ShowEq{f,g:A->B}
Производная удовлетворяет соотношению
\ShowEq{differential of product, algebra}
\ShowEq{derivative of product, algebra}
}

\DefDefinition{norm of polylinear map}
{
Пусть $A$ - банаховый $D$\Hyph модуль с нормой $\|x\|_A$.
Пусть $B$ - банаховый $D$\Hyph модуль с нормой $\|x\|_B$.
Для отображения
\ShowEq{f:An->B}
величина
\ShowEq{norm of polymap}
\ShowEq{norm of map, module}
называется
\AddIndex{нормой отображения}{norm of map} $f$.
}

\DefTheorem{|f(a)|<|f||a| 1n}
{
Для отображения
\ShowEq{f:An->B}
банахового $D$\Hyph модуля $A$ с нормой $\|x\|_A$
в банаховый $D$\Hyph модуль $B$ с нормой $\|x\|_B$
\ShowEq{|f(a)|<|f||a| 1n}
}

\DefProof{|f(a)|<|f||a| 1n}
{
Неравенство
\ShowEq{|f(a)|/|a|<max}
является следствием равенства
\EqRef{norm of map, module}.
Неравенство
\EqRef{|f(a)|<|f||a| 1n}
является следствием неравенства
\EqRef{|f(a)|/|a|<max}.
}

\DefTheorem{|on|->0 ona1p->0}
{
Пусть
\ShowEq{f:A->B}{o_n}{A^n}B
последовательность отображений банахова $D$\Hyph модуля $A$
в банаховый $D$\Hyph модуль $B$ такая, что
\ShowEq{|on|->0}
Тогда для любых $B$\Hyph чисел
\ShowEq{a1n}p{}
\ShowEq{ona1p->0}
}

\DefProof{|on|->0 ona1p->0}
{
Из теоремы
\RefTheorem{|f(a)|<|f||a| 1n}
следует, что
\ShowEq{|oa1p|<}
Утверждение
\EqRef{ona1p->0}
является следствием утверждений
\EqRef{|on|->0},
\EqRef{|oa1p|<}.
}

\DefTheorem{derivative x2}
{
Пусть $D$ - полное коммутативное кольцо характеристики $0$.
Пусть $A$ - ассоциативная банаховая $D$\Hyph алгебра.
Тогда\,\footnote{
Утверждение теоремы аналогично примеру VIII,
\citeBib{Hamilton Elements of Quaternions 1}, с. 451.
Если произведение коммутативно, то равенство
\EqRef{derivative x2, algebra}
принимает вид
\ShowEq{derivative x2, field}}
\ShowEq{derivative x2, algebra}
\ShowEq{derivative x2 differential, algebra}
\ShowEq{derivative x2 component, algebra}
}

\DefProof{derivative x2}
{
Рассмотрим приращение функции $f(x)=x^2$.
\ShowEq{derivative x2, algebra, 1}
Равенство
\EqRef{derivative x2 differential, algebra}
является следствием равенства
\EqRef{derivative x2, algebra, 1}
и определения
\RefDefinition{differentiable map, algebra}.
Равенство
\EqRef{derivative x2, algebra}
является следствием равенств
\EqRef{a ox b c=},
\EqRef{derivative x2 differential, algebra}
и определения
\RefDefinition{differential of map}.
Равенство
\EqRef{derivative x2 component, algebra}
является следствием равенства
\EqRef{derivative x2, algebra}.
}

\DefExample{differential equation y=xx, real number}
{
Рассмотрим
\AddIndex{метод последовательного дифференцирования}
{method of successive differentiation}
для решения дифференциального уравнения
\ShowEq{differential equation y=xx, real number}
\DrawEq{differential equation, initial}{y=xx, real number}
над полем действительных чисел.
Последовательно дифференцируя уравнение
\EqRef{differential equation y=xx, real number},
мы получаем цепочку уравнений
\ShowEq{differential equation y=xx, 2...n, real number}
Разложение в ряд Тейлора
\DrawEq{y=x3+C}{}
следует из уравнений
\ShowEq{differential equation y=xx, ref, real number}
}

\DefTheorem{int=x3 algebra}
{
Пусть $A$ - банахова алгебра над коммутативным кольцом $D$.
\DrawEq{int=x3}{integral}
где $C$ - произвольное $A$\Hyph число.
}

\DefProof{int=x3 algebra}
{
Согласно определению
\RefDefinition{indefinite integral},
отображение $y$ является интегралом
\eqRef{int=x3}{integral},
если отображение $y$ удовлетворяет дифференциальному уравнению
\DrawEq{differential equation y=xx, 1, algebra}{integral}
и начальному условию
\DrawEq{differential equation, initial}{y=xx, algebra}
Мы воспользуемся методом последовательного дифференцирования,
чтобы решить дифференциальное уравнение
\eqRef{differential equation y=xx, 1, algebra}{integral}.
Последовательно дифференцируя уравнение
\eqRef{differential equation y=xx, 1, algebra}{integral},
мы получаем цепочку уравнений
\ShowEq{differential equation y=xx, 2, algebra}
\ShowEq{differential equation y=xx, 3, algebra}
\ShowEq{differential equation y=xx, 4, algebra}
Разложение в ряд Тейлора
\DrawEq{y=x3+C}{algebra}
следует из уравнений
\ShowEq{differential equation y=xx, ref, algebra}
Равенство
\eqRef{int=x3}{integral}
является следствием
\eqRef{differential equation y=xx, 1, algebra}{integral},
\eqRef{differential equation, initial}{y=xx, algebra},
\eqRef{y=x3+C}{algebra}.
}

\DefRemark{int=x3 algebra}
{
Согласно определению
\EqRef{a ox b c=},
мы можем записать интеграл
\eqRef{int=x3}{integral}
следующим образом
\ShowEq{int=x3 1}
}

\DefRemark{notation int=x3 algebra}
{
В доказательстве теоремы
\RefTheorem{int=x3 algebra}
я пользовался записью вида
\ShowEq{notation theorem int=x3 algebra}
Я записываю  следующие равенства для того,
чтобы показать как работает производная. 
\ShowEq{differential equation y=xx, algebra, 1}
}

\DefRemark{differential equation 3x^2 does not possess a solution}
{
Дифференциальное уравнение
\DrawEq{differential equation y=xx, 1, a, algebra}{integral}
\DrawEq{differential equation, initial}{}
так же приводит к решению $y=x^3$. Очевидно, что
отображение $y=x^3$ не удовлетворяет дифференциальному уравнению
\eqRef{differential equation y=xx, 1, a, algebra}{integral}.
Это говорит о том, что дифференциальное уравнение
\eqRef{differential equation y=xx, 1, a, algebra}{integral}
не имеет решений.

Я советую обратить внимание на то, что
вторая производная не
является симметричным многочленом (смотри разложение Тейлора).
}

\DefTheorem{derivative of the sum}
{
Пусть $A$ - банаховый $D$\Hyph модуль.
Пусть $B$ - банаховая $D$\Hyph алгебра.
Пусть $f$, $g$ - дифференцируемые отображения
\ShowEq{f,g:A->B}
Отображение
\ShowEq{derivative of the sum, 2}
дифференцируемо и
производная удовлетворяет соотношению
\ShowEq{derivative of the sum, 3}
}

\AddEq [4]{definition: differentiable map}
{
\begin{definition}
\labelDefinition{differentiable map, #4}
{\it
Пусть $#2$ - банаховый $#1$\Hyph модуль с нормой $\|a\|_#2$.
Пусть $#3$ - банаховый $#1$\Hyph модуль с нормой $\|a\|_#3$.
Отображение
\ShowEq{f:A->B}f{#2}{#3}
называется
\AddIndex{дифференцируемым}{differentiable map}
на множестве $U\subset #2$,
если в каждой точке $x\in U$
изменение отображения $f$ может быть представлено в виде
\ShowEq{derivative of map}
\DrawEq{derivative of map, def}{#4}
где
\ShowEq{df:A->B}{#2}{#3}
линейное отображение $#1$\Hyph модуля $#2$ в $#1$\Hyph модуль $#3$ и
\ShowEq{f:A->B}o{#2}{#3}
такое непрерывное отображение, что
\ShowEq{lim |o|/|a|}{#2}{#3}
Линейное отображение
\ShowEq{show derivative of map}
называется
\AddIndex{производной отображения}{derivative of map}
$f$.
}
\qed
\end{definition}
}

\AddEq [4]{remark: derivative as differential form}
{
\begin{remark}
\labelRemark{derivative as differential form, #4}
Согласно определению
\RefDefinition{differentiable map, #4}
при заданном $x$, производная
\ShowEq{df/dx in L(A->B)}{#1}{#2}{#3}
Следовательно, производная отображения $f$ является
дифференциальной $#3$\Hyph значной $1$\Hyph формой
\ShowEq{df/dx:A->L(A->B)}{#1}{#2}{#3}
\qed
\end{remark}
}

\AddEq [4]{remark: differential of map}
{
\begin{remark}
\labelRemark{differential of map, #4}
В математическом анализе, отображение
\ShowEq{differential of independent variable}
\ShowEq{dx=delta}{#1}{#2}
называется
\AddIndex{дифференциалом независимой переменной}
{differential of independent variable}.
Дифференциальная $#3$\Hyph значная $1$\Hyph форма
\ShowEq{df/dx:A->L(A->B)}{#1}{#2}{#3}
записанная в виде
\ShowEq{differential of independent variable}
\ShowEq{differential of map}
\DrawEq{differential of map =}{#4}
называется
\AddIndex{дифференциалом отображения}{differential of map}
$f$.
Впрочем равенство
\eqRef{differential of map =}{#4}
имеет другую интерпретацию.
А именно, мы рассматриваем приращение $df$ отображения $f$
как функцию
\eqRef{differential of map =}{#4}
приращения $dx$ независимой переменной.
\qed
\end{remark}
}

\DefRemark{differential L(A,A)}
{
Согласно определению
\RefDefinition{differentiable map, algebra},
производная отображения $f$ является отображением
\EqParm{x->df/dx in L(A,B)}{A=AB}
Выражения $d_x f(x)$ и
\ShowEq{df/dx}
являются разными обозначениями одного и того же отображения.
}

\DefEq
{
\begin{theorem}
\labelTheorem{representation of derivative, algebra A->B}
Пусть $A$ - свободный банаховый $D$\Hyph модуль.
Пусть $B$ - свободная банаховая $D$\Hyph алгебра.
Пусть $\Basis F$ - базис левого \BoxB{B}модуля
\ShowEq{L(A;B)}DAB.
Мы можем представить производную отображения
\ShowEq{f:A->B}fAB
в виде
\ShowEq{coordinates of derivative}
\ShowEq{df/dx=dkf/dx Ik}
\end{theorem}
}
{theorem: representation of derivative, algebra A->B}
%\DefEq

\DefEq
{
\begin{definition}
\labelDefinition{coordinates of derivative, algebra A->B}
{\it
%Согласно определению
%\RefDefinition{coordinates of vector},
Выражение
\ShowEq{show coordinates of derivative}
называется
\AddIndex{координатами}{coordinates}
производной
\ShowEq{df/dx}
относительно базиса $\Basis F$.
Выражение
\ShowEq{component of derivative A->B}
\ShowEq{component of derivative A->B =}
называется
\AddIndex{компонентой производной}
{component of derivative} отображения $f(x)$.
}
\qed
\end{definition}
}
{definition: coordinates of derivative, algebra A->B}
%\DefEq

\DefEq
{
\begin{theorem}
\labelTheorem{representation of differential, algebra A->B}
Пусть $A$ - свободный банаховый $D$\Hyph модуль.
Пусть $B$ - свободная банаховая $D$\Hyph алгебра.
Пусть $\Basis F$ - базис левого \BoxB{B}модуля
\ShowEq{L(A;B)}DAB.
Мы можем представить дифференциал отображения
\ShowEq{f:A->B}fAB
в виде
\ShowEq{df=sum dsf/dx dx A->B}
\end{theorem}
}
{theorem: representation of differential, algebra A->B}
%\DefEq

\DefTheorem{dfa1p/dx=df/dx a1p}
{
Пусть $B$ - банаховый модуль над коммутативным кольцом $D$.
Пусть $U$ - открытое множество банахового $D$\Hyph модуля $A$.
Пусть
\ShowEq{U->L(Ap,B)}
дифференцируемое отображение.
Тогда
\ShowEq{dfa1p/dx=df/dx a1p}
}

\AddEq{proof: dfa1p/dx=df/dx a1p}
{
\begin{proof}
Пусть
\ShowEq{a0 in U}
Согласно определению
\RefDefinition{differentiable map, algebra},
изменение отображения
$f$ может быть представлено в виде
\ShowEq{derivative of map, U->L(B)}
где
\ShowEq{derivative in L(L)}
и
\ShowEq{o:A->LB}
такое непрерывное отображение, что
\ShowEq{o:A->LB, lim o}
Так как
\ShowEq{f(x) in LB}
то для любых
\ShowEq{a1n}p{}
равенство
\ShowEq{derivative of map, U->B}
является следствием равенства
\EqRef{derivative of map, U->L(B)}.
Согласно теореме
\RefTheorem{|on|->0 ona1p->0},
равенство
\ShowEq{o:A->LB, lim o a1p}
является следствием равенства
\EqRef{o:A->LB, lim o}.
Рассматривая выражение
\ShowEq{f(x) o a1p}
как отображение
\ShowEq{x->f(x) o a1p}
мы получим, что изменение этого отображения
может быть представлено в виде
\ShowEq{derivative of map, U->B 1}
где
\ShowEq{derivative in L}
и
\ShowEq{f:A->B}{o_1}AB
такое непрерывное отображение, что
\ShowEq{o1:A->B, lim o}
Равенство
\ShowEq{derivative of map, U->B = +o}
является следствием равенств
\EqRef{derivative of map, U->B},
\EqRef{derivative of map, U->B 1}.
Равенство
\ShowEq{lim o a1p-o1}
является следствием равенств
\EqRef{o:A->LB, lim o a1p},
\EqRef{o1:A->B, lim o}.
Равенство
\EqRef{dfa1p/dx=df/dx a1p}
является следствием равенств
\EqRef{derivative of map, U->B = +o},
\EqRef{lim o a1p-o1}.
\end{proof}
}

\DefEq
{
\begin{theorem}
\labelTheorem{derivative, representation in algebra}
Определения производной
\eqRef{derivative of map, def}{algebra}
эквивалентно определению
\ShowEq{derivative, linear path}
\end{theorem}
}
{theorem: derivative, representation in algebra}
%\DefEq

\DefDefinition{derivative of Second Order, algebra}
{
Полилинейное отображение
\ShowEq{derivative of Second Order}
\ShowEq{derivative of Second Order, algebra}
называется
\AddIndex{производной второго порядка}
{derivative of Second Order} отображения $f$.
}

\DefTheorem{Differential of Second Order, algebra, representation}
{
Пусть $A$ - свободный банаховый $D$\Hyph модуль.
Пусть $B$ - свободная ассоциативная банаховая $D$\Hyph алгебра.
Пусть $\Basis F$ - базис левого \BoxB{B}модуля
\ShowEq{L(A;B)}DAB.
Мы можем представить
производную второго порядка отображения $f$
в виде
\ShowEq{Differential of Second Order, algebra, representation}
Мы будем называть выражение
\ShowEq{component of derivative of Second Order, algebra}
\AddIndex{компонентой производной второго порядка}
{component of derivative of Second Order} отображения $f(x)$.
}

\DefDefinition{derivative of Order n, algebra}
{
По индукции, предполагая, что определена производная
\ShowEq{partial n-1 f}
порядка $n-1$, мы определим
\ShowEq{derivative of Order n}
\ShowEq{derivative of Order n, algebra}
\AddIndex{производную порядка $n$}
{derivative of Order n} отображения $f$.

Мы будем также полагать
\ShowEq{d0f(x)}
}

\DefTheorem{n derivative equal 0, algebra}
{
Если для отображения $f(x)$ выполняется условие
\ShowEq{n derivatives of function, algebra}
то при $t\rightarrow 0$ выражение $f(x+th)$ является бесконечно малой порядка
выше $n$ по сравнению с $t$
\[
f(x_0+th)=o(t^n)
\]
}

\AddEq{Taylor polynomial}
{
Составим многочлен
\ShowEq{Taylor polynomial, f(x), algebra}
Согласно теореме \RefTheorem{n derivative equal 0, algebra}
\[
f(x_0+t(x-x_0))-p(x_0+t(x-x_0))=o(t^n)
\]
Следовательно, полином $p(x)$ является хорошей апроксимацией отображения $f(x)$.
}

\AddEq{Taylor series}
{
Если отображение $f(x)$ имеет производную любого порядка, то переходя к пределу
$n\rightarrow\infty$, мы получим разложение в ряд
\ShowEq{Taylor series, f(x), algebra}
который называется \AddIndex{рядом Тейлора}{Taylor series, algebra}.
}

\DefDefinition{indefinite integral}
{
Пусть $A$ - банаховый $D$\Hyph модуль.
Пусть $B$ - банаховая $D$\Hyph алгебра.
Отображение
\ShowEq{g:A->BoxB}
называется
\AddIndex{интегрируемым}{integrable map},
если существует отображение
\ShowEq{f:A->B}fAB
такое, что
\ShowEq{df=g}
Тогда мы пользуемся записью
\ShowEq{indefinite integral}
\ShowEq{f=int g}
и отображение $f$ называется
\AddIndex{неопределённым интегралом}{indefinite integral}
отображения $g$.
}

\DefTheorem{derivative of tensor product}
{
Пусть $A$ - банаховый $D$\Hyph модуль.
Пусть $B$, $C$ - банаховые $D$\Hyph алгебры.
Пусть $f$, $g$ - дифференцируемые отображения
\ShowEq{f,g:A->BC}
Производная удовлетворяет соотношению
\ShowEq{differential of tensor product, algebra}
\ShowEq{derivative of tensor product, algebra}
}

\DefTheorem{map is continuous, derivative}
{
Пусть $A$ - банаховый $D$\Hyph модуль с нормой $\|a\|_A$.
Пусть $B$ - банаховая $D$\Hyph алгебра с нормой $\|b\|_B$.
Если производная
\ShowEq{df/dx}
отображения
\ShowEq{f:A->B}fAB
существует в точке $x$ и имеет конечную норму,
то отображение $f$ непрерывно в точке $x$.
}

\DefTheorem{composite map, derivative, D algebra}
{
Пусть $A$ - банаховый $D$\Hyph модуль с нормой $\|a\|_A$.
Пусть $B$ - банаховый $D$\Hyph модуль с нормой $\|b\|_B$.
Пусть $C$ - банаховый $D$\Hyph модуль с нормой $\|c\|_C$.
Пусть отображение
\ShowEq{f:A->B}fAB
дифференцируемо в точке
$x$
и норма производной отображения $f$
конечна
\ShowEq{composite map, norm f, D algebra}
Пусть отображение
\ShowEq{f:A->B}gBC
дифференцируемо в точке
\ShowEq{composite map, y fx, D algebra}
и норма производной отображения $g$
конечна
\ShowEq{composite map, norm g, D algebra}
Отображение\,\footnote{
Запись
\ShowEq{dg/df}
означает выражение
\ShowEq{dg/df=}
Аналогичное замечание верно для компонент производной.
}
\ShowEq{composite map, gfx, D algebra}
дифференцируемо в точке
\labelItem{composite map is differentiable}
$x$
\ShowEq{composite map, derivative, D algebra}
}


==> Stmt.Module.Russian.tex <==
%auto-ignore
\input{Stmt.Module.Eq}

\DefEq
{
\begin{definition}
\labelDefinition{module over ring}
Пусть коммутативное кольцо $D$ имеет единицу $1$.
Эффективное представление
\DrawEq{D->*V}{def}
кольца $D$
в абелевой группе $V$
называется
\AddIndex{модулем над кольцом}{module over ring} $D$
или
\AddIndex{$D$\Hyph модулем}{D module}.
Эффективное представление
\eqRef{D->*V}{def}
поля $D$ в абелевой группе $V$
называется
\AddIndex{векторным пространством над полем}{vector space over field} $D$
или
\AddIndex{$D$\Hyph векторным пространством}{D vector space}.
\qed
\end{definition}
}
{... definition: module over ring}
%\DefEq

\DefTheorem{tensor product of D-algebras is D-algebra}
{
Пусть
\ShowEq{A1...n}
- $D$\Hyph алгебры.
Тензорное произведение
$\Tensor A$
$D$\Hyph модулей
\ShowEq{A1...n}
является $D$\Hyph алгеброй,
если мы определим произведение согласно правилу
\ShowEq{xA1n*xA1n->oxA1n=}
}

\DefTheorem{representation of algebra A2 in LA}
{
Пусть $A$ является $D$\Hyph алгеброй.
Пусть произведение в алгебре
\ShowEq{AoxA}
определено согласно правилу
\DrawEq{product in algebra AA}{}
Представление
\ShowEq{h:AoxA->L(A)}
$D$\Hyph алгебры
\ShowEq{AoxA}
в модуле
\ShowEq{L(A;B)}DAA,
определённое равенством
\ShowEq{representation AA in LA}
позволяет отождествить тензор
\ShowEq{d in AxoA}
с линейным отображением
\ShowEq{product in algebra AA 2},
где
\ShowEq{product in algebra AA 3}
- тождественное отображение.
Линейное отображение
\ShowEq{a ox b}
имеет вид
\ShowEq{a ox b c=}
}

\DefDefinition{module over commutative ring}
{
Эффективное представление коммутативного кольца $D$
в абелевой группе $V$
\DrawEq{D->*V}{module}
называется
\AddIndex{модулем над кольцом}{module over ring} $D$
или
\AddIndex{$D$\Hyph модулем}{D module}.
$V$\Hyph число называется
\AddIndex{вектором}{vector}.
\ePrints{1610.309618526,CACAA.06}
\ifx\Semafor\ValueOn
Если $D$ - поле, то абелевая группа $V$
называется
\AddIndex{векторным пространством}{vector space} над полем $D$
или
\AddIndex{$D$\Hyph векторным пространством}{D vector space}.
\fi
}

\DefTheorem{definition of module over commutative ring}
{
Элементы $D$\Hyph модуля $V$ удовлетворяют соотношениям
\StartLabelItem
\begin{enumerate}
\item
\AddIndex{закону ассоциативности}{associative law}
\DrawEq{associative law, module}2
\item 
\AddIndex{закону дистрибутивности}{distributive law}
\ShowEq{distributive law, module}
\item 
\AddIndex{закону унитарности}{unitarity law}
\ShowEq{unitarity law, D-module}
\end{enumerate}
для любых
\ShowEq{c,d in Z, a,b in D, v,w in V}
}

\AddEq{definition: module over algebra}
{
\begin{definition}
\labelDefinition{\SideWS module over algebra}
Эффективное \SideRu востороннее представление
\DrawEq{\SideWS A->*V}{def}
ассоциативной $D$\Hyph алгебры $A$
в $D$\Hyph модуле $V$
называется
\AddIndex{\SideRu вым модулем}{\SideWS module} над $D$\Hyph алгеброй $A$.
Мы также будем говорить, что $D$\Hyph модуль $V$ является
\AddIndex{\SideRu вым $A$\Hyph модулем}{\SideWS A module}
или
\AddIndex{$\SideA$\Hyph модулем}{\SideA-module}.
$V$\Hyph число называется
\AddIndex{вектором}{vector}.
Если $A$ - алгебра с делением, то \SideRu вый $A$\Hyph модуль
называется
\AddIndex{\SideRu вым векторным пространством}{\SideWS vector space}
над $D$\Hyph алгеброй $A$.
Мы также будем говорить, что $D$\Hyph модуль $V$ является
\AddIndex{\SideRu вым $A$\Hyph векторным пространством}{\SideWS A vector space}
или
\AddIndex{$\SideA$\Hyph векторным пространством}{\SideA-vector space}.
\qed
\end{definition}
}

\AddEq{theorem: module over algebra}
{
\begin{theorem}
\labelTheorem{\SideWS module over algebra}
Следующая диаграмма представлений описывает \SideRu вый $\Base$\Hyph модуль $V$
\ShowEq{diagram of representations, \SideWS module}
В диаграмме представлений
\EqRef{diagram of representations, \SideWS module}
верна
\AddIndex{коммутативность представлений}{commutativity of representations}
\BaseRings
в абелевой группе $V$
\ShowEq{\SideWS module, a d v}
\end{theorem}
}

\DefProof{module over algebra}
{
Диаграмма представлений
\EqRef{diagram of representations, \SideWS module}
является следствием определения
\def\Temp{}
\ifx\SideNS\Temp
\RefDefinition{module over commutative ring}
и теоремы
\RefTheorem{action of ring of rational integers in Abelian group}.
\else
\RefDefinition{\SideWS module over algebra}
и следствия
\RefCorollary{Free Algebra over Ring}.
\fi
Равенство
\EqRef{\SideWS module, a d v}
является следствием утверждения, что
\SideRu\HSide преобразование $\ATransf(a)$
является эндоморфизмом $\CBase$\Hyph модуля $V$.
}

\AddEq{theorem: A module -> alebra is associative}
{
\begin{theorem}
\labelTheorem{\SideWS A module -> alebra is associative}
Пусть $g$ - эффективное левостороннее представление $D$\Hyph алгебры $A$
в $D$\Hyph модуле $V$.
Тогда $D$\Hyph алгебра $A$ ассоциативна.
\end{theorem}
}

\DefProof{A module -> alebra is associative}
{
Пусть
\ShowEq{abc in A, v in v}
Равенство
\DrawEq{\SideWS module, associative law}0
является следствием утверждения, что \SideRu востороннее представление
$g$ является
\SideRu восторонним представлением
мультипликативной группы $D$\Hyph алгебры $A$.
Равенство
\ShowEq{a(b(cv))=(a(bc))v \SideNS}
является следствием равенства
\eqRef{\SideWS module, associative law}0.
Так как
\ShowEq{cv \SideNS}
равенство
\ShowEq{a(b(cv))=((ab)c)v \SideNS}
является следствием равенства
\eqRef{\SideWS module, associative law}0.
Равенство
\ShowEq{(a(bc))v=((ab)c)v \SideNS}
является следствием равенств
\EqRef{a(b(cv))=(a(bc))v \SideNS},
\EqRef{(a(bc))v=((ab)c)v \SideNS}.
Поскольку $v$ - произвольный вектор $A$\Hyph модуля $V$,
равенство
\ShowEq{a(bc)=(ab)c \SideNS}
является следствием равенства
\EqRef{(a(bc))v=((ab)c)v \SideNS}.
Следовательно, $D$\Hyph алгебра $A$ ассоциативна.
}

\AddEq{theorem: definition of A module}
{
\begin{theorem}
\labelTheorem{definition of \SideWS module}
Пусть $V$ является \SideRu\What $\Base$\Hyph модулем.
Для любого вектора $v\in V$,
вектор, порождённый диаграммой представлений
\EqRef{diagram of representations, \SideWS module},
имеет следующий вид
\ShowEq{\SideWS module, (a+n)v=av+nv}
\StartLabelItem
\begin{enumerate}
\item
Множество отображений
\ShowEq{\SideWS module, a+n:V->V}
порождает\,\footnote{
Смотри аналогичное утверждение на странице
\citeBib{McCrimmon: Jordan Algebras}-52.
}
\algebrad $\Base_{(1)}$
где сложение определено равенством
\DrawEq{(a+n)+(b+m)=}{\SideWS module}
и произведение определено равенством
\DrawEq{(a+n)(b+m)=}{\SideWS module}
\algebraD $\Base_{(1)}$ называется
\AddIndex{унитальным расширением}{unital extension}
кольца $\Base$.
\item
\algebraD $\Base$ является \SideRu\What идеалом \algebrab $\Base_{(1)}$.
\labelItem{Algebra is \SideWS ideal of algebra (1)}
\item
Множество преобразований
\EqRef{\SideWS module, (a+n)v=av+nv}
порождает \SideRu\HSide представление \algebrab $\Base_{(1)}$ в абелевой группе $V$.
\labelItem{\SideWS representation of D1 in Abelian group}
\end{enumerate}
Элементы \SideRu\From $\Base$\Hyph модуля $V$ удовлетворяют соотношениям
\begin{itemize}
\item
\AddIndex{закон ассоциативности}{associative law}
\DrawEq{associative law, \SideWS module}1
\item
\AddIndex{закон дистрибутивности}{distributive law}
\ShowEq{distributive law, \SideWS module}
\item
\AddIndex{закон унитарности}{unitarity law}
\ShowEq{unitarity law, \SideWS \Base-module}
\end{itemize}
для любых
\ShowEq{p,q in \Base 1, v,w in V}
\end{theorem}
}

\DefProof{definition of A module}
{
Пусть $v\in V$.

\begin{lemma}
\labelLemma{\SideWS module, map a+n:V->V is endomorphism of Abelian group}
{\it
Пусть 
\ShowEq{module, d in D}
\ShowEq{module, a in A}
Отображение
\EqRef{\SideWS module, a+n:V->V}
является эндоморфизмом абелевой группы $V$.
}
\end{lemma}

{\sc Доказательство.}
Утверждения
\ShowEq{\SideWS module, dv in V}
\ShowEq{\SideWS module, av in V}
являются следствием теорем
\RefTheorem[\RefRepresentation]{structure of subrepresentations},
\RefTheorem{\SideWS module over algebra}.
Так как $V$ является абелевой группой, то
\ShowEq{\SideWS module, dv+av in V}
Следовательно,
для любого $\CBase$\Hyph числа $\DArg$
и любого $\Base$\Hyph числа $a$,
мы определили отображение
\EqRef{\SideWS module, a+n:V->V}.
Поскольку преобразование $\DTransf(\DArg)$
и \SideRu\HSide преобразование $\ATransf(a)$
являются эндоморфизмами абелевой группы $V$,
то отображение
\EqRef{\SideWS module, a+n:V->V}
является эндоморфизмом абелевой группы $V$.
\hfill\(\odot\)

Пусть $\Base_{(1)}$ - множество отображений
\EqRef{\SideWS module, a+n:V->V}.
Равенство
\EqRef{distributive law, \SideWS module, 1}
является следствием леммы
\RefLemma{\SideWS module, map a+n:V->V is endomorphism of Abelian group}.

Пусть
\ShowEq{p,q in D1}
Согласно утверждению
\RefItem{representation of D1 in Abelian group},
мы определим сумму $\Base_{(1)}$\Hyph чисел $p$ и $q$ равенством
\EqRef{distributive law, \SideWS module, 2}.
Равенство
\ShowEq{\SideWS module, (a+n)+(b+m)=, 1}
является следствием равенства
\EqRef{distributive law, \SideWS module, 2}.
Равенство
\ShowEq{distributive law, \CBase, \SideWS module, 2}
является следствием утверждения, что представление
$\DTransf$ является гомоморфизмом аддитивной группы кольца $\CBase$.
Равенство
\ShowEq{distributive law, \Base, \SideWS module, 2}
является следствием утверждения, что \SideRu\HSide представление
$\ATransf$ является гомоморфизмом аддитивной группы \algebrab $\Base$.
Так как $V$ является абелевой группой, то равенство
\ShowEq{\SideWS module, (a+n)+(b+m)=}
является следствием равенств
\EqRef{\SideWS module, (a+n)+(b+m)=, 1},
\EqRef{distributive law, \CBase, \SideWS module, 2},
\EqRef{distributive law, \Base, \SideWS module, 2}.
Из равенства
\EqRef{\SideWS module, (a+n)+(b+m)=}
следует, что определение
\eqRef{(a+n)+(b+m)=}{\SideWS module}
суммы на множестве $\Base_{(1)}$ не зависит от вектора $v$.

Равенства
\eqRef{associative law, \SideWS module}1,
\EqRef{unitarity law, \SideWS \Base-module}
являются следствием утверждения
\RefItem{\SideWS representation of D1 in Abelian group}.
Пусть
\ShowEq{p,q in D1}
\def\Temp{}
\ifx\SideNS\Temp
Равенство
\DrawEq{associative law, \CBase, \SideWS module}1
является следствием утверждения, что представление $\DTransf$
является представлением мультипликативной группы кольца $\CBase$.
Равенство
\DrawEq{\SideWS module, associative law}1
является следствием утверждения, что представление $g_2$
является представлением мультипликативной группы кольца $D$.
Равенство
\DrawEq{associative law, \CBase\Base, \SideWS module}1
является следствием утверждения, что кольцо $D$
является абелевой группой.
Равенство
\ShowEq{module, (a+n)(b+m)=}
является следствием равенств
\ShowEq{ref module, (a+n)(b+m)=}%
Равенство
\eqRef{(a+n)(b+m)=}{\SideWS module}
является следствием равенства
\EqRef{module, (a+n)(b+m)=}.
\else%
Так как произведение в $D$\Hyph алгебре $A$ может быть неассоциативным,
то опираясь на теорему
мы рассмотрим произведение
$\Base_{(1)}$\Hyph чисел $p$ и $q$
как билинейное отображение
\ShowEq{f:D1xD1->D1}
такое, что верны равенства
\DrawEq{fab=ab}{\SideWS module}
\DrawEq{f1p=p}{\SideWS module}
Равенство
\DrawEq{pq=fpq}{\SideWS module}
является следствием равенств
\eqRef{fab=ab}{\SideWS module},
\eqRef{f1p=p}{\SideWS module}.
Равенство
\eqRef{(a+n)(b+m)=}{\SideWS module}
является следствием равенства
\eqRef{pq=fpq}{\SideWS module}.
\fi%

Утверждение
\RefItem{Algebra is \SideWS ideal of algebra (1)}
является следствием равенства
\eqRef{(a+n)(b+m)=}{\SideWS module}.
}

\AddEq{definition: submodule}
{
\begin{definition}
\labelDefinition{submodule, \SideWS module}
Подпредставление $D$\Hyph \SideRu вого модуля $V$ называется
\AddIndex{подмодулем}{submodule}
\SideRu вого $D$\Hyph модуля $V$.
\qed
\end{definition}
}

\AddEq{theorem: submodule}
{
\begin{theorem}
\labelTheorem{submodule, \SideWS module}
Пусть
\ShowEq{vi V}{}
- множество векторов \SideRu вого $\Base$\Hyph модуля $V$.
Если векторы
\ShowEq{set vi}
принадлежат подмодулю $V'$ \SideRu вого $\Base$\Hyph модуля $V$,
то линейная комбинация векторов
\ShowEq{set vi}
принадлежат подмодулю $V'$.
\end{theorem}
}

\DefProof{submodule}
{
Теорема является следствием
теоремы
\RefTheorem{set of vectors generated by set of vectors, \SideWS module}
и определений
\RefDefinition{\SideWS linear combination of vectors},
\RefDefinition{submodule, \SideWS module}.
}

\AddEq{theorem: set of vectors generated by set of vectors}
{
\begin{theorem}
\labelTheorem{set of vectors generated by set of vectors, \SideWS module}
Пусть $V$ - \SideRu\To $\Base$\Hyph модуль.
Множество векторов, порождённое множеством векторов
\ShowEq{vi V},
имеет вид\,\footnote{
Для множества $A$,
мы обозначим $|A|$ мощность множества $A$.
Запись $|A|<\infty$ означает, что множество $A$ конечно.
}
\ShowEq{w=sum vi, \SideWS module}
\end{theorem}
}

\DefProof{set of vectors generated by set of vectors}
{
Согласно теореме
\RefTheorem[\RefRepresentation]{structure of subrepresentations},
для доказательства теоремы мы должны доказать следующие утверждения:
%Мы докажем теорему по индукции, опираясь на теорему
\ShowEq{vectors generated by set of vectors}

\begin{itemize}
\item
Для произвольного
\ShowEq{vk in v}
положим
\ShowEq{ci=dik}
Тогда
\ShowEq{vk=sum vi, \SideWS module}
Утверждение
\RefItem{\SideWS module, vk in Jv}
следует из
\EqRef{w=sum vi, \SideWS module},
\EqRef{vk=sum vi, \SideWS module}.
\item
Утверждение
\RefItem{\SideWS module, cvk in Jv}
являются следствием теорем
\RefTheorem[\RefRepresentation]{structure of subrepresentations},
\RefTheorem{definition of \SideWS module}
и утверждения
\RefItem{\SideWS module, vk in Jv}.
\item
Так как $V$ является абелевой группой,
то утверждение
\RefItem{\SideWS module, sum cvk in Jv}
следует из утверждения
\RefItem{\SideWS module, cvk in Jv}
и теорем
\RefTheorem[\RefRepresentation]{structure of subrepresentations},
\RefTheorem{structure of Abelian group}.
\item
Пусть
\ShowEq{w12 in Jv}wv
Так как $V$ является абелевой группой,
то, согласно утверждению
\RefItem[\RefRepresentation]{x1n omega in Xk+1},
\ShowEq{w1+w2 in Jv}wv
Согласно равенству
\EqRef{w=sum vi, \SideWS module},
существуют $\Base_{(1)}$\Hyph числа
\ShowEq{gi12}w
такие, что
\DrawEq[w]{w12= \SideNS}{module}
где множества
\DrawEq[w]{|ci12 ne 0|}{\SideWS module}
конечны.
Так как $V$ является абелевой группой,
то из равенства
\eqRef{w12= \SideNS}{module}
следует, что
\DrawEq[w]{w1+w2= \SideNS}{module}
Равенство
\DrawEq[w]{w1+w2= 1 \SideNS}{module}
является следствием равенств
\EqRef{distributive law, \SideWS module, 2},
\eqRef{w1+w2= \SideNS}{module}.
Из равенства
\eqRef{|ci12 ne 0|}{\SideWS module}
следует, что
множество
\ShowEq{|gi 1+2 ne 0|}w
конечно.
Из равенства
\eqRef{w1+w2= 1 \SideNS}{module}
следует, что
\ShowEq{w1+w2 in Jv}wv
\item
Пусть
\ShowEq{w in Jv}
Согласно утверждению
\RefItem[\RefRepresentation]{ax in Xk+1},
для любого $\Base_{(1)}$\Hyph числа $a$,
\ShowEq{aw in Xk \SideWS module}
Согласно равенству
\EqRef{w=sum vi, \SideWS module},
существуют $\Base_{(1)}$\Hyph числа
\ShowEq{wi}
такие, что
\ShowEq{w= \SideWS module}
где
\DrawEq{|wi ne 0|}{\SideWS module}
Из равенства
\EqRef{w= \SideWS module}
следует, что
\ShowEq{aw= \SideWS module}
Из утверждения
\eqRef{|wi ne 0|}{\SideWS module}
следует, что
множество
\ShowEq{\SideWS module, |awi ne 0|}
конечно.
Из равенства
\EqRef{aw= \SideWS module}
следует, что
\ShowEq{aw in Jv \SideWS module}
\end{itemize}
}

\AddEq{definition: linear combination of vectors}
{
\begin{definition}
\labelDefinition{\SideWS linear combination of vectors}
Пусть
\ShowEq{vi V}{}
- множество векторов.
\ShowEq{\SideWS linear combination}%
Выражение
\ShowEq{A linear combination =}
называется
\AddIndex{линейной комбинацией}{linear combination} векторов
\ShowEq{vi}
Вектор
\ShowEq{w=wi vi\SideNS}
называется
\AddIndex{линейно зависимым}{linearly dependent}
от векторов
\ShowEq{vi}
\qed
\end{definition}
}

\AddEq{definition: generating set of module}
{
\begin{definition}
\labelDefinition{generating set of \SideWS module}
$J(v)$
называется
\AddIndex{подмодулем, порождённым множеством}
{submodule generated by set} $v$,
а $v$ -
\AddIndex{множеством образующих}{generating set}
подмодуля $J(v)$.
В частности,
\AddIndex{множеством образующих}{generating set}
\SideRu\From $D$\Hyph модуля $V$
будет такое подмножество $X\subset V$, что
\ShowEq{generating set of module}
\qed
\end{definition}
}

\AddEq{remark: generating set of module}
{
Следующее определение является следствием теорем
\RefTheorem{set of vectors generated by set of vectors, \SideWS module},
\RefTheorem[\RefRepresentation]{structure of subrepresentations}
и определения
\RefDefinition[\RefRepresentation]{generating set of representation}.
}

\AddEq{remark: basis of module}
{
Следующее определение является следствием теорем
\RefTheorem{set of vectors generated by set of vectors, \SideWS module},
\RefTheorem[\RefRepresentation]{structure of subrepresentations}
и определения
\RefDefinition[\RefRepresentation]{basis of representation}.
}

\AddEq{definition: basis of module}
{
\begin{definition}
\labelDefinition{basis of \SideWS module}
Если множество $X\subset V$ является множеством образующих
\SideRu\From $D$\Hyph модуля $V$, то любое множество $Y$, $X\subset Y\subset V$
также является множеством образующих \SideRu\From $D$\Hyph модуля $V$.
Если существует минимальное множество $X$, порождающее
\SideRu\To $D$\Hyph модуль $V$, то такое множество $X$ называется
\AddIndex{базисом \SideRu\From $D$\Hyph модуля}{basis, module} $V$.
\qed
\end{definition}
}

\AddEq{theorem: linearly depends on rest of vectors}
{
\begin{theorem}
\labelTheorem{linearly depends on rest of vectors, \SideWS module}
Пусть $\Base$ - \Algebra.
Если уравнение
\ShowEq{\SideWS wi vi=0}
предполагает существования индекса
\ShowEq{i=j}
такого, что
\ShowEq{wj ne 0},
то вектор $v_{\gij}$
линейно зависит от остальных векторов $v$.
\end{theorem}
}

\AddEq{proof: linearly depends on rest of vectors}
{
\begin{proof}
Теорема является следствием равенства
\ShowEq{\SideWS vj=sum vi}v
и определения
\RefDefinition{\SideWS linear combination of vectors}.
\end{proof}
}

\AddEq{remark: 0=0vi}
{
Очевидно, что для любого множества векторов $v_{\gii}$,
\ShowEq{\SideWS 0=0vi}
}

\AddEq{remark: scalars and vectors as matrix}
{
Представим множество $\Base_{(1)}$\Hyph чисел
\ShowEq{wi}
в виде матрицы
\ShowEq{w=wi}
Представим множество векторов
\ShowEq{set vi}
в виде матрицы
\ShowEq{v=vi}
Тогда мы можем записать линейную комбинацию векторов
\ShowEq{w=wi vi\SideNS}
в виде
\ShowEq{w=w cr v}
}

\AddEq{definition: linearly independent vectors}
{
\begin{definition}
\labelDefinition{\SideWS linearly independent vectors}
{\it
Множество векторов\,\footnote{
Я следую определению в
\citeBib{Serge Lang}, страница 100.}
\ShowEq{set vi}
\SideRu\From $\Base$\Hyph модуля $V$
\AddIndex{линейно независимо}{linearly independent set},
если $w=0$ следует из уравнения
\ShowEq{\SideWS wi vi=0}
В противном случае, множество векторов
\ShowEq{set vi}
\AddIndex{линейно зависимо}{linearly dependent set}.
}
\qed
\end{definition}
}

\AddEq{theorem: basis of module}
{
\begin{theorem}
\labelTheorem{basis of \SideWS module}
Множество векторов
\ShowEq{basis for module over algebra}
является базисом \SideRu\From $\Base$\Hyph модуля
$V$, если верны следующие утверждения.
\StartLabelItem
\begin{enumerate}
\item
\labelItem{vector is linear combination of set, \SideWS module}
Произвольный вектор $v\in V$
является линейной комбинацией
векторов множества $\Basis e$.
\item
\labelItem{cannot be represented as a linear combination, \SideWS module}
Вектор $e_{\gii}$
нельзя представить в виде линейной комбинации
остальных векторов множества $\Basis e$.
\end{enumerate}
\end{theorem}
}

\DefProof{basis of module}
{
Согласно утверждению
\RefItem{vector is linear combination of set, \SideWS module},
теореме
\RefTheorem{set of vectors generated by set of vectors, \SideWS module}
и определению
\RefDefinition{\SideWS linear combination of vectors},
множество $\Basis e$ порождает \SideRu\To $\Base$\Hyph модуль $V$
(определение
\RefDefinition{generating set of \SideWS module}).
Согласно утверждению
\RefItem{cannot be represented as a linear combination, \SideWS module},
множество $\Basis e$ является минимальным множеством,
порождающим \SideRu\To $\Base$\Hyph модуль $V$.
Согласно определению
\RefDefinition{basis of \SideWS module},
множество $\Basis e$ является базисом  \SideRu\From $\Base$\Hyph модуля $V$.
}

\AddEq{theorem: division algebra, basis}
{
\begin{theorem}
\labelTheorem{division algebra, \SideWS basis}
Пусть $\Base$ - \Algebra.
Множество векторов
\ShowEq{basis, module}
является
\AddIndex{базисом \SideRu\From $\Base$\Hyph векторного пространства}{basis, vector space}
$V$, если векторы $e_{\gii}$ линейно независимы и любой вектор $v\in V$
линейно зависит от векторов $e_{\gii}$.
\end{theorem}
}

\DefProof{division algebra, basis}
{
Пусть множество векторов
\ShowEq{ei, i in I}
линейно зависимо. Тогда в равенстве
\DrawEq[w]{c*e=0, \SideWS module}{}
существует индекс $\gii=\gij$ такой, что
\ShowEq{wj ne 0}.
Согласно теореме
\RefTheorem{linearly depends on rest of vectors, \SideWS module},
вектор $e_{\gij}$
линейно зависит от остальных векторов множества $\Basis e$.
Согласно определению
\RefDefinition{basis of \SideWS module},
множество векторов
\ShowEq{ei, i in I}
не является базисом \SideRu\From $\Base$\Hyph векторного пространства $V$.

Следовательно, если множество векторов
\ShowEq{ei, i in I}
является базисом, то эти векторы
линейно независимы.
Так как произвольный вектор $v\in V$
является линейной комбинацией векторов
\ShowEq{ei, i in I},
то множество векторов $v$,
\ShowEq{ei, i in I}
не является линейно независимым.
}

\AddEq{convention: we use separate color for index of element}
{
\begin{convention}
\labelConvention{we use separate color for index of element}
Пусть $A$ - свободная алгебра
с конечным или счётным базисом.
При разложении элемента алгебры $A$ относительно базиса $\Basis e$
мы пользуемся одной и той же корневой буквой для обозначения этого
элемента и его координат.
В выражении $a^2$ не ясно - это компонента разложения элемента
$a$ относительно базиса или это операция возведения в степень.
Для облегчения чтения текста мы будем индекс элемента алгебры выделять
цветом. Например,
\ShowEq{Expansion relative basis in algebra}
\qed
\end{convention}
}

\AddEq{convention: unit of algebra in basis}
{
\begin{convention}
Пусть $\Basis e$ - базис свободной алгебры $A$ над кольцом $D$.
Если алгебра $A$ имеет единицу,
положим $e_{\gi 0}$ - единица алгебры $A$.
\qed
\end{convention}
}

\DefDefinition{linear map from D1 A1 to D2 A2, module}
{
Морфизм представлений
\ShowEq{h:D1->D2 f:A1->A2}h\Base fV
$D_1$\Hyph модуля $A_1$
в $D_2$\Hyph модуль $A_2$
называется
\AddIndex{линейным отображением}{linear map}
$D_1$\Hyph модуля $A_1$ в $D_2$\Hyph модуль $A_2$.
Обозначим
\ShowEq{set linear maps, D12 module}
множество линейных отображений
$D_1$\Hyph модуля $A_1$ в $D_2$\Hyph модуль $A_2$.
}

\ifx\texFuture\Defined
\AddEq{linear map from D1 A1 to D2 A2, module}
{
\begin{definition}
\labelDefinition{linear map from D1 A1 to D2 A2, \SideNS module}
{\it
Морфизм представлений
\ShowEq{h:D1->D2 f:A1->A2}h\Base fV
\SideRu\From $D_1$\Hyph модуля $A_1$
в \SideRu\To $D_2$\Hyph модуль $A_2$
называется
\AddIndex{линейным отображением}{linear map}
\SideRu\From $D_1$\Hyph модуля $A_1$ в \SideRu\To $D_2$\Hyph модуль $A_2$.

Обозначим
\ShowEq{set linear maps, D12 module}
множество линейных отображений
$D_1$\Hyph модуля $A_1$ в $D_2$\Hyph модуль $A_2$.
}
\qed
\end{definition}
}
\fi

\DefEq
{
\begin{definition}
\labelDefinition{linear map from A1 to A2, commutative module}
Пусть $A_1$, $A_2$ - $D$\Hyph модули.
Морфизм представлений
\ShowEq{f:A->B}f{A_1}{A_2}
$D$\Hyph модуля $A_1$
в $D$\Hyph модуль $A_2$
называется
\AddIndex{линейным отображением}{linear map}
$D$\Hyph модуля $A_1$ в $D$\Hyph модуль $A_2$.
Обозначим
\ShowEq{set linear maps, module}
множество линейных отображений
$D$\Hyph модуля $A_1$ в $D$\Hyph модуль $A_2$.
\qed
\end{definition}
}
{definition: linear map from A1 to A2, commutative module}
%\DefEq

\DefEq
{
\begin{theorem}
\labelTheorem{linear map from A1 to A2, commutative module}
Линейное отображение
\ShowEq{f:A->B}f{A_1}{A_2}
$D$\Hyph модуля $A_1$
в $D$\Hyph модуль $A_2$
удовлетворяет равенствам\,\footnote{В некоторых книгах
(например, \citeBib{Serge Lang}, с. 94) теорема \RefTheorem{linear map from A1 to A2, commutative module}
рассматривается как определение.}
\ShowEq{linear map from A1 to A2, 1}
\end{theorem}
}
{theorem: linear map from A1 to A2, commutative module}
%\DefEq

\DefEq
{
\begin{theorem}
\labelTheorem{set of A->B is D module}
Пусть $A$ - банаховый $D$\Hyph модуль с нормой $|x|_A$.
Пусть $B$ - банаховый $D$\Hyph модуль с нормой $|y|_B$.
\StartLabelItem
\begin{enumerate}
\item
Множество
$B^A$
отображений
\ShowEq{f:A->B}fAB
является $D$\Hyph модулем.
\labelItem{set of A->B is D module}
\item
Отображение
\ShowEq{f in BA->|f|}
определённое равенством
\ShowEq{norm of map}
\ShowEq{norm of map, algebra}
является нормой в $D$\Hyph модуле $B^A$
и величина
\ShowEq{show|f|}
называется
\AddIndex{нормой отображения $f$}{norm of map}.
\labelItem{norm of map}
\end{enumerate}
\end{theorem}
}
{theorem: set of A->B is D module}
%\DefEq

\DefDefinition{coordinates of vector 2016}
{
Пусть $\Basis e$ - базис \SideRu\From $\Base$\Hyph модуля $V$,
и вектор
\ShowEq{vv in V}
имеет разложение
\DrawEq{vv=ve \SideWS module}{}
относительно базиса $\Basis e$.
$\Base$\Hyph числа $v^{\gii}$ называются
\AddIndex{координатами}{coordinates}
вектора $\Vector v$ относительно базиса $\Basis e$.
\ePrints{1610.309618526,CACAA.06}
\ifx\Semafor\ValueOn
Матрица $\Base$\Hyph чисел
\ShowEq{coordinate matrix of vector}
называется
\AddIndex{координатной матрицей вектора}{coordinate matrix of vector}
$\Vector v$ в базисе $\Basis e$.
\fi
}

\AddEq{definition: coordinates of vector}
{
\begin{definition}
\labelDefinition{coordinates of vector, \SideWS module}
{\it
Пусть $\Basis e$ - базис \SideRu\From $\Base$\Hyph модуля $V$,
и вектор
\ShowEq{vv in V}
имеет разложение
\DrawEq{vv=ve \SideWS module}{}
относительно базиса $\Basis e$.
$\Base_{(1)}$\Hyph числа $v^{\gii}$ называются
\AddIndex{координатами}{coordinates}
вектора $\Vector v$ относительно базиса $\Basis e$.
Матрица $\Base_{(1)}$\Hyph чисел
\ShowEq{coordinate matrix of vector}
называется
\AddIndex{координатной матрицей вектора}{coordinate matrix of vector}
$\Vector v$ в базисе $\Basis e$.
}
\qed
\end{definition}
}

\AddEq{theorem: linear dependence between vectors of basis}
{
\begin{theorem}
\labelTheorem{linear dependence between vectors of basis, \SideWS module}
Пусть $\Base$ - \algebra.
Пусть $\Basis e$ - базис \SideRu\From $\Base$\Hyph модуля $V$.
Пусть
\DrawEq[w]{c*e=0, \SideWS module}{1}
линейная зависимость векторов базиса $\Basis e$.
Тогда
\StartLabelItem
\begin{enumerate}
\item
$\Base_{(1)}$\Hyph число
\ShowEq{wi i in I}
не имеет обратного элемента
в \algebraa $\Base_{(1)}$.
\item
Множество $\Base'$ матриц
\ShowEq{w=wi i in I}
порождает \SideRu\To $\Base$\Hyph модуль.
\end{enumerate}
\end{theorem}
}

\DefProof{linear dependence between vectors of basis}
{
Допустим существует матрица
\ShowEq{w=wi i in I}
такая, что равенство
\eqRef{c*e=0, \SideWS module}{1}
верно и существует индекс
\ShowEq{i=j}
такой, что
\ShowEq{wj ne 0}.
Если мы положим, что $\Base_{(1)}$\Hyph число $c^{\gij}$
имеет обратный, то равенство
\ShowEq{\SideWS vj=sum vi}e
является следствием равенства
\eqRef{c*e=0, \SideWS module}{1}.
Следовательно вектор $e_{\gij}$
является линейной комбинацией остальных векторов множества $\Basis e$
и множество $\Basis e$ не является базисом.
Следовательно, наше предположение неверно,
и $\Base_{(1)}$\Hyph число $c^{\gij}$ не имеет обратного.

Пусть матрицы
\ShowEq{b in D'}b,
\ShowEq{b in D'}c.
Из равенств
\DrawEq[b]{c*e=0, \SideWS module}{}
\DrawEq[c]{c*e=0, \SideWS module}{}
следует
\ShowEq{(b+c)*e, \SideWS module}
Следовательно, множество $\Base'$ является абелевой группой.

Пусть матрица
\ShowEq{b in D'}c{}
и $a\in\Base$.
Из равенства
\DrawEq[c]{c*e=0, \SideWS module}{}
следует
\ShowEq{(ac)*e, \SideWS module}
Следовательно, абелевая группа $\Base'$ является \SideRu\What $\Base$\Hyph модулем.
}

\AddEq{theorem: coordinates of vector with linear dependence}
{
\begin{theorem}
\labelTheorem{coordinates of vector with linear dependence, \SideWS module}
Пусть \SideRu\To $\Base$\Hyph модуль $V$
имеет базис $\Basis e$ такой, что в равенстве
\DrawEq[w]{c*e=0, \SideWS module}{2}
существует индекс
\ShowEq{i=j}
такой, что
\ShowEq{wj ne 0}.
Тогда
\StartLabelItem
\begin{enumerate}
\item
Матрица
\ShowEq{w=wi i in I}
определяет координаты вектора $0\in V$ относительно базиса $\Basis e$.
\labelItem{coordinates of vector 0 with linear dependence, \SideWS module}
\item
Координаты вектора $\Vector v$ относительно базиса $\Basis e$
определены однозначно с точностью до выбора координат вектора $0\in V$.
\labelItem{coordinates of vector with linear dependence, \SideWS module}
\end{enumerate}
\end{theorem}
}

\DefProof{coordinates of vector with linear dependence}
{
Утверждение
\RefItem{coordinates of vector 0 with linear dependence, \SideWS module}
является следствием равенства
\eqRef{c*e=0, \SideWS module}{2}
и определения
\RefDefinition{coordinates of vector, \SideWS module}.

Пусть вектор $\Vector v$ имеет разложение
\DrawEq{vv=ve \SideWS module}{2}
относительно базиса $\Basis e$.
Равенство
\ShowEq{v=v+0, \SideWS module}
является следствием равенств
\eqRef{c*e=0, \SideWS module}{2},
\eqRef{vv=ve \SideWS module}{2}.
Утверждение
\RefItem{coordinates of vector with linear dependence, \SideWS module}
является следствием равенств
\eqRef{vv=ve \SideWS module}{2},
\EqRef{v=v+0, \SideWS module}
и определения
\RefDefinition{coordinates of vector, \SideWS module}.
}

\AddEq{definition: free module over ring}
{
\begin{definition}
\labelDefinition{free \SideWS module}
\SideRuC\To $\Base$\Hyph модуль $V$ -
\AddIndex{свободный \SideRu\To $\Base$\Hyph модуль}{free module},\,\footnote{
Я следую
определению в \citeBib{Serge Lang}, страница 103.}
если \SideRu\To $\Base$\Hyph модуль $V$ имеет базис
и векторы базиса линейно независимы.
\qed
\end{definition}
}

\AddEq{theorem: coordinates of vector of free module}
{
\begin{theorem}
\labelTheorem{coordinates of vector of free \SideWS module}
Координаты вектора $v\in V$ относительно базиса $\Basis e$
свободного \SideRu\From $\Base$\Hyph модуля $V$
определены однозначно.
\end{theorem}
}

\DefProof{coordinates of vector of free module}
{
Теорема является следствием теоремы
\RefTheorem{coordinates of vector with linear dependence, \SideWS module}
и определений
\RefDefinition{\SideWS linearly independent vectors},
\RefDefinition{free \SideWS module}.
}

\DefTheorem{standard representation of map A1 A2, associative algebra}
{
Пусть $A_1$ - свободный $D$\Hyph модуль.
Пусть $A_2$ - свободная конечно мерная ассоциативная $D$\Hyph алгебра.
Пусть $\Basis e$ - базис $D$\Hyph модуля $A_2$.
Пусть $\Basis F$
- базис левого \BoxB{A_2}модуля
\ShowEq{L(A;B)}D{A_1}{A_2}.\,\footnote{
Если $D$\Hyph модуль $A_1$ или $D$\Hyph модуль $A_2$
не является свободным $D$\Hyph модулем,
то мы будем рассматривать множество
\ShowEq{Ik 1n}
линейно независимых линейных отображений. Теорема верна для любого линейного отображения
\ShowEq{f:A->B}f{A_1}{A_2}
порождённого множеством линейных отображений $\Basis F$.
}
\StartLabelItem
\begin{enumerate}
\item
Отображение
\ShowEq{f:A->B}f{A_1}{A_2}
имеет следующее разложение
\labelItem{map f generated by basis I}
\DrawEq{map f generated by basis I}{expansion}
где
\ShowEq{fk= in A2xA2}
\item
Отображение $f$ имеет стандартное представление
\labelItem{standard representation of map A1 A2, associative algebra}
\ShowEq{standard representation of map A1 A2, associative algebra}
\end{enumerate}
}

\DefDefinition{component of linear map}
{
Выражение
\ShowEq{component of linear map}
в равенстве
\eqRef{map f generated by basis I}{expansion}
называется
\AddIndex{компонентой линейного отображения}
{component of linear map} $f$.
Выражение
\ShowEq{standard component of linear map}
в равенстве
\EqRef{standard representation of map A1 A2, associative algebra}
называется \AddIndex{стандартной компонентой линейного отображения}
{standard component of linear map} $f$.
}

\DefEq
{
\begin{proof}
Поскольку $\Basis F$ является базисом левого \BoxB{A_2}модуля
\ShowEq{L(A;B)}D{A_1}{A_2},
то согласно определению
\ShowEq{ref definition: basis of representation}
и теореме
\RefTheorem{set of vectors generated by set of vectors, \SideWS module},
существует разложение
\ShowEq{expansion of linear map with respect to basis}
линейного отображения $f$ относительно базиса $\Basis I$.
Согласно определению
\ShowEq{ref map j, representation, tensor product}
\ShowEq{f=fkxfk}
Равенство
\eqRef{map f generated by basis I}{expansion}
является следствием равенств
\EqRef{expansion of linear map with respect to basis},
\EqRef{f=fkxfk}.
Согласно теореме
\RefTheorem{standard component of tensor, algebra},
стандартное представление тензора $f^k$ имеет вид
\ShowEq{standard representation of map A1 A2, 3, associative algebra}
Равенство
\EqRef{standard representation of map A1 A2, associative algebra}
следует из равенств
\eqRef{map f generated by basis I}{expansion},
\EqRef{standard representation of map A1 A2, 3, associative algebra}.
\end{proof}
}
{proof: standard representation of map A1 A2, associative algebra}
%\DefEq

\DefTheorem{Free Algebra over Ring}
{
Представление
\ShowEq{endomorphism of module from product}
$D$\Hyph модуля $A$ в $D$\Hyph модуле $A$
эквивалентно структуре $D$\Hyph алгебры $A$.
}

\DefEq
{
Пусть $D$ - коммутативное кольцо и $A$ - абелевая группа.
%Мы сперва рассматриваем вертикальное представление,
%а затем горизонтальные.
Диаграмма представлений
\DrawEq[{}{}{}g]{diagram of representations of D algebra}{}
порождает структуру $D$\Hyph алгебры $A$.
}
{text: Free Algebra over Ring}

\AddEq [2]{definition: linear map of A module}
{
\begin{definition}
\labelDefinition{linear map of #1 A module}
{\it
Пусть $V$ и
$W$ - {#2}вые $A$\Hyph модули.
Отображение
\ShowEq{f:A->B}fVW
назывется
\AddIndex{линейным отображением}{linear map},
если отображение $f$
является линейным отображением
$D$\Hyph модуля $V$ в $D$\Hyph модуль $W$.
Обозначим
\ShowEq{set linear maps, D vector space}
множество линейных отображений
{#2}вого $A$\Hyph модуля $V$ в {#2}вый $A$\Hyph модуль $W$.
}
\qed
\end{definition}
}

\DefTheorem{linear map of A module}
{
Линейное отображение
\ShowEq{f:A->B}fVW
относительно базиса \eV V
левого $A$\Hyph модуля $V$ и
базиса \eV W
левого $A$\Hyph модуля $W$
имеет вид
\ShowEq{linear map in A module}
где $f_{\gi i}^{\gi j}\circ v^{\gi i}$ линейно зависят от
одной переменной $v^{\gi i}$ и не зависят от остальных
координат вектора
\ShowEq{v=veV}
}

\DefProof{linear map of A module}
{
Согласно определению
\RefDefinition{linear map of A module}
\ShowEq{vector expansion, linear map, D vector space, 1}
Для любого заданного $\gi i$ вектор
\ShowEq{vector expansion, linear map, D vector space, 2}
имеет единственное разложение
\ShowEq{vector expansion, linear map, D vector space, 3}
относительно базиса \eV W.
Из равенств
\begin{align*}
A_{\gi i}^{\gi j}(v^{\gi i}_1+v^{\gi i}_2)&=
A_{\gi i}^{\gi j}(v^{\gi i}_1)+A_{\gi i}^{\gi j}(v^{\gi i}_2)
\\
A_{\gi i}^{\gi j}(pv^{\gi i})&=
pA_{\gi i}^{\gi j}(v^{\gi i})\ \ \ p\in F
\end{align*}
следует, что отображение
\[A_{\gi i}^{\gi j}:D\rightarrow D\]
линейно.
Следовательно, мы можем пользоваться записью
\ShowEq{Aij vj}
Равенство
\EqRef{linear map in vector space}
является следствием равенств
\EqRef{vector expansion, linear map, D vector space, 1},
\EqRef{vector expansion, linear map, D vector space, 3},
\EqRef{Aij vj}.
}

\DefTheorem{representation of algebra An in LAnA}
{
Рассмотрим $D$\Hyph алгебру $A$.
Представление
\ShowEq{representation An in LAnA}
алгебры $\AOn$
в модуле $\LAnA$,
определённое равенством
\DrawEq{representation An in LAnA, 1}{}
позволяет отождествить тензор
\ShowEq{product in algebra An 1}
и перестановку $\sigma\in S^n$
с отображением
\ShowEq{product in algebra An 2} где
\ShowEq{product in algebra AA 3}
- тождественное отображение.
}

\AddEq{definition: linear map from A1 to A2, algebra}
{
\begin{definition}
\labelDefinition{linear map from A1 to A2, algebra}
Пусть $A_1$ и
$A_2$ - алгебры над коммутативным кольцом $D$.
Линейное отображение
$D_{\DF}$\Hyph модуля $A_\VF$
в $D_{\DT}$\Hyph модуль $A_\VT$
называется
\AddIndex{линейным отображением}{linear map}
$D_{\DF}$\Hyph алгебры $A_\VF$ в $D_{\DT}$\Hyph алгебру $A_\VT$.

Обозначим
\ShowEq{set linear maps, module}
множество линейных отображений
$D$\Hyph алгебры
$A_\VF$
в $D$\Hyph алгебру
$A_\VT$.
\qed
\end{definition}
}

\DefTheorem{linear map times constant, algebra}
{
Пусть отображение
\ShowEq{f:A->B}f{A_1}{A_2}
является линейным отображением $D$\Hyph алгебры $A_1$ в $D$\Hyph алгебру $A_2$.
Тогда отображения
\ShowEq{linear map times constant, algebra}
определённые равенствами
\ShowEq{linear map times constant, 0, algebra}
также являются линейными.
}

\DefTheorem{linear map AA LAA}
{
\ePrints{1502.04063}
\ifx\Semafor\ValueOn
Рассмотрим $D$\Hyph алгебры $A_1$ и $A_2$.
Для заданного отображения
\ShowEq{f in L(A->B)}{A_1}{A_2}{}
\else
Для заданного отображения
\ShowEq{f in L(A->B)}{A_1}{A_2}{}
$D$\Hyph алгебры $A_1$ в $D$\Hyph алгебру $A_2$
\fi
существует линейное отображение
\ShowEq{linear map AA LAA}
определённое равенством
\ShowEq{linear map AA LAA, 1}
}

\DefEq
{
\begin{theorem}
\labelTheorem{conjugation transformation}
Пусть $A_1$ - свободный $D$\Hyph модуль.
Пусть $A_2$ - свободная ассоциативная $D$\Hyph алгебра.
Пусть $\Basis F$ - базис левого \BoxB{A_2}модуля
\ShowEq{L(A;B)}D{A_1}{A_2}.
Для любого отображения
\ShowEq{Ik in I}
существует множество линейных отображений
\ShowEq{conjugation transformation}
\ShowEq{conjugation transformation:}
$D$\Hyph модуля
$A_1\otimes A_1$
в $D$\Hyph модуль
$A_2\otimes A_2$
таких, что
\ShowEq{conjugation transformation =}
Отображение
\ShowEq{show conjugation transformation}
называется
\AddIndex{преобразованием сопряжения}{conjugation transformation}.
\end{theorem}
}
{theorem: conjugation transformation}
%\DefEq

\DefEq
{
\begin{proof}
Согласно теореме
\RefTheorem{product of linear map, algebra},
для произвольного тензора
$a\in A_1\otimes A_1$,
отображение
\ShowEq{x->Ik a x}
является линейным.
Согласно утверждению
\RefItem{map f generated by basis I},
существует разложение
\ShowEq{expansion Ik a x}
Положим
\ShowEq{b=Ikl a}
Равенство
\EqRef{conjugation transformation =}
является следствием равенств
\EqRef{expansion Ik a x},
\EqRef{b=Ikl a}.
Из равенств
\ShowEq{Ikl a1+a2}
\ShowEq{Ikl d a}
следует, что отображение $I_k^l$ является линейным.
\end{proof}
}
{proof: conjugation transformation}
%\DefEq

\DefEq
{
\begin{theorem}
\labelTheorem{representation of composition of linear maps}
Пусть $A_1$ - свободный $D$\Hyph модуль.
Пусть $A_2$, $A_3$ - свободные ассоциативные $D$\Hyph алгебры.
Пусть $\Basis F$ - базис левого \BoxB{A_2}модуля
\ShowEq{L(A;B)}D{A_1}{A_2}.
Пусть $\Basis G$ - базис левого \BoxB{A_3}модуля
\ShowEq{L(A;B)}D{A_2}{A_3}.
\StartLabelItem
\begin{enumerate}
\item
Множество отображений
\labelItem{basis of composition of linear maps}
\DrawEq{JlIk}{linear map}
является базисом левого \BoxB{A_3}модуля
\ShowEq{L(A;B)}D{A_1\rightarrow A_2}{A_3}.
\item
Пусть линейное отображение
\ShowEq{f:A->B}f{A_1}{A_2}
имеет разложение
\ShowEq{expansion of f with respect to basis I}
относительно базиса $\Basis I$.
Пусть линейное отображение
\ShowEq{f:A->B}g{A_2}{A_3}
имеет разложение
\ShowEq{expansion of g with respect to basis J}
относительно базиса $\Basis J$.
Тогда линейное отображение
\DrawEq{h=g o f}{123}
имеет разложение
\labelItem{hlk=glfk}
\ShowEq{expansion of h with respect to basis K}
относительно базиса $\Basis K$, где
\ShowEq{hlk=glfk}
\end{enumerate}
\end{theorem}
}
{theorem: representation of composition of linear maps}
%\DefEq

\DefEq
{
\begin{proof}
Равенство
\ShowEq{h(a)1}
является следствием равенств
\EqRef{expansion of f with respect to basis I},
\EqRef{expansion of g with respect to basis J},
\eqRef{h=g o f}{123}.
Равенство
\ShowEq{h(a)2}
является следствием равенств
\eqRef{JlIk}{linear map},
\EqRef{h(a)1}
и теоремы
\RefTheorem{conjugation transformation}.
Из равенства
\EqRef{h(a)2}
следует, что множество отображений $\Basis K$ порождает
левый \BoxB{A_3}модуля\newline
\ShowEq{L(A;B)}D{A_1\rightarrow A_2}{A_3}.
Из равенства
\ShowEq{aK=aJI}
следует, что
\ShowEq{aJ=0}
и, следовательно, $a^{lk}=0$.
Следовательно, множество $\Basis K$ является базисом
левого \BoxB{A_3}модуля
\ShowEq{L(A;B)}D{A_1\rightarrow A_2}{A_3}.
\end{proof}
}
{proof: representation of composition of linear maps}
%\DefEq

\DefEq
{
\begin{theorem}
\labelTheorem{representation of composition of linear maps A->A}
Пусть $A$ - свободная ассоциативная $D$\Hyph алгеба.
Пусть левый \BoxB{A}модуль
\ShowEq{L(A;B)}DAA{}
порождён тождественным отображением $F_0=\delta$.
Пусть линейное отображение
\ShowEq{f:A->B}fAA
имеет разложение
\ShowEq{expansion of f A->A}
Пусть линейное отображение
\ShowEq{f:A->B}gAA
имеет разложение
\ShowEq{expansion of g A->A}
Тогда линейное отображение
\DrawEq{h=g o f}{A}
имеет разложение
\ShowEq{expansion of h A->A}
где
\ShowEq{hlk=glfk 01}
\end{theorem}
}
{theorem: representation of composition of linear maps A->A}
%\DefEq

\DefEq
{
\begin{proof}
Равенство
\ShowEq{h(a)}
является следствием равенств
\EqRef{expansion of f A->A},
\EqRef{expansion of g A->A},
\eqRef{h=g o f}{A}.
Равенство
\EqRef{hlk=glfk 01}
является следствием равенства
\EqRef{h(a)}.
\end{proof}
}
{proof: representation of composition of linear maps A->A}
%\DefEq

\DefTheorem{linear map in L(A,A), associative algebra}
{
Пусть $A_1$ - $D$\Hyph алгебра.
Пусть $A_2$ - свободная конечно мерная ассоциативная $D$\Hyph алгебра.
Пусть $\Basis e$ - базис $D$\Hyph модуля $A_2$.
Левый \BoxB{A_2}модуль
\ShowEq{L(A;B)}D{A_1}{A_2}{}
имеет конечный
\AddIndex{базис}{basis of algebra L(A,A)} $\Basis I$.
\StartLabelItem
\begin{enumerate}
\item
Линейное отображение
\ShowEq{f in L(A->B)}{A_1}{A_2}{}
имеет вид
\labelItem{f in L(A,A), 1, associative algebra}
\ShowEq{f in L(A,A), 1, associative algebra}
\item
Его стандартное представление имеет вид
\labelItem{f in L(A,A), 2, associative algebra}
\ShowEq{f in L(A,A), 2, associative algebra}
\end{enumerate}
}

\DefEq
{
\begin{theorem}
\labelTheorem{h generated by f, associative algebra}
Рассмотрим $D$\Hyph алгебру $A_1$
и ассоциативную $D$\Hyph алгебру $A_2$.
Рассмотрим представление алгебры $\ATwo$
в модуле $\mathcal L(D;A_1;A_2)$.
Отображение
\ShowEq{h:A1->A2}
порождённое отображением
\ShowEq{f:A->B}f{A_1}{A_2}
имеет вид
\ShowEq{h generated by f, associative algebra}
\end{theorem}
}
{theorem: h generated by f, associative algebra}
%\DefEq

\DefEq
{
\begin{theorem}
\labelTheorem{coordinates of map A1 A2, algebra}
Пусть $\Basis e_1$ - базис свободного конечно мерного
$D$\Hyph модуля $A_1$.
Пусть $\Basis e_2$ - базис свободной конечно мерной ассоциативной
$D$\Hyph алгебры $A_2$.
Пусть
\ShowEq{structural constants, algebra}
- структурные константы алгебры $A_2$.
Пусть $\Basis F$ - базис
левого \BoxB{A_2}модуля
\ShowEq{L(A;B)}D{A_1}{A_2}{}
и
\ShowEq{coordinates of map Ik}
- координаты отображения $F_k$ относительно базисов $\Basis e_1$ и $\Basis e_2$.
Координаты
\ShowEq{Coordinates of map f}
отображения
\ShowEq{f in L(A->B)}{A_1}{A_2}{}
и его стандартные компоненты
\ShowEq{standard components of map f}
связаны равенством
\ShowEq{coordinates of map A1 A2, 2, associative algebra}
\end{theorem}
}
{theorem: coordinates of map A1 A2, algebra}
%\DefEq

\DefEq
{
\begin{proof}
Относительно базисов
$\Basis e_1$ и $\Basis e_2$, линейные отображения $f$ и $I_k$ имеют вид
\ShowEq{coordinates of map f, associative algebra}
\ShowEq{coordinates of map Ik, associative algebra}
Равенство
\ShowEq{coordinates of map A1 A2, 3, associative algebra}
является следствием равенств
\EqRef{standard representation of map A1 A2, associative algebra},
\EqRef{coordinates of map f, associative algebra},
\EqRef{coordinates of map Ik, associative algebra}.
Так как векторы $\Vector e_{2\cdot\gik}$
линейно независимы и $x^{\gi i}$ произвольны,
то равенство
\EqRef{coordinates of map A1 A2, 2, associative algebra}
следует из равенства
\EqRef{coordinates of map A1 A2, 3, associative algebra}.
\end{proof}
}
{proof: coordinates of map A1 A2, algebra}
%\DefEq

\DefEq
{
\begin{theorem}
\labelTheorem{sum of linear maps, D module}
Пусть $A_1$, $A_2$ - $D$\Hyph модули.
Отображение
\ShowEq{sum of maps,,D module}
\ShowEq{sum of maps, 1, D module}
определённое равенством
\ShowEq{sum of maps, D module}
называется
\AddIndex{суммой отображений}{sum of maps}
$f$ и $g$
и является линейным отображением.
Множество
$\mathcal L(D;A_1;A_2)$
является абелевой группой
относительно суммы отображений.
\end{theorem}
}
{theorem: sum of linear maps, D module}
%\DefEq

\DefEq
{
\begin{theorem}
\labelTheorem{sum of polylinear maps, module}
Пусть $D$ - коммутативное кольцо.
Пусть $A_1$, ..., $A_n$, $S$ - $D$\Hyph модули.
Отображение
\ShowEq{sum of maps,,polylinear}
\ShowEq{sum of maps, 1, polylinear}
определённое равенством
\ShowEq{sum of  maps, polylinear}
называется
\AddIndex{суммой полилинейных отображений}{sum of maps}
$f$ и $g$
и является полилинейным отображением.
Множество
\ShowEq{module of polylinear maps}
является абелевой группой
относительно суммы отображений.
\end{theorem}
}
{theorem: sum of polylinear maps, module}
%\DefEq

\AddEq{corollary: sum of linear maps, D module}
{
\begin{corollary}
\labelCorollary{sum of linear maps, D module}
Пусть $A_1$, $A_2$ - $D$\Hyph модули.
Отображение
\ShowEq{sum of maps,,D module}
\ShowEq{sum of maps, 1, D module}
определённое равенством
\ShowEq{sum of maps, D module}
называется
\AddIndex{суммой отображений}{sum of maps}
$f$ и $g$
и является линейным отображением.
Множество
$\mathcal L(D;A_1;A_2)$
является абелевой группой
относительно суммы отображений.
\qed
\end{corollary}
}

\AddEq{definition: linear map A module}
{
\begin{definition}
\labelDefinition{linear map \SideWS A module}
Пусть
\ShowEq{Ai, i=}A
- алгебра над коммутативным кольцом $D_i$.
Пусть
\ShowEq{Ai, i=}V
-
\ShowEq{\SideWS column module}{A_i}
модуль.
Морфизм диаграммы представлений
\ShowEq{A module diagram for linear}1
в диаграмму представлений
\ShowEq{A module diagram for linear}2
называется
\AddIndex{линейным отображением}{linear map}
%
\ShowEq{\SideWS column module}{A_1}
модуля $V_1$ в
\ShowEq{\SideWS column module}{A_2}
модуль $V_2$.
Обозначим
\ShowEq{set linear maps, \SideWS A12 module}
множество линейных отображений
%
\ShowEq{\SideWS column module}{A_1}
модуля $V_1$ в
\ShowEq{\SideWS column module}{A_2}
модуль $V_2$.
\qed
\end{definition}
}

\AddEq{definition: homomorphism A module}
{
\begin{definition}
\labelDefinition{homomorphism \SideWS A module}
Пусть
\ShowEq{Ai, i=}A
- алгебра над коммутативным кольцом $D_i$.
Пусть
\ShowEq{Ai, i=}V
-
\ShowEq{\SideWS column module}{A_i}
модуль.
Морфизм диаграммы представлений
\ShowEq{A module diagram for homomorphism}1
в диаграмму представлений
\ShowEq{A module diagram for homomorphism}2
называется
\AddIndex{гомоморфизмом}{homomorphism}
%
\ShowEq{\SideWS column module}{A_1}
модуля $V_1$ в
\ShowEq{\SideWS column module}{A_2}
модуль $V_2$.
Обозначим
\ShowEq{set homomorphisms, \SideWS A12 module}
множество гомоморфизмов
%
\ShowEq{\SideWS column module}{A_1}
модуля $V_1$ в
\ShowEq{\SideWS column module}{A_2}
модуль $V_2$.
\qed
\end{definition}
}

\DefTheorem{L(An;B) is free D module}
{
Пусть $A_1$, ..., $A_n$, $B$ - свободные модули над коммутативным кольцом $D$.
$D$\Hyph модуль
\ShowEq{L(A;B)}D{A_1\times...\times A_n}B{}
является свободным $D$\Hyph модулем.
}

\DefEq
{
\begin{definition}
\labelDefinition{linear map from A1 to A2, module}
Приведенный морфизм представлений
\ShowEq{f:A->B}f{A_1}{A_2}
$D$\Hyph модуля $A_1$
в $D$\Hyph модуль $A_2$
называется
\AddIndex{линейным отображением}{linear map}
\SideRu вого $D$\Hyph модуля $A_1$ в \SideRu вый $D$\Hyph модуль $A_2$.

Обозначим
\ShowEq{set linear maps, module}
множество линейных отображений
\SideRu вого $D$\Hyph модуля $A_1$ в \SideRu вый $D$\Hyph модуль $A_2$.
\qed
\end{definition}
}
{definition: linear map from A1 to A2, module}
%\DefEq

\AddEq{theorem: linear map of module}
{
\begin{theorem}
\labelTheorem{linear map from \Base\DF \Module\DF to \Base\DT \Module\DT, \SideWS module}
Линейное отображение
\ShowEq{show linear map \MapE}f
\SideRu\From $\Base_\DF$\Hyph модуля $\Module_\DF$
в \SideRu\To $\Base_\DT$\Hyph модуль $\Module_\DT$
удовлетворяет равенствам\,\footnote{
В некоторых книгах
(например, на странице \citeBib{Serge Lang}\Hyph 94) теорема
\RefTheorem{linear map from \Base\DF \Module\DF to \Base\DT \Module\DT, \SideWS module}
рассматривается как определение.}
\ShowEq{property linear map \MapE}
\end{theorem}
}

\DefProof{linear map of module}
{
Из определений
\RefDefinition[\RefRepresentation]{morphism of representations of universal algebra},
\RefDefinition{linear map from D1 A1 to D2 A2, module}
следует, что
отображение $h$ является гомоморфизмом кольца $D_1$
в кольцо $D_2$ (равенства
\eqRef{h(d1+d2)=...}{\SideWS module},
\eqRef{h(d1d2)=...}{\SideWS module})
и отображение $f$ является гомоморфизмом абелевой группы $A_1$
в абелеву группу $A_2$ (равенство
\eqRef{f(a+b)=...}{D1 D2 \SideWS module}).
Равенство
\EqRef{\DFDT, f(da)=... \SideWS module}
является следствием равенства
\EqRef[\RefRepresentation]{morphism of representations of F algebra, definition, 2m}.
%\eqRef[\RefRepresentation]{morphism of representations of universal algebra, 2m}{definition}.
}

\AddEq{theorem: linear map of module, coordinates}
{
\begin{theorem}
\labelTheorem{linear map of \SideWS \DFDT module, coordinates}
Пусть
\ShowEq{basis, module V1}
базис в свободном \SideRu\From $\Base_\DF$\Hyph модуле $\Module_1$
и
\ShowEq{basis, module V2}
базис в свободном \SideRu\From $\Base_\DT$\Hyph модуле $\Module_2$.
Тогда линейное отображение
\ShowEq{show linear map \MapE}{\Vector f}
имеет представление
\ShowEq{r2:A1->A2, \SideWS \DFDT module}
относительно заданных базисов. Здесь
\begin{itemize}
\item $a$ - координатная матрица вектора
$\Vector a$ относительно базиса $\Basis e_1$
\DrawEq [a1]{va=ae1, \SideWS module}{a \DFDT}
\def\Temp{D1 D2 }
\ifx\DFDT\Temp
\item
\ShowEq{h(a)=...}
- матрица $D_2$\Hyph чисел.
\fi
\item $b$ - координатная матрица вектора
\DrawEq{vb=f(va)}{\DFDT\SideWS module}
относительно базиса $\Basis e_2$
\DrawEq[b2]{va=ae1, \SideWS module}{b \DFDT}
\item $f$ - координатная матрица множества векторов
\ShowEq{Vector f(e1) \SideWS module}
относительно базиса $\Basis e_2$.
Мы будем называть матрицу $f$
\AddIndex{матрицей линейного отображения}{matrix of linear map}
относительно базисов $\Basis e_1$ и $\Basis e_2$.
\end{itemize}
\end{theorem}
}

\DefProof{linear map of module, coordinates}
{
Так кaк
\ShowEq{show linear map \MapE}{\Vector f}
линейное отображение, то на основании
\EqRef{\DFDT, f(da)=... \SideWS module},
\eqRef{va=ae1, \SideWS module}{a \DFDT},
\eqRef{vb=f(va)}{\DFDT\SideWS module}
следует, что
\ShowEq{\DFDT vb=h(e1)a \SideNS}
\ShowEq{f(e1) \SideNS}
является вектором свободного \SideRu\From $\Base_\DT$\Hyph модуля $V_2$ и имеет
разложение
\DrawEq{f(e1)= \SideNS}{\DFDT}
относительно базиса $\Basis e_2$.
Комбинируя \EqRef{\DFDT vb=h(e1)a \SideNS}
и \eqRef{f(e1)= \SideNS}{\DFDT}, мы получаем
\ShowEq{\DFDT vb=a f e \SideNS}
\EqRef{r2:A1->A2, \SideWS \DFDT module}
следует из сравнения
\eqRef{va=ae1, \SideWS module}{b \DFDT}
и \EqRef{\DFDT vb=a f e \SideNS} и
теоремы \RefTheorem{coordinates of vector of free \SideWS module}.
}

\DefDefinition{algebra over ring}
{
Пусть $D$ - коммутативное кольцо.
$D$\Hyph модуль $A$ называется
\AddIndex{алгеброй над кольцом}{algebra over ring} $D$
или
\AddIndex{$D$\Hyph алгеброй}{D algebra},
если определена операция произведения\,\footnote{
Я следую определению,
приведенному в
\citeBib{Richard D. Schafer}, страница 1,
\citeBib{0105.155}, страница 4. Утверждение,
верное для произвольного $D$\Hyph модуля,
верно также для $D$\Hyph алгебры.} в $A$
\DrawEq{product in D algebra}{definition}
где $C$ - билинейное отображение
\ShowEq{product in algebra, definition 1}
Если $A$ является свободным
$D$\Hyph модулем, то $A$ называется
\AddIndex{свободной алгеброй над кольцом}{free algebra over ring} $D$.
}

\DefDefinition{commutator of algebra}
{
\AddIndex{Коммутатор}{commutator of algebra}
\ShowEq{commutator of algebra}
служит мерой коммутативности в $D$\Hyph алгебре $A$.
$D$\Hyph алгебра $A$ называется
\AddIndex{коммутативной}{commutative D algebra},
если
\ShowEq{commutative D algebra}
}

\DefDefinition{nucleus of algebra}
{
\AddIndex{Ядро $D$\Hyph алгебры $A$}{nucleus of algebra}
- это
множество\,\footnote{
Определение дано на базе
аналогичного определения в
\citeBib{Richard D. Schafer}, с. 13}
\ShowEq{nucleus of algebra}
}

\DefDefinition{associator of algebra}
{
\AddIndex{Ассоциатор}{associator of algebra}
\ShowEq{associator of algebra}
служит мерой ассоциативности в $D$\Hyph алгебре $A$.
$D$\Hyph алгебра $A$ называется
\AddIndex{ассоциативной}{associative D algebra},
если
\ShowEq{associative D algebra}
}

\DefEq
{
\begin{definition}
\labelDefinition{center of algebra}
\AddIndex{Центр $D$\Hyph алгебры $A$}{center of algebra}
- это
множество\,\footnote{
Определение дано на базе
аналогичного определения в
\citeBib{Richard D. Schafer}, страница 14}
\ShowEq{center of algebra}
\qed
\end{definition}
}
{definition: center of algebra}
%\DefEq

\DefEq
{
\begin{definition}
\labelDefinition{otimes -}
Билинейное отображение
\ShowEq{otimes -}
определено равенством
\ShowEq{otimes -, 1}
\qed
\end{definition}
}
{definition: otimes -}
%\DefEq


==> Stmt.Omega.Russian.tex <==
%auto-ignore
\input{Stmt.Omega.Eq}

\DefDefinition{polyadditive map}
{
Отображение
\ShowEq{f:A->B}g{A^n}A
называется
\AddIndex{полиаддитивным отображением}{polyadditive map},
если для любого
\ShowEq{fi(a+b)=}
}

\DefDefinition{semiring of sets}
{
Непустая система множеств $\mathcal S$ называется
\AddIndex{полукольцом множеств}{semiring of sets},\,\footnote{
Смотри так же определение
\citeBib{Kolmogorov Fomin}\Hyph 2, страница 43.}
если
\ifx\setCACAA\undefined
\StartLabelItem
\else
\StartLabelItem[definition]
\fi
\begin{enumerate}
\item
\ShowEq{empty in S}
\item
Если
\ShowEq{A, B in S}
то
\ShowEq{AB in S}
\item
Если
\ShowEq{A, A1 in S},
то множество \(A\) может быть представлено в виде 
\DrawEq{A=+Ai}{def}
где
\ShowEq{Ai*Aj=0}
\labelItem{A=+Ai}
\end{enumerate}
Представление
\eqRef{A=+Ai}{def}
множества \(A\) называется
\AddIndex{конечным разложением множества}{finite expansion of set}
\(A\).
}

\DefDefinition{norm on Omega group}
{
\AddIndex{Норма на $\Omega$\Hyph группе}
{norm on Omega group} $A$\,\footnote{
Определение дано согласно определению из \citeBib{Bourbaki: General Topology: Chapter 5 - 10},
гл. IX, \S 3, п${}^\circ$2, а также согласно
определению \citeBib{Arnautov Glavatsky Mikhalev}-1.1.12,
с. 23.} - это отображение
\ShowEq{d->|d|}
такое, что
\ifx\setCACAA\undefined
\StartLabelItem
\else
\StartLabelItem[definition]
\fi
\begin{enumerate}
\ShowEq{|a|>=0}
\ShowEq{|a|=0}
равносильно $a=0$
\ShowEq{|a+b|<=|a|+|b|}
\ShowEq{|-a|=|a|}
\end{enumerate}

$\Omega$\Hyph группа $A$,
наделённая структурой, определяемой заданием на $A$ нормы, называется
\AddIndex{нормированной $\Omega$\Hyph группой}{normed Omega group}.
}

\DefTheorem{h=f1...fn omega, converges uniformly}
{
Пусть $A$ - полная $\Omega$\Hyph группа.
Пусть
\ShowEq{omega in Omega}{}{}
- $n$\Hyph арная операция.
Пусть последовательность отображений
\ShowEq{fim M(X,A)}
в полную $\Omega$\Hyph группу $A$
сходится равномерно
к отображению $f_i$.
Пусть множество значений отображения
$f_i$
компактно.
Тогда последовательность отображений
\ShowEq{hm=f1m...fnm omega}
в полную $\Omega$\Hyph группу $A$
сходится равномерно
к отображению
\DrawEq{h=f1...fn omega}{converges uniformly}
}

\DefTheorem{|int h|<int|omega||f1n|}
{
Пусть
\ShowEq{omega in Omega}{}{}
- $n$\Hyph арная операция в
абелевой \(\Omega\)\Hyph группе \(A\).
Пусть
\ShowEq{fi:X->A}
$\mu$\Hyph измеримое отображение
с компактным множеством значений.
Если отображение \(f_i\), \(i=1\), ..., \(n\),
интегрируемо, то отображение
\DrawEq{h=f1...fn omega}{}
интегрируемо и
\DrawEq{|int h|<int|omega||f1n|}{measurable}
}

\DefTheorem{h=fX g1 g2 representation}
{
Пусть на множестве $X$ определена \(\sigma\)\Hyph аддитивная мера $\mu$.
Пусть
\ShowEq{f:A->*B}g{A_1}{A_2}
представление
$\Omega_1$\Hyph группы $A_1$ с нормой $\|x\|_1$
в $\Omega_2$\Hyph группе $A_2$ с нормой $\|x\|_2$.
Пусть
\ShowEq{gi:X->A 12}
интегрируемое отображение
с компактным множеством значений.
Тогда отображение
\ShowEq{h=fX g1 g2}
интегрируемо и
\DrawEq{|int h|<int|g1||g2|}{measurable}
}

\DefTheorem{polymorphism of representations}
{
Пусть отображение
\ShowEq{map r1n,R}
является полиморфизмом
представлений $f_1$, ..., $f_n$ в представление $f$.
Для любого
\ShowEq{k,1n}
отображение
\ShowEq{map r,R}{r_{1k}}{r_2}{}
удовлетворяет равенству
\ShowEq{polymorphism of representation, ak}
Пусть $\omega_1\in\Omega_1(p)$.
Для любого
\ShowEq{k,1n}
отображение $r_{1k}$ удовлетворяет равенству
\ShowEq{polymorphism of representation, omega1}
Пусть $\omega_2\in\Omega_2(p)$.
Для любого
\ShowEq{k,1n}
отображение $r_2$ удовлетворяет равенству
\ShowEq{polymorphism of representation, omega2}
}

\DefDefinition{polymorphism of representations}
{
Пусть
\ShowEq{A1n A}
- $\Omega_1$\Hyph алгебры.
Пусть
\ShowEq{B1n}
- $\Omega_2$\Hyph алгебры.
Пусть, для любого
\ShowEq{k,1n}
\ShowEq{f:A->*B}{f_k}{A_k}{B_k}
представление $\Omega_1$\Hyph алгебры $A_k$
в $\Omega_2$\Hyph алгебре $B_k$.
Пусть
\ShowEq{f:A->*B}fAB
представление $\Omega_1$\Hyph алгебры $A$
в $\Omega_2$\Hyph алгебре $B$.
Отображение
\ShowEq{polymorphism of representation}
называется
\AddIndex{полиморфизмом представлений}
{polymorphism of representations}
$f_1$, ..., $f_n$ в представление $f$,
если, для любого
\ShowEq{k,1n}
при условии, что все переменные кроме переменных
\ShowEq{ak bk in}
имеют заданное значение, отображение
\ShowEq{map r,R}{r_{1k}}{r_2}{}
является морфизмом представления $f_k$ в представление $f$.

Если $f_1=...=f_n$, то мы будем говорить, что отображение
\ShowEq{map r1n,R}
является полиморфизмом представления $f_1$ в представление $f$.

Если $f_1=...=f_n=f$, то мы будем говорить, что отображение
\ShowEq{map r1n,R}
является полиморфизмом представления $f$.
}

\DefDefinition{Omega group}
{
Пусть в $\Omega_1$\Hyph алгебре
$A$ определена операция сложения,
которая не обязательно коммутативна.
Мы пользуемся символом $+$ для обозначения операции суммы.
Положим
\ShowEq{Omega=...-+}
Если $\Omega_1$\Hyph алгебра $A$ является группой
относительно операции сложения
и любая операция $\omega\in\Omega$
является полиаддитивным отображением,
то $\Omega_1$\Hyph алгебра $A$ называется
\AddIndex{$\Omega$\Hyph группой}{Omega group}.
Если $\Omega$\Hyph группа $A$ является ассоциативной группой
относительно операции сложения,
то $\Omega_1$\Hyph алгебра $A$ называется
\AddIndex{ассоциативной $\Omega$\Hyph группой}{associative Omega group}.
Если $\Omega$\Hyph группа $A$ является абелевой группой
относительно операции сложения,
то $\Omega_1$\Hyph алгебра $A$ называется
\AddIndex{абелевой $\Omega$\Hyph группой}{Abelian Omega group}.
}

\DefTheorem{operation is distributive over addition}
{
Пусть
\EqParm{omega n ari}{=z}
- полиаддитивное отображение.
Операция $\omega$
\AddIndex{дистрибутивна}{distributive law}
относительно сложения
\ShowEq{omega is distributive over addition}
}

\DefDefinition{multiplicative Omega group}
{
Пусть произведение
\DrawEq{c=ab}{}
является операцией $\Omega_1$\Hyph алгебры $A$.
Положим
\ShowEq{Omega=...-o}
Если $\Omega_1$\Hyph алгебра $A$ является группой
относительно произведения
и для любой операции
\EqParm{omega n ari}{=z}
умножение дистрибутивно относительно операция $\omega$
\DrawEq{a omega=omega a left}{}
\DrawEq{a omega=omega a right}{}
то $\Omega_1$\Hyph алгебра $A$ называется
\AddIndex{мультипликативной $\Omega$\Hyph группой}
{multiplicative Omega group}.
}

\DefDefinition{Abelian multiplicative Omega group}
{
Если
\ShowEq{Abelian multiplicative Omega group}
то мультипликативная $\Omega$\Hyph группа называется
\AddIndex{абелевой}{Abelian multiplicative Omega group}.
}

\DefDefinition{Omega ring}
{
Пусть сложение
\ShowEq{c1=a+b}
которое не обязательно коммутативно,
и произведение
\DrawEq{c=ab}{}
являются операциями $\Omega_1$\Hyph алгебры $A$.
Положим
\ShowEq{Omega=...-o+}
Если $\Omega_1$\Hyph алгебра $A$ является
$\Omega\cup\{*\}$\Hyph группой
и
мультипликативной $\Omega\cup\{+\}$\Hyph группой,
то $\Omega_1$\Hyph алгебра $A$ называется
\AddIndex{$\Omega$\Hyph кольцом}{Omega ring}.
}

\DefTheorem{product in Omega ring is distributive over addition}
{
Произведение в $\Omega$\Hyph кольце
\AddIndex{дистрибутивно}{distributive law}
относительно сложения
\ShowEq{a*(b1+b2)=}
}

\DefProof{product in Omega ring is distributive over addition}
{
Теорема является следствием определений
\RefDefinition{Omega group},
\RefDefinition{multiplicative Omega group},
\RefDefinition{Omega ring}.
}

\DefDefinition{matrix over Omega ring}
{
Пусть $A$ - $\Omega$\Hyph кольцо.
\AddIndex{Матрица}{matrix}
над $\Omega$\Hyph кольцом $A$ - это таблица $A$\Hyph чисел $a^i_j$,
где индекс $i$ - это номер строки
и индекс $j$ - это номер столбца.
}


==> Stmt.Representation.Russian.tex <==
%auto-ignore
\input{Stmt.Representation.Eq}

\DefDefinition{morphism of representations of universal algebra}
{
Пусть
\ShowEq{f:A->*B}f{A_1}{A_2}
представление $\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $A_2$ и 
\ShowEq{f:A->*B}g{B_1}{B_2}
представление $\Omega_1$\Hyph алгебры $B_1$
в $\Omega_2$\Hyph алгебре $B_2$.
Для
\EqParm{i=1,2}{=c}
пусть отображение
\ShowEq{ri:A->B}
является гомоморфизмом $\Omega_i$\Hyph алгебры.
Матрица отображений
\ShowEq{map r,R}{r_1}{r_2}{}
таких, что
\ShowEq{morphism of representations of universal algebra, definition, 2}
называется
\AddIndex{морфизмом представлений из $f$ в $g$}
{morphism of representations from f into g}.
Мы также будем говорить, что определён
\AddIndex{морфизм представлений $\Omega_1$\Hyph алгебры
в $\Omega_2$\Hyph алгебре}
{morphism of representations of Omega1 algebra in Omega2 algebra}.
}

\DefTheorem{reduced polymorphism of representations}
{
Пусть отображение $r_2$ - приведенный полиморфизм
эффективных представлений $f_1$, ..., $f_n$ в эффективное представление $f$.
\begin{itemize}
\item
Для любого
\ShowEq{k,1n}
отображение $r_2$ удовлетворяет равенству
\ShowEq{reduced polymorphism of representation, ak}
\item
Для любого
\ShowEq{kl,1n}
отображение $r_2$ удовлетворяет равенству
\ShowEq{reduced polymorphism of representation, akl}
\item
Пусть $\omega_2\in\Omega_2(p)$.
Для любого
\ShowEq{k,1n}
отображение $r_2$ удовлетворяет равенству
\ShowEq{reduced polymorphism of representation, omega2}
\end{itemize}
}

\DefEq
{
\begin{remark}
\labelRemark{notation for effective \SideNS-side representation of algebra}
Если \SideRu востороннее представление мультипликативной $\Omega$\Hyph группы эффективно, мы будем отождествлять
элемент мультипликативной $\Omega$\Hyph группы с его образом и записывать \SideRu востороннее преобразование,
порождённое $A_1$\Hyph числом $a_1$,
в форме
\ShowEq{effective \SideNS-side representation}
Отображение
\ShowEq{A12->A2 \SideNS}
порождённый \SideRu восторонним эффективным представлением $f$ называется
\AddIndex{\SideRu восторонним произведением}{\SideNS-side product}
$A_2$\Hyph числа на $A_1$\Hyph число.
Если представления
\ShowEq{f:A->*B}fAM
\ShowEq{f:A->*B}gBN
эффективны, то мы можем записать равенство
\eqRef{morphism of representations of universal algebra, 2m}{definition}
следующим образом
\ShowEq{morphism of \SideWS representation of Omega group}
Орбита представления $f$ имеет вид
\ShowEq{orbit of effective \SideNS-side representation}
Мы будем пользоваться обозначением
\ShowEq{space of orbits of effective \SideNS-side representation}
для пространства орбит \SideRu востороннего эффективного $A_1$\Hyph представления.
\qed
\end{remark}
}
{remark: notation for effective representation}
%DefEq

\DefDefinition{product in category}
{
Пусть $\mathcal A$ - категория.
Пусть
\ShowEq{set Bi}B
- множество объектов из $\mathcal A$.
Объект
\ShowEq{product in category}
и множество морфизмов
\ShowEq{set f:A->B}fP{B_i}
называется
\AddIndex{произведением множества объектов
\ShowEq{set Bi}B
в категории $\mathcal A$}
{product in category}\,\footnote{
Определение дано согласно \citeBib{Serge Lang},
страница 45.}, если для любого объекта $R$ и множество морфизмов
\ShowEq{set f:A->B}gR{B_i}
существует единственный морфизм
\ShowEq{f:A->B}hRP
такой, что диаграмма
\ShowEq{product in category diagram}
коммутативна для всех $i\in I$.

Если $|I|=n$, то для произведения множества объектов
$\{B_i,\Ii\}$ в $\mathcal A$
мы так же будем пользоваться записью
\ShowEq{product in category, 1 n}
}

\DefDefinition{coproduct in category}
{
Пусть $\mathcal A$ - категория.
Пусть
\ShowEq{set Bi}B
- множество объектов из $\mathcal A$.
Объект
\ShowEq{coproduct in category}
и множество морфизмов
\ShowEq{set f:A->B}f{B_i}P
называется
\AddIndex{копроизведением множества объектов
\ShowEq{set Bi}B
в категории $\mathcal A$}
{coproduct in category}\,\footnote{
Определение дано согласно \citeBib{Serge Lang}, страница 46.},
если для любого объекта $R$ и множество морфизмов
\ShowEq{set f:A->B}g{B_i}R
существует единственный морфизм
\ShowEq{f:A->B}hPR
такой, что диаграмма
\ShowEq{coproduct in category diagram}
коммутативна для всех $i\in I$.

Если $|I|=n$, то для копроизведения множества объектов
\ShowEq{set Bi}B
в $\mathcal A$
мы так же будем пользоваться записью
\ShowEq{coproduct in category, 1 n}
}

\DefTheorem{structure of subrepresentations}
{
Пусть\,\footnote{Утверждение теоремы аналогично
утверждению теоремы 5.1, \citeBib{Cohn: Universal Algebra}, страница 94.}
\ShowEq{f:A->*B}g{A_1}{A_2}
представление $\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $A_2$.
Пусть $X\subset A_2$.
Определим подмножество $X_k\subset A_2$ индукцией по $k$.
\ShowEq{structure of subrepresentations}
Тогда
\ShowEq{structure of subrepresentations, 1}
}

\DefDefinition{direct sum of Abelian groups}
{
Копроизведение в категории абелевых групп $Ab$ называется
\AddIndex{прямой суммой}{direct sum}.\,\footnote{
Определение дано согласно \citeBib{Serge Lang}, страница 55.}
Мы будем пользоваться записью
\ShowEq{direct sum of Abelian groups}
для прямой суммы абелевых групп $A$ и $B$.
}

\DefTheorem{direct sum of Abelian groups}
{
Пусть
\ShowEq{set Bi}A
- семейство абелевых групп.
Пусть
\ShowEq{A in xAi}
такое множество, что
\ShowEq{(xi)in A},
если
$x_i\ne 0$
для конечного числа индексов $i$.
Тогда\,\footnote{
Смотри также предложение \citeBib{Serge Lang}-10, страница 55.}
\ShowEq{A=o+Ai}
}

\DefProof{direct sum of Abelian groups}
{
Согласно построению
$A$ является подгруппой абелевой группы $\prod A_i$.
Отображение
\ShowEq{f:A->B}{\lambda_j}{A_j}A
определённое равенством
\ShowEq{lj(x)=0x0}
является инъективным гомоморфизмом.

Пусть
\ShowEq{set f:A->B}f{A_i}B
семейство гомоморфизмов в абелевую группу $B$.
Мы определим отображение
\ShowEq{f:A->B}fAB
пользуясь равенством
\ShowEq{fxi,i=sum fxi}
Сумма в правой части равенства
\EqRef{fxi,i=sum fxi}
конечна, так как все слагаемые, кроме конечного числа, равна $0$.
Из равенства
\ShowEq{fi(x+y)=}
и равенства
\EqRef{fxi,i=sum fxi}
следует, что
\ShowEq{f(x+y)i=}
Следовательно, отображение $f$ является гомоморфизмом абелевой группы.
Равенство
\ShowEq{flj=fj}
является следствием равенств
\EqRef{lj(x)=0x0},
\EqRef{fxi,i=sum fxi}.
Так как отображение $\lambda_i$ инъективно,
то отображение $f$ определено однозначно.
Следовательно, теорема является следствием определений
\RefDefinition{coproduct in category},
\RefDefinition{direct sum of Abelian groups}.
}

\DefEq
{
Пусть эндоморфизм $f$ действует на $A_2$\Hyph число $a$ с\SideRu ва
\ShowEq{f(a) \SideNS}
Пусть
\ShowEq{End O2}{A_2}{}
- мультипликативная $\Omega$\Hyph группа с произведением
\ShowEq{fga= \SideNS}
и $\delta$ - единица группы
\ShowEq{End O2}{A_2}.
Мы можем рассматривать равенство
\EqRef{fga= \SideNS}
как
\AddIndex{закон ассоциативности}{associative law},
который позволяет записывать равенство
\EqRef{fga= \SideNS}
без использования скобок
\ShowEq{fga= 1 \SideNS}

\begin{definition}
\labelDefinition{\SideNS-side representation of group} 
Пусть $A_1$ - мультипликативная $\Omega$\Hyph группа.
Мы будем называть гомоморфизм мультипликативной $\Omega$\Hyph группы
\DrawEq{representation of group, map}{\SideNS-side}
\AddIndex{\SideRu восторонним представлением}{\SideNS-side representation}
мультипликативной $\Omega$\Hyph группы $A_1$
или
\AddIndex{\SideRu восторонним $A_1$\Hyph представлением}{\SideNS-side A representation}
в $\Omega_2$\Hyph алгебре $A_2$, если отображение $f$ удовлетворяет условиям
\DrawEq{\SideNS-side representation of group}{def}
\qed
\end{definition}
}
{definition: side representation of group}
%DefEq

\DefDefinition{reduced morphism of representations}
{
Пусть
\ShowEq{f:A->*B}f{A_1}{A_2}
представление $\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $A_2$ и 
\ShowEq{f:A->*B}g{A_1}{B_2}
представление $\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $B_2$.
Пусть
\ShowEq{id:A1->A1 A2->B2}
морфизм представлений.
В этом случае мы можем отождествить морфизм
\ShowEq{map r,R}{\id}{r_2}{}
представлений $\Omega_1$\Hyph алгебры и соответствующий гомоморфизм $r_2$ $\Omega_2$\Hyph алгебры
и будем называть гомоморфизм $r_2$
\AddIndex{приведенным морфизмом представлений}
{reduced morphism of representations}.
Мы будем пользоваться диаграммой
\ShowEq{morphism id,R of representations}
для представления приведенного морфизма $r_2$ представлений
$\Omega_1$\Hyph алгебры.
Из диаграммы следует
\ShowEq{morphism of representations of universal algebra}
Мы будем также пользоваться диаграммой
\ShowEq{morphism id,R of representations 2}
вместо диаграммы
\EqRef{morphism id,R of representations}.
}

\DefEq
{
\begin{definition}
\labelDefinition{tensor product of representations}
Пусть $A$ является абелевой мультипликативной $\Omega_1$\Hyph группой.
Пусть
\EqParm{A1n}{=z}
- $\Omega_2$\Hyph алгебры.\,\footnote{
Я определяю
тензорное произведение представлений универсальной алгебры
по аналогии с определением в \citeBib{Serge Lang}, с. 456 - 458.
}
Пусть для любого
\ShowEq{k,1n}
\ShowEq{representation A Ak 1}
эффективное представление мультипликативной $\Omega_1$\Hyph группы $A$
в $\Omega_2$\Hyph алгебре $A_k$.
Рассмотрим категорию $\mathcal A$ объектами которой являются
приведенные полиморфизмы представлений $f_1$, ..., $f_n$
\ShowEq{polymorphisms category}
где $S_1$, $S_2$ - $\Omega_2$\Hyph алгебры и
\ShowEq{representation of algebra in S1 S2}
эффективные представления мультипликативной $\Omega_1$\Hyph группы $A$.
Мы определим морфизм
\ShowEq{r1->r2}
как приведенный морфизм представлений $h:S_1\rightarrow S_2$,
для которого коммутативна диаграмма
\ShowEq{polymorphisms category, diagram}
Универсальный объект
\ShowEq{tensor product of representations}
категории $\mathcal A$ называется
\AddIndex{тензорным произведением}{tensor product}
представлений
\EqParm{A1n}{=.}
\qed
\end{definition}
}
{definition: tensor product of representations}
%DefEq

\DefEq
{
\begin{theorem}
\labelTheorem{tensor product of representations}
Если существует полиморфизм представлений,
то тензорное произведение представлений существует.
\end{theorem}
}
{theorem: tensor product of representations}
%DefEq

\DefEq
{
\begin{theorem}
\labelTheorem{representation, tensor product}
Пусть
\ShowEq{equivalence, 1, representation, tensor product}
Тензорное произведение дистрибутивно относительно операции $\omega$
\ShowEq{tensors 1, representation, tensor product}
Представление мультипликативной $\Omega_1$\Hyph группы $A$
в тензорном произведении определено равенством
\ShowEq{tensors 2, representation, tensor product}
\end{theorem}
}
{theorem: representation, tensor product}
%DefEq

\DefEq
{
\begin{theorem}
\labelTheorem{tensor product and polymorphism}
Пусть $B_1$, ..., $B_n$ -
$\Omega_2$\Hyph алгебры.
Пусть
\ShowEq{map f, 1, representation, tensor product}
приведенный полиморфизм, определённый равенством
\ShowEq{map f, representation, tensor product}
Пусть
\ShowEq{map g, representation, tensor product}
приведенный полиморфизм в $\Omega_2$\Hyph алгебру $V$.
Существует морфизм представлений
\ShowEq{map h, representation, tensor product}
такой, что диаграмма
\ShowEq{map gh, representation, tensor product}
коммутативна.
\end{theorem}
}
{theorem: tensor product and polymorphism}
%DefEq

\DefEq
{
\begin{theorem}
\labelTheorem{B times->B otimes}
Отображение
\ShowEq{B times->B otimes}
является полиморфизмом.
\end{theorem}
}
{theorem: B times->B otimes}
%DefEq

\DefTheorem{|a-b|>|a|-|b|}
{
Пусть $A$ - нормированная $\Omega$\Hyph группа.
Тогда
\ShowEq{|a-b|>|a|-|b|}
}

\DefDefinition{continuous map, Omega group}
{
Отображение
\ShowEq{f:A->B}f{A_1}{A_2}
нормированной $\Omega_1$\Hyph группы $A_1$ с нормой $\|x\|_1$
в нормированную $\Omega_2$\Hyph группу $A_2$ с нормой $\|y\|_2$
называется \AddIndex{непрерывным}{continuous map}, если
для любого сколь угодно малого $\epsilon>0$
существует такое $\delta>0$, что
\ShowEq{|x'-x|<delta}
влечёт
\ShowEq{|f(x)-f(x')|<epsilon}
}

\DefTheorem{continuous map, open set}
{
Отображение
\ShowEq{f:A->B}f{A_1}{A_2}
нормированной $\Omega_1$\Hyph группы $A_1$ с нормой $\|x\|_1$
в нормированную $\Omega_2$\Hyph группу $A_2$ с нормой $\|y\|_2$
непрерывно тогда и только тогда, когда
прообраз открытого множества
является открытым множеством.
}

\DefTheorem{image of interval is interval, real field}
{
Пусть
\ShowEq{f:A->B}fRR
непрерывное отображение поля действительных чисел.
Тогда образ интервала является интервалом.
}

\DefEq
{
\begin{definition}
\labelDefinition{norm of operation}
Пусть $A$
- нормированная $\Omega$\Hyph группа.
Для $n$\Hyph арной операции $\omega$, величина
\ShowEq{norm of operation}
\ShowEq{norm of operation, definition}
называется
\AddIndex{нормой операции}{norm of operation} $\omega$.
\qed
\end{definition}
}
{definition: norm of operation}
%\DefEq

\DefTheorem{|fx|<|f||x|1n}
{
Пусть $A$ - нормированная $\Omega$\Hyph группа.
Для $n$\Hyph арной операции $\omega$,
\ShowEq{|a omega|<|omega||a|1n}
}

\DefEq
{
\begin{definition}
\labelDefinition{norm of representation}
Пусть
\ShowEq{f:A->*B}g{A_1}{A_2}
представление\
\ePrints{1305.4547}
\ifx\Semafor\ValueOn
\footnote{
Смотри определение
\EqParm{ref definition: left-side representation of algebra}{=z}
представления универсальной алгебры.
Согласно определению
\Ref[1211.6965]{definition: module over ring},
модуль - это представление кольца в абелевой группе.
Так как кольцо и абелева группа являются $\Omega$\Hyph группами,
то модуль - это представление $\Omega$\Hyph группы.
}
\fi
$\Omega_1$\Hyph группы $A_1$ с нормой $\|x\|_1$
в $\Omega_2$\Hyph группе $A_2$ с нормой $\|x\|_2$.
Величина
\ShowEq{norm of representation}
\ShowEq{norm of representation, definition}
называется
\AddIndex{нормой представления}{norm of representation} $f$.
\qed
\end{definition}
}
{definition: norm of representation}
%\DefEq

\DefTheorem{|fab|<|f||a||b|}
{
Пусть
\ShowEq{f:A->*B}g{A_1}{A_2}
представление
$\Omega_1$\Hyph группы $A_1$ с нормой $\|x\|_1$
в $\Omega_2$\Hyph группе $A_2$ с нормой $\|x\|_2$.
Тогда
\ShowEq{|fab|<|f||a||b|}
}

\DefEq
{
\begin{definition}
\labelDefinition{open set}
Пусть $A$ - нормированная $\Omega$\Hyph группа.
Множество
$U\subset A$
называется
\AddIndex{открытым}{open set},\,\footnote{
В топологии
обычно сперва определяют открытое множество,
а затем базу топологии.
В случае метрического или нормированного пространства,
удобнее дать определение открытого множества,
опираясь на определение базы топологии.
В этом случае определение основано на одном из свойств
базы топологии. Непосредственная проверка
позволяет убедиться, что определённое таким образом
открытое множество удовлетворяет основным свойствам.
}
если для любого $A$\Hyph числа
\EqParm{a in U}{=z}
существует
\ShowEq{epsilon in R}
такое, что
\ShowEq{B(a) subset U}
\qed
\end{definition}
}
{definition: open set}
%\DefEq

\DefEq
{
\begin{definition}
\labelDefinition{compact set}
Множество $T$ топологического пространства называется
\AddIndex{компактным}{compact set},
если любое его открытое покрытие содержит
конечное подпокрытие.\,\footnote{
Смотри также определение в
\citeBib{Kolmogorov Fomin}, страница 98.
}
\qed
\end{definition}
}
{definition: compact set}
%\DefEq

\DefTheorem{c1+c2 in B}
{
Пусть $A$ - нормированная $\Omega$\Hyph группа.
Для
\ShowEq{c1 c2 in A}
пусть
\ShowEq{c1 c2 in B}
Тогда
\ShowEq{c1+c2 in B}
}

\AddEq{definition: limit of sequence}
{
\begin{definition}
\labelDefinition{limit of sequence, normed \Algebrac}
Пусть $\Module$
- нормированн\WhatA $\SideA$\Hyph \Algebrab.
$\Module$\Hyph число $a$ называется 
\AddIndex{пределом последовательности}{limit of sequence}
\ShowEq{[an] in A}
\ShowEq{limit of sequence}
если для любого
\ShowEq{epsilon in R}
существует, зависящее от $\epsilon$, натуральное число $n_0$ такое, что
\DrawEq{|an-a|<epsilon}{-}
для любого $n>n_0$.
Мы будем также говорить, что
\AddIndex{последовательность $a_n$ сходится}{sequence converges}
к $a$.
\qed
\end{definition}
}

\AddEq{theorem: limit of sequence}
{
\begin{theorem}
\labelTheorem{limit of sequence, normed \Algebrac}
Пусть $\Module$
- нормированн\WhatA $\SideA$\Hyph \Algebrab.
$\Module$\Hyph число $a$ является 
пределом последовательности
\ShowEq{[an] in A}
\DrawEq{a=lim an}{}
если для любого
\ShowEq{epsilon in R}
существует, зависящее от $\epsilon$, натуральное число $n_0$ такое, что
\DrawEq{an in B(a)}{}
для любого $n>n_0$.
\end{theorem}
}

\DefProof{limit of sequence}
{
Следствие определений
\RefDefinition{open ball},
\RefDefinition{limit of sequence, normed \Algebrac}.
}

\AddEq{definition: fundamental sequence}
{
\begin{definition}
\labelDefinition{fundamental sequence, normed \Algebrac}
Пусть $\Module$
- нормированн\WhatA $\SideA$\Hyph \Algebrab.
Последовательность
\ShowEq{[an] in A}
называется 
\AddIndex{фундаментальной}{fundamental sequence}
или \AddIndex{последовательностью Коши}{Cauchy sequence},
если для любого
\ShowEq{epsilon in R}
существует, зависящее от $\epsilon$, натуральное число $n_0$ такое, что
\DrawEq{|ap-aq|<epsilon}{-}
для любых $p$, $q>n_0$.
\qed
\end{definition}
}

\AddEq{theorem: fundamental sequence}
{
\begin{theorem}
\labelTheorem{fundamental sequence, normed \Algebrac}
Пусть $\Module$
- нормированн\WhatA $\SideA$\Hyph \Algebrab.
Последовательность
\ShowEq{[an] in A}
является фундаментальной последовательностью,
тогда и только тогда, когда для любого
\ShowEq{epsilon in R}
существует, зависящее от $\epsilon$, натуральное число $n_0$ такое, что
\ShowEq{aq in B(ap)}
для любых $p$, $q>n_0$.
\end{theorem}
}

\DefProof{fundamental sequence}
{
Следствие определений
\RefDefinition{open ball},
\RefDefinition{fundamental sequence, normed \Algebrac}.
}

\DefTheorem{norm of compact set is bounded}
{
Пусть $C$ - компактное множество
нормированной $\Omega$\Hyph группы $A$.
Тогда норма
\ShowEq{|x in C|}
ограничена сверху и снизу.
}

\DefTheorem{lim a=lim b}
{
Пусть $A$ - нормированная $\Omega$\Hyph группа.
Пусть $a_n$, $b_n$, $n=1$, ..., - фундаментальные последовательности.
Пусть
\DrawEq{lim a-b=0}{limit}
Если последовательность $a_n$ сходится, то
последовательность $b_n$ сходится и
\ShowEq{lim a=lim b}
}

\DefEq
{
\begin{definition}
\labelDefinition{complete Omega group}
Нормированная $\Omega$\Hyph группа $A$ называется 
\AddIndex{полной}{complete Omega group}
если любая фундаментальная последовательность элементов
$\Omega$\Hyph группы $A$ сходится, т. е.
имеет предел в этой $\Omega$\Hyph группе.
\qed
\end{definition}
}
{definition: complete Omega group}
%\DefEq

\DefEq
{
\begin{definition}
\labelDefinition{limit of sequence, map to Omega group}
Пусть
\ShowEq{fn M(X,A)}
- последовательность отображений в нормированную
$\Omega$\Hyph группу $A$.
Отображение
\ShowEq{f M(X,A)}
называется
\AddIndex{пределом последовательности}{limit of sequence}
$f_n$, если для любого $x\in X$
\DrawEq{f(x)=lim}{}
Мы будем также говорить, что
\AddIndex{последовательность $f_n$ сходится}{sequence converges}
к отображению $f$.
\qed
\end{definition}
}
{definition: limit of sequence, map to Omega group}
%\DefEq

\DefEq
{
\begin{definition}
\labelDefinition{sequence converges uniformly}
Пусть
\ShowEq{fn M(X,A)}
- последовательность отображений в нормированную
$\Omega$\Hyph группу $A$.
\AddIndex{Последовательность $f_n$ сходится равномерно}
{sequence converges uniformly}
к отображению $f$,
если для любого
\ShowEq{epsilon in R}
существует $N$ такое, что
\ShowEq{fn(x) - f(x)}
для любого $n>N$.
\qed
\end{definition}
}
{definition: sequence converges uniformly}
%\DefEq

\DefEq
{
\begin{theorem}
\labelTheorem{sequence converges uniformly, fn-fm}
Последовательность отображений
\ShowEq{fn M(X,A)}
в нормированную
$\Omega$\Hyph группу $A$ сходится равномерно
к отображению $f$,
если для любого
\ShowEq{epsilon in R}
существует $N$ такое, что
\ShowEq{|fn(x)-fm(x)|<e}
для любых \(n\), \(m>N\).
\end{theorem}
}
{theorem: sequence converges uniformly, fn-fm}
%\DefEq

\DefTheorem{h=f+g, converges uniformly}
{
Пусть последовательность отображений
\ShowEq{fn M(X,A)}
в полную $\Omega$\Hyph группу $A$
сходится равномерно
к отображению $f$.
Пусть последовательность отображений
\ShowEq{gn M(X,A)}
в полную $\Omega$\Hyph группу $A$
сходится равномерно
к отображению $g$.
Тогда последовательность отображений
\ShowEq{hn=fn+gn}
в полную $\Omega$\Hyph группу $A$
сходится равномерно
к отображению
\DrawEq{h=f+g}{converges uniformly}
}

\DefTheorem{representation f generates representation fX}
{
Представление
\ShowEq{f:A->*B}g{A_1}{A_2}
$\Omega_1$\Hyph группы $A_1$ с нормой $\|x\|_1$
в $\Omega_2$\Hyph группе $A_2$ с нормой $\|x\|_2$
порождает представление
\ShowEq{f:A->*B}{f_X}{M(X,A_1)}{M(X,A_2)}
$\Omega_1$\Hyph группы
\ShowEq{M(X,A1)}
в $\Omega_2$\Hyph группе
\ShowEq{M(X,A2)}
где (
\ShowEq{g1 in M(X,A1)},
\ShowEq{g2 in M(X,A2)}
)
\ShowEq{f(x)g(x):X->A2}
}

\DefTheorem{fX(g1)(g2), converges uniformly}
{
Пусть
\ShowEq{f:A->*B}g{A_1}{A_2}
представление
полной $\Omega_1$\Hyph группы $A_1$ с нормой $\|x\|_1$
в полной $\Omega_2$\Hyph группе $A_2$ с нормой $\|x\|_2$.
Пусть последовательность отображений
\ShowEq{g1n M(X,A1)}
сходится равномерно
к отображению $g_1$.
Пусть последовательность отображений
\ShowEq{g2n M(X,A2)}
сходится равномерно
к отображению $g_2$.
Пусть множество значений отображения $g_i$, $i=1$, $2$,
компактно.
Тогда последовательность отображений
\ShowEq{f(g1n)(g2n)}
сходится равномерно
к отображению
\ShowEq{fX(g1)(g2)}.
}

\DefTheorem{set of maps to Omega group}
{
Пусть
\ShowEq{set of maps to Omega group}
- множество отображений множества $X$ в $\Omega$\Hyph группу $A$.
Мы можем определить структуру $\Omega$\Hyph группы на множестве
\EqParm{M(X,A)}{=.}
}

\DefEq
{
Так как $X$ - произвольное множество, мы не можем определить
норму в $\Omega$\Hyph группе
\EqParm{M(X,A)}{=.}
Однако мы можем определить сходимость последовательности в
\EqParm{M(X,A)}{=.c}
следовательно, мы можем определить топологию в
\EqParm{M(X,A)}{=.}
}
{remark: set of maps to Omega group}
%\DefEq

\DefDefinition{closed ball}
{
Пусть $\Module$
- нормированн\WhatA $\SideA$\Hyph \Algebrab.
Пусть $a\in \Module$.
Множество
\ShowEq{closed ball}
называется
\AddIndex{замкнутым шаром}{closed ball}
с центром в $a$.
}

\DefDefinition{open ball}
{
Пусть $\Module$
- нормированн\WhatA $\SideA$\Hyph \Algebrab.
Пусть $a\in \Module$.
Множество
\ShowEq{open ball}
называется
\AddIndex{открытым шаром}{open ball}
с центром в $a$.
}

\DefDefinition{reduced polymorphism of representations}
{
Пусть
\ShowEq{set of universal algebras 1}
- универсальные алгебры.
Пусть, для любого
\ShowEq{k,1n}
\ShowEq{f:A->*B}{f_k}A{B_k}
эффективное представление $\Omega_1$\Hyph алгебры $A$
в $\Omega_2$\Hyph алгебре $B_k$.
Пусть
\ShowEq{f:A->*B}fAB
эффективное представление $\Omega_1$\Hyph алгебры $A$
в $\Omega_2$\Hyph алгебре $B$.
Отображение
\ShowEq{reduced polymorphism of representation}
называется
\AddIndex{приведенным полиморфизмом представлений}
{reduced polymorphism of representations}
$f_1$, ..., $f_n$ в представление $f$,
если для любого
\ShowEq{k,1n}
при условии, что все переменные кроме переменной $x_k\in B_k$
имеют заданное значение, отображение $r_2$
является приведенным морфизмом представления $f_k$ в представление $f$.

Если $f_1=...=f_n$, то мы будем говорить, что отображение $r_2$
является приведенным полиморфизмом представления $f_1$ в представление $f$.

Если $f_1=...=f_n=f$, то мы будем говорить, что отображение $r_2$
является приведенным полиморфизмом представления $f$.
}

\DefEq
{
\begin{convention}
Мы будем пользоваться соглашением Эйнштейна о сумме.
Это означает, что, когда индекс присутствует в
выражении дважды (один вверху и один внизу) и множество индексов известно,
это выражение подразумевает сумму по повторяющемуся индексу.
В этом случае предполагается известным множество
индекса суммирования и знак суммы опускается
\ShowEq{av=sum av}av
Я буду явно указывать множество
индексов, если это необходимо.
\qed
\end{convention}
}
{convention: Einstein summation}
%\DefEq

\AddEq [1]{step of proof: action in Abelian group}
{
Из равенства
\EqRef{0g=0}
следует, что равенство
\EqRef{#1}
верно, когда $n=0$.
\def\TempA{(nm)a=n(ma)}
\def\TempB{#1}
\begin{itemize}
\item
Пусть равенство
\EqRef{#1}
верно, когда $n=k\ge 0$.
Тогда
\ShowEq{#1,n=k}
Равенство
\ShowEq{#1,n=k+1}
является следствием
\ifx\TempA\TempB
равенств
\EqRef{(n+1)g=},
\EqRef{(m+n)a=ma+na}.
\else
равенства
\EqRef{(n+1)g=}.
\fi
Следовательно, равенство
\EqRef{#1}
верно, когда $n=k+1$.
Согласно принципу математической индукции,
равенство
\EqRef{#1}
верно для любого $n\ge 0$.
\item
Пусть равенство
\EqRef{(m+n)a=ma+na}
верно, когда $n=k\le 0$.
Тогда
\ShowEq{#1,n=k}
Равенство
\ShowEq{#1,n=k-1}
является следствием
\ifx\TempA\TempB
равенств
\EqRef{(n-1)g=},
\EqRef{(m-n)a=ma-na}.
\else
равенства
\EqRef{(n-1)g=}.
\fi
Следовательно, равенство
\EqRef{#1}
верно, когда $n=k-1$.
Согласно принципу математической индукции,
равенство
\EqRef{#1}
верно для любого $n\le 0$.
\item
Следовательно, равенство
\EqRef{#1}
верно для любого $n\in Z$.
\end{itemize}
}

\DefDefinition{category of representations A1(mA2)}
{
Пусть $A_1$ - $\Omega_1$\Hyph алгебра.
Пусть $\mathcal A_2$ - категория $\Omega_2$\Hyph алгебр.
Мы определим \AddIndex{категорию
\ShowEq{A1(mA2) symb}
представлений}
{category of representations}
$\Omega_1$\Hyph алгебры $A_1$ в $\Omega_2$\Hyph алгебре.
Объектами этой категории являются представления
$\Omega_1$\Hyph алгебры $A_1$ в $\Omega_2$\Hyph алгебре.
Морфизмами этой категории являются приведенные морфизмы соответствующих представлений.
}

\DefEq
{
\begin{definition}
\labelDefinition{matrix operations}
{\it
Мы определим следующие операции на множестве матриц над
$\Omega$\Hyph кольцом $A$.
\StartLabelItem
\begin{enumerate}
\item
Пусть число столбцов матрицы $a$ равно числу строк матрицы $b$.
\AddIndex{\RC произведение}{rc-product}
матриц $a$ и $b$
имеет вид
\ShowEq{rc-product}
\ShowEq{rc-product of matrices}
и может быть выражено как произведение строк матрицы $a$
и столбцов матрицы $b$.\,\footnote{
Символ операции \RC произведения сформирован из двух символов операции произведения, которые записываются на
месте индекса суммирования.
}
\item
Пусть число строк матрицы $a$ равно числу столбцов матрицы $b$.
\AddIndex{\CR произведение}{cr-product}
матриц $a$ и $b$
имеет вид
\ShowEq{cr-product}
\ShowEq{cr-product of matrices}
и может быть выражено как произведение столбцов матрицы $a$
и строк матрицы $b$.\,\footnote{
Символ операции \CR произведения сформирован из двух символов операции произведения, которые записываются на
месте индекса суммирования.
}
\item
Сумма матриц $a$ и $b$ определена равенством
\ShowEq{(a+b)=}
\item
Транспонирование $a^T$ матрицы $a$
меняет местами строки и столбцы
\ShowEq{transpose of matrix, 1}
\end{enumerate}
}
\qed
\end{definition}
}
{definition: matrix operations}
%\DefEq

\DefEq
{
\begin{remark}
\labelRemark{pronunciation of product}
Мы будем пользоваться символом \RC\  или \CR\  в имени свойств
каждого произведения и в обозначениях.
Мы можем читать символы
$\RCstar$ и $\CRstar$ как $rc$\hyph произведение и $cr$\hyph произведение.
Это правило мы распространим на последующую терминологию.
\qed
\end{remark}
}
{remark: pronunciation of product}
%\DefEq

\DefEq
{
\begin{definition}
\labelDefinition{biring}
\AddIndex{Бикольцо}{biring} $A$ - это множество,
на котором мы определили унарную операцию, называемую транспозицией,
и три бинарных операции,
называемые \RC произведение, \CR произведение и сумма, такие что
\begin{itemize}
\item \RC произведение и сумма определяют структуру кольца на $A$
\item \CR произведение и сумма определяют структуру кольца на $A$
\item оба произведения имеют общую единицу $\delta$
\item произведения удовлетворяют равенству
\ShowEq{rcstar transpose}
\item транспозиция единицы есть единица
\ShowEq{transpose of identity}
\item двойная транспозиция есть исходный элемент
\ShowEq{double transpose}
\end{itemize}
\qed
\end{definition} 
}
{definition: biring}
%\DefEq

\DefEq
{
\begin{theorem}
[\AddIndex{принцип двойственности для бикольца}
{duality principle for biring}]
\labelTheorem{duality principle for biring}
Пусть $\mathcal{A}$ - истинное утверждение о
бикольце $A$.
Если мы заменим одновременно
\begin{itemize}
\item $a\in A$ и $a^T$
\item \RC произведение и \CR произведение
\end{itemize}
то мы снова получим истинное утверждение.
\end{theorem}
}
{theorem: duality principle for biring}
%\DefEq

\DefEq
{
\begin{theorem}
[\AddIndex{принцип двойственности для бикольца матриц}
{duality principle for biring of matrices}]
\labelTheorem{duality principle for biring of matrices}
Пусть $A$ является бикольцом матриц.
Пусть $\mathcal{A}$ - истинное утверждение о матрицах.
Если мы заменим одновременно
\begin{itemize}
\item строки и столбцы всех матриц
\item \RC произведение и \CR произведение
\end{itemize}
то мы снова получим истинное утверждение.
\end{theorem}
\begin{proof}
Непосредственное следствие
теоремы \RefTheorem{duality principle for biring}.
\end{proof}
}
{theorem: duality principle for biring of matrices}
%\DefEq

\DefEq
{
\begin{remark}
\labelRemark{reducible biring}
Если произведение в $\Omega$\Hyph кольце коммутативно, то
\ShowEq{reducibility of products}
\AddIndex{Приводимое бикольцо}{reducible biring}
- это бикольцо, в котором выполняется
\AddIndex{условие приводимости произведений}
{condition of reducibility of products}
\EqRef{reducibility of products}.
Поэтому в приводимом бикольце достаточно рассматривать только
\RC произведение. Однако в тех случаях, когда
порядок сомножителей существенен,
мы будем пользоваться также \CR произведением.
\qed
\end{remark}
}
{remark: reducible biring}
%\DefEq

\DefEq
{
Так как левостороннее представление и правостороннее представление
опирается на гомоморфизм $\Omega$\Hyph группы,
то верно следующее утверждение.

\begin{theorem}[принцип двойственности для представления мультипликативной $\Omega$\Hyph группы]
\labelTheorem{duality principle, algebra representation}
Любое утверждение, справедливое для
левостороннего представления мультипликативной $\Omega$\Hyph группы $A_1$,
будет справедливо для правостороннего представления мультипликативной $\Omega$\Hyph группы $A_1$, если
\begin{itemize}
\item
мы будем пользоваться правосторонним произведением на $A_1$\Hyph число $a_1$ вместо
левостороннего произведения на $A_1$\Hyph число $a_1$;
\item
мы будем пользоваться правым сдвигом $R(a_1)$ мультипликативной $\Omega$\Hyph группы $A_1$
вместо левого сдвига $L(a_1)$.
\end{itemize}
\qed
\end{theorem}
}
{theorem: duality principle, algebra representation}
%\DefEq

\DefEq
{
\begin{theorem}
\labelTheorem{left right shift}
Произведение в мультипликативной $\Omega$\Hyph группе $A_1$ определяет два различных представления
мультипликативной группы $A_1$
в $\Omega$\Hyph алгебре $A_1$:
\begin{itemize}
\EqParm{theorem: shift}{=left}
\EqParm{theorem: shift}{=right}
\end{itemize}
\end{theorem}
}
{theorem: left right shift}
%\DefEq

\DefEq
{
\item
\AddIndex{\SideRuC вый сдвиг}{\SideWS shift}
\ShowEq{\SideWS shift =}
\ShowEq{\SideWS shift}
является \SideRu восторонним представлением
\ShowEq{\SideWS shift, product}
}
{theorem: shift}
%\DefEq

\DefEq
{
Если мультипликативная $\Omega$\Hyph группа $A_1$ - абелевая,
то нет разницы между левосторонним и правосторонним представлениеми.

\begin{definition}
\labelDefinition{representation of Abelian group} 
Пусть $A_1$ - абелевая мультипликативная $\Omega$\Hyph группа.
Мы будем называть гомоморфизм мультипликативной $\Omega$\Hyph группы
\DrawEq{representation of group, map}{Abelian group}
\AddIndex{представлением}{representation of algebra}
мультипликативной $\Omega$\Hyph группы $A_1$
или
\AddIndex{$A_1$\Hyph представлением}{A representation of algebra}
в $\Omega_2$\Hyph алгебре $A_2$, если отображение $f$ удовлетворяет условиям
\DrawEq{left-side representation of group}{Abelian}
\qed
\end{definition}

Обычно мы отождествляем представление абелевой мультипликативной $\Omega$\Hyph группы $A_1$
и левостороннее представление мультипликативной $\Omega$\Hyph группы $A_1$.
Однако, если это необходимо нам,
мы можем отождествить представление абелевой мультипликативной $\Omega$\Hyph группы $A_1$
и правостороннее представление мультипликативной $\Omega$\Hyph группы $A_1$.
}
{definition: representation of Abelian group}
%\DefEq

\DefDefinition{algebra of sets}
{
Непустая система множеств $\mathcal R$ называется
\AddIndex{кольцом множеств}{ring of sets},\,\footnote{
Смотри так же определение
\citeBib{Kolmogorov Fomin}\Hyph 1, страница 41.}
если условие
\ShowEq{A, B in R}
влечёт
\ShowEq{A, B in R 1}
Множество
\ShowEq{E in R}
называется
\AddIndex{единицей кольца множеств}{unit of ring of sets},
если
\ShowEq{A cap E=A}
Кольцо множеств с единицей называется
\AddIndex{алгеброй множеств}{algebra of sets}.
}

\DefEq
{
\begin{remark}
\labelRemark{A cup/minus B}
Для любых
\ShowEq{A cup/minus B}
Следовательно, если
\ShowEq{A, B in R},
то
\ShowEq{A cup/minus B R}
\qed
\end{remark}
}
{remark: A cup/minus B}
%\DefEq

\DefDefinition{sigma algebra of sets}
{
Кольцо множеств $\mathcal R$ называется
\AddIndex{\(\sigma\)\Hyph кольцом множеств}{sigma ring of sets},\,\footnote{
Смотри аналогичное определение в
\citeBib{Kolmogorov Fomin}, страница 45, определение 3.}
если условие
\ShowEq{Ai in R}
влечёт
\ShowEq{Ai in R 1}
\(\sigma\)\Hyph Кольцо множеств с единицей называется
\AddIndex{\(\sigma\)\Hyph алгеброй множеств}{sigma algebra of sets}.
}

\DefDefinition{Borel algebra}
{
Минимальная \(\sigma\)\Hyph алгебра
\ShowEq{Borel algebra}
над совокупностью всех открытых шаров нормированной $\Omega$\Hyph группы $A$,
называется
\AddIndex{алгеброй Бореля}{Borel algebra}.\,\footnote{
Смотри определение в
\citeBib{Kolmogorov Fomin}, с. 46.
Согласно замечанию
\ref{remark: A cup/minus B},
алгебра Бореля может быть также порождена множеством
замкнутых шаров.
}
Множество,
принадлежащее алгебре Бореля,
называется
\AddIndex{борелевским множеством}{Borel set}
или
\AddIndex{$B$\Hyph множеством}{B set}.
}

\DefDefinition{C_X C_Y measurable}
{
Пусть $\mathcal C_X$ -
\(\sigma\)\Hyph алгебра множеств множества $X$.
Пусть $\mathcal C_Y$ -
\(\sigma\)\Hyph алгебра множеств множества $Y$.
Отображение
\ShowEq{f:A->B}fXY
называется
$(\mathcal C_X,\mathcal C_Y)$\Hyph измеримым,\,\footnote{
Смотри аналогичное определение в
\citeBib{Kolmogorov Fomin}, с. 282.}
если для всякого множества
\ShowEq{CX CY measurable map}
}

\DefEq
{
\begin{example}
\labelExample{measurable map}
Пусть на множестве $X$ определена \(\sigma\)\Hyph аддитивная мера $\mu$.
Пусть
\ShowEq{algebra of sets measurable with respect to measure}
- \(\sigma\)\Hyph алгебра измеримых относительно меры $\mu$ множеств.
Пусть
$\mathcal B(A)$
- алгебра Бореля
нормированной $\Omega$\Hyph группы $A$.
Отображение
\ShowEq{f:A->B}fXA
называется
\AddIndex{$\mu$\Hyph измеримым}{mu measurable map},\,\footnote{
Смотри аналогичное определение в
\citeBib{Kolmogorov Fomin}, с. 282, определение 1.
Если мера $\mu$ на множестве $X$ определена в контексте,
мы также будем называть отображение
\ShowEq{f:A->B}fXA
\AddIndex{измеримым}{measurable map}.
}
если для всякого множества
\ShowEq{measurable map}
\qed
\end{example}
}
{example: measurable map}
%\DefEq

\DefDefinition{simple map}
{
Пусть на множестве $X$ определена \(\sigma\)\Hyph аддитивная мера $\mu$.
Отображение
\ShowEq{f:A->B}fXA
в нормированную $\Omega$\Hyph группу $A$ называется
\AddIndex{простым отображением}{simple map},
если это отображение $\mu$\Hyph измеримо и
принимает не более, чем счётное множество значений.
}

\DefTheorem{measurable simple map}
{
Пусть отображение
\ShowEq{f:A->B}fXA
принимает не более, чем счётное множество значений
\ShowEq{range f}
.
Отображение $f$ $\mu$\Hyph измеримо тогда и только тогда, когда
все множества
\DrawEq{Fn=}{}
$\mu$\Hyph измеримы.\,\footnote{
Смотри аналогичную теорему в
\citeBib{Kolmogorov Fomin}, страница 292, теорема 1.}
}

\DefDefinition{measure}
{
Пусть \(\mathcal C_m\) - полукольцо множеств.\,\footnote{
Смотри также определение
\citeBib{Kolmogorov Fomin}\Hyph 1 на странице 265.}
Отображение
\ShowEq{f:A->B}f{\mathcal C_m}R
называется
\AddIndex{мерой}{measure},
если
\StartLabelItem
\begin{enumerate}
\item
\ShowEq{m(A)>0}
\item
Отображение \(m\) аддитивно.
Если множество
\ShowEq{A in Cm}
имеет конечное разлоение
\DrawEq{A=+Ai Cm}{}
где
\ShowEq{Ai*Aj=0},
то
\ShowEq{m A=+m Ai}
\end{enumerate}
}

\DefDefinition{complete measure}
{
Мера \(\mu\) называется
\AddIndex{полной}{complete measure},
если из условий
\ShowEq{B in A, mu(A)=0}
следует,
что множество \(B\) измеримо.
}

\DefDefinition{sigma-additive measure}
{
Пусть $\mathcal C_{\mu}$ -
\(\sigma\)\Hyph алгебра множеств множества $F$.\,\footnote{
Смотри аналогичные определения в
\citeBib{Kolmogorov Fomin}, определение 1 на странице 265
и определение 3 на странице 268.}
Отображение
%\ShowEq{mu:CF->A}
%в нормированную $\Omega$\Hyph группу $A$ называется
\ShowEq{f:A->B}{\mu}{\mathcal C_{\mu}}R
в поле действительных чисел $R$ называется
\AddIndex{\(\sigma\)\Hyph аддитивной мерой}{sigma-additive measure},
если для любого множества
\ShowEq{X in Cmu}
выполнены следующие условия.
\StartLabelItem
\begin{enumerate}
\item
\ShowEq{muX>0}
\item
Пусть
\DrawEq{X=+Xi}{}
конечное или счётное объединение множеств
\ShowEq{Xn in Cmu}
Тогда
\DrawEqParm{mu(X=+Xi)}X{}
где ряд в правой части сходится абсолютно.
\labelItem{mu(X=+Xi)}
\end{enumerate}
}

\DefEq
{
Пусть на множестве $X$ определена \(\sigma\)\Hyph аддитивная мера $\mu$.
Пусть определено эффективное представление поля действительных чисел \(R\)
в полной абелевой \(\Omega\)\Hyph группе \(A\).\,\footnote{
Другими словами,
\(\Omega\)\Hyph группа \(A\) является
\(R\)\Hyph векторным пространством.}
}
{remark - measure - effective representation of real field}
%\DefEq

\DefDefinition{series converges normally}
{
Пусть \(a_i\) - последовательность \(A\)\Hyph чисел.
Если
\ShowEq{sum |ai|<infty}
то мы будем говорить, что {\bf ряд}
\ShowEq{sum ai}
\AddIndex{сходится нормально}
{series converges normally}.\,\footnote{Смотри также
определение нормальной сходимости ряда
на странице \citeBib{Cartan differential form}-12.}
}

\DefDefinition{Integral of Map over Set of Finite Measure}
{
\(\mu\)\Hyph измеримое отображение
\ShowEq{f:A->B}fXA
называется
\AddIndex{интегрируемым}{integrable map}
по множеству \(X\),\,\footnote{
Смотри также определение
\citeBib{Kolmogorov Fomin}\Hyph 3, страницы 294, 295.
}
если существует последовательность
простых  отображений
\ShowEq{f:A->B}{f_n}XA
сходящаяся равномерно к \(f\).
Если отображение \(f\) интегрируемо,
то предел
\ShowEq{integral of map}
\ShowEq{integral of measurable map}
называется
\AddIndex{интегралом Лебега}{Lebesgue integral}
отображения \(f\) по множеству \(X\).
}

\DefDefinition{integrable map}
{
Для простого отображения
\ShowEq{f:A->B}fXA
рассмотрим ряд
\DrawEq{sum mu(F) f}{integral}
где
\begin{itemize}
\item
Множество
\ShowEq{f1...}
является областью определения отображения \(f\)
\item
Если \(n\ne m\), то
\ShowEq{fn ne fm}
\item
\DrawEq{Fn=}{-}
\end{itemize}
Простое отображение
\ShowEq{f:A->B}fXA
называется
\AddIndex{интегрируемым}{integrable map}
по множеству \(X\),
если ряд
\eqRef{sum mu(F) f}{integral}
сходится нормально.\,\footnote{
Смотри аналогичное определение в
\citeBib{Kolmogorov Fomin}, определение 2, с. 293.}
Если отображение \(f\) интегрируемо,
то сумма ряда
\eqRef{sum mu(F) f}{integral}
называется
\AddIndex{интегралом Лебега}{Lebesgue integral}
отображения \(f\) по множеству \(X\)
\ShowEq{integral of map}
\ShowEq{integral of simple map}
}

\DefTheorem{|int f|<int|f|}
{
Пусть
\ShowEq{f:A->B}fXA
измеримое отображение.
Интеграл
\ShowEq{int f X}
существует
тогда и только тогда, когда
интеграл
\ShowEq{int |f| X}
существует.
Тогда
\DrawEq{|int f|<int|f|}{measurable}
}

\DefTheorem{int |f|<M mu}
{
Пусть $\mu$\Hyph измеримое отображение
\ShowEq{f:A->B}fXA
удовлетворяет условию
\DrawEq{|f(x)|<M}{}
Если мера множества \(X\) конечна, то
\DrawEq{int |f|<M mu}{measurable}
}

\DefTheorem{int f+g X}
{
Пусть
\ShowEq{f:A->B}fXA
\ShowEq{f:A->B}gXA
$\mu$\Hyph измеримые отображения
с компактным множеством значений.
Если существуют интегралы
\ShowEq{int f X}
\ShowEq{int g X}
то существует интеграл
\ShowEq{int f+g X}
и
\DrawEq{int f+g X =}{measurable}
}


==> Summary.Calculus.Russian.tex <==
%auto-ignore

\input{Summary.Calculus.Eq}

\chapter{Сводка теорем}

Пусть $D$ - полное коммутативное кольцо характеристики $0$.

\section{Таблица производных}

\begin{theorem}
\labelTheorem{derivative of const, algebra}
Для любого $b\in A$
\ShowEq{derivative of const, algebra}
\end{theorem}
\begin{proof}
Непосредственное следствие определения
\RefDefinition{differentiable map, algebra}.
\end{proof}

\begin{theorem}
\labelTheorem{dx/dx=1}
\ShowEq{dx/dx=1}
\end{theorem}
\begin{proof}
Согласно определению
\ShowEq{ref derivative, representation in algebra}
\ShowEq{dx/dx=}
Равенство
\EqRef{dx/dx=1}
является следствием
\EqRef{dx/dx=}.
\end{proof}

\begin{theorem}
\labelTheorem{derivative, product over constant, algebra}
Для любых $b$, $c\in A$
\ShowEq{derivative, product over constant, algebra}
\end{theorem}
\begin{proof}
Непосредственное следствие равенств
\ShowEq{ref derivative of product}
и теоремы
\RefTheorem{derivative of const, algebra}.
\end{proof}

\begin{theorem}
\labelTheorem{d(f+g)=df+dg}
Пусть
\ShowEq{f:A->B}fAB
\ShowEq{f:A->B}gAB
отображения банахова $D$\Hyph модуля $A$
в ассоциативную банахову $D$\Hyph алгебра $B$.
Если производные
\ShowEq{df,dg}
существуют,
то существует
производная
\ShowEq{d(f+g)}
\ShowEq{d(f+g)dx=df+dg}
\ShowEq{d(f+g)=df+dg}
Если
\ShowEq{df=+}
\ShowEq{dg=+}
то
\ShowEq{d(f+g)=+}
\end{theorem}
\begin{proof}
Если производные
\ShowEq{df,dg}
существуют,
то согласно определению
\ShowEq{ref derivative, representation in algebra}
\ShowEq{df=}
\ShowEq{dg=}
Согласно определению
\ShowEq{ref derivative, representation in algebra}
\ShowEq{d(f+g)=}
Равенство
\EqRef{d(f+g)dx=df+dg}
является следствием
\EqRef{df=},
\EqRef{dg=},
\EqRef{d(f+g)=}.
Равенство
\EqRef{d(f+g)=df+dg}
является следствием
\ShowEq{ref sum of maps}
\EqRef{d(f+g)dx=df+dg}.
Равенство
\EqRef{d(f+g)=+}
является следствием
\EqRef{df=+},
\EqRef{dg=+},
\EqRef{d(f+g)=df+dg}.
\end{proof}

\begin{theorem}
\labelTheorem{derivative, fx=axb, algebra}
Для любых $b$, $c\in A$
\ShowEq{derivative, fx=axb, algebra}
\end{theorem}
\begin{proof}
Следствие теорем
\RefTheorem{dx/dx=1},
\RefTheorem{derivative, product over constant, algebra},
когда $f(x)=x$.
\end{proof}

\begin{theorem}
\labelTheorem{derivative of linear map}
Пусть $f$ - линейное отображение
\ShowEq{derivative linear map associative algebra}
Тогда
\ShowEq{derivative linear map associative algebra, 1}
\end{theorem}
\begin{proof}
Следствие теорем
\ShowEq{ref derivative of the sum}
\end{proof}

\begin{corollary}
Для любого $b\in A$
\ShowEq{derivative, xb-bx, algebra}
\qed
\end{corollary}

\begin{convention}
\labelConvention{set of permutations SO}
Для $n\ge 0$, пусть
\ShowEq{set of permutations SO}
- множество перестановок
\EqParm{s in SO(kn)}{K=n}
таких, что каждая перестановка $\sigma$
сохраняет порядок переменных $x_i$:
если $i<j$, то в кортеже
\ShowEq{s(y1kxn)}
$x_i$
предшествует
$x_j$.
\qed
\end{convention}

\begin{lemma}
\labelLemma{enumerate set of permutations S(1,n)}
{\it
Множество перестановок $S(1,n)$
мы можем пронумеровать индексом
\ShowEq{i 1n}
таким образом, что
\StartLabelItem
\begin{enumerate}
\item
\ShowEq{s1(y)=y}
\item
Если $i>1$, то
\ShowEq{si(xi)=y}
\end{enumerate}
}
\end{lemma}
\begin{proof}
Так как порядок переменных
\ShowEq{x2...n}
в перестановке
\ShowEq{s in S1n}
не зависит от перестановки, перестановки
\ShowEq{s in S1n}
отличаются местом, которое занимает переменная $y$.
Соответственно, мы можем пронумеровать
множество перестановок $S(1,n)$ индексом,
значение которого соответствует номеру позиции переменной $y$.
\end{proof}

Лемма
\RefLemma{enumerate set of permutations S(1,n)}
имеет простую интерпретацию.
Предположим, что $n-1$ белых шаров и один чёрный лежат в пенале.
Чёрный шар - самый левый шар, и белые шары
пронумерованы от $2$ до $n$ в том порядке, как они лежат в пенале.
Суть перестановки $\sigma_k$ состоит в том, что мы вынимаем
чёрный шар из пенала и затем мы ложим его в ячейку с номером $k$.
При этом, белые шары с номером, не превышающим $k$, сдвигаются влево.

\begin{lemma}
\labelLemma{S(1,n+1)=S(1,n)+}
{\it
Для $n>0$, пусть
\ShowEq{S+(1,n)=}
Тогда
\ShowEq{S(1,n+1)=S(1,n)+}
}
\end{lemma}
\begin{proof}
Пусть
\ShowEq{sigma in S+}
Согласно определению
\EqRef{S+(1,n)=},
существует перестановка
\ShowEq{tau in S1n}
такая, что
\ShowEq{tau x1n n+1}
Согласно соглашению
\RefConvention{set of permutations SO},
из утверждения
\ShowEq{i<j<n+1}
следует, что в кортеже
\ShowEq{tau x1n n+1}
переменная $x_j$ расположена между переменными $x_i$ и $x_{n+1}$.
Согласно соглашению
\RefConvention{set of permutations SO},
\ShowEq{sigma in S1n}
Следовательно
\ShowEq{S+ subset S}
Согласно лемме
\RefLemma{enumerate set of permutations S(1,n)},
множество
\ShowEq{S+(1,n)}
имеет $n$ перестановок.

Пусть
\ShowEq{sigma=x2n y}
Согласно соглашению
\RefConvention{set of permutations SO},
\ShowEq{sigma in S}
Согласно определению
\EqRef{S+(1,n)=},
\ShowEq{sigma not in S+}

Следовательно, мы перечислили $n+1$ элемент множества $S(1,n+1)$.
Согласно лемме
\RefLemma{enumerate set of permutations S(1,n)},
утверждение
\EqRef{S(1,n+1)=S(1,n)+}
является следствием утверждений
\EqRef{S+ subset S},
\EqRef{sigma in S}.
\end{proof}

\begin{theorem}
\labelTheorem{dpn dx=+SO}
Для произвольного одночлена
\ShowEq{pn(x)=a xn}
производная имеет вид
\ShowEq{dpn dx=+SO}
\end{theorem}
\begin{proof}
Для $n=1$,
отображение
\ShowEq{p1(x)=}
является линейным отображением.
Согласно теореме
\RefTheorem{derivative, fx=axb, algebra}
и соглашению
\RefConvention{set of permutations SO}
\ShowEq{dp1(x)=}

Пусть утверждение справедливо для $n-1$
\ShowEq{dpn-1}
Если
\ShowEq{pn(x)=}
то согласно теореме
\ShowEq{ref derivative of product, theorem}
и определению
\EqRef{pn(x)=}
\ShowEq{dpn(x)=}
Равенство
\ShowEq{dpn(x)= 1}
следует из
\EqRef{dx/dx=1},
\EqRef{derivative, product over constant, algebra},
\EqRef{dpn-1},
\EqRef{dpn(x)=}.
Равенство
\ShowEq{dpn(x)= 2}
следует из
\EqRef{dpn(x)= 1}
и правила перемножения одночленов (определения
\RefDefinition{otimes -},
\RefDefinition{product of homogeneous polynomials}).
Согласно лемме
\RefLemma{S(1,n+1)=S(1,n)+},
равенство
\EqRef{dpn dx=+SO}
является следствием равенства
\EqRef{dpn(x)= 2}.
\end{proof}

\begin{lemma}
\labelLemma{sigma->(mu,nu)}
{\it
Пусть
\ShowEq{k<n}
Для любой перестановки
\ShowEq{s in S(k+1,n)}
существует единственная пара перестановок
\ShowEq{mn in S(k,n)}
такая, что
\ShowEq{s=nu(mu)}
}
\end{lemma}
\begin{proof}
\end{proof}

\begin{lemma}
\labelLemma{(mu,nu)->sigma}
{\it
Пусть
\ShowEq{k<n}
Для любой пары перестановок
\ShowEq{mn in S(k,n)}
существует единственная перестановка
\ShowEq{s in S(k+1,n)}
такая, что
\ShowEq{s=nu(mu)}
}
\end{lemma}
\begin{proof}
\end{proof}

\begin{theorem}
\labelTheorem{dkpn dx=+SO}
Для произвольного одночлена
\ShowEq{pn(x)=a xn}
производная порядка $k$ имеет вид
\ShowEq{dkpn dx=+SO}
\end{theorem}
\begin{proof}
Для $k=1$ утверждение теоремы
является утверждением теоремы
\RefTheorem{dpn dx=+SO}.
Пусть теорема верна для $k-1$. Тогда
\ShowEq{dk-1pn dx=+SO}
\end{proof}

\ifx\texFuture\Defined
\begin{theorem}
\labelTheorem{derivative of pn is symmetric, m < n, algebra}
Производная
\ShowEq{derivative of pn is symmetric}
является симметричным многочленом по переменным $h_1$, ..., $h_m$.
\end{theorem}
\begin{proof}
Для доказательства теоремы мы рассмотрим алгебраические свойства
производной и дадим эквивалентное определение.
Мы начнём с построения одночлена.

\begin{lemma}
{\it
Производная порядка $k$ многочлена  имеет вид
\ShowEq{derivative of monomial, algebraic definition, algebra}
}
\end{lemma}
Согласно построению многочлен $r_n(h_1,...,h_k,x_{k+1},...,x_n)$
симметричен по переменным $h_1$, ..., $h_k$, $x_{k+1}$, ..., $x_n$.
Следовательно, многочлен
\EqRef{derivative of monomial, algebraic definition, algebra}
симметричен по переменным $h_1$, ..., $h_k$.

При $k=1$ мы докажем, что определение
\EqRef{derivative of monomial, algebraic definition, algebra}
производной совпадает с определением
\ShowEq{ref derivative of map}

Докажем теперь, что определение
\EqRef{derivative of monomial, algebraic definition, algebra}
производной совпадает с определением
\ShowEq{ref derivative of Order n}
для $k>1$.

Пусть равенство
\EqRef{derivative of monomial, algebraic definition, algebra}
верно для $k-1$.
Рассмотрим произвольное слагаемое многочлена $r_n(h_1,...,h_{k-1},x_k,...,x_n)$.
Отождествляя переменные $h_1$, ..., $h_{k-1}$
с элементами тела $D$, мы рассмотрим многочлен
\begin{equation}
R_{n-k}(x_k,...,x_n)=r_n(h_1,...,h_{k-1},x_k,...,x_n)
\EqLabel{reduced polynom, algebra}
\end{equation}
Положим $P_{n-k}(x)=R_{n-k}(x_k,...,x_n)$, $x_k=...=x_n=x$.
Следовательно
\ShowEq{derivative of pn is symmetric, 2}
Согласно определению
\ShowEq{ref derivative of Order n}
производной
\ShowEq{derivative of Order n, 1, algebra}
Согласно определению
\EqRef{derivative of monomial, algebraic definition, algebra}
производной
\ShowEq{derivative of monomial, algebraic definition, 1, algebra}
Согласно определению \EqRef{reduced polynom, algebra},
из равенства
\EqRef{derivative of monomial, algebraic definition, 1, algebra}
следует
\begin{equation}
\partial P_{n-k}(x)(h_k)=r_n(h_1,...,h_k,x_{k+1},...,x_n)\ \ \ x_{k+1}=x_n=x
\EqLabel{derivative of monomial, algebraic definition, 2, algebra}
\end{equation}
Из сравнения \EqRef{derivative of Order n, 1, algebra}
и \EqRef{derivative of monomial, algebraic definition, 2, algebra}
следует
\[
\partial^k p_n(x)(h_1;...;h_k)=r_n(h_1,...,h_k,x_{k+1},...,x_n)\ \ \ x_{k+1}=x_n=x
\]
Следовательно равенсто
\EqRef{derivative of monomial, algebraic definition, algebra}
верно для любых $k$ и $n$.

Утверждение теоремы доказано.
\end{proof}
\fi

\ShowTheorem{derivative x2}
\ShowProof{derivative x2}

\begin{remark}
Теорема
\RefTheorem{derivative x2}
также является следствием теоремы
\RefTheorem{dpn dx=+SO}
так как
\ShowEq{x2=1x1x1}
\qed
\end{remark}

\begin{theorem}
\labelTheorem{derivative x3}
Пусть $D$ - полное коммутативное кольцо характеристики $0$.
Пусть $A$ - ассоциативная банаховая $D$\Hyph алгебра.
Тогда
\ShowEq{derivative x3, algebra}
\ShowEq{derivative x3 differential, algebra}
\end{theorem}
\begin{proof}
Согласно теореме
\RefTheorem{derivative of product, algebra},
\ShowEq{derivative x3 =}
Равенство
\EqRef{derivative x3, algebra}
является следствием равенства
\EqRef{derivative x3 =}.
Равенство
\EqRef{derivative x3 differential, algebra}
является следствием равенства
\EqRef{derivative x3, algebra}
и определения
\RefDefinition{differential of map}.
\end{proof}

\begin{theorem}
Пусть $D$ - полное коммутативное кольцо характеристики $0$.
Пусть $A$ - ассоциативная $D$\Hyph алгебра с делением.
Тогда\,\footnote{
Утверждение теоремы аналогично примеру IX,
\citeBib{Hamilton Elements of Quaternions 1}, с. 451.
Если произведение коммутативно, то равенство
\EqRef{derivative x power -1, algebra}
принимает вид
\ShowEq{derivative x power -1, field}}
\ShowEq{derivative x power -1, algebra}
\ShowEq{differential x power -1, algebra}
\ShowEq{derivative x power -1 component, algebra}
\end{theorem}
\begin{proof}
Подставим $f(x)=x^{-1}$ в определение
\ShowEq{ref derivative, representation in algebra}
\ShowEq{derivative x power -1, algebra, 1}
Равенство \EqRef{derivative x power -1, algebra}
следует из цепочки равенств
\EqRef{derivative x power -1, algebra, 1}.
Равенство
\EqRef{differential x power -1, algebra}
является следствием равенства
\EqRef{derivative x power -1, algebra}
и определения
\RefDefinition{differential of map}.
Равенство
\EqRef{derivative x power -1 component, algebra}
является следствием равенства
\EqRef{derivative x power -1, algebra}.
\end{proof}

\begin{theorem}
Пусть $D$ - полное коммутативное кольцо характеристики $0$.
Пусть $A$ - ассоциативная $D$\Hyph алгебра с делением.
Тогда\,\footnote{
Если произведение коммутативно, то
\[
y=xax^{-1}=a
\]
Соответственно производная обращается в $0$.}
\ShowEq{derivative xax power -1, algebra}
\ShowEq{differential xax power -1, algebra}
\ShowEq{derivative xax power -1 component, algebra}
\end{theorem}
\begin{proof}
Равенство \EqRef{derivative xax power -1, algebra}
является следствием равенств\newline
\ShowEq{ref derivative, fx=axb}
Равенство
\EqRef{differential xax power -1, algebra}
является следствием равенства
\EqRef{derivative xax power -1, algebra}
и определения
\RefDefinition{differential of map}.
Равенство
\EqRef{derivative xax power -1 component, algebra}
является следствием равенства
\EqRef{derivative xax power -1, algebra}.
\end{proof}

\begin{theorem}
\labelTheorem{dex=ex}
\ShowEq{dex=ex}
\end{theorem}
\begin{proof}
Теорема является следствием теоремы
\RefTheorem{exponent}.
\end{proof}

\begin{theorem}
\labelTheorem{dsh dch}
\ShowEq{dsh=ch}
\ShowEq{dch=sh}
\end{theorem}
\begin{proof}
Теорема является следствием теоремы
\RefTheorem{sh ch}.
\end{proof}

\begin{theorem}
\labelTheorem{dsin dcos}
\ShowEq{dsin=cos}
\ShowEq{dcos=sin}
\end{theorem}
\begin{proof}
Теорема является следствием теоремы
\RefTheorem{sin cos}.
\end{proof}

\section{Таблица интегралов}

\begin{theorem}
Пусть отображение
\ShowEq{f:A->B}fAB
дифференцируемо.
Тогда
\ShowEq{int df=f}
\end{theorem}
\begin{proof}
Теорема является следствием определения
\RefDefinition{indefinite integral}.
\end{proof}

\begin{theorem}
\ShowEq{int=axb}
\ShowEq{int=axb=}
\end{theorem}
\begin{proof}
Согласно определению
\RefDefinition{indefinite integral},
отображение $y$ является интегралом
\EqRef{int=axb},
если отображение $y$ удовлетворяет дифференциальному уравнению
\ShowEq{differential equation, additive function, algebra}
и начальному условию
\DrawEq{differential equation, initial}{y=axb, algebra}
Согласно теореме
\RefTheorem{derivative of const, algebra},
из равества
\EqRef{differential equation, additive function, algebra}
следует, что вторая производная имеет вид
\ShowEq{differential equation, additive function, 1, algebra}
Разложение в ряд Тейлора
\ShowEq{differential equation, additive function, solution, algebra}
следует из
\ShowEq{differential equation y=axb, ref, algebra}
Равенство
\EqRef{int=axb}
является следствием равенств
\EqRef{differential equation, additive function, algebra},
\eqRef{differential equation, initial}{y=axb, algebra},
\EqRef{differential equation, additive function, solution, algebra}.
\end{proof}

\begin{remark}
Согласно определению
\EqRef{a ox b c=}
мы можем записать интеграл
\EqRef{int=axb}
следующим образом
\ShowEq{int=axb 1}
\qed
\end{remark}

\begin{theorem}
\ShowEq{int ex=ex+C}
\end{theorem}
\begin{proof}
Теорема является следствием теоремы
\RefTheorem{dex=ex}
и определения
\RefDefinition{indefinite integral}.
\end{proof}

\begin{remark}
Согласно определению
\EqRef{a ox b c=}
мы можем записать интеграл
\EqRef{int ex=ex+C}
следующим образом
\ShowEq{int ex=ex+C 1}
\qed
\end{remark}

\begin{theorem}
\ShowEq{int sh=ch+C}
\ShowEq{int ch=sh+C}
\end{theorem}
\begin{proof}
Теорема является следствием теоремы
\RefTheorem{dsh dch}
и определения
\RefDefinition{indefinite integral}.
\end{proof}

\begin{remark}
Согласно определению
\EqRef{a ox b c=}
мы можем записать интегралы
\EqRef{int sh=ch+C},
\EqRef{int ch=sh+C}
следующим образом
\ShowEq{int sh=ch+C 1}
\ShowEq{int ch=sh+C 1}
\qed
\end{remark}

\begin{theorem}
\ShowEq{int sin=cos+C}
\ShowEq{int cos=sin+C}
\end{theorem}
\begin{proof}
Теорема является следствием теоремы
\RefTheorem{dsin dcos}
и определения
\RefDefinition{indefinite integral}.
\end{proof}

\begin{remark}
Согласно определению
\EqRef{a ox b c=}
мы можем записать интегралы
\EqRef{int sin=cos+C},
\EqRef{int cos=sin+C}
следующим образом
\ShowEq{int sin=cos+C 1}
\ShowEq{int cos=sin+C 1}
\qed
\end{remark}



==> Symbol.Russian.tex <==
%auto-ignore
\def\indexname{Специальные символы и обозначения}
\OpenIndex

\SetIndexSpace%0%0
\Symb%
   {прямая сумма}%
   {direct sum}%
   {0}{0}%
\Symb%
   {единичный интервал}%
   {unit interval}%
   {0}{0}%

\SetIndexSpace%A%0
\Symb%
   {минорная матрица}%
   {A from b a}%
   {A}{0}%
\Symb%
   {минорная матрица}%
   {A from columns T}%
   {A}{0}%
\Symb%
   {минорная матрица}%
   {A from rows S}%
   {A}{0}%
\Symb%
   {множество векторов, разложение которых относительно базиса $\Basis e$ сходится нормально}%
   {A plus Schauder}%
   {A}{0}%
\Symb%
   {минорная матрица}%
   {A without column a}%
   {A}{0}%
\Symb%
   {минорная матрица}%
   {A without columns T}%
   {A}{0}%
\Symb%
   {минорная матрица}%
   {A without row b}%
   {A}{0}%
\Symb%
   {минорная матрица}%
   {A without rows S}%
   {A}{0}%
\Symb%
   {активное представление группы $G(f)$ в многообразии базисов $\mathcal B(f)$}%
   {active representation in basis manifold}%
   {A}{0}%
\Symb%
   {активное представление группы $G(\Vector  f)$ в многообразии базисов $\mathcal B(\Vector f)$}%
   {active representation in basis manifold, tower of representations}%
   {A}{0}%
\Symb%
   {$A$\Hyph алгебра многочленов над $D$\Hyph алгеброй $A$}%
   {algebra of polynomials over algebra}%
   {A}{0}%
\Symb%
   {алгебра многочленов над $D$\Hyph алгеброй $A$}%
   {algebra of polynomials over D algebra}%
   {A}{0}%
\Symb%
   {алгебра рациональных отображений алгебры $A$}%
   {algebra of rational mappings of algebra}%
   {A}{0}%
\Symb%
   {аффинное пространство}%
   {An}%
   {A}{0}%
\Symb%
   {ассоциатор $D$\Hyph алгебры}%
   {associator of algebra}%
   {A}{0}%
\Symb%
   {\subs строка ($c$\hyph строка) матрицы}%
   {c row}%
   {A}{0}%
\Symb%
   {категория левосторонних представлений $\Omega_1$\Hyph алгебры $A$}%
   {category of left-side representations of Omega1 algebra}%
   {A}{0}%
\Symb%
   {категория представлений}%
   {category of representations}%
   {A}{0}%
\Symb%
   {коммутатор $D$\Hyph алгебры}%
   {commutator of algebra}%
   {A}{0}%
\Symb%
   {компонента линейного отображения}%
   {component of linear map, vector}%
   {A}{0}%
\Symb%
   {компонента $p$ полилинейного отображения $\Vector A$}%
   {component of polyadditive map, D vector space}%
   {A}{0}%
\Symb%
   {компонента полилинейного отображения}%
   {component of polylinear map, vector}%
   {A}{0}%
\Symb%
   {сопряжённый $D$\Hyph  модуль}%
   {conjugated D module}%
   {A}{0}%
\Symb%
   {\CR степень элемента $A$ бикольца}%
   {cr power}%
   {A}{0}%
\Symb%
   {\crd вектор}%
   {crd vector}%
   {A}{0}%
\Symb%
   {\CR обратный элемент бикольца}%
   {cr-inverse element}%
   {A}{0}%
\Symb%
   {\CR произведение}%
   {cr-product}%
   {A}{0}%
\Symb%
   {\dcr вектор}%
   {dcr vector}%
   {A}{0}%
\Symb%
   {производная левого сдвига}%
   {derivative of left shift}%
   {A}{0}%
\Symb%
   {производная левого сдвига в $1$\Hyph параметрической группе Ли}%
   {derivative of left shift, 1-Parameter Group}%
   {A}{0}%
\Symb%
   {производная левого сдвига в $1$\Hyph параметрической D группе Ли}%
   {derivative of left shift, 1-Parameter Group, algebra}%
   {A}{0}%
\Symb%
   {производная правого сдвига}%
   {derivative of right shift}%
   {A}{0}%
\Symb%
   {производная правого сдвига в $1$\Hyph параметрической группе Ли}%
   {derivative of right shift, 1-Parameter Group}%
   {A}{0}%
\Symb%
   {производная правого сдвига в $1$\Hyph параметрической D группе Ли}%
   {derivative of right shift, 1-Parameter Group, algebra}%
   {A}{0}%
\Symb%
   {производная левого сдвига}%
   {derivative of Tstar shift}%
   {A}{0}%
\Symb%
   {\drc вектор}%
   {drc vector}%
   {A}{0}%
\Symb%
   {координаты вектора $a$ относительно базиса Гамеля}%
   {Hamel basis, coordinates}%
   {A}{0}%
\Symb%
   {эрмитово сопряжение в теле}%
   {hermitian conjugation, division ring}%
   {A}{0}%
\Symb%
   {тензор, обратный тензору $a$}%
   {inverse tensor}%
   {A}{0}%
\Symb%
   {изоморфны}%
   {isomorphic}%
   {A}{0}%
\Symb%
   {$(^j_i)$\hyph\CR квазидетерминант}%
   {j i CR quasideterminant definition}%
   {A}{0}%
\Symb%
   {$(ji)$\hyph квазидетерминант матрицы $\bfA$}%
   {j i quasideterminant definition}%
   {A}{0}%
\Symb%
   {$(^j_i)$\hyph $\RCcirc$\Hyph квазидетерминант}%
   {j i RCcirc-quasideterminant definition}%
   {A}{0}%
\Symb%
   {$(^j_i)$\hyph \RC квазидетерминант}%
   {j i RC-quasideterminant definition}%
   {A}{0}%
\Symb%
   {левая дробь}%
   {left fraction}%
   {A}{0}%
\Symb%
   {левый главный идеал}%
   {left principal ideal}%
   {A}{0}%
\Symb%
   {левый сдвиг в $D$\Hyph алгебре}%
   {left shift, D algebra}%
   {A}{0}%
\Symb%
   {линейная комбинация}%
   {linear combination}%
   {A}{0}%
\Symb%
   {малая группа}%
   {little group}%
   {A}{0}%
\Symb%
   {преобразование матрицы}%
   {matrix, replacing its column}%
   {A}{0}%
\Symb%
   {преобразование матрицы}%
   {matrix, replacing its row}%
   {A}{0}%
\Symb%
   {$A$\Hyph модуль однородных многочленов над $D$\Hyph алгеброй $A$}%
   {module of homogeneous polynomials over algebra}%
   {A}{0}%
\Symb%
   {норма в $D$\Hyph модуле}%
   {norm on D module}%
   {A}{0}%
\Symb%
   {$\Omega$\Hyph алгебра}%
   {Omega-algebra}%
   {A}{0}%
\Symb%
   {алгебра, противоположная алгебре $A$}%
   {opposite algebra}%
   {A}{0}%
\Symb%
   {орбита эффективного левостороннего представления}%
   {orbit of effective left-side representation}%
   {A}{0}%
\Symb%
   {орбита эффективного правостороннего представления}%
   {orbit of effective right-side representation}%
   {A}{0}%
\Symb%
   {орбита линейного отображения}%
   {orbit of linear map}%
   {A}{0}%
\Symb%
   {производная}%
   {overline nabla_l, definition 2}%
   {A}{0}%
\Symb%
   {частное линейное отображение}%
   {partial linear map}%
   {A}{0}%
\Symb%
   {главный идеал}%
   {principal ideal}%
   {A}{0}%
\Symb%
   {квазидетерминант матрицы $\bfA$}%
   {quasideterminant definition}%
   {A}{0}%
\Symb%
   {\sups строка ($r$\hyph строка) матрицы}%
   {r row}%
   {A}{0}%
\Symb%
   {\RC степень элемента $A$ бикольца}%
   {rc power}%
   {A}{0}%
\Symb%
   {$\RCcirc$\Hyph квазидетерминант}%
   {RCcirc-quasideterminant definition}%
   {A}{0}%
\Symb%
   {\rcd вектор}%
   {rcd vector}%
   {A}{0}%
\Symb%
   {\RC обратный элемент бикольца}%
   {rc-inverse element}%
   {A}{0}%
\Symb%
   {\RC произведение}%
   {rc-product}%
   {A}{0}%
\Symb%
   {\RC квазидетерминант}%
   {RC-quasideterminant definition}%
   {A}{0}%
\Symb%
   {правый главный идеал}%
   {right principal ideal}%
   {A}{0}%
\Symb%
   {правый сдвиг в $D$\Hyph алгебре}%
   {right shift, D algebra}%
   {A}{0}%
\Symb%
   {координаты вектора $a$ относительно базиса Шаудера}%
   {Schauder basis, coordinates}%
   {A}{0}%
\Symb%
   {множество аддитивных отображений}%
   {set additive maps}%
   {A}{0}%
\Symb%
   {множество обратимых элементов алгебры $A$}%
   {set of invertible elements of algebra}%
   {A}{0}%
\Symb%
   {множество нулей алгебры $A$}%
   {set of zeros of algebra}%
   {A}{0}%
\Symb%
   {множество полилинейных отображений колец $R_1$, ..., $R_n$ в модуль $S$}%
   {set polylinear maps, ring}%
   {A}{0}%
\Symb%
   {симплекс}%
   {simplex}%
   {A}{0}%
\Symb%
   {косое произведение векторов $\Vector a_1$, ..., $\Vector a_m$}%
   {skew product of vectors}%
   {A}{0}%
\Symb%
   {пространство орбит эффективного левостороннего представления}%
   {space of orbits of effective left-side representation}%
   {A}{0}%
\Symb%
   {пространство орбит эффективного правостороннего представления}%
   {space of orbits of effective right-side representation}%
   {A}{0}%
\Symb%
   {пространство орбит левостороннего представления}%
   {space of orbits of left side representation}%
   {A}{0}%
\Symb%
   {квадратный корень}%
   {square root}%
   {A}{0}%
\Symb%
   {группа стабилизации}%
   {stability group}%
   {A}{0}%
\Symb%
   {\sT сдвиг}%
   {starT shift, fibered group}%
   {A}{0}%
\Symb%
   {тензорная степень алгебры $A$}%
   {tensor power of algebra}%
   {A}{0}%
\Symb%
   {неголономные координаты вектора}%
   {vector anholonomic coordinates}%
   {A}{0}%
\Symb%
   {голономные координаты вектора}%
   {vector holonomic coordinates}%
   {A}{0}%

\SetIndexSpace%B%0
\Symb%
   {многообразие базисов \rcd векторного пространства $\Vector V$}%
   {basis manifold of rcd vector space}%
   {B}{0}%
\Symb%
   {многообразие базисов векторного пространства}%
   {basis manifold of vector space}%
   {B}{0}%
\Symb%
   {многообразие базисов представления $f$}%
   {basis manifold representation F algebra}%
   {B}{0}%
\Symb%
   {многообразие базисов башни представлений $\Vector f$}%
   {basis manifold tower of representations}%
   {B}{0}%
\Symb%
   {многообразие базисов аффинного пространства}%
   {Basis Manifold, Affine Space}%
   {B}{0}%
\Symb%
   {многообразие базисов центро-аффинного пространства}%
   {BCAn}%
   {B}{0}%
\Symb%
   {многообразие базисов евклидова пространства}%
   {BEn}%
   {B}{0}%
\Symb%
   {алгебра Бореля}%
   {Borel algebra}%
   {B}{0}%
\Symb%
   {каноническое частное от деления}%
   {canonical remainder of the division}%
   {B}{0}%
\Symb%
   {декартова степень}%
   {Cartesian power}%
   {B}{0}%
\Symb%
   {декартова степень $\Bundle A$ расслоения $\Bundle B$}%
   {Cartesian power A of bundle B}%
   {B}{0}%
\Symb%
   {декартова степень $A$ множества $B$}%
   {Cartesian power of set}%
   {B}{0}%
\Symb%
   {замкнутый шар}%
   {closed ball}%
   {B}{0}%
\Symb%
   {замыкание множества}%
   {closure of set}%
   {B}{0}%
\Symb%
   {копроизведение в категории}%
   {coproduct in category}%
   {B}{0}%
\Symb%
   {многообразие базисов центро-аффинного пространства}%
   {FCAn}%
   {B}{0}%
\Symb%
   {многообразие базисов евклидова пространства}%
   {FEn}%
   {B}{0}%
\Symb%
   {структура всех подпредставлений представления $f$}%
   {lattice of subrepresentations}%
   {B}{0}%
\Symb%
   {структура башен подпредставлений башни представлений $\Vector f$}%
   {lattice of subrepresentations, tower of representations}%
   {B}{0}%
\Symb%
   {открытый шар}%
   {open ball}%
   {B}{0}%
\Symb%
   {произведение в категории}%
   {product in category}%
   {B}{0}%
\Symb%
   {правая дробь}%
   {right fraction}%
   {B}{0}%
\Symb%
   {тензорная степень представления}%
   {tensor power of representation}%
   {B}{0}%

\SetIndexSpace%C%0
\Symb%
   {$\sigma$\Hyph алгебра измеримых относительно меры $\mu$ множеств}%
   {algebra of sets measurable with respect to measure}%
   {C}{0}%
\Symb%
   {центро-аффинное пространство}%
   {CAn}%
   {C}{0}%
\Symb%
   {центро-аффинное пространство}%
   {central affine space}%
   {C}{0}%
\Symb%
   {класс непрерывности}%
   {class Cn}%
   {C}{0}%
\Symb%
   {столбцовый определитель по $j$-му столбцу  матрицы $\bfA$}%
   {column determinant}%
   {C}{0}%
\Symb%
   {косинус}%
   {cosine}%
   {C}{0}%
\Symb%
   {$\CRcirc$\Hyph произведение матриц отображений}%
   {cr product of matrices of maps}%
   {C}{0}%
\Symb%
   {гиперболический косинус}%
   {hyperbolic cosine}%
   {C}{0}%
\Symb%
   {левые структурные константы алгебры Ли}%
   {left structural constant of Lie algebra}%
   {C}{0}%
\Symb%
   {правые структурные константы алгебры Ли}%
   {right structural constant of Lie algebra}%
   {C}{0}%
\Symb%
   {множество непрерывных отображений нескольких переменных}%
   {set continuous multivariable maps}%
   {C}{0}%
\Symb%
   {структурные константы}%
   {structural constants}%
   {C}{0}%

\SetIndexSpace%D%0
\Symb%
   {базовый вектор представления группы Ли над алгеброй $A$}%
   {basis vector of representation of Lie group over algebra A}%
   {D}{0}%
\Symb%
   {координаты базового вектора представления группы Ли над алгеброй $A$}%
   {basis vector of representation of Lie group over algebra A, coordinates}%
   {D}{0}%
\Symb%
   {компонента производной отображения $f(x)$}%
   {component of derivative}%
   {D}{0}%
\Symb%
   {компонента производной второго порядка отображения $f(x)$}%
   {component of derivative of Second Order}%
   {D}{0}%
\Symb%
   {компонента производной Гато отображения $f(x)$}%
   {component of Gateaux derivative}%
   {D}{0}%
\Symb%
   {компонента производной Гато отображения $f(x)$}%
   {component of Gateaux derivative of map, D vector space, short}%
   {D}{0}%
\Symb%
   {компонента производной Гато второго порядка отображения $f(x)$}%
   {component of Gateaux derivative of Second Order}%
   {D}{0}%
\Symb%
   {компонента производной Гато второго порядка отображения $f(x)$}%
   {component of Gateaux derivative of Second Order, D vector space}%
   {D}{0}%
\Symb%
   {компонента производной Гато отображения $f(x)$}%
   {component of Gateaux derivative, vector space}%
   {D}{0}%
\Symb%
   {сопряжение в алгебре}%
   {conjugation in algebra}%
   {D}{0}%
\Symb%
   {сопряжение в кольце}%
   {conjugation in ring}%
   {D}{0}%
\Symb%
   {координатное \rcd векторное пространство}%
   {coordinate rcd vector space}%
   {D}{0}%
\Symb%
   {координатная система отсчёта}%
   {coordinate reference frame, extensive definition}%
   {D}{0}%
\Symb%
   {координатное векторное расслоение}%
   {coordinate vector bundle}%
   {D}{0}%
\Symb%
   {производная отображения $f$}%
   {derivative of map}%
   {D}{0}%
\Symb%
   {производная отображения $f$}%
   {derivative of map inline}%
   {D}{0}%
\Symb%
   {производная порядка $n$}%
   {derivative of Order n}%
   {D}{0}%
\Symb%
   {производная порядка $n$}%
   {derivative of Order n inline}%
   {D}{0}%
\Symb%
   {производная второго порядка}%
   {derivative of Second Order}%
   {D}{0}%
\Symb%
   {производная второго порядка}%
   {derivative of Second Order inline}%
   {D}{0}%
\Symb%
   {диагональ в расслоении $\Bundle A$}%
   {diagonal in bundle, 1}%
   {D}{0}%
\Symb%
   {дифференциал независимой переменной}%
   {differential of independent variable}%
   {D}{0}%
\Symb%
   {дифференциал отображения $f$}%
   {differential of map}%
   {D}{0}%
\Symb%
   {прямое произведение тел $D_1$, ..., $D_n$}%
   {direct product of division rings, 1 n}%
   {D}{0}%
\Symb%
   {двойной определитель матрицы $\bfA$}%
   {double determinant}%
   {D}{0}%
\Symb%
   {внешний дифференциал}%
   {exterior differential}%
   {D}{0}%
\Symb%
   {\Ds производная Фреше функции $f$ тела}%
   {Frechet Dstar derivative of map, division ring}%
   {D}{0}%
\Symb%
   {\dcr производная Гато отображения $\Vector f$ $D$\Hyph векторного пространства $V$ в $D$\Hyph векторное пространство $W$}%
   {Gateaux dcr derivative of map, D vector space}%
   {D}{0}%
\Symb%
   {производная Гато отображения $f$}%
   {Gateaux derivative of map}%
   {D}{0}%
\Symb%
   {производная Гато отображения $f$}%
   {Gateaux derivative of map, fraction}%
   {D}{0}%
\Symb%
   {производная Гато порядка $n$}%
   {Gateaux derivative of Order n}%
   {D}{0}%
\Symb%
   {производная Гато порядка $n$ отображения $f$ тела}%
   {Gateaux derivative of Order n, division ring}%
   {D}{0}%
\Symb%
   {производная Гато порядка $n$ отображения $f$ алгебры}%
   {Gateaux derivative of Order n, fraction, algebra}%
   {D}{0}%
\Symb%
   {производная Гато порядка $n$ отображения $f$ тела}%
   {Gateaux derivative of Order n, fraction, division ring}%
   {D}{0}%
\Symb%
   {производная Гато второго порядка}%
   {Gateaux derivative of Second Order}%
   {D}{0}%
\Symb%
   {производная Гато второго порядка отображения $f$ алгебры}%
   {Gateaux derivative of Second Order, fraction, algebra}%
   {D}{0}%
\Symb%
   {производная Гато второго порядка отображения $f$ тела}%
   {Gateaux derivative of Second Order, fraction, division ring}%
   {D}{0}%
\Symb%
   {дифференциал Гато отображения $f$}%
   {Gateaux differential of map, vector}%
   {D}{0}%
\Symb%
   {\Ds производная Гато функции $f$ тела $D$}%
   {Gateaux Dstar derivative of map, division ring}%
   {D}{0}%
\Symb%
   {якобиан Гато отображения $D$\Hyph векторного пространства}%
   {Gateaux Jacobian of map, D vector space}%
   {D}{0}%
\Symb%
   {частная \dcr производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial dcr derivative of map, 1, D vector space}%
   {D}{0}%
\Symb%
   {частная \dcr производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial dcr derivative of map, 2, D vector space}%
   {D}{0}%
\Symb%
   {частная \dcr производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial dcr derivative of map, 3, D vector space}%
   {D}{0}%
\Symb%
   {частная производная Гато}%
   {Gateaux partial derivative}%
   {D}{0}%
\Symb%
   {смешанная частная производная Гато}%
   {Gateaux partial derivative of Second Order}%
   {D}{0}%
\Symb%
   {частная \rcd производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial rcd derivative of map, 1, D vector space}%
   {D}{0}%
\Symb%
   {частная \rcd производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial rcd derivative of map, 2, D vector space}%
   {D}{0}%
\Symb%
   {частная \rcd производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial rcd derivative of map, 3, D vector space}%
   {D}{0}%
\Symb%
   {\rcd производная Гато отображения $f$ $D$\hyph векторного пространства $V$ в $D$\hyph векторное пространство $W$}%
   {Gateaux rcd derivative of map, D vector space}%
   {D}{0}%
\Symb%
   {\sD производная Гато функции $f$ тела $D$}%
   {Gateaux starD derivative of map, division ring}%
   {D}{0}%
\Symb%
   {векторное пространство матриц}%
   {matrices vector space}%
   {D}{0}%
\Symb%
   {производная Картана}%
   {overbrace D}%
   {D}{0}%
\Symb%
   {производная}%
   {overline D}%
   {D}{0}%
\Symb%
   {частная производная}%
   {partial derivative}%
   {D}{0}%
\Symb%
   {частная производная второго порядка}%
   {partial derivative of second order}%
   {D}{0}%
\Symb%
   {производная вдоль векторного поля $e_{(k)}$}%
   {partial(k)}%
   {D}{0}%
\Symb%
   {произведение отображения на скаляр}%
   {product of map over scalar}%
   {D}{0}%
\Symb%
   {скорость отклонения}%
   {speed of deviation}%
   {D}{0}%
\Symb%
   {стандартная компонента производной}%
   {standard component of derivative}%
   {D}{0}%
\Symb%
   {стандартная компонента производной Гато}%
   {standard component of Gateaux derivative}%
   {D}{0}%
\Symb%
   {тип векторного пространства}%
   {vector space type}%
   {D}{0}%

\SetIndexSpace%E%0
\Symb%
   {матрица Якоби левого сдвига}%
   {aE, quaternion, Jacobian matrix}%
   {E}{0}%
\Symb%
   {аффинный базис}%
   {Affine Basis}%
   {E}{0}%
\Symb%
   {базис векторного пространства}%
   {Basis e}%
   {E}{0}%
\Symb%
   {базис модуля}%
   {basis for module}%
   {E}{0}%
\Symb%
   {базис в векторном пространстве $\Vector V$}%
   {basis in V}%
   {E}{0}%
\Symb%
   {базис $D$\Hyph модуля $\mathcal L(D;A_1;A_2)$}%
   {basis L(A1,A2)}%
   {E}{0}%
\Symb%
   {базис \crd векторного пространства}%
   {basis, crd vector space}%
   {E}{0}%
\Symb%
   {базис $D$\Hyph векторного пространства}%
   {basis, D vector space}%
   {E}{0}%
\Symb%
   {базис \dcr векторного пространства}%
   {basis, dcr vector space}%
   {E}{0}%
\Symb%
   {базис \drc векторного пространства}%
   {basis, drc vector space}%
   {E}{0}%
\Symb%
   {базис \rcd векторного пространства}%
   {basis, rcd vector space}%
   {E}{0}%
\Symb%
   {базис в векторного расслоения}%
   {basis, vector bundle}%
   {E}{0}%
\Symb%
   {базис $(n)$\hyph векторного пространства}%
   {basis,n vector space}%
   {E}{0}%
\Symb%
   {декартова степень расслоенного пространства}%
   {Cartesian power of total spaces}%
   {E}{0}%
\Symb%
   {декартово произведение расслоенных пространств}%
   {Cartesian product of total spaces, definition 1}%
   {E}{0}%
\Symb%
   {центро-аффинный базис}%
   {Central Affine Basis}%
   {E}{0}%
\Symb%
   {форма системы отсчёта}%
   {dual forms, reference frame}%
   {E}{0}%
\Symb%
   {евклидово пространство}%
   {Euclid space}%
   {E}{0}%
\Symb%
   {евклидово пространство}%
   {Euclid space, division ring}%
   {E}{0}%
\Symb%
   {экспонента}%
   {exponent}%
   {E}{0}%
\Symb%
   {базис Гамеля}%
   {Hamel basis}%
   {E}{0}%
\Symb%
   {тождественное преобразование расслоения}%
   {identical transformation of bundle}%
   {E}{0}%
\Symb%
   {линейный автоморфизм алгебры кватернионов}%
   {mapping E, quaternion}%
   {E}{0}%
\Symb%
   {линейный автоморфизм алгебры кватернионов}%
   {mapping E_1, quaternion}%
   {E}{0}%
\Symb%
   {линейный автоморфизм алгебры кватернионов}%
   {mapping E_2, quaternion}%
   {E}{0}%
\Symb%
   {ортонормированный базис}%
   {Orthonornal Basis}%
   {E}{0}%
\Symb%
   {псевдоевклидово пространство}%
   {pseudo Euclid space}%
   {E}{0}%
\Symb%
   {псевдоевклидово пространство}%
   {pseudo Euclid space, division ring}%
   {E}{0}%
\Symb%
   {алгебра кватернионов над полем $F$}%
   {quaternion algebra over the field}%
   {E}{0}%
\Symb%
   {алгебра кватернионов с делением над полем $F$}%
   {quaternion division algebra over the fieldL}%
   {E}{0}%
\Symb%
   {приведенное декартово произведение расслоенных пространств}%
   {reduced Cartesian product of total spaces, definition 1}%
   {E}{0}%
\Symb%
   {базис Шаудера}%
   {Schauder basis}%
   {E}{0}%
\Symb%
   {множество эндоморфизмов}%
   {set of endomorphisms}%
   {E}{0}%
\Symb%
   {множество невырожденных \sT преобразований расслоения $\Bundle E$}%
   {set of starT nonsingular transformations of bundle}%
   {E}{0}%
\Symb%
   {множество преобразований универсальной алгебры}%
   {set of transformations}%
   {E}{0}%
\Symb%
   {множество невырожденных \Ts преобразований расслоения $\Bundle E$}%
   {set of Tstar nonsingular transformations of bundle}%
   {E}{0}%
\Symb%
   {стандартные координаты базиса}%
   {standard coordinates of basis}%
   {E}{0}%
\Symb%
   {стандартные координаты системы отсчёта}%
   {standard coordinates of reference frame}%
   {E}{0}%
\Symb%
   {векторное поле системы отсчёта}%
   {vector field of reference frame}%
   {E}{0}%
\Symb%
   {вектор базиса}%
   {vector of basis}%
   {E}{0}%

\SetIndexSpace%F%0
\Symb%
   {альтернация полилинейного отображения}%
   {alternation of polylinear map}%
   {F}{0}%
\Symb%
   {компонента линейного отображения $f$ тела}%
   {component of linear map, division ring}%
   {F}{0}%
\Symb%
   {компонента полилинейного отображения}%
   {component of polylinear map}%
   {F}{0}%
\Symb%
   {преобразование сопряжения}%
   {conjugation transformation}%
   {F}{0}%
\Symb%
   {внешнее произведение}%
   {exterior product}%
   {F}{0}%
\Symb%
   {расслоенный морфизм из расслоения $\Bundle A$ в $\Bundle B$}%
   {fibered morphism from A into B}%
   {F}{0}%
\Symb%
   {фильтр $\mathfrak{F}$ сходится к множеству $A$}%
   {filter converges}%
   {F}{0}%
\Symb%
   {гомоморфизм расслоенных универсальных алгебр}%
   {homomorphism of fibered universal algebras}%
   {F}{0}%
\Symb%
   {обратное расслоенное соответствие}%
   {inverse fibered correspondence, 1}%
   {F}{0}%
\Symb%
   {обратное приведенное расслоенное соответствие}%
   {inverse reduced fibered correspondence, 1}%
   {F}{0}%
\Symb%
   {отображение в декартово произведение}%
   {map to Cartesian product}%
   {F}{0}%
\Symb%
   {норма функционала}%
   {norm of functional}%
   {F}{0}%
\Symb%
   {норма отображения}%
   {norm of map}%
   {F}{0}%
\Symb%
   {норма полилинейного отображения}%
   {norm of polymap}%
   {F}{0}%
\Symb%
   {норма представления}%
   {norm of representation}%
   {F}{0}%
\Symb%
   {орбита представления}%
   {orbit of representation}%
   {F}{0}%
\Symb%
   {ортонормированный базис}%
   {Orthonormal Basis, division ring}%
   {F}{0}%
\Symb%
   {кватернионная алгебра над полем ${\rm {\mathbb{F}}}$}%
   {quaternion algebra F a b}%
   {F}{0}%
\Symb%
   {система отсчёта}%
   {reference frame}%
   {F}{0}%
\Symb%
   {система отсчёта, расширенное определение}%
   {reference frame, extensive definition}%
   {F}{0}%
\Symb%
   {стандартная компонента биаддитивного отображения $f$ над полем $F$}%
   {standard component of biadditive map, division ring}%
   {F}{0}%
\Symb%
   {стандартная компонента линейного отображения }%
   {standard component of linear map, G}%
   {F}{0}%
\Symb%
   {стандартная компонента полилинейного отображения}%
   {standard component of polylinear map}%
   {F}{0}%
\Symb%
   {стандартная компонента квадратичного отображения $f$ над полем $F$}%
   {standard component of quadratic map, division ring}%
   {F}{0}%
\Symb%
   {стандартная компонента тензора}%
   {standard component of tensor}%
   {F}{0}%
\Symb%
   {сумма отображений}%
   {sum of maps}%
   {F}{0}%
\Symb%
   {симметрирование полилинейного отображения}%
   {symmetrization of polylinear map}%
   {F}{0}%

\SetIndexSpace%G%0
\Symb%
   {группа аффинных преобразований}%
   {affine transformation group}%
   {G}{0}%
\Symb%
   {группа аффинных преобразований}%
   {affine transformation group}%
   {G}{0}%
\Symb%
   {декартово произведение групп $G_1$, ..., $G_n$}%
   {Cartesian product of groups, 1 n}%
   {G}{0}%
\Symb%
   {\CR матричная группа}%
   {cr-matrix group}%
   {G}{0}%
\Symb%
   {расслоенная малая группа сечения $h$}%
   {fibered little group}%
   {G}{0}%
\Symb%
   {расслоенная группа стабилизации сечения $h$}%
   {fibered stability group}%
   {G}{0}%
\Symb%
   {группа автоморфизмов представления $f$}%
   {group of automorphisms of representation}%
   {G}{0}%
\Symb%
   {группа гомоморфизмов векторного пространства $\Vector V$}%
   {GV}%
   {G}{0}%
\Symb%
   {неопределённый интеграл}%
   {indefinite integral}%
   {G}{0}%
\Symb%
   {определённая слева алгебра Ли группы Ли}%
   {left defined Lie algebra of Lie group}%
   {G}{0}%
\Symb%
   {алгебра Ли группы Ли}%
   {Lie algebra of Lie group}%
   {G}{0}%
\Symb%
   {группа линейных преобразований}%
   {linear transformation group}%
   {G}{0}%
\Symb%
   {малая группа}%
   {little group}%
   {G}{0}%
\Symb%
   {орбита эффективного	\Ts представления группы}%
   {orbit of effective starT representation of fibered group}%
   {G}{0}%
\Symb%
   {орбита эффективного		\Ts представления расслоенной группы}%
   {orbit of effective Tstar representation of fibered group}%
   {G}{0}%
\Symb%
   {\RC матричная группа}%
   {rc-matrix group}%
   {G}{0}%
\Symb%
   {определённая справа алгебра Ли группы Ли}%
   {right defined Lie algebra}%
   {G}{0}%
\Symb%
   {группа стабилизации}%
   {stability group}%
   {G}{0}%

\SetIndexSpace%H%0
\Symb%
   {обращение Адамара матрицы}%
   {Hadamard inverse of matrix}%
   {H}{0}%
\Symb%
   {горизонтальная компонента вектора}%
   {horizontal component of vector}%
   {H}{0}%
\Symb%
   {горизонтальное подпространство}%
   {horizontal subspace}%
   {H}{0}%
\Symb%
   {алгебра кватернионов}%
   {quaternion algebra}%
   {H}{0}%
\Symb%
   {кватернионная алгебра}%
   {quaternion algebra H a b}%
   {H}{0}%
\Symb%
   {множество гомоморфизмов}%
   {set of homomorphisms}%
   {H}{0}%

\SetIndexSpace%I%0
\Symb%
   {инфинитезимальные образующие представления}%
   {infinitesimal generator i of representation}%
   {I}{0}%
\Symb%
   {инфинитезимальные образующие представления}%
   {infinitesimal generator of representation}%
   {I}{0}%
\Symb%
   {инфинитезимальные образующие группы Ли}%
   {Lie group infinitesimal generators}%
   {I}{0}%
\Symb%
   {модуль векторов алгебры $A$}%
   {vector module of algebra}%
   {I}{0}%
\Symb%
   {модуль векторов кольца $D$}%
   {vector module of ring}%
   {I}{0}%
\Symb%
   {вектор элемента $d$ алгебры}%
   {vector of algebra}%
   {I}{0}%
\Symb%
   {вектор элемента $d$ кольца}%
   {vector of ring}%
   {I}{0}%

\SetIndexSpace%J%0
\Symb%
   {оператор замыкания представления $f$}%
   {closure operator, representation}%
   {J}{0}%
\Symb%
   {оператор замыкания башни представлений $\Vector f$}%
   {closure operator, tower of representations}%
   {J}{0}%
\Symb%
   {матрица Якоби правого сдвига}%
   {Ea, quaternion, Jacobian matrix}%
   {J}{0}%
\Symb%
   {подпредставление, порождённое множеством $X$}%
   {subrepresentation generated by set}%
   {J}{0}%
\Symb%
   {башня подпредставлений башни представлений $\Vector f$, порождённая кортежем множеств $\VX X$}%
   {subrepresentation generated by tuple of sets}%
   {J}{0}%

\SetIndexSpace%K%0
\Symb%
   {ядро гомоморфизма}%
   {kernel of homomorphism}%
   {K}{0}%
\Symb%
   {ядро линейного отображения}%
   {kernel of linear map}%
   {K}{0}%

\SetIndexSpace%L%0
\Symb%
   {декартова степень систем подмножеств}%
   {Cartesian power of systems of subsets}%
   {L}{0}%
\Symb%
   {декартово произведение систем подмножеств}%
   {Cartesian product of systems of subsets}%
   {L}{0}%
\Symb%
   {левое алгебраическое дополнение элемента  $a_{i{\kern 1pt} j} $ матрицы}%
   {left cofactor, matrix}%
   {L}{0}%
\Symb%
   {левое двойное алгебраическое дополнение элемента $a_{ij}$ матрицы}%
   {left double cofactor}%
   {L}{0}%
\Symb%
   {левый сдвиг}%
   {left shift}%
   {L}{0}%
\Symb%
   {производная Ли связности}%
   {Lie derivative of connection}%
   {L}{0}%
\Symb%
   {производная Ли метрики}%
   {Lie derivative of metric}%
   {L}{0}%
\Symb%
   {предел соответствия $\Phi$ по фильтру $\mathfrak{F}$}%
   {limit of correspondence with respect to the filter}%
   {L}{0}%
\Symb%
   {предел последовательности}%
   {limit of sequence}%
   {L}{0}%
\Symb%
   {линейная комбинация}%
   {linear combination}%
   {L}{0}%
\Symb%
   {модуль косо симметричных полилинейных отображений}%
   {module of skew symmetric polylinear maps}%
   {L}{0}%
\Symb%
   {пассивное преобразование}%
   {passive transformation}%
   {L}{0}%
\Symb%
   {$D$\Hyph модуль непрерывных линейных отображений нормированного $D$\Hyph модуля $A_1$ в нормированный $D$\Hyph модуль $A_2$}%
   {set continuous linear mappings, module}%
   {L}{0}%
\Symb%
   {множество непрерывных линейных отображений}%
   {set continuous linear maps, vector}%
   {L}{0}%
\Symb%
   {множество непрерывных полилинейных отображений}%
   {set continuous polylinear maps}%
   {L}{0}%
\Symb%
   {множество линейных отображений}%
   {set linear maps}%
   {L}{0}%
\Symb%
   {множество левосторонних невырожденных преобразований универсальной алгебры $M$}%
   {set of left-side nonsingular transformations}%
   {L}{0}%
\Symb%
   {множество полилинейных отображений}%
   {set polylinear maps}%
   {L}{0}%
\Symb%
   {множество $n$\hyph линейных отображений}%
   {set polylinear maps An}%
   {L}{0}%
\Symb%
   {множество полилинейных отображений}%
   {set polylinear maps, D vector space}%
   {L}{0}%
\Symb%
   {множество полилинейных отображений алгебр $A_1$, ..., $A_n$ в алгебру $A$}%
   {set polylinear maps, finite dimensional algebra}%
   {L}{0}%

\SetIndexSpace%M%0
\Symb%
   {множество левосторонних преобразований универсальной алгебры $M$}%
   {set of left-side transformations}%
   {M}{0}%
\Symb%
   {множество отображений в $\Omega$\Hyph группу $A$}%
   {set of maps to Omega group}%
   {M}{0}%
\Symb%
   {множество правосторонних преобразований универсальной алгебры $M$}%
   {set of right-side transformations}%
   {M}{0}%
\Symb%
   {пространство орбит \Ts{G}представления}%
   {space of orbits of G* representation}%
   {M}{0}%

\SetIndexSpace%N%0
\Symb%
   {норма кватерниона $x$}%
   {norm, quaternion algebra}%
   {N}{0}%
\Symb%
   {ядро $D$\Hyph алгебры $A$}%
   {nucleus of algebra}%
   {N}{0}%

\SetIndexSpace%O%0
\Symb%
   {геометрический объект в координатном представлении, определённом в \rcd векторном пространстве}%
   {geometric object, coordinate rcd vector space}%
   {O}{0}%
\Symb%
   {геометрический объект в координатном представлении}%
   {geometric object, coordinate vector space}%
   {O}{0}%
\Symb%
   {геометрический объект, определённый в \rcd векторном пространстве}%
   {geometric object, rcd vector space}%
   {O}{0}%
\Symb%
   {алгебра октонионов}%
   {octonion algebra}%
   {O}{0}%
\Symb%
   {орбита представления расслоенной группы $\Bundle G$}%
   {orbit of representation of fibered group}%
   {O}{0}%
\Symb%
   {орбита \Ts{G}представления группы}%
   {orbit of representation of group}%
   {O}{0}%
\Symb%
   {тензорное произведение}%
   {tensor product}%
   {O}{0}%

\SetIndexSpace%P%0
\Symb%
   {расслоение}%
   {bundle}%
   {P}{0}%
\Symb%
   {расслоение уровня $2$}%
   {bundle of level 2}%
   {P}{0}%
\Symb%
   {расслоение уровня $n$}%
   {bundle of level n}%
   {P}{0}%
\Symb%
   {декартова степень $n$ расслоения $\bundle{}{p}{E}{}$}%
   {Cartesian power of bundle}%
   {P}{0}%
\Symb%
   {декартово произведение расслоений}%
   {Cartesian product of bundles, definition 1}%
   {P}{0}%
\Symb%
   {пассивное представление группы $G(f)$ в многообразии базисов $\mathcal B(f)$}%
   {passive representation in basis manifold}%
   {P}{0}%
\Symb%
   {пассивное представление группы $G(\Vector f)$ в многообразии базисов $\mathcal B(\Vector f)$}%
   {passive representation in basis manifold, tower of representations}%
   {P}{0}%
\Symb%
   {приведенное декартово произведением расслоений}%
   {reduced Cartesian product of bundles, definition 1}%
   {P}{0}%
\Symb%
   {множество невырожденных \sT преобразований расслоения $\bundle{}pE{}$}%
   {set of starT nonsingular transformations of bundle, projection}%
   {P}{0}%
\Symb%
   {множество невырожденных \Ts преобразований расслоения $\bundle{}pE{}$}%
   {set of Tstar nonsingular transformations of bundle, projection}%
   {P}{0}%

\SetIndexSpace%R%0
\Symb%
   {активное преобразование}%
   {active transformation}%
   {R}{0}%
\Symb%
   {кривизна Картана}%
   {Cartan curvature}%
   {R}{0}%
\Symb%
   {\CR ранг матрицы}%
   {cr-rank of matrix}%
   {R}{0}%
\Symb%
   {диагональ в расслоении $\bundle{}pA{}$}%
   {diagonal in bundle, 2}%
   {R}{0}%
\Symb%
   {диагональ в расслоении $\Bundle A$}%
   {diagonal in reduced bundle, 2}%
   {R}{0}%
\Symb%
   {образ $m$ при эндоморфизме $R$ эффективного представления}%
   {endomorphism image, effective representation}%
   {R}{0}%
\Symb%
   {образ кортежа $\VX a$ при эндоморфизме $\VX r$ башни эффективных представлений}%
   {endomorphism image, tower of effective representations}%
   {R}{0}%
\Symb%
   {кривизна}%
   {GLn curvature_overline}%
   {R}{0}%
\Symb%
   {произведение колец множеств}%
   {product of rings of sets}%
   {R}{0}%
\Symb%
   {$\RCcirc$\Hyph произведение матриц отображений}%
   {rc product of matrices of maps}%
   {R}{0}%
\Symb%
   {\RC ранг матрицы}%
   {rc-rank of matrix}%
   {R}{0}%
\Symb%
   {правое алгебраическое дополнение элемента  $a_{i{\kern 1pt} j} $ матрицы}%
   {right cofactor, matrix}%
   {R}{0}%
\Symb%
   {правое двойное алгебраическое дополнение элемента $a_{ij}$ матрицы}%
   {right double cofactor}%
   {R}{0}%
\Symb%
   {правый сдвиг}%
   {right shift}%
   {R}{0}%
\Symb%
   {строчный определитель по  $i$-й строке матрицы $\bfA$}%
   {row determinant}%
   {R}{0}%
\Symb%
   {алгебра скаляров алгебры $A$}%
   {scalar algebra of algebra}%
   {R}{0}%
\Symb%
   {алгебра скаляров кольца $D$}%
   {scalar algebra of ring}%
   {R}{0}%
\Symb%
   {скаляр элемента $d$ алгебры}%
   {scalar of algebra}%
   {R}{0}%
\Symb%
   {скаляр элемента $d$ кольца}%
   {scalar of ring}%
   {R}{0}%
\Symb%
   {множество правосторонних невырожденных преобразований универсальной алгебры $M$}%
   {set of right-side nonsingular transformations}%
   {R}{0}%
\Symb%
   {сферические координаты}%
   {spherical coordinates}%
   {R}{0}%

\SetIndexSpace%S%0
\Symb%
   {произведение расслоенных соответствий}%
   {composition of fibered correspondences}%
   {S}{0}%
\Symb%
   {гиперболический синус}%
   {hyperbolic sine}%
   {S}{0}%
\Symb%
   {обратное расслоенное соответствие}%
   {inverse fibered correspondence, 2}%
   {S}{0}%
\Symb%
   {обратное приведенное расслоенное соответствие}%
   {inverse reduced fibered correspondence, 2}%
   {S}{0}%
\Symb%
   {интеграл Лебега}%
   {Lebesgue integral}%
   {S}{0}%
\Symb%
   {линейная оболочка в векторном пространстве}%
   {linear span, vector space}%
   {S}{0}%
\Symb%
   {образ базиса $X$ при пассивном преобразовании $S$}%
   {passive transformation of basis, representation}%
   {S}{0}%
\Symb%
   {образ базиса $\VX X$ при пассивном преобразовании $\VX s$}%
   {passive transformation of basis, tower of representations}%
   {S}{0}%
\Symb%
   {множество перестановок}%
   {set of permutations}%
   {S}{0}%
\Symb%
   {множество перестановок}%
   {set of transpositions}%
   {S}{0}%
\Symb%
   {синус}%
   {sine}%
   {S}{0}%
\Symb%
   {симметрическая группа}%
   {symmetric group}%
   {S}{0}%

\SetIndexSpace%T%0
\Symb%
   {категория левосторонних представлений}%
   {category of left-side representations}%
   {T}{0}%
\Symb%
   {касательная плоскость к группе Ли $G$}%
   {tangent plane to Lie group}%
   {T}{0}%
\Symb%
   {след кватерниона $x$}%
   {trace, quaternion algebra}%
   {T}{0}%

\SetIndexSpace%V%0
\Symb%
   {аффинное пространство}%
   {affine space}%
   {V}{0}%
\Symb%
   {сопряжённое аффинное пространство}%
   {conjugated affine space}%
   {V}{0}%
\Symb%
   {сопряжённое векторное пространство}%
   {conjugated vector space}%
   {V}{0}%
\Symb%
   {координатное векторное пространство}%
   {coordinate vector space}%
   {V}{0}%
\Symb%
   {координаты в векторном пространстве}%
   {coordinates in vector space}%
   {V}{0}%
\Symb%
   {прямое произведение $\RCstar D_i$\hyph векторных пространств $\Vector V_1$, ..., $\Vector V_n$}%
   {direct product, rcd vector space, 1 n}%
   {V}{0}%
\Symb%
   {дуальное пространство к \rcd векторному пространству $\Vector V$}%
   {dual space of rcd vector space}%
   {V}{0}%
\Symb%
   {эрмитово сопряжённый вектор}%
   {hermitian conjugated vector}%
   {V}{0}%
\Symb%
   {линейная комбинация векторов}%
   {linear composition of vectors}%
   {V}{0}%
\Symb%
   {векторное пространство}%
   {V}%
   {V}{0}%
\Symb%
   {вертикальная компонента вектора}%
   {vertical component of vector}%
   {V}{0}%
\Symb%
   {вертикальное подпространство}%
   {vertical subspace}%
   {V}{0}%

\SetIndexSpace%W%0
\Symb%
   {множество координат представления $J(f,X)$}%
   {coordinate set of representation}%
   {W}{0}%
\Symb%
   {множество кортежей координат башни представлений $\Vector J(\Vector f,\VX X)$}%
   {coordinate set of tower of representations}%
   {W}{0}%
\Symb%
   {координаты базиса $X'$ относительно базиса $X$ представления}%
   {coordinates of basis relative to basis, representation}%
   {W}{0}%
\Symb%
   {координаты элемента $m$ представления $f$ относительно множества $X$}%
   {coordinates of element relative to generating set, representation}%
   {W}{0}%
\Symb%
   {координаты элемента $m$ относительно множества $X$}%
   {coordinates of element relative to set, representation}%
   {W}{0}%
\Symb%
   {кортеж координат элемента $\Vector a$ относительно кортежа множеств $\VX X$}%
   {coordinates of element, tower of representations}%
   {W}{0}%
\Symb%
   {геометрический объект в координатном представлении, определённом в $\Omega_2$\Hyph алгебре $M$}%
   {geometric object, coordinate representation g}%
   {W}{0}%
\Symb%
   {геометрический объект в координатном представлении, определённом в кортеже $\VX\Omega$\Hyph алгебр $\VX A$}%
   {geometric object, coordinate tower of representations g}%
   {W}{0}%
\Symb%
   {геометрический объект, определённый в $\Omega_2$\Hyph алгбре $M$}%
   {geometric object, representation g}%
   {W}{0}%
\Symb%
   {геометрический объект, определённый в кортеже $\VX\Omega$\Hyph алгебр $\VX A$}%
   {geometric object, tower of representations g}%
   {W}{0}%
\Symb%
   {геометрический объект в векторном пространстве}%
   {geometric object, vector space}%
   {W}{0}%
\Symb%
   {множество координат множества $B\subset J(f,X)$}%
   {subset of coordinates of representation}%
   {W}{0}%
\Symb%
   {координаты кортежа множеств $\VX B$ относительно кортежа множеств $\VX X$}%
   {subset of coordinates of tower of representations}%
   {W}{0}%
\Symb%
   {координаты множества $B_k$ относительно кортежа множеств $\VX X$}%
   {subset of coordinates of tower of representations, k}%
   {W}{0}%
\Symb%
   {множество $\Omega_2$\Hyph слов, представляющих множество $B\subset J(f,X)$}%
   {subset of words of representation}%
   {W}{0}%
\Symb%
   {суперпозиция координат эндоморфизма представления $f$ и точки $m$}%
   {superposition of coordinates, representation}%
   {W}{0}%
\Symb%
   {суперпозиция координат эндоморфизма башни представлений $\Vector f$ и элемента $\VX a$}%
   {superposition of coordinates, tower of representations}%
   {W}{0}%
\Symb%
   {$\Omega_2$\Hyph слово, представляющее элемент $m\in J(f,X)$}%
   {word of element relative to generating set, representation}%
   {W}{0}%
\Symb%
   {множество $\Omega_2$\Hyph слов представления $J(f,X)$}%
   {word set of representation}%
   {W}{0}%
\Symb%
   {множество кортежей $\VX{\Omega}$\Hyph слов башни представлений $\Vector J(\Vector f,\VX X)$}%
   {word set of tower of representations}%
   {W}{0}%
\Symb%
   {кортеж слов элемента $\Vector a$ относительно кортежа множеств $\VX X$}%
   {words of element, tower of representations}%
   {W}{0}%

\SetIndexSpace%X%0
\Symb%
   {кватернион, сопряженный к кватерниону $x$}%
   {conjugate of quaternion}%
   {X}{0}%
\Symb%
   {локальный базис аффинного пространства}%
   {local basis of affine space}%
   {X}{0}%
\Symb%
   {неголономная координата}%
   {x(k)}%
   {X}{0}%

\SetIndexSpace%Z%0
\Symb%
   {центр $D$\Hyph алгебры $A$}%
   {center of algebra}%
   {Z}{0}%
\Symb%
   {центр кольца $D$}%
   {center of ring}%
   {Z}{0}%

\SetIndexSpace%Delta%1
\Symb%
   {отклонение траекторий}%
   {deviation of trajectories}%
   {Delta}{1}%
\Symb%
   {тождественное преобразование}%
   {identical transformation}%
   {Delta}{1}%
\Symb%
   {образ вектора $\Vector e_k\in\Basis e$ при изоморфизме в координатное векторное пространство}%
   {image of vector e_k, coordinate vector space}%
   {Delta}{1}%
\Symb%
   {символ Кронекерa}%
   {Kronecker symbol}%
   {Delta}{1}%

\SetIndexSpace%Gamma%1
\Symb%
   {неголономные координаты связности}%
   {anholonomic coordinates of connection}%
   {Gamma}{1}%
\Symb%
   {символ Картана}%
   {Cartan symbol}%
   {Gamma}{1}%
\Symb%
   {связность}%
   {conection overline}%
   {Gamma}{1}%
\Symb%
   {коэффициенты связности в $D$\Hyph аффинном пространстве}%
   {connection coefficients, D affine space}%
   {Gamma}{1}%
\Symb%
   {связность в $D$\Hyph аффинном пространстве}%
   {connection, affine manifold}%
   {Gamma}{1}%
\Symb%
   {коэффициенты $D$\Hyph аффинной связности на многообразии}%
   {D affine connection coefficients, manifold}%
   {Gamma}{1}%
\Symb%
   {голономные координаты связности}%
   {holonomic coordinates of connection}%
   {Gamma}{1}%
\Symb%
   {связность Картана}%
   {overbrace Gamma i kl}%
   {Gamma}{1}%
\Symb%
   {множество сечений расслоения}%
   {set of sections of bundle}%
   {Gamma}{1}%

\SetIndexSpace%Lambda%1
\Symb%
   {обратный оператор оператора $\psi_l$}%
   {inverse operator to operator psi l}%
   {Lambda}{1}%
\Symb%
   {обратный оператор оператора $\psi_r$}%
   {inverse operator to operator psi r}%
   {Lambda}{1}%

\SetIndexSpace%Mu%1
\Symb%
   {декартово произведение мер}%
   {Cartesian product of measures}%
   {Mu}{1}%
\Symb%
   {степень меры}%
   {power of measure}%
   {Mu}{1}%
\Symb%
   {произведение мер}%
   {product of measures}%
   {Mu}{1}%
\Symb%
   {произведение мер}%
   {product of measures, otimes}%
   {Mu}{1}%

\SetIndexSpace%Omega%1
\Symb%
   {объект неголономности}%
   {anholonomity object}%
   {Omega}{1}%
\Symb%
   {определённый интеграл}%
   {definite integral}%
   {Omega}{1}%
\Symb%
   {интеграл дифференциальной $1$\Hyph формы вдоль пути}%
   {integral of differential 1 form along path}%
   {Omega}{1}%
\Symb%
   {норма операции}%
   {norm of operation}%
   {Omega}{1}%
\Symb%
   {область операторов}%
   {operator domain}%
   {Omega}{1}%
\Symb%
   {множество дифференциальных $p$\Hyph форм}%
   {set of differential p forms}%
   {Omega}{1}%
\Symb%
   {множество $n$\Hyph арных операций $\Omega$\Hyph алгебры}%
   {set of n-ary operations}%
   {Omega}{1}%
\Symb%
   {множество $n$\Hyph арных операторов}%
   {set of n-ary operators}%
   {Omega}{1}%

\SetIndexSpace%Psi%1
\Symb%
   {левый базовый оператор группы Ли над алгеброй $A$}%
   {L basic operator of Lie group over algebra A}%
   {Psi}{1}%
\Symb%
   {левый базовый оператор группы Ли}%
   {Lie Basic Operator L}%
   {Psi}{1}%
\Symb%
   {левый базовый оператор однопараметрической группы Ли}%
   {Lie Basic Operator L, 1-Parameter Group}%
   {Psi}{1}%
\Symb%
   {левый базовый оператор однопараметрической группы Ли над алгеброй $A$}%
   {Lie Basic Operator L, 1-Parameter Group, algebra}%
   {Psi}{1}%
\Symb%
   {правый базовый оператор группы Ли}%
   {Lie Basic Operator R}%
   {Psi}{1}%
\Symb%
   {правый базовый оператор однопараметрической группы Ли}%
   {Lie Basic Operator R, 1-Parameter Group}%
   {Psi}{1}%
\Symb%
   {правый базовый оператор однопараметрической группы Ли над алгеброй $A$}%
   {Lie Basic Operator R, 1-Parameter Group, algebra}%
   {Psi}{1}%
\Symb%
   {правый базовый оператор группы Ли над алгеброй $A$}%
   {R basic operator of Lie group over algebra A}%
   {Psi}{1}%

\SetIndexSpace%Sigma%1
\Symb%
   {расслоенное подмножество}%
   {fibered subset}%
   {Sigma}{1}%
\Symb%
   {чётность перестановки}%
   {parity of permutation}%
   {Sigma}{1}%
\Symb%
   {подрасслоение}%
   {subbundle}%
   {Sigma}{1}%

\SetIndexSpace%Nabla%2
\Symb%
   {производная Картана}%
   {overbrace nabla_l}%
   {Nabla}{2}%
\Symb%
   {производная}%
   {overline nabla_l, definition 1}%
   {Nabla}{2}%

\SetIndexSpace%Phi%1
\Symb%
   {операция на группе Ли}%
   {Lie group composition law}%
   {Phi}{1}%
\Symb%
   {сужение соответсвия $\Phi$ на множество $C$}%
   {restriction of correspondence}%
   {Phi}{1}%

\SetIndexSpace%Pi%1
\Symb%
   {декартово произведение расслоений}%
   {Cartesian product of bundles, definition 2}%
   {Pi}{1}%
\Symb%
   {декартово произведение групп $G_i$, $i\in I$}%
   {Cartesian product of groups}%
   {Pi}{1}%
\Symb%
   {декартово произведение групп $G_1$, ..., $G_n$}%
   {Cartesian product of groups, i 1 n}%
   {Pi}{1}%
\Symb%
   {декартово произведение расслоенных пространств}%
   {Cartesian product of total spaces, definition 2}%
   {Pi}{1}%
\Symb%
   {копроизведение в категории}%
   {coproduct in category}%
   {Pi}{1}%
\Symb%
   {прямое произведение тел $D_i$, $i\in I$}%
   {direct product of division rings}%
   {Pi}{1}%
\Symb%
   {прямое произведение тел $D_1$, ..., $D_n$}%
   {direct product of division rings, i 1 n}%
   {Pi}{1}%
\Symb%
   {прямое произведение $\RCstar D_i$\hyph векторных пространств $\Vector V_i$, $i\in I$}%
   {direct product, rcd vector space}%
   {Pi}{1}%
\Symb%
   {прямое произведение $\RCstar D_i$\hyph векторных пространств $\Vector V_1$, ..., $\Vector V_n$}%
   {direct product, rcd vector space, i 1 n}%
   {Pi}{1}%
\Symb%
   {произведение в категории}%
   {product in category}%
   {Pi}{1}%
\Symb%
   {приведенное декартово произведением расслоений}%
   {reduced Cartesian product of bundles, definition 2}%
   {Pi}{1}%
\Symb%
   {приведенное декартово произведение расслоенных пространств}%
   {reduced Cartesian product of total spaces, definition 2}%
   {Pi}{1}%

\CloseIndex


==> Two.Integrals.Russian.tex <==
%auto-ignore

\input{Two.Integrals.Eq}

\ePrints{1702.01}
\ifx\Semafor\ValueOff
\Chapter{Интеграл Лебега}

Я решил выделить теоремы
\RefTheorem{Lebesgue Integral along Linear Path},
\RefTheorem{Lebesgue Integral along Path}
\ifx\setCACAA\undefined
в отдельную главу,
\else
в отдельный раздел,
\fi
поскольку я считаю эти теоремы очень важными.
Важно отметить, что теоремы
\RefTheorem{Lebesgue Integral along Linear Path},
\RefTheorem{Lebesgue Integral along Path}
предлагают альтернативный метод решения дифференциального уравнения
\ShowEq{df=g}

\Section{Интеграл Лебега вдоль линейного пути}
\fi

\begin{theorem}
\labelTheorem{Lebesgue Integral along Linear Path}
Пусть $A$ - банаховый $D$\Hyph модуль.
Пусть $B$ - банаховая $D$\Hyph алгебра.
Пусть
\ShowEq{g:A->BoxB}
интегрируемое отображение
\DrawEq{f=int g.}{linear}
и
$\|g\|=G<\infty$.
Для любых $A$\Hyph чисел $a$, $x$,
пусть
\ShowEq{h:[01]->A}
линейный путь в $D$\Hyph алгебре $A$
\ShowEq{h=a+tb}
Тогда
\DrawEq{int hn= 2}{linear path}
\end{theorem}
\begin{proof}
Из равенства
\EqRef{h=a+tb}
следует, что
\ShowEq{dx=dt b-a}
\ShowEq{h'=b-a}
и равенство
\ShowEq{g(x)=g(h(t))}
является следствием равенства
\EqRef{dx=dt b-a}.
Чтобы посчитать интеграл
\ShowEq{int h=int 01}
рассмотрим разбиение
\DrawEq{t0...tn}{}
отрезка $[0,1]$
на равные интервалы.
В этом случае мы можем использовать простое отображение\,\footnote{
Согласно определению
\ShowEq{ref: simple map}
и теореме
\ShowEq{ref: measurable simple map}
отображение является простым, если
область значений - конечное или счётное множество
и прообраз каждого значения - измеримое множество.
}%
\ShowEq{gn(t)=}
вместо подынтегрального выражения.
Из
\EqRef{g(x)=g(h(t))}, \EqRef{gn(t)=}
следует, что
\ShowEq{|g-gn|}
если
\ShowEq{ti<t<ti+1}
Из
\EqRef{|g-gn|}
следует, что
\ShowEq{g(h)=lim gn}
и следовательно
\ShowEq{g(b-a)=lim...}
Равенство
\ShowEq{g(x)dx=}
является следствием равенства
\eqRef{f=int g.}{linear}
и определений
\RefDefinition{differentiable map, algebra},
\RefDefinition{indefinite integral}.
Здесь
$o:A\rightarrow A$
- отображение такое, что
\ShowEq{lim |o(a)|=0}
Из
\EqRef{gn(t)=}, \EqRef{g(x)dx=}
следует, что
\ShowEq{dt gn (b-a)}
где
\ShowEq{lim o1/n}
Из
\EqRef{dt gn (b-a)},
следует, что
отображение
$g_n(t)\circ(x-a)$
интегрируемо и
\ShowEq{int gn=...}
Из
\EqRef{lim o1/n}
следует, что
\ShowEq{lim no=0}
Из
\EqRef{g(b-a)=lim...},
\EqRef{lim no=0}
и определения
\EqParm{ref: Integral of Map over Set of Finite Measure}{=z}
следует, что
отображение
\ShowEq{g(h)o(b-a)}
интегрируемо на отрезке $[0,1]$ и
равенство
\eqRef{int hn= 2}{linear path}
является следствием
\eqRef{f=int g.}{linear}.
\end{proof}

\ePrints{1702.01}
\ifx\Semafor\ValueOff
\Section{Интеграл Лебега вдоль пути}
\fi

\begin{theorem}
\labelTheorem{Lebesgue Integral along Path}
Пусть существует неопределённый интеграл
\DrawEq{f=int g.}{}
Для любого непрерывного спрямляемого пути
\ShowEq{h:[01]->A}
из $a$ в $x$ в $D$\Hyph модуле $A$
\DrawEq{int hn= 2}{path}
\end{theorem}
\begin{proof}
Пусть
\DrawEq{t0...tn}{path}
множество точек отрезка $[0,1]$
таких, что
\ShowEq{lim max dt = 0}
Мы определим путь $\gamma_n$ согласно равенству
\ShowEq{hn=htiti1}
%На каждом отрезке
%\ShowEq{[titi1]}
%мы определим отображение
%\ShowEq{hi:01->A}
Последовательность отображений $\gamma_n$
сходится к отображению $\gamma$.
Мы можем потребовать равномерную сходимость.
Из теории интегрирования следует, что
\ShowEq{int h=lim int hn}
Согласно разбиению
\eqRef{t0...tn}{path}
интеграл
\ShowEq{int hn}
можно представить в виде суммы
\ShowEq{int hn=sum}
Для каждого $i$, мы заменим переменную
\ShowEq{s=...ti}
Тогда
\ShowEq{int hin=}
Согласно теореме
\RefTheorem{Lebesgue Integral along Linear Path},
\ShowEq{int hin= 1}
Из
\EqRef{int hn=sum},
\EqRef{int hin= 1}
следует, что
\ShowEq{int hn=}
\end{proof}

\Section{Решение дифференциального уравнения}

Мы ещё раз рассмотрим дифференциальное уравнение
\DrawEq{differential equation y=xx, 1, algebra}{path}
и начальное условие
\DrawEq{differential equation, initial}{y=xx, path}
Согласно определению
\RefDefinition{indefinite integral},
отображение $y$ является интегралом
\ShowEq{int=x3 path}
Поэтому мы можем применить теорему
\RefTheorem{Lebesgue Integral along Linear Path}
для решения дифференциального уравнения
\eqRef{differential equation, initial}{y=xx, path}.
Рассмотрим путь
\ShowEq{h:[01]->A}
в $D$\Hyph алгебре $A$
\ShowEq{h=tx}
Тогда интеграл
\eqRef{int hn= 2}{linear path}
принимает вид
\ShowEq{int=x3 path tx}

%Согласно доказательству теоремы
%\RefTheorem{Lebesgue Integral along Linear Path},
%мы разобьём интервал $[0,1]$ на $n$ равных частей
%и рассмотрим сумму
%\ShowEq{sum x3 1}
%Из равенства
%\EqRef{sum x3 1}
%следует, что
%\DrawEq{int=x3}{}%{path}

Как легко мы решили дифференциальное уравнение.
Однако, так ли это?

Чтобы получить ответ на этот вопрос, рассмотрим также дифференциальное уравнение
\DrawEq{differential equation y=xx, 1, a, algebra}{path}
\DrawEq{differential equation, initial}{}
Рассмотрев путь
\EqRef{h=tx},
мы получим, что
\ShowEq{int 3x2=x3}
Однако мы знаем, что это неверно.

Для решения дифференциального уравнения
мы рассмотрели линейный путь.
Однако путь может быть произвольным.
Рассмотрим путь
\ShowEq{path 0ax}
Интеграл
\ShowEq{int h gx dx}
может быть представлен в виде суммы
\ShowEq{int h gx dx sum}
где $\gamma_1$ - путь
\ShowEq{path h1}
и $\gamma_2$ - путь
\ShowEq{path h2}
Мы только что рассмотрели интеграл
\ShowEq{int h1=a3}
Поэтому нам надо рассмотреть интеграл
\ShowEq{int h2=int 12}
\begin{itemize}
\item
Пусть
\ShowEq{gx=xx+}
Тогда интеграл
\EqRef{int h2=int 12}
принимает вид
\ShowEq{int h2=int 12 xx+}
Равенство
\ShowEq{int h2 xx+ =}
\ePrints{1702.01}
\ifx\Semafor\ValueOff
является следствием равенств
\EqRef{int h2=int 12 xx+},
\EqRef{int h2=int 12 xx+ 5}.
\else
является следствием равенства
\EqRef{int h2=int 12 xx+}.
\fi
Равенство
\ShowEq{int h xx+ =}
является следствием равенств
\EqRef{int h gx dx sum},
\EqRef{int h1=a3},
\EqRef{int h2 xx+ =}.
\item
Пусть
\ShowEq{gx=3x2}
Тогда интеграл
\EqRef{int h2=int 12}
принимает вид
\ShowEq{int h2=int 12 3x2}
Равенство
\ShowEq{int h2 3x2 =}
является следствием равенств
\ePrints{1702.01}
\ifx\Semafor\ValueOff
является следствием равенств
\EqRef{int h2=int 12 3x2},
\EqRef{int h2=int 12 3x2 3}.
\else
является следствием равенства
\EqRef{int h2=int 12 3x2}.
\fi
Равенство
\ShowEq{int h 3x2 =}
является следствием равенств
\EqRef{int h gx dx sum},
\EqRef{int h1=a3},
\EqRef{int h2 3x2 =}.
\end{itemize}

Таким образом, интеграл
\ShowEq{int h 3x2 dx}
зависит от выбора пути $\gamma$ из $0$ в $x$,
и дифференциальное уравнение
\eqRef{differential equation y=xx, 1, a, algebra}{path}
не имеет решений.
\ePrints{1702.01}
\ifx\Semafor\ValueOff
Таким образом, прежде чем применять интеграл Лебега
для решения дифференциального уравнения,
мы должны ответить на один из следующих вопросов.
Как доказать, что интеграл
не зависит от выбора пути, либо как найти путь,
который докажет зависимость интеграла от пути.

Мы неожиданно оказались на новой территории.
Имя этой территории - дифференциальные формы.
\fi

